Practical Low Latency Proof of Work Consensus

Bitcoin is the first fully-decentralized permissionless blockchain protocol to achieve a high level of security, but at the expense of poor throughput and latency. Scaling the performance of Bitcoin has a been a major recent direction of research. One successful direction of work has involved replacing proof of work (PoW) by proof of stake (PoS). Proposals to scale the performance in the PoW setting itself have focused mostly on parallelizing the mining process, scaling throughput; the few proposals to improve latency have either sacrificed throughput or the latency guarantees involve large constants rendering it practically useless. Our first contribution is to design a new PoW blockchain Prism++ that has provably low latency and high throughput; the design retains the parallel-chain approach espoused in Prism but invents a new confirmation rule to infer the permanency of a block by combining information across the parallel chains. We show security at the level of Bitcoin with very small confirmation latency (a small constant factor of block interarrival time). A key aspect to scaling the performance is to use a large number of parallel chains, which puts significant strain on the system. Our second contribution is the design and evaluation of a practical system to efficiently manage the memory, computation, and I/O imperatives of a large number of parallel chains. Our implementation of Prism++ achieves a throughput of over 80,000 transactions per second and confirmation latency of tens of seconds on networks of up to 900 EC2 Virtual Machines.

==> Prism Systems Paper (CCS)/ack.tex <==
\section*{Acknowledgments}

We thank Ertem Nusret Tas for feedback and fruitful discussions.

==> Prism Systems Paper (CCS)/background.tex <==
\section{The Longest Chain Protocol}
\label{sec:background}
% In this section, we review Nakamoto's longest chain protocol~\cite{bitcoin} and discuss the fundamental limitations in scaling its latency and throughput. These limitations motivate \prism's design, as we discuss in the next section. 

% %as a natural design to remove these limitations. 
% %%We will explain the design of \prism incrementally, first addressing throughput and then latency.



% \subsection{The longest chain protocol}

The most basic blockchain consensus protocol is Nakamoto's longest chain protocol, used in many systems including \bitcoin and \ethereum.  The basic object is a {\em block}, consisting of {\em transactions} and a reference link to another block. 
%A transaction is a payment signed by a sender's public key, and addressed to a recipient's public key. 
As transactions arrive into the system, a set of nodes, called {\em miners}, construct blocks and broadcast them to other nodes. The goal of the protocol is for all nodes to reach consensus on an ordered log of blocks (and the transactions therein), referred to as the {\em ledger}.

Starting with the {\em genesis} block as the root, each new block mined by a miner is added to create an evolving {\em blocktree}. In the longest chain protocol, honest miners append each block to the leaf block of the longest chain\footnote{In case of variable proof of work, honest miners mine on the "heaviest chain".} in the current blocktree, and the transactions in that block are added to the transaction ledger maintained by the blocks in the longest chain. 
A miner earns the right to append a block after solving a cryptographic puzzle, which requires finding a solution to a hash inequality.
 %the leaf block \ma{and the contents of the block being mined?}.  
 The miner includes the solution in the block as a {\em proof of work} (PoW), which other nodes can verify.  The time to solve the puzzle is random and exponentially distributed, with a mining rate $f$ that can be tuned by adjusting the difficulty of the puzzle. How fast an individual miner can solve the puzzle and mine the block is proportional to its hashing power, i.e. how fast it can compute hashes. 
 
 A block is confirmed to be in the ledger when it is $k$-deep in the ledger, i.e. the block is on the longest chain and a chain of $k-1$ blocks have been appended to it. It is proven that as long as the adversary has less than $50\%$ hashing power, the ledger has consistency and liveness properties~\cite{backbone}: blocks that are deep enough in the longest chain will remain in the longest chain with high probability, and honest miners will be able to enter a non-zero fraction of blocks into the ledger. 

\begin{figure}
\begin{center}
\includegraphics[width=0.4\textwidth]{fast_confirmation_comparision_2.pdf}
\end{center}
\caption{\small Depth of confirmation: longest chain vs. \prism. (a) The longest chain protocol requires a block $Ho$ to be many blocks deep for reliable confirmation, so that an adversary mining in private cannot create a longer chain to reverse block $Ho$. (b) \prism allows each voter block to be very shallow but relies on many voter chains to increase the reliability.}
\label{fig:double_spend}
\end{figure}

\subsection{Latency Limitation}
\label{s:lc-latency}
A critical attack on the longest chain protocol is the {\em private  double-spend} attack \cite{bitcoin}, as shown in Figure \ref{fig:double_spend}(a). Here, an adversary is trying to revert a block after it is confirmed, by mining a chain in private and broadcasting it when it is longer than the public chain. If the hashing power of the adversary is greater than that of aggregate of the honest nodes, this attack can be easily executed no matter what $k$ is, since the adversary can mine blocks faster on the average than the honest nodes and will eventually  overtake the public chain. On the other hand, when the adversary has less than half the power, the probability of success of this attack can be made exponentially small by choosing the confirmation depth $k$ to be large \cite{bitcoin}. The price to pay for choosing $k$ large is increased latency in confirmation. For example, to achieve a reversal probability of  $0.001$, a depth of $24$ blocks is needed if the adversary has $\beta = 30\%$ of the total hashing power~\cite{bitcoin}.  Figure ~\ref{fig:rd} shows the tradeoff between confirmation depth (and therefore latency) and reliability.


%%With Bitcoin's block mining rate of 1 block every 10 minutes, this translates into a latency of 4 hours! Increasing the block mining rate to, say, 1 block per 10 seconds, improves latency to 240 seconds, but the latency to achieve a high level of reliability is still very high. To achieve a reversal probability of $10^{-6}$, a depth of $50$ blocks is required, translating into a latency of $500$ seconds. Figure ~\ref{fig:rd} shows the tradeoff between confirmation depth (and therefore latency) and reliability. \pv{This is a pretty long section and if we are in a space crunch, then its fine to cut a bit.} 

%In Bitcoin, the mining rate is set much more conservatively, a block roughly every 10 minutes, leading to very long confirmation latency. 

%\ma{I've been assuming this figure also shows the reliability-depth tradeoff for Prism?}
% \begin{figure}
%     \centering
%     \begin{subfigure}[b]{\textwidth}
%         \centering
%         \includegraphics[width=0.35\linewidth]{fast_confirmation_comparision_a.pdf}%
%         \hfill
%         \includegraphics[width=0.35\linewidth]{fast_confirmation_comparision_b.pdf}
%     \end{subfigure}
%     \tion{\small Depth of confirmation: longest chain vs. \prism. (a) The longest chain protocol requires a block to be many blocks deep for reliable confirmation, so that an adversary mining in private cannot create a longer chain. (b) \prism allows each voter block to be very shallow but relies on many voter chains to increase the reliability. \ma{please increase the font size of the subfigure labels, or better, separate this into two figures and use latex's subfig environment}} 
% \end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=0.32\textwidth]{figures/reliability-depth.pdf}
\end{center}
\caption{\label{fig:rd} \small Reliability as a function of confirmation depth. The reversal probability of \prism has a factor $m$ improvement over the longest chain protocol in the exponential rate of decrease, where $m$ is the number of voter chains (introduced in \S\ref{sec:overview}).}
\end{figure}
\subsection{Throughput Limitation}
\label{s:lc-thput}

If $B$ is the block size in number of transactions, then the throughput of the longest chain protocol is at most $fB$ transactions per second (tps). 
However, the mining rate $f$ and the block size $B$ are constrained by the security requirement. Increasing the mining rate increases the amount of {\em forking} of the blockchain due to multiple blocks being mined on the same leaf block by multiple miners within the network delay~$\Delta$. Forking reduces throughput since it reduces the growth rate of the longest chain; recall that only blocks on the longest chain contribute to the ledger. More importantly, forking hurts the security of the protocol because the adversary requires less compute power to overtake the longest chain. In fact, the adversarial power that can be tolerated by the longest chain protocol goes from $50\%$ to $0\%$ as the mining rate $f$ increases \cite{backbone}. 
%(Figure \ref{fig:forking}). 
Similarly, increasing the block size $B$ also increases the amount of forking since the network delay $\Delta$ increases with the block size \cite{decker}.

A back-of-the-envelope calculation of the impact of the forking can be done based on a simple model of the network delay: 
$$ \Delta = \frac{hB}{C} + D,$$
where $h$ is the average number of hops for a block to travel, $C$ is the communication bandwidth per link in transactions per second, and $D$ is the end-to-end propagation delay.  This model is consistent with the linear relation between the network delay and the block size as measured empirically by \cite{decker}. 
%\ma{do we have to mention the possibility of cut-through routing? i think we can skip it and maybe mention it in the discussion section towards the end.}
%\vb{Thats a good idea. There are works (like bloxroute) out there which propose cut-through routing to improve the latency.}
Hence, the utilization, i.e. the throughput as a fraction of the communication bandwidth, is upper bounded by
$$ \frac{fB}{C} < \frac{f\Delta}{h},$$
where $f\Delta$ is the average number of blocks ``in flight'' at any given time, and reflects the amount of forking in the block tree.  %%which is nothing but the \textit{forking rate} on the longest chain. \ma{how is forking rate defined?}
In the longest chain protocol, to be secure against an adversary with $\beta < 50\%$ of hash power, this parameter should satisfy \cite{backbone}
$$f\Delta<\frac{1-2\beta}{\beta}.$$
For example, to achieve security against an adversary with $\beta = 45\%$ of the total hashing power, one needs $f\Delta \approx 0.2$. With $h = 5$, this translates to a utilization of at most $4\%$. The above bound holds regardless of block size; the utilization of the longest chain protocol cannot exceed 4\% for $\beta = 45\%$ and $h=5$.
In summary, to not compromise on security, $f\Delta$ must be kept much smaller than $1$. 
Hence, the security requirement (as well as the number of hops) limits the bandwidth utilization.  

%%$$ \ma{I still don't understand why this is different from the analysis in Appendix %%D.2 of the Prism paper.}
%%\vb{The analysis in D.2 is a conservative necessary condition. Whereas the above %%formula is only a necessary condition. It comes from the simple fact that the %%honest nodes grow at rate $\frac{(1-\beta)}{1+f\Delta}$ and adversary grows at rate %%$f\beta$.}
%%\gf{The phrasing above the equation makes it sound like a necessary condition.} %%\vb{Typo. It is indeed a necessary condition

% \ma{Can we state how security depends on $f\Delta$ here precisely, and replace Figure 3 with one that shows maximum possible $f\Delta$ vs. $\beta$. The next sentence gives the specific point $\beta=0.45$ as an example. The nice thing about this is that it highlights that in the longest chain protocol, to meet the security requirement, one cannot have too many blocks in flight at the same time. Prism doesn't have this limitation. However, if my understanding is correct, it will show that $f\Delta$ can be 1 for $\beta < 0.33$, and drops sharply only for higher security levels. This would mean that the possible utilization for Bitcoin in practice is really $1/h$. Is this correct? Prism can only improve throughput from $1/h$ to $1$, unless we're concerned with very high security?} 
% \vb{The effective throughput due to forking is $fB\big(\frac{1}{1+f\Delta}\big)$} \ly{$f\Delta = \frac{1-2\beta}{\beta}$ See Figure~\ref{fig:forking-new}} \ma{Is this consistent with the Prism theory paper, Appendix D.2? I'm still not happy with our explanation here. My hope is that we can remove Fig. 3, and use the fact that f$\Delta$ must be small for security, and the equation above to show that the utilization of the longest chain protocol is limited. @Vivek: please see if this makes sense and update this section.}


%%In summary, in the longest chain protocol, security of the system is fundamentally at odds with low latency and high throughput. To achieve a low reversal probability, blocks must be deep in the longest chain, increasing confirmation latency. At the same time, increasing the mining rate or block size would compromise security because of forking. As we discuss next, \prism removes these limitations to achieve high throughput, low latency, and security simultaneously. 

%\red{GF: Maybe explain in words why we can hope to fix this problem? The dependency on  graph diameter is fundamental, since all honest nodes have to come to consensus, but the effect of Bitcoin's security requirement could  be circumvented by designing a system that trades latency for communication in its confirmation rule.}

\if 0
\begin{figure}
\begin{center}
\includegraphics[width=0.4\textwidth]{figures/forking_security.pdf}
\end{center}
\caption{ Increasing mining rate or block size increases forking and reduces security. 
\red{GF: Are we going to add numbers to the x-axis? This looks a bit cartoonish, I think having actual nubmers on the axes would help,  if we want to keep this figure at all (not sure it clarifies too much?).} \ly{Shall I redo the plot to put numbers on x-axis and make it the same style as figure 8 to 12?}
\vb{I have added numbers to x-axis for now.}
\gw{Caption says "or block size", but it's not in the figure.}}
\label{fig:forking}
\end{figure}

\fi

% \begin{figure}
% \centering
% \input{figures/fdelta-fig.tex}
% \caption{ Increasing mining rate or block size increases forking and reduces security. \gw{Is this the correct caption for the figure?}} \ma{No. This figure might actually work better with $f\Delta$ on the x-axis. The focus should probably be the region where $f\Delta$ is small, say less than 2 or 3. I'm not sure the figure is correct. @Vivek: please double check} \vb{This figure look correct}
% \label{fig:forking-new}
% \end{figure}






==> Prism Systems Paper (CCS)/commands.tex <==

\usepackage[utf8]{inputenc}
\usepackage[english]{babel}

\setcounter{secnumdepth}{3} % numbering section depth
\setcounter{tocdepth}{4}
\newtheorem{thm}{Theorem}[section]
\newtheorem{defn}[thm]{Definition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{prop}{Proposition}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{constr}[thm]{Construction}


\newcommand{\bpf}{\begin{proof}}
\newcommand{\epf}{\end{proof}}
\newcommand{\bprf}{{\em Proof: }}
\newcommand{\bproof}{{\em Proof of }}
\newcommand{\eproof}{\hfill $\Box$}
\newcommand{\argmin}{\operatornamewithlimits{arg \ min}}
\newcommand{\argmax}{\operatornamewithlimits{arg \ max}}
\newcommand{\indep}{\mathrel{\text{\scalebox{1.07}{$\perp\mkern-10mu\perp$}}}}


\newcommand{\red}[1]{\textcolor{red}{#1}}

\newcommand{\beqa}{\begin{eqnarray}}

\newcommand{\eeqa}{\end{eqnarray}}

\newcommand{\beqan}{\begin{eqnarray*}}

\newcommand{\eeqan}{\end{eqnarray*}}

\newcommand{\beq}{\begin{equation}}

\newcommand{\eeq}{\end{equation}}

\newcommand{\prf}{\noindent {\bf Proof}\ \ \ }

\newcommand{\lra}{\Longleftrightarrow}

\newcommand{\lbr}{\left \{ }

\newcommand{\rbr}{\right \} }

\newcommand{\Lbr}{\left [}

\newcommand{\Rbr}{\right ]}

\newcommand{\lp}{\left (}

\newcommand{\rp}{\right )}

\renewcommand{\r}{\right}

\renewcommand{\l}{\left}

\newcommand{\df}{\stackrel{{\rm def}}{=}}

\newcommand{\real}{{\Bbb {R}}}

\newcommand{\complex}{{\Bbb {C}}}

\newcommand{\prob}{{\Bbb {P}}}

\newcommand{\expect}{{E}}

% \newcommand{\eqref}[1]{(\ref{#1})}




\renewcommand{\C}{{\cal C}}
\newcommand{\X}{{\mathcal X}}

\renewcommand{\S}{{\cal S}}

\newcommand{\bmk}{\beta_m^{(K)}}



\newcommand{\vu}{{\bf u}}

\newcommand{\vd}{{\bf d}}

\newcommand{\Ummse}{U_{{\rm mmse}}}

\newcommand{\vp}{{\bf p}}

\newcommand{\vq}{{\bf q}}

\newcommand{\vone}{{\bf 1}}

\newcommand{\vh}{{\bf h}}
\newcommand{\hh}{\hat h}
\newcommand{\vw}{{\bf w}}

\newcommand{\SNR}{\sf SNR}
\newcommand{\SINR}{\sf SINR}
\newcommand{\rot}{\sf RoT}
\newcommand{\penal}{\sf penalty}
\newcommand{\PR}{\sf PR}

\newcommand{\eapprox} {\stackrel {.}{=}}
\newcommand{\al}{\stackrel{.}{<}}
\newcommand{\ag}{\stackrel{.}{>}}

\newcommand{\SINRt}{{\sf SINR^{(t)}}}
\newcommand{\lambdat}{\lambda^{(t)}}
\newcommand{\It}{I^{(t)}}
\newcommand{\vwt}{{\bf w}^{(t)}}
\newcommand{\vwn}{{\bf w}^{(t+1)}}
\newcommand{\vv}{{\bf v}}
\newcommand{\uu}{{\bf u}}
\newcommand{\ww}{{\bf w}}
\newcommand{\eps}{\varepsilon}
\newcommand{\vz}{{\bf z}}
\newcommand{\bvh}{\bar{\vh}}



\newcommand{\singlespacing}{\let\CS=\@currsize\renewcommand{\baselinestretch}{0.95}\tiny\CS}



\newcommand{\oneandahalfspacing}{\let\CS=\@currsize\renewcommand{\baselinestretch}{1.25}\tiny\CS}



\newcommand{\doublespacing}{\let\CS=\@currsize\renewcommand{\baselinestretch}{1.39}\tiny\CS}



% Start with double spacing:

%%\singlespacing

%\oneandahalfspacing

%\doublespacing

\newcommand{\be}{\begin{equation}}

\newcommand{\ee}{\end{equation}}

\newcommand{\tr}{{\rm trace}}

\newcommand{\rref}[1]{(\ref{#1})}

\newcommand{\CN}{{\cal CN}}





\newcommand{\bc}{\begin{center}}

\newcommand{\ec}{\end{center}}

\newcommand{\bfl}{\begin{flushleft}}

\newcommand{\efl}{\end{flushleft}}

\newcommand{\blob}{\hfill \rule{.1in}{0.1in}}

\newcommand{\scheme}{{\sf Prism} }
\newcommand{\schemenosp}{{\sf Prism}\ignorespaces}
\newcommand{\schemelite}{{\sf Prism 1.0 } }
\newcommand{\schemelitenosp}{{\sf Prism 1.0}\ignorespaces}
\newcommand{\schemebackbone}{{\sf Prism Backbone} }
\newcommand{\schemebackbonenosp}{{\sf Prism Backbone}\ignorespaces}
\newcommand{\fruitchains}{{\sf Fruitchains } }
\newcommand{\fruitchainsnosp}{{\sf Fruitchains}\ignorespaces}
\newcommand{\bitcoinNG}{{\sf BitcoinNG } }
\newcommand{\bitcoinNGnosp}{{\sf BitcoinNG}\ignorespaces}
\newcommand{\disccoin}{{\sf DiscCoin } }
\newcommand{\disccoinnosp}{{\sf DiscCoin}\ignorespaces}
\newcommand{\byzcoin}{{\sf ByzCoin } }
\newcommand{\byzcoinnosp}{{\sf ByzCoin}\ignorespaces}
\newcommand{\hybrid}{{\sf Hybrid } }
\newcommand{\thunderella}{{\sf Thunderella }}
\newcommand{\inclusive}{{\sf Inclusive }}
\newcommand{\spectre}{{\sf Spectre }}
\renewcommand{\phantom}{{\sf Phantom }}
\newcommand{\conflux}{{\sf Conflux }}
\newcommand{\avalanche}{{\sf Avalanche }}

\newcommand{\bitcoin}{{\sf Bitcoin} }
\newcommand{\bitcoinnosp}{{\sf Bitcoin}\ignorespaces}

\newcommand{\ghost}{{\sf GHOST} }
\newcommand{\ghostnosp}{{\sf GHOST}\ignorespaces}

\newcommand{\prism}{{\sf Prism} }

\newcommand{\pois}{{\sf Poiss}}
\newcommand{\geom}{{\sf Geometric}}
\newcommand{\bin}{{\sf Bin}}

\makeatletter
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                       {-18\p@ \@plus -4\p@ \@minus -4\p@}%
                       {4\p@ \@plus 2\p@ \@minus 2\p@}%
                       {\normalfont\normalsize\bfseries\boldmath
                        \rightskip=\z@ \@plus 8em\pretolerance=10000 }}

\newcommand{\ext}{{\sf ext} }

\newcommand{\N}{{\mathcal{N}}}
\newcommand{\Z}{{\mathcal{Z}}}
\newcommand{\fv}{\bar{f}_v}
\newcommand{\fp}{\bar{f}_p}
\newcommand{\Rl}{R_{\ell}}



\newcommand{\Vo}{{\sf{V}}}
\renewcommand{\H}{{\mathcal{H}}}
\renewcommand{\C}{{\mathcal{C}}}
\newcommand{\A}{{\mathcal{A}}}
\newcommand{\T}{{\mathcal{T}}}
\newcommand{\R}{{\mathcal{R}}}
\newcommand{\rmax}{r_{\rm max}}
\newcommand{\rmin}{r_{\rm min}}
\newcommand{\bmin}{b_{\rm min}}
\newcommand{\kmin}{k_{\rm min}}
\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\E}{\mathbb{E}}
\renewcommand{\P}{{\mathcal P}}
\newcommand{\Dr}{{\Delta_r}}
\newcommand{\Dmax}{{\Delta_{\text{max}}}}
\newcommand{\cone}{\frac{1-2\beta}{16}}


\makeatother
\newcommand{\blue}{\color{blue}}

\newcommand{\tE}{\texttt{E}}
\newcommand{\tT}{\texttt{T}}
\newcommand{\tF}{\texttt{F}}
\newcommand{\Rc}{R^{\text{stop}}}
\newcommand{\Rconf}{R^{\text{conf}}}
\newcommand{\Dll}{D_{\ell', \ell}}
\newcommand{\Dllf}{\big\{D_{\ell', \ell}\big\}_{\ell'\leq \ell}}
\newcommand{\Rfirst}{R_0}
\newcommand{\Rlast}{R_{\text{last}}}
\newcommand{\LS}{\texttt{LedSeq}}
\renewcommand{\epsilon}{\varepsilon}

\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{xcolor}
\definecolor{azure}{rgb}{0.54, 0.17, 0.89}
\newcommand{\colorcomment}[1]{\Comment{ {\color{azure} #1}} }
\newcommand{\av}[1]{$#1$}
\newcommand{\maincolorcomment}[1]{{\color{azure}// #1 } }
\def\NoNumberLine#1{{\def\alglinenumber##1{}\State #1}\addtocounter{ALG@line}{-1}}
\usepackage{enumitem,kantlipsum}

\renewcommand{\bmin}{B_{\rm min}}

==> Prism Systems Paper (CCS)/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this paper, we have presented \newprism, the first practical PoW consensus protocol to achieve low latency, high throughput, and Bitcoin-level security. \newprism retains the mining and the chain structure of \prism \cite{prism-theory}, and invents a new confirmation rule based on a novel methodology of co-designing the confirmation rule with an explicit identification of the worst-case attack. We proved that this confirmation rule is crucial in achieving low latency in practical settings. In the second part of the paper, we have converted the \newprism protocol to an efficient software system.  Our implementation supports over 80,000 transactions per second at a confirmation latency of tens of seconds with Bitcoin-level security. Our results validate the theoretical analysis of the new confirmation rule, and highlight the importance of optimizing transaction execution and the databases for high throughput. We also demonstrated experimentally that \newprism is robust to several active attacks, and showed that a simple random delay is effective at mitigating spamming. 


==> Prism Systems Paper (CCS)/confirmation-rule.tex <==
\section{Confirmation Rule}
\label{apx:confirmation}

In this section we give the detailed calculation of the confidence intervals of the votes a proposer block receives. It is used when confirming a leader proposer block, as mentioned in Section~\ref{sec:confirmation}.

Consider the scenario where there are $n$ proposer blocks at level $l$, and let $\mathcal P =\{B^P_1, B^P_2, \ldots, B^P_n\}$ denote the set of proposer blocks at level $l$. Now we want to count the number of votes each block will get with confidence $1-\epsilon$.

Suppose $B^P_i$ gets $v_i$ votes. Here a vote stands for a voter block which is on the longest chain of its voter tree and votes for $B^P_i$. 
Let $\mathcal V_i =\{B^V_{i_1}, B^V_{i_2}, \ldots, B^V_{i_{v_i}}\}$ denote the set of votes that $B^P_i$ has. For every vote $B^V_{i_j}$, let $d_{i_j}$ denote its depth, which is the number of blocks appended to voter block $B^V_{i_j}$ in the longest chain, plus one.

Now, for each vote $B^V_{i_j}$ with depth $d_{i_j}$, we want to calculate the probability $P_{i_j}$ of it being permanent. 
% \textit{not} being overtaken by a hypothetical, unreleased adversarial chain any time in the future. 
To do so, we consider a potential private double-spend attack, assuming an adversarial party is trying to overturn the voting results to elect a different proposer block $B^P_A$ as the leader block of level $l$. 
Note that $B^P_A$ could either be a block in $\mathcal P$, i.e. publicly known, or a block the adversary has privately mined but not released. 
To elect $B^P_A$ as the leader block of level $l$, the adversarial party would need to mine its own voter chains to overturn some existing votes to vote for $B^P_A$. 

We want to compute the probability of this happening.
% we need to reason about the blocks the adversary has already mined as well as those it will mine in the future. 
However, we do not know when the adversary started mining voter blocks for $B^P_A$.
% , which means we do not know how long the adversary could have been mining its private blocks. 
% However, from the visible state of the blockchain, we can estimate when $B^P_i$ was mined; assuming $B^P_A$ was mined at least as late as $B^P_i$, this gives us a bound. 
Notice that the adversary has no incentive to mine voter blocks for $B^P_A$ until $B^P_i$ has been mined and released. 
%Since the honest nodes are always releasing blocks, we can use the average depth of the votes for $B^P_i$ in the public voter trees to estimate the time passed since $B^P_i$ was released, hence  bounding the expected number of votes the adversary could have accumulated on their private fork in the same amount of time. 
Since the honest nodes are always releasing blocks, we can use the average depth of the votes in the public voter trees to estimate the time passed since level $l$ was released, hence  bounding the expected number of votes the adversary could have accumulated on their private fork in the same amount of time. 
That is, since block inter-arrivals are exponentially distributed, the number of blocks mined since blocks in $\mathcal P$ was proposed is a Poisson random variable, with rate equal to its mean. 
This quantity can be related to the time elapsed since blocks in $\mathcal P$ was released via the block mining rate.
%That is, since block inter-arrivals are exponentially distributed, the number of blocks mined since block $B^P_i$ was proposed is a Poisson random variable, with rate equal to its mean. 
%This quantity can be related to the time elapsed since $B^P_i$ was released via the block mining rate.
% To do this, we estimating how deep those private voter chains are on average. 

More precisely, as an honest node, we assume the fraction of adversarial hashing power is $\beta$, and we can empirically estimate the average depth of existing public votes as $\bar{d}=\sum_{ij}{d_{i_j}}/\sum_{i}{v_i}$ and the forking rate $\alpha$~\footnote{The fraction of blocks not on the longest chain out of all blocks.} of public voter chains. 
Since there are many voter chains, these estimates converge quickly to their true means. 
Then, we calculate the estimated average depth of a \emph{private} voter chain, denoted as $\bar{d_A}$, to be
% \gf{Yes, the sentences starting with "we observe that" to the end of this para  (through the following equations) need a good bit more explanation. Minor nits: In the defn of $\bar{d}$, $v_i$ was earlier defined as the total number of votes, not the honest number  of votes,
% but $\bar{d}$ is defined as the average depth of honest votes. How are you defining an "honest vote" here? 
% Also, the sentence starting with "We observe" doesn't parse.}
% \ly{``honest'' is better defined as ``public'' here, and I have changed the definitions correspondingly. Also, I added the sentence below the next equation. Does this sound like enough explanantion?}
$$\bar{d_A} = \frac{\beta \bar{d}}{(1-\alpha)(1-\beta)}.$$
Here the $1/(1-\alpha)$ term accounts for forking in public voter chains and assumes that the malicious private voter chains do not fork. The $\beta / (1-\beta)$ term accounts for the ratio of hashing power between the honest users ($1-\beta$) and the malicious users ($\beta$).
This expected depth $\bar{d_A}$ can be used as an estimate of the rate of the Poisson random variable of the number of blocks in the adversary's  private chain. 


Since each voter chain follows the longest-chain rule, the calculation for $P_{i_j}$ is the same as in \bitcoin
$$P_{i_j} = F_{\text{Pois}}(d_{i_j};\bar{d_A}) - \sum_{k=0}^{d_{i_j}}f_{\text{Pois}}(k;\bar{d_A})\frac{\beta}{1-\beta}^{d_{i_j} + 1 - k}.$$
Here $F_{\text{Pois}}(x;\lambda)$ is the cumulative distribution function and $f_{\text{Pois}}(x;\lambda)$ is the probability mass function of Poisson distribution with rate parameter $\lambda$.
In this expression, the first term is the probability that the adversary has mined fewer than $d_{i_j}+1$ blocks, in which case it cannot currently overtake the main chain. 
The second term computes, for each possible length of the adversary's chain, the probability that the adversary overtakes the public voter chain in the future by mining faster. 

Given $P_{i_j}$, we can now calculate the confidence interval of votes on each proposer block. For proposer block $B_i^P$ and each of its votes $B^V_{i_j}$, let $\tilde V_{i_j}$ be the random variable where
$$\tilde V_{i_j} = \begin{cases}
    1, & \text{if vote } B^V_{i_j} \text{ is secure forever (permanent)} \\
    0, & \text{if vote } B^V_{i_j} \text{ will be overturned}
  \end{cases}.$$
With some abuse of notation, let $v_i$ be the random variable equal to the number of secure votes of $B^P_i$. We have
$$v_i = \sum_{j}B^V_{i_j}.$$
Note that $\tilde V_{i_j}\sim \text{Bernoulli}(P_{i_j})$. Then the lower confidence bound of votes on $B_i^P$ (denoted as $\left \lfloor v_{i} \right \rfloor$) can be obtained by calculating in $\epsilon$-quantile of random variable $v_i$.

In real-world implementations, given the complexity of such computation, its closed-form approximation may be used. We can approximate $v_i$ using a Gaussian distribution $\mathcal N(\mu_i, \sigma_i^2)$ where
$$\mu_i=\sum_j P_{i_j}.$$
$$\sigma_i^2 = \sum_j P_{i_j}(1-P_{i_j}).$$
Using the closed-form approximation of the quantile function of normal distribution, we have
$$\left \lfloor v_{i} \right \rfloor \approx \mu_i - \sigma_i \sqrt{\ln{
\frac{1}{\epsilon^2}} - \ln{\ln{\frac{1}{\epsilon^2}}} - \ln{(2\pi)}}.$$

Now, we consider the upper confidence bound of votes on $B_i^P$ (denoted as $\left \lceil v_{i} \right \rceil$). Here, we want to defend against the worst case where for each $B_i^P$, only $\left \lfloor v_{i} \right \rfloor$ votes are retained, and the adversarial party controls the remaining votes (we let $\left \lceil v_A \right \rceil$ denote the number of such votes). Recall that each voter chain can only vote for each proposer level once. For a system with $m$ voter chains, we have
$$\left \lceil v_A \right \rceil = m - \sum_{i}\left \lfloor v_{i} \right \rfloor.$$
The adversarial party will use those votes to vote for $B^P_A$. Since $B^P_A$ could be any block in $\mathcal P$, we have
$$\left \lceil v_i \right \rceil = \left \lfloor v_{i} \right \rfloor + \left \lceil v_A \right \rceil.$$
$B^P_A$ could also be a block which the adversarial party mines but has not released. In such case, the upper bound of votes on $B^P_A$ is just $\left \lceil v_A \right \rceil$. Finally, to select the leader of level $l$, we search for the block $B^P_L \in \mathcal P$ satisfying $\left \lfloor v_{L} \right \rfloor > \left \lceil v_i \right \rceil$ for every $i \neq L$ and $\left \lfloor v_{L} \right \rfloor > \left \lceil v_A \right \rceil$. In words, we select the block whose lower bound of votes is higher than the upper bound of any other known or unknown proposer block in the same level.

==> Prism Systems Paper (CCS)/datapoints.tex <==
\section{Parameters Used in Evaluations}
\label{apx:datapoints}

Here we present the parameters used in the experiment in \S\ref{sec:eval-performance} for \prism (Table~\ref{table:prism-params}, Table~\ref{table:prism-beta}), \algorand (Table~\ref{table:algorand-params}), \bng (Table~\ref{table:bng-params}), and the longest chain protocol (Table~\ref{table:lc-params}).

\begin{table}[t]
	\centering
	\caption{Parameters of \prism.}
	%\resizebox{\columnwidth}{!}{
	\begin{tabular}{ r | c } 
	 \hline
	 Parameter & Value \\ [0.5ex] 
	 \hline\hline
	 Transaction Block Size & 228 transactions \\
	 Voter Block Size & 1000 votes \\
	 Proposer Block Size & 7000 references \\
	 Voter Chains ($m$) & 1000 \\
	 Transaction Mining Rate & 350 Blocks/s \\
	 Voter Mining Rate & Table~\ref{table:prism-beta}\\
	 Proposer Mining Rate & Table~\ref{table:prism-beta}\\
	 \hline
	\end{tabular}
	%}
\label{table:prism-params}
\end{table}

\begin{table}[t]
	\centering
	\caption{Mining rate $f$ of proposer and voter blocks for different $\beta$ in \prism. The unit is Blocks/s.}
	%\resizebox{\columnwidth}{!}{
	\begin{tabular}{ r | c } 
	 \hline
	 $\beta$ & Mining Rate ($f$) \\ [0.5ex] 
	 \hline\hline
	 0.20 & 0.535 \\
	 0.33 & 0.185 \\
	 0.40 & 0.097 \\
	 0.42 & 0.081 \\
	 0.43 & 0.069 \\
	 0.44 & 0.054 \\
	 \hline
	\end{tabular}
	%}
\label{table:prism-beta}
\end{table}


\begin{table}[t]
	\centering
	\caption{Parameters of \algorand. Block Size: number of transactions in a block. Assembly Time: maximum time spent on assembling a block (this limit was never hit in the experiment). $\lambda$: expected time to reach consensus on block hash. $\Lambda$: expected time to reach consensus on the actual block. Detailed definition in~\cite{algorand}.}
	%\resizebox{\columnwidth}{!}{
	\begin{tabular}{ r | c | c | c } 
	 \hline
	 Block Size & Assembly Time (s) & $\lambda$ (s) & $\Lambda$ (s) \\ [0.5ex] 
	 \hline\hline
	 1287 & 0.5 & 0.6 & 1.6 \\
	 4366 & 0.8 & 1.2 & 3.0 \\
	 8733 & 1.6 & 1.9 & 6.5 \\
	 13100 & 1.6 & 1.9 & 10.0 \\
	 17294 & 1.6 & 2.0 & 13.0 \\
	 21504 & 1.9 & 2.3 & 16.0 \\
	 42334 & 3.5 & 3.9 & 38.0 \\
	 64614 & 5.0 & 5.4 & 56.0 \\
	 85513 & 7.0 & 7.4 & 73.0 \\
	 85836 & 7.0 & 7.4 & 68.0 \\
	 103004 & 8.4 & 8.8 & 84.0 \\
	 116580 & 9.5 & 9.9 & 99.0 \\
	 133766 & 11.0 & 11.4 & 110.0 \\
	 \hline
	\end{tabular}
	%}
\label{table:algorand-params}
\end{table}

\begin{table}[t]
	\centering
	\caption{Parameters of \bng.}
	\begin{tabular}{ r | c } 
	 \hline
	 Parameter & Value \\ [0.5ex] 
	 \hline\hline
	 Key Block Mining Rate & 0.10 Block/s \\
	 Micro Block Interval & 15000 $\mu\text{s}$ \\
	 Block Size & 500 transactions \\
	 \hline
	\end{tabular}
\label{table:bng-params}
\end{table}

\begin{table}[t]
	\centering
	\caption{Mining rate $f$ for different $\beta$ and block sizes in the longest chain protocol. Here block sizes are in terms of transactions.}
	%\resizebox{\columnwidth}{!}{
	\begin{tabular}{ r | r | c } 
	 \hline
	 $\beta$ & Block Size & Mining Rate ($f$) \\ [0.5ex] 
	 \hline\hline
	 \multirow{8}{*}{0.20} & 10 & 0.404 \\
	                       & 260 & 0.262 \\
	                       & 1000 & 0.221 \\
	                       & 4000 & 0.144 \\
	                       & 10000 & 0.110 \\
	                       & 20000 & 0.079 \\
	                       & 60000 & 0.064 \\
	                       & 200000 & 0.027 \\
	 \hline
	 \multirow{4}{*}{0.33} & 10 & 0.168 \\
	                       & 260 & 0.117 \\
	                       & 1000 & 0.119 \\
	                       & 4000 & 0.065 \\
	 \hline
	\end{tabular}
	%}
\label{table:lc-params}
\end{table}






==> Prism Systems Paper (CCS)/design.tex <==
\section{System Implementation}
\label{sec:design}
% So far, we have established that Prism achieves a natural scaling of both the throughput and latency of Nakamoto consensus. However, 
An end-to-end cryptocurrency system based on the \prism structure is significantly more complex than one based on a single longest chain. 
This makes it challenging to design and implement a client software that can approach physical network limits without encountering other bottlenecks (e.g I/O). 
% In this section, we quickly look at some of these complexities, while deferring detailed description of the protocol to \S\ref{sec:pseudocode} in the  appendix. 
In this section, we describe the design and implementation of the \newprism client, the first client that achieves high-throughput and low-latency PoW consensus.
% the system in the next section.

% \smallskip \noindent
% \textbf{Mining.}\label{sec:mining} In Prism, miners should not be able to choose \emph{a priori} which type of block they are mining; this is essential for the security of the scheme, since otherwise the adversary could concentrate all of its power on a subset of block trees and overpower them.
% \emph{Cryptographic sortition} is used to ensure that miners cannot choose which type of block they mine.
% Nodes combine the contents of the transaction block, the proposer block, and the $m$ voter blocks (one for each voter chain) they are mining into a \emph{superblock} and perform proof-of-work mining on it.
% We divide the range of a valid proof of work into $m+2$ sections, each corresponding to one type of block.
% The concrete type \textbf{T} of a superblock is then decided by looking at which section its proof-of-work falls into.
% Here, the proof-of-work value essentially serves as a random oracle % \ly{please confirm it is technically correct.}
%  that dictates the type of a mined block.
% However, there is still one more problem: once we know the concrete type \textbf{T} of a superblock, we want it to contain only the content of type \textbf{T} but not other types, otherwise we will waste bandwidth. As a solution, miners summarize the contents of the $m+2$ consisting blocks using a Merkle tree and perform mining on the Merkle root instead of on the plain hash of the combined content. When the concrete type \textbf{T} of the superblock is decided, the miner keeps only the content of type \textbf{T} and inserts a Merkle proof to show that the miner have committed to this particular content when the block is mined.

% \smallskip \noindent
% \textbf{Ledger Formation.}\label{sec:confirmation} Prism achieves high throughput in part by mining multiple transaction blocks simultaneously and allowing all of them to contribute to the final ledger. 
% A key consequence is that transaction blocks mined concurrently may contain redundant or conflicting transactions.
% If Prism were to discard blocks that contain inconsistent transactions, it would needlessly reduce throughput by not confirming the transactions that \emph{are} consistent.
% % This would also slow down transaction confirmation, because it means 
% To prevent this, Prism separates the process of confirming blocks and forming a ledger.
% This is a key difference between Prism and many other blockchain protocols. The key observation is that given a confirmed leader sequence of proposer blocks, the ordering of transaction blocks is uniquely determined. This gives us a total ordering of transactions since the beginning of the protocol, and enables us to determine the validity of each individual transactions by executing them following this ordering. For example, among transactions that try to spend the same coin, only the first is considered valid.

% \smallskip \noindent
% \textbf{Spam Mitigation.}
% \label{sec:spamming-design}
% In Prism, miners do not validate transactions before including them in blocks.
% This introduces the possibility of spamming, where an adversary could generate a large number of conflicting transactions and send them to different nodes across the network.  
% The nodes would then mine all of these transactions into blocks, causing miners and validators to waste storage and computational resources (we note that transaction fees alone cannot prevent such spamming: since   nodes only pay for transactions that make it to into the ledger, the adversary would not be charged for conflicting transactions that get removed during sanitization). 
% %spam/duplicate transactions
% % There are a few practical mechanisms for circumventing this. 
%  Bitcoin is not susceptible to this attack because transactions are  validated  {\em prior} to block creation. 
% We propose a simple mechanism to mitigate spamming. Miners validate transactions with respect to their latest ledger state and other unconfirmed transactions, giving the adversary only a small window of network delay to spam the system. 
% This then allows miners to mitigate spamming attacks by adding a random timing jitter prior to mining transactions, thus increasing the chance that a miner can detect that a conflicting transaction is already present in a transaction block, in  which case it will choose to not include that transaction.
% We evaluate the effectiveness of this method in \S\ref{sec:spamming-eval}.


==> Prism Systems Paper (CCS)/design2.tex <==
\section{Design}
\label{sec:design}

% \vb{ A possible notation is to use capital letters for tuples and small letters otherwise. Header $H$, Content $C$, Block $B=(H,C)$.
% $H=(P,n,D)$, $P$ is the content, $n$ is nonce and $D$ is $\texttt{digest}(C)$.
% Tx block $B^T$, Tx header $H^T$, Tx parent $P^T$, Tx digest $D^T$ and Tx content $C^T$ (similar for prop. and voter block). $B \in \{B^T, B^P, B^V\}$ and so on..}

\subsection{Notation}
\label{sec:blocktypes}
Each block $B=(H,C)$ is a tuple containting a header $H$ and content $C$.
As discussed in  \S\ref{sec:overview}, there are three types of blocks: transaction blocks, proposer blocks,  and voter blocks.
In all three types, the header $H=(P, n, D)$ is a tuple containing: (1) the hash $P$ of the parent block,
%(\vb{conceptually parent blocks also differ}) \ma{seems ok to me} 
(2)  a valid PoW nonce $n$, and (3) a content digest $D=\texttt{Digest}(C)$. % proving that the block was mined in the correct category (transaction, proposer, or voter). 
We add a superscript to the above notations to denote the type of block being referred. 
For example, we refer  to proposer blocks by $B^P$, transaction blocks by $B^T$, and voter blocks by $B^V$.
% Along the same lines, a proposer block's header, content, and parent are denoted by $H^P$, $C^P$, and $P^P$, respectively, and its content digest by $D^P$.

% The nonce $n$ and content digest $D$ are explained further in the mining procedure (\S\ref{sec:mining}).

%\todo{I intentionally did not  describe what is actually done in the code w.r.t. parent blocks because I think it may confuse people more. Let me know what you think.}
% \ma{I think this is at the right level}

%\paragraph{Transaction blocks.}
% \smallskip
% \noindent{\bf Transaction blocks.}
% Transaction blocks do not need a parent block,  so  $P^T=\emptyset$.
% The content of a transaction block is an ordered list of transactions: $C^T := [t_1, \ldots, t_m]$.
% drawn from the miner's local a memory pool \texttt{mempool} of transactions that have not yet been  incorporated into a transaction block.
% Note that a transaction $t$ is a payment from a sender's public key to a recipient's public key, signed by the sender. 
% \gw{Do we want to mention about multiple senders and recipients?}


% They contain a list of transactions, and a pointer to a parent proposer block. \ma{why do transaction blocks need a pointer to a proposer block? this is also not shown in in Fig. 4} \ma{It might be useful to define a transaction, e.g., it is a payment from a sender public key to a recipient public key, signed by the sender}

% \vb{Below we have described both the content and the mining procedure of the proposer and voter blocks. We can explicitly state that perhaps} \ma{I think this is ok} 

% \smallskip
% \noindent{\bf Proposer blocks.}
% Since the proposer tree is built in a longest-chain fashion, proposer blocks choose as their parent $P^P$  the tip of the longest chain in the proposer tree. 
% Each proposer block's content, $C^P$, is an ordered list of references to other proposer and/or transaction blocks.  
% We compute $B$'s set of \emph{ancestors} by following the chain of parent links in the proposer tree.
% For proposer block $B$, let $C^P_1 =[B^P_{i_1}, B^P_{i_2}, \ldots]$ denote an ordered list of proposer blocks that are neither indirectly referenced or among content of $B$'s ancestors.
% Let $C^P_2 = [B^T_{j_1}, B^T_{j_2},\ldots]$ denote an ordered list of transaction blocks that are not referenced (directly or indirectly) by any of $B$'s ancestors or by any of the proposer blocks in $C^P_1$.
% The content of the proposer block is the concatenation of these two ordered lists: $C^P  :=(C^P_1, C^P_2)$.
% Note that $C^P$ actually stores references to the listed blocks, but we describe them as blocks here to reduce notation.
% Honest nodes mine proposer blocks on the longest chain in the proposer blocktree, but the longest chain does not determine the final confirmed sequence of proposer blocks, known as the  \emph{leader sequence}. 
% We define the \emph{level} of a proposer block as its distance from the genesis block (Figure \ref{}), and the \emph{height} of the proposer tree as the maximum level that contains any proposer blocks. 
% The confirmed leader sequence of proposer blocks contains one block at every level up to the height of the proposer blocktree, and is  determined by the \emph{voter trees}. 
% \smallskip
% \noindent{\bf Voter blocks.}
% There are $m$ voter trees, where $m \gg 1$ is a fixed parameter chosen by the system designers. 
% The $i^{th}$ voter tree is comprised of voter blocks that are mined on the longest chain of the voter tree. 
% Voter trees are also  built in a longest-chain fashion,  so for a voter block  $B^{V_i}$ in the $i^{th}$ voter tree,  its parent $P^{V_i}$ is the tip of the longest chain in the $i^{th}$ voter tree.
% The block's contents $C^{V_i}$ are a list of references to proposer blocks, or \emph{votes}.
% Recall that the \emph{level} of a proposer block denotes its distance from the genesis block, and the \emph{height} $h$ of the proposer tree is the maximum level that contains any proposer blocks.
% Let $L=\{1,\ldots, h\}$ denote the set of all levels in the proposer blocktree.
% Voter trees are built in a longest-chain fashion; each voter tree's longest chain is allowed to vote at most once on any level in  $L$.
% For a voter block $B^V$, let $\ell'_{B}$ be the latest level of proposer block voter by $B^V$'s ancestors and thus $B^V$ has to vote on levels $\{\ell'_{B}+1,\cdots,h\}$.
% % let $L'_{B}$ denote the set of levels that have already been voted on by $B$'s ancestors. (\vb{$L'_{B}$ is a continuous set. To simplify the notation we can say that `for voter block $B$, let $\ell'_{B}$ be the latest level of proposer block voter by $B$'s ancestors and thus $B$ has to vote on levels $\{\ell'_{B}+1,\cdots,h\}$})
% % Let $L_{B} = L \cap L'_{B}$ be the set of remaining levels, and let $\mathcal P_i$ denote the set of proposer blocks at level  $i$. \gw{You mean $L - L'_B$?}
% The content of the voter block, $C^V := [B^P_{\ell'_{B}+1},\ldots,B^P_{h}]$ is a list of proposer blocks where with some abuse of notation, $B^P_{\ell}$ denotes a vote for  (pointer to) a proposer block at level $\ell$. 
% In words,  the voter block contains a list of one vote per unvoted level in the block's ancestor list. 
% \ma{It seems we can simplify this description per Vivek's suggestion} \vb{done}
% this list includes at most one pointer to a proposer block at every level of the proposer blocktree that has not yet been voted on by any of $B$'s ancestors in the $i$th voter tree. 
% We call such a pointer a \emph{vote}, since it is effectively endorsing a given proposer block. 
% In other words, each voter tree is allowed  at most one vote for each level of the proposer tree, where only the votes contained in the longest chain of each voter tree are counted. 
% We explain how these votes are used to confirm transactions in Section \ref{sec:confirmation}


% \todo{Mention database, mempool, etc. data structures as well. These will be discussed in more detail in the Implementation subsection, but we just explain what they are here so that the pseudocode makes sense. }

% \subsection{Protocol}
% The protocol has two primary components: mining and ledger formation. 

% \ma{One thing that would be good to mention is that the lists in the different blocks have bounded length. Perhaps discuss how a block picks among its options when the list doesn't fit everything.}
% \vb{The list of different blocks will vary in length but for simplicity we can leave it unbounded. In expectation, the size of the list is $1$.}

\subsection{Mining}
\label{sec:mining}
Miners should not be able to choose \emph{a priori} which type of block they are mining; this is essential for the security of the scheme, since otherwise the adversary could concentrate all  of its power on a subset of block trees and overpower them. 
\emph{Cryptographic sortition} is used to ensure that miners cannot choose which type of block they mine.
Nodes simultaneously mine one transaction block, one proposer block, and $m$ voter blocks (one for each tree). 
Only after a valid proof of work is found does the miner learn if the mined block is a transaction, proposer, or voter block. 
The mining process has three steps (four including validation): 

\noindent \textbf{(1) Superblock generation.} 
When a miner starts mining, it creates a \emph{superblock} that simultaneously contains the parents and contents for all $m+2$ possible sub-blocks (1 transaction sub-block, 1 proposer, and $m$ voter sub-blocks). The parents and contents differ for each type of block.
This superblock is updated whenever the miner receives a new network message that changes either the header or the content of any of the sub-blocks. 

\emph{Transaction sub-block $B^T$:} 
%The miner chooses a parent $R_{B^T}$ as described in Section  \ref{sec:blocktypes}. 
Transaction blocks do not need a parent block,  so  $P^T=\emptyset$.
The content of a transaction block, $C^T$, is an ordered list of transactions,  drawn from a data structure similar to the Bitcoin \texttt{mempool}, except in Bitcoin, \texttt{mempool} stores all transactions that have not yet been included in the main chain; in Prism, once a transaction is included in a valid transaction block, it is permanently removed from the \texttt{mempool}.
This is because the transaction block (hence its contained transactions), is guaranteed to eventually be included in the ledger (\S\ref{sec:confirmation}).
Upon receiving a new transaction block over the network, the miner should remove the transactions in the new block from its own mempool and transaction block content. 

\emph{Proposer sub-block $B^P$:} 
Proposer tree is built in a longest-chain fashion; proposer blocks choose as their parent $P^P$  the tip of the longest chain in the proposer tree. 
Each proposer block's content, $C^P  :=(C^P_1, C^P_2)$, is an ordered list of references to other proposer and transaction blocks, where
$C^P_1$ is an ordered list of proposer blocks that are neither referenced nor among content of $B^P$'s ancestor block\footnote{ Ancestor blocks are computed by following the chain of links from $B^P$ in the prop. tree.}, and
 $C^P_2$ is an ordered list of transaction blocks that are not referenced (directly or indirectly) by any of $B^P$'s ancestors or by any of the proposer blocks in $C^P_1$.
% Note that $C^P$ actually stores references to the listed blocks.
A miner updates content $C^P$ upon receiving a new transaction block or a new proposer block. 
% The miner chooses a parent $P^P$ and block contents $C^P$ as described in  \S\ref{sec:blocktypes}. 
% That  is, miners store a list of references to proposer and transaction blocks that have not been referenced by any other proposer blocks in $B^P$'s ancestry. 
% In the former case, it can choose to add a reference to the new transaction block to the miner's proposer block content.
% In the latter case, if the newly-received proposer block is at the same level as the miner's in-progress block, the miner should update the in-progress proposer block's parent so as to extend the longest chain and also update the content $C^P$.
%(\vb{and the content?)} \ma{yep, i think it should be `parent and content'}. 

\emph{Voter sub-block $B^{V_i}$ in the $i^{th}$ voter tree:} 
Voter trees are also  built in a longest-chain fashion; the  parent of voter block  $B^{V_i}$, $P^{V_i}$, is the tip of the longest chain in the $i^{th}$ voter tree.
The content, $C^{V_i}$, is a list of references to proposer blocks, or \emph{votes}.
% , and the \emph{height} $h$ of the proposer tree is the maximum level that contains any proposer blocks.
Each voter tree's longest chain is allowed to vote at most one proposer block on any level\footnote{
Level of a proposer block is its distance from the genesis block.} of the proposer tree.
Let $h$ denote the last level in the proposer blocktree and $\ell_B$ denote the last level voted by $B_{V_i}$'s ancestors.
% For a voter block $B^{V_i}$, let $\ell'_{B}$ be the latest level of proposer block voter by $B^{V_i}$'s ancestors and thus $B^{V_i}$ has to vote on levels $\{\ell'_{B}+1,\cdots,h\}$.
% let $L'_{B}$ denote the set of levels that have already been voted on by $B$'s ancestors. (\vb{$L'_{B}$ is a continuous set. To simplify the notation we can say that `for voter block $B$, let $\ell'_{B}$ be the latest level of proposer block voter by $B$'s ancestors and thus $B$ has to vote on levels $\{\ell'_{B}+1,\cdots,h\}$})
% Let $L_{B} = L \cap L'_{B}$ be the set of remaining levels, and let $\mathcal P_i$ denote the set of proposer blocks at level  $i$. \gw{You mean $L - L'_B$?}
Then the content of the voter block $B^{V_i}$ is $C^V := [B^P_{\ell'_{B}+1},\ldots,B^P_{h}]$, list of proposer blocks where with some abuse of notation, $B^P_{\ell}$ denotes a vote for  (pointer to) a proposer block at level $\ell$. 
In words,  the voter block contains a list of one vote per unvoted level in the block's ancestors. 

% The miner chooses a parent $P^{V_i}$ as described in   \S\ref{sec:blocktypes}. 
% Its content $C^{V_i}$  is references to one proposer block on each level that have not yet been voted on by any of its ancestors. 
% \ma{Feels a bit repetitive with 4.1, but i think it's OK}
By default, nodes will vote for the first proposer block they see at a given level.
Notice that the content $C^{V_i}$ is updated if the miner receives either a new proposer block at a previously-unseen level or a new voter block for the $i^{th}$ tree that changes the longest chain of that voter tree. 
In  the former case, the miner adds a vote for that level. 
In the latter case, the miner updates its parent block $P^{V_i}$ so as to extend the longest chain and also updates the content $C^{V_i}$.
All the contents and parent links are concatenated into a superblock $B=(H,C)$ with header 
$H=(P:=[P^T,  P^P, P^{V_1}, \ldots, P^{V_m}], n, D)$ 
% \ma{nit. do we need the $\emptyset$?} \vb{nope..}
and content 
$ C := [ C^T, C^P, C^{V_1}, \ldots, C^{V_m}]$.
The content digest $D$ is explained next.


\noindent \textbf{(2) PoW and sortition.}
Once the superblock is formed, the miner mines by searching for a nonce $n$ such that $Hash( H)\leq q$, where $Hash(\cdot)$ denotes a hash function, and $q$ denotes a difficulty threshold. 
For a one-way hash function, the miner can do no better than brute-force search, so it cycles through difference values of nonces $n$ until  finding one such that $Hash(H) \leq q$. Upon finding a valid nonce,  sortition  occurs. 
We divide the numbers from $0$ to $q$ into regions corresponding to different block types. 
For example, $[0,q_T]$ denotes a transaction block, $[q_T+1,q_P]$ denotes a  proposer block, and $[q_P+1,q]$ denotes voter blocks,  split evenly into  $m$ regions, one per voter tree.
The output region of $Hash(H)$ determines the block type.


\noindent \textbf{(3) Block pruning.}
Passing around a large superblock after mining would waste unnecessary bandwidth. 
Hence, to improve space efficiency, instead of using the full concatenated parent block and content lists, only the relevant content is retained after mining and the type of the block is known.
For example, a mined proposer block would contain only the proposer parent reference , $P^P$, and proposer content, $ C^P$; it would \emph{not} store transactions or votes.
However,  if we do this naively, block validators would not be able to tell if the cryptographic sortition was correctly executed.
To address this, we alter our header to contain the following:
$H=\left(\textsf{MerkleRoot}(P), n, D := \textsf{MerkleRoot}(C)\right)$, 
 where $\textsf{MerkleRoot}(\cdot)$ denotes the Merkle root of a Merkle tree \cite{merkle} 
%  \ma{cite something for Merkle tree} 
generated from the contained array.
%To avoid the overhead of including all $m+2$ parents and content hashes in every block, Prism block headers contain: a) the Merkle root of a tree with $m+2$ parent blocks, b) the Merkle root of a tree with $m+2$ contents, and c) a nonce. \gw{"a)" is different from our implementation. In implementation, every block has a proposer parent. And every voter block has a voter parent which is stored inside content.}
%Upon finding a valid nonce, the hash of the block deterministically determines if the block is a proposer block, a transaction block, or a voter block on one  of the $m$ voter trees.  
%The mined, sortitioned block includes a header, the appropriate parent and content for the soritioned block type, and the respective Merkle proofs.
In addition to the pruned content and header, we include \textit{sortition proofs}, Merkle proofs attesting to the fact that the block  was mined correctly.
In our proposer block example, the Merkle proof would include the sibling node for every  node in the path from the proposer content $C^P$ to the root $\textsf{MerkleRoot}(C)$ in the Merkle tree. 
Hence $\textsf{MerkleProof}( C)$ (resp. $\textsf{MerkleProof}(P)$) is an array of  size $\log_2 (m)$ -- a primary source of storage overhead in Prism blocks. 


\noindent \textbf{(4) Block validation.}
Upon  receiving a mined Prism block $B=(H,C)$, a validator checks two things. 
First, it  checks that $Hash( H) \leq q$ and that the cryptographic sortition is correct  (i.e., that the hash  maps to the correct region for the block type).
Next, it checks the sortition proof.  
To do this, it takes content $C$ (resp. parent) in  the block, and ensures that the Merkle proof validation gives the content (resp. parent) digest in the header \cite{merkle}. 
% \ma{This is perfect}


\begin{figure}
   \centering
   \includegraphics[width=\linewidth]{figures/ledger_generation.png}
   \vspace{-5mm}
    \caption{\small Ledger formation has three parts:  
   (1)  confirming a leader  sequence of proposer blocks;
   (2)  creating a list  of transactions;
   and (3) sanitizing the transaction list for conflicts. 
   In this figure, each transaction  block has only one transaction; suppose transactions  (c) and (d) are inconsistent (e.g., a double spend).
   A proposer block's black reference link denotes a parent link. 
    Blue links denote reference links; a proposer block can include reference links to transaction blocks as well as proposer blocks.}
   %   \gw{A typo: unrefererred $\to$ unreferred? Do we need to use the word unrefererred? Referred blocks are okay in links.}
%   Each shade of grey corresponds to an epoch. In Step 1 (line:\ref{code:txbksOrdering}), all the transaction blocks are incorporated, and in Step 2 (line:\ref{code:sanitizeLedger}), they are combined to build the ledger.
   \label{fig:leader_ledger}
    \vspace{-5mm}

 \end{figure}


\subsection{Ledger Formation}
\label{sec:confirmation}
% Unlike many blockchain designs, Prism allows transactions to be confirmed before they are ordered. 
% This is possible because confirmation is often an easier task than ordering. 
% For example, consider the following two transactions: a) Alice pays Bob 10\$, and b) Carol pays Drake 10\$. Both these transactions can be individually confirmed without deciding which transaction occurred first.
% The decision to separate transaction confirmation from ordering helps Prism achieve low latency. 
% However, as a result, conflicting or duplicate transactions can become part of the blockchain; these conflicts must be eliminated during transaction ordering (i.e., during ledger formation). 
% % It handles such conflicts by separating the process of confirming blocks and that of generating a ledger from the set of confirmed blocks. 
% % Without it, blockchains must maintain a single, self-consistent sequence of blocks; this causes simultaneously-mined blocks to be wasted, while slowing down the generation of the ledger. 
% % We separately discuss the two procedures of block confirmation and ledger formation. 

% \paragraph{Transaction confirmation}
Prism achieves high throughput in part by mining multiple transaction blocks simultaneously and allowing all of them to contribute to the final ledger. 
A key consequence is that blocks mined concurrently may contain redundant or conflicting transactions.
If Prism were to discard blocks that contain inconsistent transactions, it would needlessly reduce throughput by not confirming the transactions that \emph{are} consistent.
% This would also slow down transaction confirmation, because it means 
To prevent this, Prism separates the process of confirming blocks and forming a ledger. 
This is a key difference between Prism and many other blockchain protocols.
% Since the same transaction can appear in multiple Prism transaction blocks \ma{we need to give more context about why this is a problem. it's all about having a large number of transaction blocks in flight at the same time, so it's fundamentally impossible for a miner to know that a transaction it is mining has not already been included in some other transaction block by another miner}, transaction confirmation is not necessarily the same thing as transaction block confirmation. 
The formation of a ledger in Prism  occurs in three steps, as shown in Figure \ref{fig:leader_ledger}. 

\noindent{\bf (1) Proposer block confirmation.}
First, we must confirm a contiguous sequence of leader proposer blocks at each level.  
    Recall that the proposer block with the most votes on level $\ell$ is defined as the \textit{leader block} at level $\ell$, and the sequence of leader blocks for each level of the proposer tree is defined as the {\em leader sequence}. 
Once we can guarantee that this leader sequence is permanent for all levels up to some level $\ell$ with probability at least $1-\epsilon$, where $\epsilon$ is the target reversal probability, we can confirm a leader block sequence. This process is described in more detail below.

\noindent{\textbf{(2) Transaction  ordering.}}
    Given a proposer block leader sequence, we iterate over the sequence and list the referred transaction blocks in the  order they are referred. 
    We use $L_i$ to denote the leader at level $i$. 
    In Figure \ref{fig:leader_ledger}, we  start  with the leader at level 1 $L_1$, the left proposer block.
    $L_1$ refers to only one transaction  block containing transaction $a$, so our ledger starts with $a$.
    Next, we consider $L_2$. It starts by referring to its parent, the right proposer block at level 1.
    Since that proposer block has not yet been included in the ledger, we include its referred transactions---namely, $a$ and $b$. 
    $L_2$ then adds $L_1$, followed by transaction blocks containing $d$ and $c$, in that order.
    Since $L_1$ was already added to our ledger, we ignore it, but add $d$ and $c$.
    This process continues until we reach the end of our leader sequence.

\noindent{\textbf{(3) Ledger sanitization.}} In the previous step, we may have added redundant or conflicting transactions. 
    Hence, we now execute the transaction list in the previously-specified order. Any duplicate or invalid transactions are discarded. 
    In Figure~\ref{fig:leader_ledger}, we discard the second instance of $a$ (since it's a duplicate), and we discard $c$ (since it conflicts with $d$).

\if 0
\begin{enumerate}
    \item  \textbf{Proposer block confirmation.} First, we must confirm a contiguous sequence of leader proposer blocks at each level.  
    Specifically, the proposer block with the most votes on level $\ell$ is defined as the \textit{leader block} at level $\ell$. 
% This phenomenon is at the core of \schemenosp's security.
The sequence of leader blocks for each level of the proposer blocktree is defined as the {\em leader sequence}. 
Once we can guarantee that this leader sequence is permanent for all levels up to some level $\ell$ with probability at least $1-\epsilon$, we can confirm a leader block sequence. This process is described in more detail below.
    \item \textbf{Transaction  ordering.} 
    Given a proposer block leader sequence, we iterate over the sequence and list the referred transaction blocks in the  order they are referred. 
    We use $L_i$ to denote the leader at level $i$. 
    In Figure \ref{fig:leader_ledger}, we  start  with the leader at level 1 $L_1$, the left proposer block.
    $L_1$ refers to only one transaction  block containing transaction $a$, so our ledger starts with $a$.
    Next, we consider $L_2$. It starts by referring to its parent, the right proposer block at level 1.
    Since that proposer block has not yet been included in the ledger, we include its referred transactions---namely, $a$ and $b$. 
    $L_2$ then adds $L_1$, followed by transaction blocks containing $d$ and $c$, in that order.
    Since $L_1$ was already added to our ledger, we ignore it, but add $d$ and $c$.
    This process continues until we reach the end of our leader sequence.
    \item \textbf{Ledger sanitization.} In the previous step, we may have added redundant or conflicting transactions. 
    Hence, we now execute the transaction list in the previously-specified order. Any duplicate or invalid transactions are discarded. 
    In Figure \ref{fig:leader_ledger}, we discard the second instance of $a$ (since it's a duplicate), and we discard $c$ (since it conflicts with $d$).
\end{enumerate}

\fi
   
%   (3) Iterate over the transactions ledger and \emph{sanitize} it by  removing all  transactions  that conflict with a prior transaction.

% Ultimately, transaction confirmation hinges on confirmation of the proposer blocks that refer to transaction block(s) containing the transaction.
% A transaction block is confirmed once a proposer block pointing to the transaction block is confirmed.
% We thus start by explaining the confirmation of proposer blocks, then explain how this leads to transaction confirmation.


% Specifically, the proposer block with the most votes on level $\ell$ is defined as the \textit{leader block} at level $\ell$. 
% % This phenomenon is at the core of \schemenosp's security.
% The sequence of leader blocks for each level of the proposer blocktree is defined as the {\em leader sequence}. 
% Once we can confirm a contiguous leader sequence, e.g. at levels $1,\ldots, \ell$ with our desired reliability $1-\epsilon$, we can confirm an ordered ledger of transactions. 
% This ledger is formed by iterating over the sequence, and for each leader block, looping over all the transaction blocks referenced within. 
% The list of transactions from each transaction block is added sequentially to the ledger; each transaction's validity is checked for validity (e.g., double spends) and duplicate entries (since the same transaction can be added to multiple transaction blocks). 
% This process is illustrated in Figure \ref{fig:leader_ledger}. \ma{I don't really like Fig. 6. It would be better to create an example which actually shows duplicate transactions and double spends after the ordering step, and than shows the sanitized ledger. BTW, the step of going from ordered transaction blocks to order transactions doesn't seem that important (it's pretty obvious). But the most important point is that you have to do sanitization, and this has to be done after transactions are ordered. }


%\paragraph{Proposer block confirmation.} 
\smallskip
The key to the above confirmation process is leader proposer block confirmation (step 1).
The leader block at a given level $\ell$ can initially fluctuate when the voter trees start voting on level $\ell$. 
However, as the voter trees grow, votes on level $\ell$ are embedded deeper into their respective voter trees, which (probabilistically) prevents the votes from being reverted.
% A leader proposer block at a given level $\ell$ is confirmed based on the votes of the voter trees. 
Hence, we can confirm the leader block when: (1) a plurality of voter trees have voted for it, and (2) that plurality is guaranteed not to change with probability at least $1-\epsilon$, where $\epsilon$ is a user-selected target reversal probability.

%Because there are many voter trees, each individual voter tree needs  only a weak confirmation guarantee to still give a strong confirmation guarantee to the aggregate majority vote. 
% \gw{Do we need to define what is weakly confirm?}

Our confirmation procedure calculates this probability by computing a $(1-\epsilon)$-confidence interval over the number of votes on each leader block, as well as a hypothetical ``private'' block that has not yet been released by a hypothetical adversary that controls a fraction $\beta$ of the hash power. 
Once the leader block's confidence interval is strictly larger than any of the other candidates' confidence intervals, we can be sure (with probability at least $1-\epsilon$) that the current leader will remain the leader for all time, so we confirm that proposer block. 
The details of this confidence interval calculation are included in Appendix~\ref{apx:confirmation}.

\subsection{Spam Mitigation}
\label{sec:spamming-design}

In Prism, miners do not validate transactions before including them in blocks.
This introduces the possibility of spamming, where an adversary could generate a large number of conflicting transactions and send them to different nodes across the network.  
The nodes would then mine all of these transactions into blocks, causing miners and validators to waste storage  and computational  resources.\footnote{While a discussion of incentives is beyond the scope of this paper, it is important to note that fees alone cannot prevent such spamming. Assuming nodes only pay for transactions that make it to into the ledger, the adversary would not be charged for conflicting transactions that get removed during sanitization.}
%spam/duplicate transactions
% There are a few practical mechanisms for circumventing this. 
Notice that protocols like the longest chain are not susceptible to this attack because transactions are validated prior to block creation. 
We propose a simple mechanism to mitigate spamming. Miners validate transactions with respect to their latest ledger state and other unconfirmed transactions, giving the adversary only a small window of network delay to spam the system. 
This then allows miners to mitigate spamming attacks by adding a random timing jitter prior to mining transactions, thus increasing the chance that a miner can detect that a conflicting transaction is already present in a transaction block, in  which case it will choose to not include that transaction.
We evaluate the effectiveness of this method in \S\ref{sec:spamming-eval}.

% \smallskip


%We believe such practical countermeasures will be important in  practical settings.
%mitigations:  jitter,  mempool optimization, sortition? 

%\ma{more generally, i think we need to expand this section to explain the important parts of the design in more detail. I don't think the long pseudocode blocks are that helpful. no one will read them, and they don't distinguish the important stuff from the mundane. let's remove the pseudocode to make room to expand on things like: (1) more formal description of block contents (a diagram might help); (2) what exactly is the proof of work puzzle in prism; (3) how does sortition work; (4) how do you get the final block that is sent over the network; (5) how do we get a ledger from all these blocks; (6) how does transaction confirmation work; how and why is it different from bitcoin. there might be other stuff worth mentioning, but we should ideally describe at least each of these points at a decent level of detail} 




% Consider a proposer block sequence from levels $1$ to $\ell$, $\{p_1,\cdots,p_{\ell}\}$, represented by blue blocks in Fig. \ref{fig:leader_ledger}(a).
% Let $L_{p_i}$, represented by green blocks in the grey shaded area in Fig. \ref{fig:leader_ledger}(a), be an ordered list of all the transaction blocks directly or indirectly referred by block $p_i$. 
% Let $\{L_{p_1}, \cdots, L_{p_{\ell}}\}$ be the \textit{transaction block list} of sequence $\{p_1,\cdots,p_{\ell}\}$ as shown in Fig. \ref{fig:leader_ledger}(b). 
% We consider this transaction block list confirmed once each proposer block in the underlying sequence is confirmed. 
% Our proposer block confirmation policy is a simplified version of the policy from \cite{prism}. 
% To confirm a proposer block as leader with reliability parameter $\epsilon$, we consider the votes from all $m$ voter trees. 
% Each voter tree has some maximum probability of ending up with a vote against the block at level $1\leq i \leq \ell$.
% Once we


% While confirming a leader block can take time, 
% we quickly narrow down a set of proposer blocks, defined as the \textit{proposer set}, which is guaranteed probabilistically to contain the eventual leader block for that level. 
% The proposer set is defined as in \todo{XXX--HOW MUCH DETAIL DO WE WANT TO GO INTO? }
% % This procedure first gets all the votes from the voter trees and then gets the proposer set for each 
% % level from the genesis to the last level for which the proposer set can be realized (lines:\ref{code:getvotes_start}-\ref{code:appendPrpList}). 
% Upon  defining a proposer set for each realizable level, Prism takes an outer product of all the proposer sets to  enumerate the set of all possible proposer block leader sequences (line:\ref{code:outerproduct}). 
% Note that by design, one of these sequence will eventually be the leader block sequence.
% It then builds a ledger for each of these proposer block sequences and confirms the given transaction if it is present in \textit{all} of these ledgers (lines:\ref{code:ledgers_for_start}-\ref{code:fastConfirmTx}). 



% \textit{Confirmation and Ordering:} A set of transactions can often be individually confirmed before being ordered among themselves. 
% For this reason, confirming transactions is easier than ordering the transactions.
% For example, consider the following two transactions a) Alice pays Bob 10\$, and b) Carol pays Drake 10\$. Both these transactions can be individually confirmed without deciding which transaction occurred first.
% In Bitcoin, transactions are simultaneously confirmed and ordered; 
% however, in Prism, transactions can be confirmed before being ordered.
% The procedure \textsc{IsTxConfirmed()} in Algorithm \ref{alg:prism_con} defines the transaction confirmation rule $g$ and the procedure \textsc{GetOrderedConfirmedTxs()} defines the rule for ordering the confirmed transactions. Both these procedures use \textsc{BuildLedger()} which is described next.



% \paragraph{Transaction Ordering}
% Once a sequence of leader blocks is confirmed, the ledger is formed by iterating over the sequence, and for each leader block, looping over all the transaction blocks referenced within. 
% The list of transactions from each transaction block is added sequentially to the ledger; each transaction's validity is checked for validity (e.g., double spends) and duplicate entries (since the same transaction can be added to multiple transaction blocks). 
% This process is illustrated in Figure \ref{fig:leader_ledger}(c). 




%\ma{let's move discussion of spamming to the discussion section}


==> Prism Systems Paper (CCS)/discussion.tex <==

\section{Discussion}
\label{sec:discussion}

% \ly{
% \begin{enumerate}
%     \item throttling
%     \item Compare with existing blockchain protocols and discuss their practicability (performance on a store-and-forward network)
% \end{enumerate}
% }

We discuss some potential extensions to \prism.


% \smallskip

 
% \smallskip
\noindent \textbf{Light clients.} 
 SPV (Simple payment verification) are short proofs~\cite{spv} to verify the validity of a given transaction (payment) for a \textit{light user} who only downloads the blocks headers in a blockchain.
In the longest chain protocol, every transaction in the block is valid so a Merkle proof of a transaction with respect to its block header proves payment validity.
However, this is not enough in \prism, where transaction blocks can potentially contain invalid transactions. We can facilitate SPV proofs in \prism by this simple modification: We store all the unspent coins in the ledger formed by leader blocks until level $\ell$ in a Merkle-Patricia tree and add the root of this tree to the proposer block(s) at level $\ell+e$ (for a large value of $e$, say $20$). Since this tree contains only unspent coins generated by valid transactions, the merkle proof of the output coins of a payment with respect to to this commit proves the validity of the payment.

% \smallskip
\noindent \textbf{Bootstrapping a new user.} 
Longest chain blockchains like Bitcoin use a small fraction of network bandwidth, so new users can simply download and process all the blocks to join the system. 
Since Prism runs near network capacity,  expecting a new user to download and process all the old blocks is not practical. 
The modification suggested in the previous paragraph can be also used to bootstrap as follows: a new user downloads all proposer and voter tree blocks (which consume less than $0.1\%$ of the capacity). Say the new user's proposer tree has confirmed leader block at level $\ell$. 
We know that this leader block stores the commit of all the unspent coins up to level $\ell-e$. 
Now the new user asks an existing user for the UTXO set for the ledger up to level $\ell-e$. The user can verify the correctness of this set by comparing it with the UTXO set commitment stored in the leader block at level $\ell$.
% \gw{"the commit of stored the leader block" contains a typo?}
This UTXO set contains all the information required from transaction blocks
% \gw{can we abbr transaction to tx?}
referred by proposer blocks until level $\ell-e$ and thus the new user can join the system by downloading full blocks starting from level $\ell-e$.



\noindent \textbf{Smart contracts.} 
 Our current implementation achieves high throughput and low latency on an UTXO based scripting layer. 
 A natural question is whether we can achieve similar performance on a smart contract layer. 
 \prism's latency depends only on the block structure at the consensus layer and is independent of the scripting layer. Thus a smart contract version of Prism will also achieve low confirmation latency. As described in \S\ref{sec:scoreboarding}, parallelizing transaction execution (via \textit{scoreboarding}) was vital in achieving high throughput. The ability to parallelize transaction execution of smart contracts will also be the key to exploit the high throughput provided by \prism consensus. 
 
 
 %%As described in section  \ref{sec:scoreboarding}, parallelizing transaction execution via \textit{scoreboarding}~\cite{scoreboarding} was vital in achieving high throughput. This technique can be extended to parallelize execution of a more generic scripting layer such as smart contracts and this is left for future work.


==> Prism Systems Paper (CCS)/eval.tex <==
\section{Evaluation}

\label{sec:eval}

Our evaluation answers the following questions:

\begin{itemize}
%\begin{itemize}[leftmargin=*]
    \item By how much does the new confirmation rule in \newprism improve the confirmation latency over \prism? (\S\ref{sec:cfm-compare})
    \item What is the performance of \newprism in terms of transaction throughput and confirmation latency, and how does it compare with other protocols? (\S\ref{sec:eval-performance})
    \item How well does \newprism scale to a large numbers of users? (\S\ref{sec:eval-scale})
    \item How does \newprism perform with limited resource, and how efficient does it utilize resource? (\S\ref{sec:eval-resource})
    %\todo{``What's the overhead of \prism in terms of CPU and network bandwidth''}
    \item How does \newprism perform when under attack? (\S\ref{sec:eval-attack})
\end{itemize}

%\smallskip

\noindent{\bf Schemes compared.} We compare the performance of \newprism with \algorand, \bng, and the longest chain protocol. We do not compare with \prism in most experiments, because its confirmation rule requires using more than 26,000 voter chains, which is impractical for real-world use. Instead, we run a targeted experiment to compare the latency of the \prism and \newprism confirmation rules under the same parameters (\S\ref{sec:cfm-compare}). For \prism, \bng, and the longest chain protocol, we modify and use our \newprism implementation. For \algorand, we use the official open-source implementation~\cite{algorandcode} written in Golang. Note that this implementation is different from the one evaluated in~\cite{algorand}. Therefore, we do not expect to reproduce the results in~\cite{algorand}.

\noindent{\bf Testbed.} We deploy our \newprism implementation on Amazon EC2's \texttt{c5d.4xlarge} instances with 16 CPU cores, 16 GB of RAM, 400 GB of NVMe SSD, and a 10 Gbps network interface. Each instance hosts one \newprism client. By default, we use 100 instances and connect them into a random 4-regular graph topology. To emulate a wide-area network, we introduce a one-way propagation delay of 120~ms on each link to match the typical delay between two distant cities~\cite{pingmeasurement}, and a rate limiter of 400~Mbps for ingress and egress traffic respectively on each instance. We also evaluate several other network topologies (up to 900 instances) and per-instance bandwidth limits.

To generate workloads for these experiments, we add a transaction generator in our testbed which continuously creates transactions at an adjustable rate. In our \newprism implementation, the main bottleneck is RocksDB and the I/O performance of the underlying SSD, which limits the throughput to about $90,000$ tps. 
We cap transaction generation rate to 80,000 tps to avoid hitting this bottleneck.

%\ly{The \algorand implementation can support at most $4,800$ tps according to our test on the same hardware. As shown later in this section, we are not bottlenecked by it. As a result, the comparison with \algorand is fair.}

%\smallskip
\noindent{\bf Performance tuning and security.} All protocols in the experiments have design parameters, and we tried our best to tune these parameters for performance and security. For \newprism, we calculate the optimal mining rate $f$ for proposer and voter blocks to achieve the best confirmation latency, given the adversarial ratio $\beta$ and desired confirmation confidence $\epsilon$. We cap the size of transaction blocks to be 40 KB, and set the mining rate for transaction blocks to support $80,000$ tps. Unless otherwise stated, we turn off the spam mitigation mechanism in \newprism (we evaluate its effectiveness in \S\ref{sec:eval-attack}).  To ensure security, we calculate the expected {\em forking rate} $\alpha$, i.e. fraction of blocks not on the main chain, given $f$ and the block propagation delay $\Delta$. We compare $\alpha$ against the forking rate actually measured in each experiment to ensure that the system has met the target security level. We follow the same process for \bng and the longest chain protocol. For \algorand, we adopt the default security parameters set in its production implementation. Then we hand-tune its latency parameters $\lambda$ and $\Lambda$. Specifically, we reduce $\lambda$ and $\Lambda$ until a round times out, and use the settings that yield the best confirmation latency. For \newprism, the longest chain protocol and \bng, we target a confirmation confidence $\epsilon$ in the order of $10^{-9}$. For \algorand, the blockchain halts with a probability in the order of $10^{-9}$.

\subsection{The New Confirmation Rule}
\label{sec:cfm-compare}

We have shown in \S\ref{sec:limitation_Prism} that the confirmation rule proposed in \prism~\cite{prism-theory} does not \textit{guarantee} low latency due to large constants. Here, we experimentally show that the rule does not \textit{achieve} optimal latency in practice by comparing it with the \newprism confirmation rule under the same parameters.

For both rules, we target a confirmation confidence of $\epsilon = 10^{-9}$. As explained in \S\ref{sec:limitation_Prism}, \prism's rule requires a large number of voter chains that depends on $\beta$, $\epsilon$, and the blockchain life span. To ensure a life span of at least 10 years under $\beta=0.3$ (the highest $\beta$ we explore in this experiment), \prism requires $m>23800$, so we set $m=23800$. We point out that this is impractically large for a real system, making the rule undeployable. In comparison, our new rule does not have such a limitation. \newprism may run for an infinite life span, and $m$ can be set independently from $\beta$ and $\epsilon$ (indeed, we use $m=1000$ for \newprism in all other experiments). Finally, we set the mining rate to 0.05 block/s per chain.

We compare the confirmation latency of \prism and \newprism under this setting. Results in Table \ref{table:real_latency} show that although the actual latency of the \prism confirmation rule is much lower than the upper bound (several hours, see \S\ref{sec:limitation_Prism}) given by \cite{prism-theory}, it is still 4--10$\times$ worse than \newprism. In comparison, the \newprism rule confirms blocks with almost-certain confidence ($\epsilon=10^{-9}$) when votes are only 3--9 blocks deep on average, achieving low latency in practice. 

\begin{table}[htb]
	\centering
	\caption{Actual confirmation latency of the \prism rule \cite{prism-theory} and the \newprism rule (\S\ref{sec:scaling}) under different $\beta$.}
	\begin{tabular}{ c || c | c | c } 
	 \hline
     $\beta$ &0.10  & 0.20 & 0.30 \\
	 \hline\hline
	 \newprism (s) & 55 & 82 & 184 \\
	 \hline
	 \prism (s) & 770   & 794 & 783 \\
	 \hline
	\end{tabular}
	\label{table:real_latency}
\end{table}

\subsection{Throughput and Latency}
\label{sec:eval-performance}

In this experiment, we measure the transaction throughput and confirmation latency of \newprism at different adversarial ratios $\beta$, and compare that with \algorand, \bng and the longest chain protocol. For \algorand, we use its default setting of security parameters, which targets $\beta=20\%$ (maximum possible is $\beta = 33\%$). %\footnote{The maximum possible security level for Algorand is $\beta = 33\%$, but its latency is expected to increase substantially as $\beta$ approaches 33\%~\cite{algorand}.}
 For \newprism, \bng and the longest chain protocol, we experiment with two adversarial ratios: $\beta=20\%$ and $\beta=33\%$. In both \algorand and the longest chain protocol, there is tradeoff between throughput and confirmation latency by choosing different block sizes. We explore this tradeoff and present it as a curve. For \algorand, we try block sizes between 300 KB to 32 MB. For the longest chain protocol, we try block sizes between 1.7 KB  to  33.6 MB. All four protocols are deployed on the same hardware and network topology as described above. We run each experiment for a minimum of 10 minutes and report the average transaction throughput and latency. The results are shown in Figure~\ref{fig:compare}.

\noindent{\bf Throughput.}
As shown in Fig. \ref{fig:compare}, \newprism is able to maintain the same transaction throughput of around $80,000$ tps regardless of the $\beta$ chosen.
This is because \newprism decouples throughput from security by using transaction blocks. In this way, \newprism is able to maintain the mining rate for transaction blocks to sustain a constant throughput, while changing the mining rate for other types of blocks to achieve the desired $\beta$. \bng offers a similar decoupling by entitling the miner of the latest key block to frequently produce micro blocks containing transactions. \algorand and the longest chain protocol do not offer such decoupling, so the block size must by increased in order to achieve a higher throughput. In such case, the confirmation latency increases, as demonstrated by the tradeoff curves in Figure~\ref{fig:compare}, to accommodate for the higher block propagation delay induced by larger blocks. %For the longest chain protocol, its throughput limit has been discussed in \S\ref{sec:limitation_LC}.
For \algorand, we observe its throughput increases marginally with block size, but does not exceed $1300$ tps.
The reason is that \algorand only commits one block every round. So at any moment, unlike \newprism, \algorand only has one block propagating in the network, causing low bandwidth utilization. For \bng, we observed a peak throughput of 21,530 tps. The reason is that, unlike \newprism, in \bng only a single node (the leader) commits transactions at a time. This results in the network becoming a bottleneck; once the throughput exceeds about 20,000 tps, we observed that the block propagation delay increases significantly for \bng (note also that \bng is susceptible to an adaptive attack that censors the chosen leader and can reduce throughput substantially~\cite{parallel}). 


\noindent{\bf Is Consensus the Throughput Bottleneck?}
A blockchain client has two roles: (1) it participates in the consensus protocol (the \textit{Block Structure Manager} and the \textit{Miner} in our implementation); (2) it executes transactions confirmed by the consensus protocol and updates the ledger (the \textit{Ledger Manager} in our implementation). The throughput can be bottlenecked by either of these stages and therefore we ask: Is the throughput limited by the consensus protocol, or the ledger updates? To answer this question, we measure the maximal throughput when no consensus protocol is involved, i.e. we start one client of each protocol and test how fast each client can execute transactions and update the ledger. For our \newprism, \bng and longest chain client, the limit is around $90,000$ tps. For \algorand, the limit is around $4,800$ tps. From Fig.~\ref{fig:compare} we see that \bitcoin, \bng, and \algorand have throughput much lower than these limits, and thus are bottlenecked by the consensus protocols. However, in the case of \newprism, its throughput is very close to the limit, and hence it is bottlenecked by the ledger updates.

\noindent{\bf Confirmation Latency.} At $\beta = 20\%$, \newprism achieves a latency of $42$ seconds, and for similar security guarantees \algorand under its default parameters achieves latency of $18$ seconds. Compared to the longest chain protocol, \newprism uses multiple voter chains in parallel ($1000$ chains in our experiments) to provide security instead of relying on a single chain. So \newprism requires each vote to be less deep in order to provide the same security guarantee. As a result, \newprism achieves a substantially lower confirmation latency. For example, for $\beta = 20\%$, the confirmation latency for \newprism is 42 seconds, compared to 607 seconds at the lowest throughput point for the longest chain protocol. As we increase the block size for the longest chain protocol, its  confirmation latency increases to 3870 seconds at a throughput of 1800 tps. The gap between \newprism and the longest chain protocol increases for higher $\beta$. For example, for \newprism the confirmation latency increases from 42 seconds to 182 seconds as $\beta$ increases from $20\%$ to $33\%$. For the longest chain protocol, the same change in $\beta$ causes the latency to increase by more than 3000 seconds. \bng exhibits similar confirmation latency as the longest chain protocol for the same value of $\beta$, since it applies the same $k$-deep rule as the longest chain protocol for key blocks to confirm transactions, and key blocks must be mined slowly to avoid frequent leader changes. Finally, we point out that the theoretical prediction of latency in \S\ref{sec:scaling} accurately translates to the real-world measurement. % confirmation latency under our new confirmation rule. 
For example, the theory predicts a latency of 150 seconds for  $\beta=0.33$, while our measurement shows a latency of 182s. The extra 32 seconds is caused by (1) a transaction needs to wait for a proposer block to refer it; (2) there is a small probability that the proposer chain forks, and thus momentarily causes higher latency.

%that is $10\times$ better than the longest chain protocol even at its lowest .

\subsection{Scalability}

\label{sec:eval-scale}
\begin{table}
	\centering
	\caption{\small Performance of \newprism with different network topologies.}
	\resizebox{\columnwidth}{!}{
	\begin{tabular}{ c || c | c c c } 
	 \hline
	 Property & \#Nodes & 100 & 300 & 900 \\ 
	 \hline\hline
	 \multirow{4}{*}{Degree $=4$}   & Diameter & 5 & 7 & 9 \\
	                                & Throughput (tps) & $8.1\times 10^4$ & $8.1\times 10^4$ & $7.8\times 10^4$ \\
	                                & Latency (s) & 42 & 71 & 76 \\
	                                & Forking & 0.15 & 0.17 & 0.15 \\
	 \hline
	 \multirow{4}{*}{Diameter $=5$} & Degree & 4 & 6 & 8 \\
	                                & Throughput (tps) & $8.1\times 10^4$ & $8.2\times 10^4$ & $8.0\times 10^4$ \\ 
	                                & Latency (s) &42 & 43 & 42 \\
	                                & Forking & 0.15 & 0.15 & 0.15 \\
	 \hline
	\end{tabular}
	}
	\label{table:scale}
	\end{table}

In this experiment, we evaluate \newprism's ability to scale to a large number of users. For each client, we use the same network and hardware configuration as in other experiments, and target an adversarial ratio $\beta=20\%$. The results are shown in Table~\ref{table:scale}.

First, we increase the number of clients while keeping the topology a random 4-regular graph, i.e., each client always connects to four random peers. In this case, the network diameter grows as the topology becomes larger, causing the block propagation delay to increase and the confirmation latency to increase correspondingly. Note that the transaction throughput is not affected because in \newprism the mining rate for transaction blocks is decoupled from that of the other types of blocks. Then, we explore the case where clients connect to more peers as the topology grows larger, so that the diameter of the network stays the same. As shown in the results, both confirmation latency and throughput are constant as the number of clients increases from 100 to 900. 

In all cases, the forking rate stays stable and is under $0.17$, proving that the system is secure for $\beta=20\%$. This suggests that \newprism is able to scale to a large number of users as long as the underlying peer-to-peer network provides a reasonable block propagation delay.

\subsection{Resource Utilization}
\label{sec:eval-resource}

In this experiment, we evaluate the resource utilization of our \newprism implementation, and how it performs with limited network bandwidth and CPU resources. 

% resources. Generally \newprism uses the following three resources: CPU, to verify cryptographic signatures, to execute transactions, and to assemble blocks. Storage, to store the ledger and blocks. Network, to receive and broadcast blocks from/to peers.

\begin{figure}
\centering
\begin{minipage}[t]{.48\columnwidth}
  \centering
  \includegraphics[width=.9\textwidth]{figures/resource-fig-bw.pdf}
    \caption{\small Performance of \newprism under different network bandwidth. }
    \label{fig:bw}
\end{minipage}\hfill%
\begin{minipage}[t]{.48\columnwidth}
  \centering
  \includegraphics[width=.9\textwidth]{figures/resource-fig-cpu.pdf}
    \caption{\small Performance of \newprism with different number of CPU cores at each client.}
    \label{fig:cpu}
\end{minipage}
\end{figure}


\begin{table}
\centering
\caption{\small Network bandwidth usage breakdown of \newprism measured on a 200 Mbps interface. Network Headroom is the unused bandwidth necessary for the block propagation delay to stay stable. Serialization overhead is wasted space when serializing in-memory objects for network transmission. Messaging stands for non-block messages.}
\resizebox{0.93\columnwidth}{!}{
\begin{tabular}{ c | c | c || r } 
 \hline
 \multicolumn{3}{c||}{Usage} & $\%$Bandwidth \\
 \hline\hline
 \multirow{5}{*}{Received} & \multirow{4}{*}{Deserialized} & Proposer Block & $0.05\%$ \\
 && Voter Block & $0.21\%$ \\
 && Transaction Block & $50.43\%$ \\ \cline{3-4}
 && Messaging &  $0.43\%$ \\ \cline{2-4} 
 & \multicolumn{2}{c||}{Serialization Overhead} & $25.80\%$ \\ \hline
 \multicolumn{3}{c||}{Network Headroom} & $23.08\%$ \\
 \hline
\end{tabular}
}

\label{table:bw-profiling}
\end{table}

\begin{figure*}
\centering
\begin{minipage}[t]{.30\textwidth}
  \centering
  \includegraphics[width=0.8\textwidth]{figures/attack-fig-spamming.pdf}
    \caption{\small Effectiveness of random delay in defending against spam attack. Spam traffic amount is normalized to the case when no delay is added.}
    \label{fig:attack-spamming}
\end{minipage}\hfill%
\begin{minipage}[t]{.30\textwidth}
  \centering
  \includegraphics[width=0.8\textwidth]{figures/attack-fig-censor.pdf}
    \caption{\small Performance of \newprism under  censorship attack.}
    \label{fig:attack-censor}
\end{minipage}\hfill%
\begin{minipage}[t]{.30\textwidth}
  \centering
  \includegraphics[width=0.8\textwidth]{figures/attack-fig-balancing.pdf}
    \caption{\small Performance of \newprism under balancing attack. We also mark the lowest confirmation latency possible for the longest chain protocol under the same security guarantee.}
    \label{fig:attack-balancing}
\end{minipage}
\end{figure*}

\noindent{\bf Network Bandwidth.} Figure~\ref{fig:bw} shows the throughput of \newprism as we throttle the bandwidth at each client. Results show that the throughput scales proportionally to the available bandwidth. The throughput stops to grow when the bandwidth is higher than 200 Mbps, because the transaction generation rate is capped at around 80,000 tps, which is near the bottleneck caused by RocksDB.

Table~\ref{table:bw-profiling} provides a breakdown of the bandwidth usage. Our implementation is able to process transaction data at a throughput about $50\%$ of the available bandwidth. (The in-memory size of a transaction is 168 bytes.) Further improvements could be made by using more efficient data serialization schemes and optimizing the underlying P2P network.

\noindent{\bf CPU.} Figure~\ref{fig:cpu} shows the throughput of \newprism as we change the number of CPU cores for each client. The throughput scales proportionally to the number of cores, and stops to grow after 7 cores because the transaction generation rate is capped. This shows that our implementation handles more than 10,000 tps per CPU core, and the parallelization techniques discussed in \S\ref{sec:implementation-highlights} are effective. 

Table~\ref{table:profiling} provides a breakdown of CPU usage across different components. More than half of CPU cycles are taken by RocksDB for which we only perform basic tuning. Less than $15\%$ are spent on overhead such as inter-thread communication, synchronization, etc. (categorized as ``Miscellaneous'' in the table). This suggests that our implementation uses CPU resources efficiently, and further improvements could be made primarily by optimizing the database. 

While we chose mid-end AWS EC2 instances for experiments, our results show that  \newprism  does not inherently require powerful machines or waste resources. For example, a laptop with 8 cores, 16 GB RAM, and 400 GB of NVMe-based SSD would cost under \$3,000 today and could easily run \newprism at 80,000 tps. %Indeed, high resource efficiency and scalability that we demonstrate in this experiment makes \prism suitable for applications with different requirements. 

%This suggests that our implementation design mentioned in Section~\ref{sec:implementation-highlights} enables efficient and scalable parallelization.

\begin{table}
\centering
\caption{\small CPU usage breakdown of our \newprism implementation.}
\resizebox{0.65\columnwidth}{!}{
\begin{tabular}{ c | c || r } 
 \hline
 \multicolumn{2}{c||}{Operation} & $\%$CPU \\  
 \hline\hline
 %\multirow{5}{*}{Ledger} & RocksDB Read & $13.2\%$ \\ %\cline{2-3}
 %                        & RocksDB Write & $13.1\%$ \\ %\cline{2-3}
 \multirow{3}{*}{Ledger} & RocksDB Read/Write & $49.5\%$ \\ %\cline{2-3}
                         & (De)serialization & $3.1\%$\\ %\cline{2-3}
    %                     & Serialization & $2.0\%$\\ %\cline{2-3}
    %                     & Deserialization & $1.1\%$ \\ %\cline{2-3}
                         & Miscellaneous & $8.9\%$\\ \hline
 \multirow{5}{*}{Blockchain}    & Signature Check & $21.7\%$ \\ %\cline{2-3}
                         & (De)serialization & $3.8\%$ \\
                         & RocksDB Read/Write & $3.9\%$ \\
 %                        & Serialization & $2.0\%$\\ %\cline{2-3}
 %                        & Deserialization & $1.8\%$ \\ %\cline{2-3}
                         & Network I/O & $0.6\%$ \\ %\cline{2-3}
                         & Miscellaneous & $5.5\%$\\ \hline
% \multicolumn{2}{|c||}{RocksDB Background Jobs} & $25.0\%$ \\ \hline
  \multicolumn{2}{c||}{Block Assembly} & $1.5\%$ \\ \hline
 \multicolumn{2}{c||}{Transaction Generation} & $0.7\%$ \\ \hline
 \multicolumn{2}{c||}{Miscellaneous} & $0.8\%$ \\ \hline
\end{tabular}
}
\label{table:profiling}
\end{table}
\subsection{Performance Under Active Attack}
\label{sec:eval-attack}



In the following experiments, we evaluate how \newprism performs in the presence of active attacks. Specifically, we consider three  types of attacks: {\em spamming}, \textit{censorship}, and \textit{balancing} attacks. Spamming and censorship attacks aim to reduce network throughput, while balancing attacks aim to increase confirmation latency. 
%For censorship and balancing attacks, we configure a variable fraction of clients to be malicious and measure the throughput and latency of the system. 
In these experiments we configure \newprism to tolerate a maximum adversarial ratio $\beta=20\%$. 

%We will demonstrate that the performance of \prism degrades gracefully under active attacks.
%\todo{cite https://eprint.iacr.org/2016/555.pdf}



\label{sec:spamming-eval}
\noindent{\bf Spamming Attack.} Recall that in a spamming attack, attackers send conflicting transactions to different nodes across the network. As described in \S\ref{sec:spamming-design}, miners can mitigate such attack by adding a random timing jitter to each transaction. In this experiment, we set up 100 miners as victims and connect them according to the same topology as in other experiments. Then for each miner we start a local process that generates a transaction every 100 ms. We synchronize those processes across the network so that each miner receives the same transaction at the same time, with a time synchronization error of several ms due to the Network Time Protocol. 
To defend against the attack, miners add a uniform random delay before including a transaction into the next transaction block. We let each attack to last for 50 seconds, and measure the fraction of spam transactions that end up in transaction blocks. 
Fig.~\ref{fig:attack-spamming} shows that adding a random jitter of at most 5 seconds can reduce the spam traffic by about 80\%. 
We point out that miners can extend this method by monitoring the reputation of clients by IP address and public key, and penalizing clients with high spam rate with longer jitter.

%\gf{Notice that the protocols we compare against (the Longest Chain protocol, Algorand, Bitcoin-NG) are not susceptible to these attacks because transactions are validated prior to block creation.}
%An adversary could generate a large number of conflicting transactions and disseminate them to different nodes across the network.  
%The 
%spam/duplicate transactions
% There are a few practical mechanisms for circumventing this. 
%To circumvent this, nodes should first validate transactions with respect to their latest ledger state and other unreferred transaction blocks, 
%\gw{I think ledger state is more proper than ledger tip.}
%giving the adversary only a small window of network delay to spam the system. % and thus significantly weakens the attack.
%Second, miners could add some timing jitter prior to mining transactions, 
%giving other miners the ability to observe if a conflicting transaction is already present in a transaction block, in  which case the miner will choose to not include that transaction. % in its block.
%We evaluate the effectiveness of this method in \S\ref{sec:spamming-eval}.

\noindent{\bf Censorship Attack.}
In a censorship attack, malicious clients mine and broadcast empty transaction blocks and proposer blocks. Censorship attack does not threaten the security of \newprism, but it reduces the system throughput because a fraction of blocks are now ``useless'' since they do not contain any data. As Figure~\ref{fig:attack-censor} shows, during a censorship attack, the transaction throughput reduces proportionally to the percentage of adversarial users, i.e. the system capacity degrades gracefully.

\label{sec:balancing}

\noindent{\bf Balancing Attack.}
In a balancing attack, attackers try to increase the confirmation latency of the system by waiting for the event when multiple proposer blocks appear on the same level and balancing the votes among them. Normally, when multiple proposer blocks appear on one level, every client votes for the proposer block with the most votes, so the system quickly converges with the vast majority of voter chains voting for one proposer block. During a balancing attack, however, the attacker votes on the proposer blocks with the second most votes to slow down such convergence, causing votes to be more evenly distributed among competing proposer blocks. In this case, clients need to wait for votes to grow deeper in order to confirm a proposer leader, resulting in longer confirmation latency. Figure~\ref{fig:attack-balancing} shows that the confirmation latency grows as the active adversarial fraction increases. But even when $20\%$ clients are malicious, the confirmation latency is still more than $6\times$ better than the longest chain protocol.



==> Prism Systems Paper (CCS)/figures/prism-chains.tex <==
\tikzstyle{proposer} = [draw, fill=blue!20, rectangle, rounded corners, minimum height=1em, minimum width=1.6em, text centered]
\tikzstyle{voter} = [draw, fill=green!20, rectangle, rounded corners, minimum height=1em, minimum width=1.6em]
\tikzstyle{transaction} = [draw, circle, fill=yellow!20]

% The block diagram code is probably more verbose than necessary
\begin{tikzpicture}[auto, node distance=0.8cm,>=latex']
\node [proposer] (p0l) {\tiny L};
\node [proposer, below of=p0l] (p1l) {\tiny L};
\node [proposer, left=0.1cm of p1l] (p1s) {};
\node [proposer, below of=p1l] (p2l) {\tiny L};
\node [proposer, right=0.1cm of p2l] (p2s) {};
\node [proposer, below of=p2l] (p3l) {\tiny L};

\node[transaction, above left = 0.01cm and 0.45cm of p0l] (t00){};
\node[transaction, below right = 0.06cm and 0.02cm of t00] (t01){};
\node[transaction, left = 0.25cm of p1s] (t10){};
\node[transaction, above right = 0.07cm and 0.02cm of t10] (t11){};
\node[transaction, below right = 0.10cm and 0.07cm of t10] (t12){};
\node[transaction, below left = 0.05cm and 0.25cm of p2l] (t20){};
\node[transaction, above left = 0.07cm and 0.13cm of t20] (t21){};
\node[transaction, left = 0.35cm of p3l] (t30){};
\node[transaction, above left = 0.05cm and 0.11cm of t30] (t31){};
\node[transaction, left = 0.25cm of t30] (t32){};
\draw[densely dashed, <-] (t00)  to [looseness=0.4] (p0l);
\draw[densely dashed, <-] (t01)  to [looseness=0.4] (p0l);
\draw[densely dashed, <-] (t10)  to [looseness=0.4] (p1l);
\draw[densely dashed, <-] (t11)  to [looseness=0.4] (p1l);
\draw[densely dashed, <-] (t12)  to [looseness=0.4] (p1l);
\draw[densely dashed, <-] (t20)  to [looseness=0.4] (p2l);
\draw[densely dashed, <-] (t21)  to [looseness=0.4] (p2l);
\draw[densely dashed, <-] (t30)  to [looseness=0.4] (p3l);
\draw[densely dashed, <-] (t31)  to [looseness=0.4] (p3l);
\draw[densely dashed, <-] (t32)  to [looseness=0.4] (p3l);


\node [voter, right=1cm of p0l] (v00) {};
\node [voter, below of=v00] (v01) {};
\node [voter, below of=v01] (v02) {};
\node [voter, below of=v02] (v03) {};
\draw[<-] (v00) to (v01);
\draw[<-] (v01) to (v02);
\draw[<-] (v02) to (v03);

\node [voter, right=0.3cm of v00] (v10) {};
\node [voter, below of=v10] (v11) {};
\node [voter, below of=v11] (v12) {};
\node [voter, below of=v12] (v13) {};
\draw[<-] (v10) to (v11);
\draw[<-] (v11) to (v12);
\draw[<-] (v12) to (v13);

\node [right=0.3cm of v10] (space0) {$\cdots$};
\node [below of=space0] (space1) {$\cdots$};
\node [below of=space1] (space2) {$\cdots$};
\node [below of=space2] (space3) {$\cdots$};

\node [voter, right=0.3cm of space0] (v20) {};
\node [voter, below of=v20] (v21) {};
\node [voter, below of=v21] (v22) {};
\node [voter, below of=v22] (v23) {};
\draw[<-] (v20) to (v21);
\draw[<-] (v21) to (v22);
\draw[<-] (v22) to (v23);

\draw[densely dashed, <-] (p0l)  to [looseness=0.3] (v00);
\draw[densely dashed, <-] (p1l)  to [looseness=0.3] (v01);
\draw[densely dashed, <-] (p2l)  to [looseness=0.3] (v02);
\draw[densely dashed, <-] (p3l)  to [looseness=0.3] (v03);

\draw[densely dashed, <-] (p0l)  to [looseness=0.3] (v10);
\draw[densely dashed, <-] (p1l)  to [looseness=0.3] (v11);
\draw[densely dashed, <-] (p2l)  to [looseness=0.3] (v12);
\draw[densely dashed, <-] (p3l)  to [looseness=0.3] (v13);

\draw[densely dashed, <-] (p0l)  to [looseness=0.3] (v20);
\draw[densely dashed, <-] (p1l)  to [looseness=0.3] (v21);
\draw[densely dashed, <-] (p2l)  to [looseness=0.3] (v22);
\draw[densely dashed, <-] (p3l)  to [looseness=0.3] (v23);

\end{tikzpicture}

==> Prism Systems Paper (CCS)/figures/system-diagram.tex <==
\tikzstyle{ledger} = [draw, fill=blue!20, rectangle, 
    minimum height=4em, minimum width=6em, text centered, text width=5em]
\tikzstyle{blockchain} = [draw, fill=red!20, rectangle, minimum height=4em, minimum width=6em, text centered, text width=5em]
\tikzstyle{miner} = [draw, fill=green!20, rectangle, minimum height=4em, minimum width=6em, text centered, text width=5em]

\tikzstyle{database} = [draw, fill=yellow!20, rectangle, rounded corners, text width=5em, minimum height=3em, minimum width=6em, text centered]


% The block diagram code is probably more verbose than necessary
\begin{tikzpicture}[auto, node distance=2.8cm,>=latex']
    \node [database] (blockchaindb) {Block Structure Database};
    \node [blockchain, above=0.5cm of blockchaindb] (blockchain) {Block Structure Manager};
    \node [ledger, left of=blockchaindb] (ledger) {Ledger Manager};
    \node [miner, right of=blockchaindb] (miner) {Miner};
    \node [database, left of=ledger] (utxodb) {UTXO Database};
    \node [database, right of=blockchain] (mempool) {Memory Pool};
    \node [database, left of=blockchain] (blockdb) {Block Database};
    \node [above=0.5cm of blockchain] (peers) {Peers};
    \node [right of=peers] (newtx) {New Transactions};
    \draw [<->] (blockchaindb) -- node[name=a] {} (blockchain);
    \draw [->] (blockchaindb) -- node[name=b] {} (miner);
    \draw [<->] (blockchaindb) -- node[name=c] {} (ledger);
    \draw [<-] (blockchain) -- node[name=d] {} (miner);
    \draw [<->] (miner) -- node[name=e]{} (mempool);
    \draw [->] (blockchain) -- node[name=f]{} (mempool);
    \draw [<->] (blockchain) -- node[name=g]{} (blockdb);
    \draw [<->] (ledger) -- node[name=h]{} (utxodb);
    \draw [<-] (ledger) -- node[name=i]{} (blockdb);
    \draw [<->] (peers) -- node[name=j]{} (blockchain);
    \draw [->] (newtx) -- node[name=k]{} (mempool);


\end{tikzpicture}

==> Prism Systems Paper (CCS)/implementation.tex <==
\section{Implementation}
\label{sec:implementation}

We have implemented a basic Prism client and wallet in about 10,000 lines of Rust code. We describe the architecture of our implementation and several design decisions that are key to its high performance.




\begin{figure}[t]
\begin{center}
\includegraphics[width=3.2in]{prism.png}
\end{center}
\caption{\label{fig:prism-system} Prism system diagram. \todo{Add persistent storage for raw blocks?}}
\end{figure}

\subsection{Architecture}

Our implementation features a simplified version of Bitcoin's scripting language, processing only pay-to-public-key (P2PK) transactions, similar to that implemented in Algorand~\cite{algorand, algorandcode}. \ma{talk about UTXO here}


Although Prism is compatible with more complex scripting languages (e.g., smart contracts), we made this choice to enable a fair comparison with other baselines \cite{algorand,ohie},
% \ly{is "alogrand1" the theory paper?} 
which make a similar choice in their  implementations \cite{ohiecode,algorandcode}. \ma{I'm not sure we should claim too strongly that Prism, as is, is compatible with smart contracts. For instance, I'm not entirely sure how miners should execute a smart contract without knowing the state of the ledger (e.g., VM state) on top of which they are mining.}
% Hence, the following design decisions will be based on the assumption that the system is processing only P2PK transactions. 


Our system architecture is illustrated in Figure \ref{fig:prism-system}. \ma{this is a useless figure!}
At a high level, it is divided into various handlers running on separate threads:
\begin{enumerate}
    \item {\em Peer handler},  which parses messages passed over the network; these messages can encapsulate protocol-relevant information such as relayed blocks.
    \item {\em Transaction/block handlers}, which process new transactions or blocks as they arrive. % For parallelism, these handlers are deployed in a worker pool with 16 threads.
    \item {\em Miner}, which updates the miner's context, i.e., its current estimate of what votes to cast and how to structure each of its block types. \gw{There are two "miner"s in this sentence and it may cause confusion.}
    \item {\em Ledger generator}, which periodically updates the confirmed order of transaction blocks. \ma{The ledger generator also updates the pending list of transactions as it confirms transaction blocks. (Is this correct? Which component is responsible for removing transactions that are already in some transaction block from the pending transaction list? I assume that can happen without  confirmation.}
    \item {\em Sanitizer}, which applies the confirmed sequence of transaction blocks to the UTXO set. \ma{Explain when this is run. It's everytime following ledger generation?}
\end{enumerate}

\ma{talk about which components have multiple threads to enable parallelism (transaction/block handlers, ledger generater/sanitizer?) and which run as a single thread}  

First, we have a network server, or \emph{peer handler}, that parses messages passed over the network; 
these messages can encapsulate protocol-relevant information such as relayed blocks.
Next, we have a worker pool of 16 threads that are opportunistically deployed as \emph{transaction or block handlers}, depending on what the system needs at a given point in time. 
These handlers deal with new transactions or blocks; because blocks are produced at such a high rate in Prism, parallelism is needed to prevent this processing from becoming a system bottleneck. 
Third, we have a \emph{miner thread}, which updates the miner's context, i.e., its current estimate of what votes to cast and how to structure each of its block types.
The \emph{ledger generation} thread periodically updates the confirmed order of transaction blocks. \gw{\emph{ledger generation} thread or ledger generator?}
Finally, the \emph{sanitization} thread applies the confirmed sequence of transaction blocks to the unspent transaction output (UTXO) set. \gw{Sanitization actually has multiple threads?}
Because ledger generation and sanitization are operating at a high rate on closely-related data, we use the scoreboarding technique from computer architecture to ensure that these processes are self-consistent.
This will be discussed further in Section \ref{sec:key_design}. \ma{I think i covered all of this.}

\smallskip
\noindent{\bf Persistent storage.} Discuss all the databases. Block database. Block DAG database (this only maintains graph structure, i.e. there aren't two copies of actual blocks). UTXO database. Wallet database (is this one important to explain. it seems this could have been a separate piece of software anyway). 

\smallskip
\noindent{\bf In-memory state.} Unresolved blocks. Mempool. Highly accessed DBs are cached in memory -- explain.


We have six types of storage. 
The first is the \emph{block database}, which stores raw blocks.
Related to the block database, the \emph{blockchain database} stores the DAG-structured relation between blocks.
Both are stored in persistent storage backed by RocksBD \cite{}.
The \emph{UTXO database} stores the set of unspent coins, and the \emph{wallet database} stores a user's own unspent coins. 
Both the UTXO and wallet databases are also kept in persistent storage (RocksDB) to enable our implementation to run for long periods of time without running out of memory. 
The \emph{unresolved blocks} database stores blocks that contain pointers to blocks that have not yet been received; 
whenever a new block is received over the network,  this database is accessed to attempt to resolve already-received blocks. 
The unresolved blocks database is stored in memory, as it does not grow with time. \ma{It doesn't grow with time only if the system is behaving correctly, right? If under attack, one could easily get a huge number of unresolved blocks. We'll have to revisit this decision.} 
Similarly, the memory pool (mempool) stores received transactions that have not yet been mined into a transaction block. 
The mempool is also stored in memory.






\subsubsection{Implementation Design Decisions}
\label{sec:key_design}
Here we outline a number of implementation design decisions that affect our performance metrics. 
Many of these issues arise implicitly in related literature \cite{ohie,algorand,conflux}; we highlight them explicitly to facilitate a fair comparison.


\paragraph{Asynchronous confirmation} 
% More tolerant on delays and frequent shift of longest chains.
In classical blockchains like Bitcoin, every block generally confirms a new set of transactions in the ledger. 
This is not the case in Prism, where confirmation occurs based on the aggregate behavior of many blockchains: each new block is individually unlikely to confirm a new transaction. 
For this reason, we have decoupled the processing of blocks from transaction confirmation by using a separate thread to periodically check the confirmation status of transactions. \gw{This thread is ledger generator?}
This wastes less processing power than checking each transaction's confirmation status every time a new block is received, and alleviated a system bottleneck for us.


\paragraph{Parallel transaction execution} 
The \emph{state} of a P2PK blockchain is the set of unspent transaction outputs, also known as the UTXO set. 
Processing transactions requires both evaluating their validity and executing them, i.e., updating the state. 
Both of these processes require accessing the UTXO database, often in quick succession. 
However, because we operate at high throughput levels (tens of thousands of transactions per second), these database accesses quickly become a bottleneck if processed sequentially. 
Hence,  we have a worker pool of eight threads accessing the UTXO database for simultaneous transaction processing. \ma{These threads are distinct from the event handler threads described in 4.1?} 
To avoid race conditions, we implement scoreboarding. \ma{We definitely need to explain this in more detail}
\todo{Lei, add more details here?}
We expect that this implementation choice would have even greater repercussions for more complex scripting languages, since the cost of processing each transaction increases. 
% (benchmark and show the advantage of parallel execution, note that the advantage on more complex transactions could be higher.)

\paragraph{State updates} 
Each node maintains a local copy of the state; different nodes' views of the state may differ due to network delays. 
In a real blockchain \ma{what do you mean `real blockchain'? traditional blockchains?}, nodes update their local state each time a new transaction is processed; this update involves checking the validity of each transaction by ensuring that the transaction draws only upon valid UTXOs, and updating the corresponding UTXO database. 
Several academic blockchain implementation papers have chosen not to implement state updates \cite{algorand,ohie}, instead generating random transactions that are not necessarily valid with respect to the current state. 
Nodes in turn do not check the validity of these transactions. 
This design choice reduces the computational load of transaction validation, which can be a substantial bottleneck in high-performance blockchains. 
Indeed, we find that state updates (e.g., transaction validation and processing updates to the UTXO database) are a bottleneck in our current implementation. 
Notice that this will also be the bottleneck in efficient centralized implementations. \ma{This discussion of previous implementations should go in the related work section. The purpose of this section is to discuss our implementation, and what we had to do to achieve good performance. So the more relevant question here is, what enables our implementation to achieve fast state updates}

% For example, Figure \ref{} illustrates the difference in throughput achievable in our implementation when we disable state updates. 
% We observe up to a \red{XXX}\% difference. 

% Talk about how many academic implementations choose to not include state updates for efficiency, which ends up being a bottleneck in practice. Show plots comparing with and without state updates. 

\paragraph{Transaction broadcasting}
Most blockchains broadcast transactions prior to incorporating them into blocks. 
This is done because it is unknown ahead of time which node will mine the next block, so transactions are widely disseminated to ensure that they are included in a block as quickly as possible. 
In contrast, our implementation does not broadcast transactions.
Prism generates blocks at much higher rate than other blockchain protocols. 
This elevated block rate means that any individual miner is likely to mine a transaction block in time comparable to the delay associated with broadcasting a block to the rest of the network (i.e., seconds).
Hence, unlike other blockchain protocols, there is little incentive for a Prism miner to broadcast its transactions.
In practice, non-mining nodes can transmit their transactions to one or more miners; however, those miners need not relay the transaction for the same reason as before.
 % Indeed, even miners may choose to broadcast transactions to ensure that their own transactions are confirmed as quickly as possible. 
% This broadcasting process may consume additional computational and network resources that are not modeled in our implementation. 
% However, such overhead can easily be limited by throttling the amount of computation and/or bandwidth used for transaction relaying. 
% In a high-performance Prism implementation, the bulk of the computation and bandwidth should be spent on processing and relaying blocks.
We want to emphasize that this decision to not broadcast transactions is \emph{not} the same thing as sharding the blockchain; all transactions end up on the same main chain and therefore have the same security guarantees. \ma{we should explain that there's nothing preventing miners from broadcasting transactions, and the impact on performance won't be significant. this is an optimization to reduce network bandwidth consumption} 
% Talk about fact that we do not broadcast transactions, why this is ok, and mention that other implementations do the same. 

\paragraph{Mining simulation} Like other academic implementations of PoW systems \cite{ohie,conflux}, we do not implement the actual proof-of-work loop used to generate blocks.
Instead, we simulate the time to mine a block by drawing an exponentially-distributed random delay for each block. 
This is done for two reasons:
first, simulating PoW wastes energy for no reason, since we have good analytical models of the (random) mining time. 
Second, in practice, PoW will happen primarily on dedicated hardware (e.g., ASICS), so the cost of mining will not contribute to the computational bottlenecks of the consensus protocol. 
Therefore, this simplification does not introduce unrealistic artifacts. 



==> Prism Systems Paper (CCS)/implementation2.tex <==
% \section{Implementation}
% \label{sec:implementation}


\label{sec:implementation-architecture}
\subsection{Architecture}
% \vb{Similar to Bitcoin, a \textit{coin} is the fundamental entity of the currency in Prism. A coin is a $256$ length binary string which has a value and an owner. A \textit{transaction} `spends' a set of input coins and produces a new set of output coins such that the sum of the value of the input coins is equal to the sum of the value of the output coins. The output coins potentially have different owners from the input coins and this is the way users exchange money in the system.
% The \textit{history} (ledger) is defined as the ordered list of transactions and for a given history, \textit{UTXO} set is defined as the set of unspent output coins of all the transactions in the history. A transaction is valid w.r.t to a ledger iff it's input coins are in the UTXO set. Our implementation uses multi- input-multi-output transactions similar to pay-to-public-key (P2PK) in Bitcoin and Algorand~\cite{algorand, algorandcode}. We use Ed25519~\cite{ed25519} for digital signatures and SHA-256~\cite{sha256} as the hashing algorithm.}


Our implementation is based on the \textit{unspent transaction output (UTXO)} model, similar to that used by \bitcoin. %UTXOs are generated by transactions. A transaction takes a list of UTXOs (\textit{inputs}) and defines a list of new UTXOs (\textit{outputs}). Each UTXO is only allowed to be spent once, and the {\em state} of the ledger, i.e., the state that results from applying the transactions that have been confirmed up to that point in the ledger, can be represented as a set of UTXOs.
We support a simplified version of Bitcoin's scripting language, processing only pay-to-public-key (P2PK) transactions, similar to that implemented in Algorand~\cite{algorand, algorandcode}. We use Ed25519~\cite{ed25519} for cryptographic signatures and SHA-256~\cite{sha256} as the hashing algorithm.

\begin{figure}
    \centering
    \resizebox{0.8\columnwidth}{!}{\input{figures/system-diagram.tex}}
    %\input{figures/system-diagram.tex}
    \caption{\small Architecture of our \newprism client implementation.}
    \label{fig:system-architecture}
\end{figure}

The system architecture is illustrated in Figure~\ref{fig:system-architecture}. Functionally it can be divided into the following three modules:

\begin{enumerate}
    \item \textit{Block Structure Manager}, which maintains the clients' view of the blockchain, and communicates with peers to exchange new blocks.
    \item \textit{Ledger Manager}, which updates the ledger based on the latest blockchain state, executes transactions, and maintains the UTXO set.
    \item \textit{Miner}, which assembles new blocks.
\end{enumerate}
%\end{CompactEnumerate}

\noindent % follow the previous paragraph
The ultimate goal of the \newprism client is to maintain up-to-date information of the blockchain and the ledger. They are stored in the following four data structures:

\begin{enumerate}
    \item \textit{Block Structure Database}, residing in persistent storage, stores the graph structure of the blockchain (i.e., the voter blocktrees, the proposer blocktree, and the transactions blocks referenced) as well as the confirmed ordering of proposer and transaction blocks.
    \item \textit{Block Database}, residing in persistent storage, stores every block a client has downloaded so far. 
    \item \textit{UTXO Database}, residing in persistent storage, stores the UTXO set.
    \item \textit{Memory Pool}, residing in memory, stores the set of transactions that have not been mined into any block.
\end{enumerate}

%For the rest of this subsection, we describe these modules and data structures, and how they interact with each other. 
%We will discuss some  highlights in detail in the next subsection.


At the core of the \textbf{Block Structure Manager} are an \textit{event loop} which sends and receives network messages to/from peers, and a \textit{worker thread pool} which handles those messages. When a new block arrives, the worker thread first checks its proof of work and sortition, according to the rules specified in \S\ref{sec:mining}, and stores the new block in the Block Database (checking proof of work at the earliest opportunity reduces the risk of DDoS attacks).  
It then proceeds to relay the block to peers that have not received it. Next, the worker thread checks whether all blocks referred by the new block, e.g. its parent, are already present in the database. If not, it buffers the block in an in-memory queue and defers further processing until all the referred block have been received. Finally, the worker validates the block (e.g., verifying transaction signatures), and inserts the block into the Block Structure Database. If the block is a transaction block, the Block Structure Manager also checks the Memory Pool against the transactions in this new block and removes any duplicates or conflicts from the Memory Pool. 

\if 0
%\smallskip
At the core of the \textbf{Block Structure Manager} are an \textit{event loop} which sends and receives network messages to/from peers, and a \textit{worker thread pool} which handles those messages. In our implementation, network messages are prefixed by their length and transported over TCP. As soon as a message is received by the event loop, it is passed on to an idle worker thread, or put into a queue if none is available. There are three types of messages: \texttt{NewBlockHashes}, which advertises the hashes of blocks that a node has just mined or received from its peers. \texttt{GetBlocks}, which asks for blocks by their hashes. And \texttt{Blocks}, which contains actual blocks. 

When a new block arrives in a \texttt{Blocks} message, the worker thread first checks its proof of work and sortition, according to the rules specified in \S\ref{sec:mining}, and stores the new block in the Block Database (again checking proof of work at the earliest opportunity reduces the risk of DDoS attacks). %, because an attacker would have to solve the proof-of-work puzzle to trigger potentially costly processing at other nodes.}
 It then proceeds to relay the block to neighbors that have not received it, following the standard procedure implemented in \bitcoin. It broadcasts a \texttt{NewBlockHashes} message to all peers to advertise this new block. Every peer that does not have this block responds with a \texttt{GetBlocks} message to request it. 

%Advertising the new block before further processing it allows us to minimize the time for a block to propagate through the network. 
Next, the worker thread checks whether all blocks referred by the new block, e.g. its parent, are already present in the databases. If not, it buffers the block in an in-memory data structure and defers further processing until all the block's references have been received. Once a block's references have all arrived, the worker performs further validation (e.g., verifying transaction signatures), and finally, the new block is inserted into the Block Structure Database. If the block is a transaction block, the Block Structure Manager also checks the Memory Pool against the transactions included in this new block, and removes any duplicates or conflicting ones. \ma{Trim the description of the block structure managerin one paragraph. We don't need the details of the messages. The important parts seem to be: event loop + workers, it relays blocks to peers similar to bitcoin after checking proof of work and sortition, it defers processing blocks if their parents are not present in db} 

\fi 

The \textbf{Ledger Manager} is a two-stage pipeline and runs asynchronously with respect to the Block Structure Manager. Its first stage, the \textit{transaction sequencer}, runs in a loop to continuously poll the Block Structure Database and try to confirm new transactions. It starts by counting the votes cast on each proposer block. To avoid doing wasteful work, it caches the vote counts and the tips of the voter chains, and on each invocation, it only scans through the new voter blocks. Then, it tries to confirm a leader for each level in the proposer block tree where new votes are cast, according to the rules specified in \S\ref{sec:scaling} Definition \ref{def:rule}.  If a leader is selected, it queries the Block Database to retrieve the transaction blocks confirmed by the new leader, and assembles a list of confirmed transactions. The list is passed on to the second stage of the pipeline, the \textit{ledger sanitizer}. This stage maintains a pool of worker threads that executes the confirmed transactions in parallel. Specifically, a worker thread queries the UTXO Database to confirm that all inputs of the transaction are unspent; their owners match the signatures of the transaction;
and the input fund is sufficient. If execution succeeds, the outputs of the transaction are inserted into the UTXO Database, and the inputs are removed.

The \textbf{Miner} module assembles new blocks according to the mining procedure described in \S\ref{sec:mining}. It is implemented as a busy-spinning loop. At the start of each round, it polls the Block Structure Database and the Memory Pool to update the block it is mining. It also implements the spam mitigation mechanism described in \S\ref{sec:spamming-design}.
Like other academic implementations of PoW systems \cite{ohie,conflux}, our miner does not actually compute hashes for the proof of work, and instead simulates mining by waiting for an exponentially-distributed random delay. Solving the PoW puzzle in our experiments would waste energy for no reason, and in practice, PoW will happen primarily on dedicated hardware, e.g., application-specific integrated circuits (ASICs). So the cost of mining will not contribute to the computational bottlenecks of the consensus protocol.

The three databases residing in the persistent storage are all built on RocksDB~\cite{rocksdb}, a high-performance key-value storage engine. We tuned the following RocksDB parameters to optimize its performance: replacing B-trees with hash tables as the index; adding bloom filters; adding a 512 MB LRU cache; and increasing the size of the write buffer to 32 MB to sustain temporary large writes. 

\if 0
% MA: if there is anything important here include it in the description of the DBs above in 1-2 sentences

The \textbf{Block Structure Database} stores different types of links between blocks as defined in the \newprism protocol: voting from voter blocks to proposer blocks; referencing from proposer blocks to proposer or transaction blocks; and parental links to proposer blocks or voter blocks. It also stores various metadata, such as the leader proposer block of a level and the order of confirmed proposer blocks. 
% the level of a voter block or a proposer block; the chain number of a voter block;  
%Although those data can all be found in the original blocks, storing them in one database allows the client to quickly follow the reference links and update the ledger. 
The \textbf{Block Database} stores every block that a node has received in its original serialized format. This allows the Block Structure Manager to forward a block to peers without paying the cost of serialization every time it is requested. The \textbf{UTXO Database} stores the mapping between a UTXO and its value and owner. This database is heavily read and written, since executing every transaction requires multiple lookups (and deletions) of the inputs and insertions of the outputs. So we tuned the following RocksDB parameters to improve its performance: replacing B-trees with hash tables as the index; adding bloom filters; adding a 512 MB LRU cache; and increasing the size of the write buffer to sustain temporary large writes. 
%Besides those persistent databases, we have the \textbf{Memory Pool} implemented as an in-memory hash table.

\fi
\subsection{Important Optimizations}

\label{sec:implementation-highlights}

We have implemented a \newprism client in about 10,000 lines of Rust code.
The key challenge to implementing the \newprism client is to handle high throughput. The client must process blocks at a rate of hundreds of blocks per second, or a throughput of hundreds of Mbps, and confirm transactions at a high rate, exceeding 80,000 tps in our implementation. To handle the high throughput, our implementation exploits opportunities for parallelism in the protocol and carefully manages race conditions to achieve high concurrency. We now discuss several key performance optimizations. 

%, and we discuss in detail those design choices in this subsection.


\noindent\textbf{Asynchronous Ledger Updates.}
In traditional blockchains like \bitcoin, blocks are mined at a low rate and clients update the ledger every time they receive a new block.  However, in the \newprism protocol, blocks are mined at a very high rate and a only a small fraction of these blocks\,---\,those that change the proposer block leader sequence\,---\,lead to changes in the ledger. Therefore, trying to update the ledger synchronously for each new block is wasteful and can introduce CPU bottleneck. 

%update the ledger for new block bottlenecks the system

Fortunately, \newprism does not require synchronous ledger updates to process blocks. Since \newprism allows conflicting or duplicate transactions to appear in the ledger and performs sanitization later (\S\ref{sec:confirmation}), the client need not update the ledger for each new block. Therefore, in our implementation, the Ledger Manager runs asynchronously with respect to the Block Structure Manager and periodically updates the ledger. 

Most blockchain protocols (e.g.,  \bitcoin, \algorand, and \bng) require that miners validate a block against the current ledger prior to mining it, and therefore cannot benefit from asynchronous ledger updates. For example, in \bitcoin's current specification, when a miner mines a block $B$, it implicitly certifies a ledger $L$ formed by tracing the blockchain from the genesis block to block $B$. 
A \bitcoin client receiving \textit{B} must therefore verify $B$ against the ledger $L$, and hence must update the ledger synchronously for each block. 
In principle, \bitcoin clients could perform \emph{post hoc} sanitization like \newprism; however, due to long block times relative to transaction verification, doing so would not improve performance.


\noindent\textbf{Parallel Transaction Execution.}
\label{sec:scoreboarding}
%The high rate of transactions asserts heavy pressure on the UTXO Database in particular, since executing every transaction requires multiple lookups and deletions for the inputs, and insertions for the outputs. 
Executing a transaction involves multiple reads and writes to the UTXO Database to (1) verify the validity of the input coins, (2) delete the input coins, and (3) insert the output coins. If handled sequentially, transaction execution can quickly become the bottleneck of the whole system. Our implementation therefore uses a pool of threads in the Ledger Manager to execute transactions in parallel. Despite the  parallelism, the UTXO database is the bottleneck for the entire system (\S\ref{sec:eval-resource}).

However, naively executing all transactions in parallel is problematic, because semantically the transactions in the ledger form an order, and must be executed strictly in this order to get to the correct final state, i.e., UTXO set. For example, suppose  transactions \textit{T} and \textit{T'} both use UTXO \textit{u} as input, and \textit{T} appears first in the ledger. In this case, \textit{T'} should fail, since it tries to reuse \textit{u} when it has already been spent by \textit{T}. If we execute \textit{T} and \textit{T'} in parallel, race condition could happen where the inputs of \textit{T'} are checked before \textit{T} deletes \textit{u} from the UTXO set, allowing \textit{T'} to execute.

To solve this problem, we borrow the \textit{scoreboarding}~\cite{scoreboarding} technique long used in processor design. A CPU employing this method schedules multiple instructions to be executed out-of-order, as long as doing so will not cause conflicts such as writing to the same register. Transactions and CPU instructions are alike, in the sense that they both need to be executed in the correct order to produce correct results, only that transactions read and write UTXOs while CPU instructions read and write CPU registers. 
In the Ledger Manager, a batch of transactions first pass through a controller thread before being dispatched to one of the idle workers in the thread pool for execution. The controller keeps track of the inputs and outputs of the transactions in the batch on a ``scoreboard'' (an in-memory hash table). Before scheduling a new transaction for execution, it checks that none of its inputs or outputs are present on the scoreboard. In this way, all worker threads are able to execute in parallel without explicit synchronization. 

\noindent\textbf{No Transaction Broadcasting.}
In most traditional blockchains, clients exchange pending transactions in their memory pools with peers. This incurs extra network usage, because each transaction will be broadcast twice: first as a pending transaction, and again as part of a block. At the throughput of \newprism, such overhead becomes even more significant.

Our implementation does not broadcast pending transactions, because it is \textit{unnecessary} in \newprism. 
In traditional blockchains like Bitcoin and Ethereum, the whole network mines a block every tens of seconds or even few minutes. 
Since we cannot predict who will mine the next block, exchanging pending transactions is necessary, so that they get included in the next block regardless of who ends up mining it. In contrast, \newprism generates hundreds of transaction blocks every second. This elevated block rate means that any individual miner is likely to mine a transaction block in time comparable to the delay associated with broadcasting a transaction to the rest of the network (i.e., seconds). As a result, unlike other blockchain protocols, there is little benefit for a \newprism client to broadcast its transactions. Non-mining clients can submit their transactions to one or more miners for redundancy; however, miners do not need to relay those transactions to peers. 

\noindent\textbf{Spam Mitigation.}
\label{sec:spamming-design}
In \newprism, miners do not validate transactions before including them in blocks.
This introduces the possibility of spamming, where an adversary could generate a large number of conflicting transactions and send them to different nodes across the network.  
The nodes would then mine all of these transactions into blocks, causing miners and validators to waste storage and computational resources. We note that transaction fees alone cannot prevent such spamming. Since nodes only pay for transactions that make it to into the ledger, the adversary would not be charged for conflicting transactions that get removed during sanitization. 
%spam/duplicate transactions
% There are a few practical mechanisms for circumventing this. 
Bitcoin is not susceptible to this attack because transactions are  validated  {\em prior to} mining. 
We propose a simple mechanism to mitigate spamming. Miners validate transactions with respect to their latest ledger state and other unconfirmed transactions, giving the adversary only a small window of network delay to spam the system. 
Miners then add a random delay prior to mining a transaction into blocks, thus increasing the chance that a miner detects a conflicting transaction in another transaction block, in which case it will drop the delayed spam transaction.
We evaluate the effectiveness of this method in \S\ref{sec:spamming-eval}.



%%%%%%%%%%%%%%%




==> Prism Systems Paper (CCS)/intro.tex <==

\section{Introduction}

In 2008, Satoshi Nakamoto invented \bitcoin and the concept of {\em blockchains}~\cite{bitcoin}. Since then, blockchains have attracted considerable interest for their applications in cross-border payments~\cite{hileman2017global,kazan2015value}, digital contracts~\cite{cong2019blockchain,wust2018you,pilkington201611} and more. At the heart of \bitcoin and many other blockchain projects is the {\em Nakamoto longest chain protocol}. It enables an open (permissionless) network of nodes to reach consensus on an ordered log of transactions and is tolerant to Byzantine adversarial attacks with no more than 50\% of the compute power in the network. To achieve this high level of security, however, the longest chain protocol severely limits transaction throughput and latency  (\S\ref{sec:background}). \bitcoin, for example, supports 3--7 transactions per second and can take hours to confirm a transaction with a high level of reliability~\cite{bitcoin}.  

%Today's cryptocurrencies have poor transaction throughput and slow confirmation times. Bitcoin supports 3--7 transactions per second and can take hours to confirm a transaction with a high level of reliability~\cite{bitcoin}.  The root cause for this poor performance is the {\em Nakamoto longest chain protocol} (\S\ref{sec:background}), a Byzantine fault-tolerant consensus protocol that lies at the heart of Bitcoin and many other cryptocurrencies~\cite{buterin2016ethereum, citeothers}. Roughly speaking, the longest chain protocol enables an open (permissionless) network of nodes to reach consensus on an ordered log of transactions, provided that at least 50\% of the compute power in the network belongs to honest nodes that follow protocol. 

The limitations of the longest chain protocol have led to a flurry of work in recent years on more scalable blockchain consensus protocols (\S\ref{sec:related} discusses related work). However, until recently, no protocol has been shown to guarantee Bitcoin-level security (up to 50\% adversarial power) as well as high throughput and low latency. Prism~\cite{prism-theory} is the first such protocol. Prism is a Proof-of-Work (PoW) blockchain consensus protocol that is  (1) secure against 50\% adversarial compute power, (2) can achieve optimal throughput (up to the network communication bandwidth), and (3) can achieve near-optimal confirmation latency (on the order of the network's propagation delay). Prism removes the throughput and latency limitations of the longest chain protocol by systematically decoupling security and throughput in the blockchain  (\S\ref{sec:overview}).  
%transaction proposal, validation, and confirmation in the blockchain (\S\ref{sec:overview}). 
A recent theoretical paper described the core protocol and analyzed its security properties~\cite{prism-theory}.

While these theoretical results are promising, there are three main limitations. (1) First, the security analysis of \prism in \cite{prism-theory} is in a limited setting (round-by-round synchronous model with a finite time horizon of blockchain operation). Further, the theoretical latency guarantees for \prism \cite{prism-theory} involve large constants (that get larger with increasing time horizon of blockchain operation) -- this  results in  large values of latency in practice.  (2) Second,  the \prism consensus protocol is much more complex than the longest chain protocol: clients must maintain over 1000 distinct blockchains, which refer to each other to create an intricate directed acyclic graph (DAG) structure, and they must process blocks at very high rates (e.g., 100-1000s of blocks per second at 100s of Mbps) to update these blockchains and confirm transactions. %Second, Prism's theoretical analysis relies on several simplifying assumptions (e.g., round-based synchronous communication and a simple network model that ignores queuing delay), and to make the analysis tractable, the performance bounds are specified up to large constants that may not be indicative of real-world performance.  
(3) Third, Prism's theory focuses on the network as the primary performance bottleneck, but a real high-throughput blockchain system must overcome other potential performance bottlenecks. For example, in addition to achieving consensus on a transaction order, clients must also {\em execute} transactions and maintain the {\em state} of the ledger to confirm transaction. Though some academic prototypes ignore transaction execution (e.g., \cite{ohiecode, conflux}),
%\cite{cite-codebases-better-than-papers},
in practice, it often turns out to be the bottleneck due to its high I/O overhead, c.f.,~\cite{raju2018mlsm},  \S\ref{sec:eval-resource}.
Finally, Prism could be vulnerable to spamming, a practical security concern that has not been fully analyzed. 


% the performance of a blockchain system depends on more than the consensus protocol. The consensus protocol orders transactions, but to confirm them, the client must {\em execute} the transactions in order and keep track of the {\em state} of the ledger. 

\begin{figure} 
    \centering
    \includegraphics{figures/compare-fig.pdf}
    \caption{\small Throughput and confirmation latency of \prism, \algorand, \bng, and the longest chain protocol on the same testbed. Note that the axes are on log scales. For \algorand and the longest chain protocol, parameters are tuned to span an optimized tradeoff between throughput and latency at a given security level. For \bng and \prism, throughput and latency are decoupled so one can simultaneously optimize both at one operating point for a given security level. However, the throughput of Bitcoin-NG drops to that of the longest chain protocol under attack, while that of \prism remains high. More details in \S\ref{sec:related} and \S\ref{sec:eval-performance}. }
    \label{fig:compare}
    \vspace{-5mm}
\end{figure}

\noindent {\bf Main Contributions}. 
In this paper, we present the design (\S\ref{sec:design}) and  implementation (\S\ref{sec:implementation}) of a Bitcoin-like system based on the \prism consensus protocol. Our implementation features payments as multi-input-multi-output transactions (payments) similar to pay-to-public-key (P2PK) in Bitcoin and Algorand~\cite{algorand, algorandcode}. We evaluate our system on a testbed of up to 1000 EC2 Virtual Machines connected via an emulated wide area network. Figure \ref{fig:compare} summarizes the results. \prism consistently achieves a throughput of over 70,000 tps for a range of security levels $\beta$ denoting the fraction of adversarial compute power.  To guarantee a reversal probability of less than $10^{-9}$, \prism's latency ranges from 13 seconds against an adversary of power $\beta = 20\%$, to $296$ seconds for $\beta = 44\%$. To our knowledge, this makes our system by far the fastest  implementation of a blockchain system with Bitcoin-level security guarantees. Compared to the longest chain protocol, \prism provides about 10,000$\times$ higher throughput and 1,000$\times$ lower latency. Compared to Algorand~\cite{algorand}, the state-of-the-art proof-of-stake system, \prism achieves 70$\times$ the throughput with about 10 seconds higher latency, and can provide a higher level of security  (up to $\beta = 50\%$ vs. $\beta=33\%$ for Algorand).

We make the following contributions:
\begin{CompactItemize}
    \item We implement a Prism client in roughly 10,000 lines of {\tt Rust} code, and quantify its performance in extensive experiments on EC2. Our result validate Prism's core modeling decisions and theory by showing that it can scale both throughput and latency of the longest chain protocol (without compromising security) in a practical setting. Our code is available here~\cite{prismcode}.
    
    \item Our implementation highlights several performance optimizations, e.g., asynchronous ledger updates, and a scoreboarding technique that enables parallel transaction execution without race conditions (see ~\S\ref{sec:implementation-highlights}). We show that with these careful optimizations, it is possible to alleviate CPU performance bottlenecks and provide linear CPU scaling up to at least 8 cores. At this point, the primary bottleneck for our implementation is the underlying database (RocksDB~\cite{rocksdb} and I/O to the SSD persistent storage). This suggests that future research on databases optimized for blockchain-specific access patterns could further improve performance. 
    
    \item We evaluate practical security concerns like censorship attack, balancing attack, and spamming (see ~\S\ref{sec:eval-attack}). Additionally, we propose a simple solution to the spamming problem that reduces spam traffic by 80\% while only adding 5 seconds to the confirmation delay. Our implementation illustrates that \prism performs well even under these attacks, and makes a stronger case for the practical viability of the system.
    
\end{CompactItemize}

%Our implementation and evaluation provide several key takeaways. First, our results validate Prism's core modeling and design decisions in a practical setting by demonstrating that it can scale both throughput and latency of the longest chain protocol independently of one another without compromising the security guarantee. Second, our implementation shows that with careful performance optimization (see ~\S\ref{sec:implementation-highlights}), it is possible to alleviate CPU performance bottlenecks and provide linear CPU scaling up to \ma{XXX cores}. At this point, the primary bottleneck for our implementation is the underlying database (RocksDB~\cite{rocksdb} and I/O to persistent storage (SSDs)). Therefore future research on databases optimized for blockchain-specific access patterns could provide further performance improvements. 


% e.g., asychoronous ledger updates, and a scoreboarding technique that enables parallel transaction execution without race conditions. We show that these optimizations alleviate CPU performance bottlenecks and provide linear CPU scaling, such that the primary bottleneck is the underlying database (RocksDB~\cite{rocksdb} and I/O to persistent storage (SSDs)). Further performance improvements may therefore be possible by optimizing the database.

The rest of the paper is organized as follows. In \S\ref{sec:related} we discuss different scaling approaches taken in blockchains. In \S\ref{sec:background} we discuss the longest chain protocol and its limitations to motivate the design of the \prism protocol in \S\ref{sec:overview} and \S\ref{sec:design}. We discuss the details of the client implementation with an interface enabling pay-to-public-key transactions in \S\ref{sec:implementation}. Evaluations are presented in \S\ref{sec:eval} to assess the impact of network resources (bandwidth, topology, propagation delay) and computation resources (memory, CPU) on the overall performance. \S\ref{sec:conclusion} concludes the paper.


%%a host of related topics of core interest to the blockchain ecosystem; this includes interfacing Prism to a smart contract programming layer, introduction of light clients (which are simply interested in making and validating specific transactions) and bootstrapping new Prism clients into a running system - each of these is a future direction of research of great interest.


\if 0

% TODO: do we include performance here? Tell the performance first or explain the protocol first?

% TODO: if to compare the performance, what are the baselines? How to compare (cite numbers, run experiments, if so, do we need to optimize their code?) For some of them, modify Prism client into our impelmentation. For algorand, run their code. But what if their implementation is flawed? Explain the results we got (cause of the bottleneck), understand their bottleneck.

% comparisons: Algorand (fame, it could be that their paper is not doing real transactions. use their real code and try to reproduce the number in the paper), Bitcoin (longest chain), OHIE (parallel chain). Remember to point out the security level. This is FINAL.
% mentions: HotStuff
% Point that Conflux is copy cat
% Use Prism 1.0 to help rationale the protocol in Design section.
% Make other system actually do transactions

% Scale of the evaluation
% Hope that the scalability curves are flat, so that reader can assume the scalability (we could provide a breakdown of the CPU/IO resource spent)

% Mention that we have included all possible functions of the client so it is real.

% TODO: make full use of the code. Change parameters to show the idea of other systems.

Text...

Takeaways from experiments. Maybe insert a figure here. % TODO: possibilities: throughput - latency, different protocols take different positions (curve for parameterized ones)

% other potential comparisons: Conflux, Prism 1.0, Bitcoin-NG



Figure 1: comparison of throughput and latency with other blockchain protocols: 

Algorand - best permissionless PoS BFT protocol

longest chain - the original blockchain protocol (frontier as we vary mining rate and block size)

Ohie - parallel chain protocol (give state execution for free)

Prism - our protocol

Network setting (first draft)

100 nodes

artificial delay 300 ms per hop (exponential)

network bandwidth: whatever is sufficient for Prism to achieve 100K Tps. (around 200 to 300Mbps)


\fi


==> Prism Systems Paper (CCS)/intro2.tex <==

\section{Introduction}

In 2008, Satoshi Nakamoto invented \bitcoin and the concept of {\em blockchains}~\cite{bitcoin}. Since then, blockchains have attracted considerable interest for their applications in cross-border payments~\cite{hileman2017global,kazan2015value}, digital contracts~\cite{cong2019blockchain,wust2018you,pilkington201611} and more. At the heart of \bitcoin and many other blockchain projects is the {\em Nakamoto longest chain protocol}. It enables an open (permissionless) network of nodes to reach consensus on an ordered log of transactions and is tolerant to Byzantine adversarial attacks with no more than 50\% of the compute power in the network. To achieve this high level of security, however, the longest chain protocol severely limits transaction throughput and latency. \bitcoin, for example, supports 3--7 transactions per second and can take hours to confirm a transaction with a high level of reliability~\cite{bitcoin}.  

%Today's cryptocurrencies have poor transaction throughput and slow confirmation times. Bitcoin supports 3--7 transactions per second and can take hours to confirm a transaction with a high level of reliability~\cite{bitcoin}.  The root cause for this poor performance is the {\em Nakamoto longest chain protocol} (\S\ref{sec:background}), a Byzantine fault-tolerant consensus protocol that lies at the heart of Bitcoin and many other cryptocurrencies~\cite{buterin2016ethereum, citeothers}. Roughly speaking, the longest chain protocol enables an open (permissionless) network of nodes to reach consensus on an ordered log of transactions, provided that at least 50\% of the compute power in the network belongs to honest nodes that follow protocol. 

\noindent {\bf Prism}. The limitations of the longest chain protocol have led to a flurry of work in recent years on more scalable blockchain consensus protocols (\S\ref{sec:related} discusses related work). 
However, a central challenge in the space has been to guarantee Bitcoin-level security (up to 50\% adversarial power) while also guaranteeing high throughput \emph{and} low latency. 
% \gf{Can we be more specific what we mean by ``high" throughput and ``low" latency? Otherwise reviewers may argue with this assertion}
Prism~\cite{prism-theory} was recently proposed as a solution to this problem.
Prism is a Proof-of-Work (PoW) blockchain consensus protocol that is theoretically shown to achieve (1) security against 50\% adversarial compute power, (2) optimal throughput (up to the network communication bandwidth), and (3) near-optimal confirmation latency. %\ma{This statement might seem in conflict with the claim in the next paragraph about Prism's current latency guarantees. Is there a better way to put this?}
% Prism removes the throughput and latency limitations of the longest chain protocol by systematically decoupling security and throughput in the blockchain.   
% %transaction proposal, validation, and confirmation in the blockchain (\S\ref{sec:overview}). 
% A recent theoretical paper described the core protocol and analyzed its security properties~\cite{prism-theory}.

\noindent {\bf Limitations of Prism}. 
While these theoretical results are promising, there are three main limitations. 
(1) First, the security analysis of \prism in \cite{prism-theory} is in a limited setting (round-by-round synchronous model with a finite time horizon of blockchain operation). The finite time horizon strictly limits the usability of the security in practice: the resulting confirmation error probability (i.e. the probability of a double-spend) depends on the duration of time horizon, getting worse as the time horizon increases.  
This shortcoming in turn forces the confirmation rule in \cite{prism-theory} to also depend on the finite time horizon, rendering the guarantees practically useless.
% and its theoretical latency bounds involving large 
% Further, the theoretical latency guarantees for \prism \cite{prism-theory} involve large constants that get larger with increasing time horizon of blockchain operation -- this  results in  high latency values in practice.  
(2) Second,  the \prism consensus protocol is more complex than the longest chain protocol: clients must maintain over 1000 distinct blockchains, which refer to each other to create an intricate directed acyclic graph (DAG) structure, and they must process blocks at very high rates (e.g., 100-1000s of blocks per second at 100s of Mbps) to update these blockchains and confirm transactions. 
A naive system design can easily introduce performance bottlenecks that would prevent Prism from achieving the theoretically-promised scaling properties.
For example, in addition to achieving consensus on a transaction order, clients must also {\em execute} transactions and maintain the {\em state} of the ledger to confirm transaction. Though some academic prototypes ignore transaction execution (e.g., \cite{ohiecode, conflux}),
%\cite{cite-codebases-better-than-papers},
in practice, it often turns out to be the bottleneck due to its high I/O overhead, c.f.,~\cite{raju2018mlsm},  \S\ref{sec:eval-resource}.
Unfortunately, \cite{prism-theory} does not explain how to design the Prism client architecture to avoid such bottlenecks. 
% It is unclear if a successful transition from algorithm to an efficient system design can be enabled.  %Second, Prism's theoretical analysis relies on several simplifying assumptions (e.g., round-based synchronous communication and a simple network model that ignores queuing delay), and to make the analysis tractable, the performance bounds are specified up to large constants that may not be indicative of real-world performance.  
(3) Third, to date there is no practical evaluation  of Prism's performance. \cite{prism-theory} provides simulations, but because of limitation (1), these simulations may not be indicative of real-world performance. 

%Finally, Prism could be vulnerable to spamming, a practical security concern that has not been fully analyzed. 

 

\begin{figure} 
    \centering
    \includegraphics{figures/compare-fig.pdf}
    \caption{\small Throughput and confirmation latency of \prism, \algorand, \bng, and the longest chain protocol on the same testbed. Note that the axes are on log scales. For \algorand and the longest chain protocol, parameters are tuned to span an optimized tradeoff between throughput and latency at a given security level (details in \S\ref{sec:eval}). 
    %\gf{This is confusing--it's not clear what parameter(s) are being varied in the Algorand and longest-chain curves. Should we add more detail?} \ly{details of tuning are provided in seciton 7.} 
    %\ly{The circle indicates the performance under the default parameters chosen by the original Algorand implementation.} 
     For \bng and \prism, throughput and latency are decoupled so one can simultaneously optimize both at one operating point for a given security level. However, the throughput of Bitcoin-NG drops to that of the longest chain protocol under attack, while that of \prism remains high. More details in \S\ref{sec:related} and \S\ref{sec:eval-performance}. 
    }
    \label{fig:compare}
    \vspace{-5mm}
\end{figure}

\noindent {\bf Main Contributions}. 
In this paper, we resolve each of these three  limitations of \prism.  Specifically: 
\begin{CompactItemize}
\item 
  {\bf Theory and Algorithms}. We  design a new, simple confirmation rule for \prism that does not depend on a finite time horizon for its security. 
  This new rule is designed to enable explicit identification of the worst-case adversarial attack, 
  which allows us to sharply characterize the confirmation error probability in    a  general, continuous-time  %cryptographic \ly{not sure if cryptographic is precise} 
  model over an infinite time  horizon of blockchain operation.  
  In general, identifying worst-case attacks on consensus protocols is considered challenging; our approach of co-designing a confirmation rule along with a worst-case attack is novel, to the best of our knowledge.
  This methodology also allows us  to sharply characterize the worst-case latency of confirmation, which we show to be a  small constant of the block interarrival time (e.g., for adversarial hash power $\beta$ of 20\%, the latency is roughly a factor of 12 of the block interarrival time). 
%   ; \prism decouples security of confirmation from latency). 
  This is elaborated in   \S\ref{sec:new_rule}.
  
  \item {\bf  Algorithms to System Design and Implementation}. We provide a system design of a Prism client that can be used to evaluate the theoretical performance scaling claims. The design includes several crucial performance optimizations, such as asynchronous ledger updates and a scoreboarding technique that enables parallel transaction execution without race conditions. We subsequently discuss the details of our implementation of a Prism client in roughly 10,000 lines of {\tt Rust} code.
  Our implementation features payments as multi-input-multi-output transactions similar to pay-to-public-key (P2PK) in Bitcoin and Algorand~\cite{algorand, algorandcode}, and includes several Prism-specific optimizations to enhance performance. 
%   Our implementation includes several optimizations
%   It also includes a simple, lightweight solution to out-of-model spamming attacks. 
  This system design is the focus of \S\ref{sec:design}.
  
  \item {\bf  Implementation and Evaluation}. 
  We evaluate our system on a testbed of up to 900 EC2 Virtual Machines connected via an emulated wide area network.   Our result (summarized in Figure~\ref{fig:compare}) validates Prism's core modeling decisions and the new confirmation rule by showing that it can scale both throughput and latency in a practical setting. 
  \prism achieves a consistent throughput of over 80,000 tps for different security levels $\beta$, denoting the fraction of adversarial compute power.  To guarantee a reversal probability of less than $10^{-9}$, \prism incurs a latency of 42 seconds against an adversary of power $\beta = 20\%$, or 182 seconds for $\beta = 33\%$. 
  %To our knowledge, this makes our system the highest-throughput blockchain implementation with Bitcoin-level security guarantees. 
  Compared to Bitcoin, \prism provides about 10,000$\times$ higher throughput and 1,000$\times$ lower latency. Compared to Algorand~\cite{algorand}, the state-of-the-art proof-of-stake system, \prism achieves 70$\times$ the throughput with about 20 seconds higher latency, and can provide a higher level of security  (up to a $\beta = 50\%$ fully-adaptive adversary vs. $\beta=33\%$ for Algorand). This is the focus of  \S\ref{sec:eval}.
  
  
 %\item We show that with these careful optimizations, it is possible to alleviate CPU performance bottlenecks and provide linear CPU scaling up to at least 8 cores. At this point, the primary bottleneck for our implementation is the underlying database (RocksDB~\cite{rocksdb} and I/O to the SSD). This suggests that future research on databases optimized for blockchain-specific access patterns could further improve performance. 

% \item
% We evaluate several practical attacks like censorship attack, balancing attack, and spamming (see ~\S\ref{sec:eval-attack}). Additionally, we propose a simple solution to the spamming problem that reduces spam traffic by 80\% while only adding 5 seconds to the confirmation delay. Our implementation illustrates that \prism performs well even under these attacks, and makes a stronger case for the practical viability of the system.
% \gf{let's remove this bullet? seems second order and raises questions about fig. 1--i.e. wasn't fig. 1 evaluated under attack?}

\end{CompactItemize}

%Our implementation and evaluation provide several key takeaways. First, our results validate Prism's core modeling and design decisions in a practical setting by demonstrating that it can scale both throughput and latency of the longest chain protocol independently of one another without compromising the security guarantee. Second, our implementation shows that with careful performance optimization (see ~\S\ref{sec:implementation-highlights}), it is possible to alleviate CPU performance bottlenecks and provide linear CPU scaling up to \ma{XXX cores}. At this point, the primary bottleneck for our implementation is the underlying database (RocksDB~\cite{rocksdb} and I/O to persistent storage (SSDs)). Therefore future research on databases optimized for blockchain-specific access patterns could provide further performance improvements. 


% e.g., asychoronous ledger updates, and a scoreboarding technique that enables parallel transaction execution without race conditions. We show that these optimizations alleviate CPU performance bottlenecks and provide linear CPU scaling, such that the primary bottleneck is the underlying database (RocksDB~\cite{rocksdb} and I/O to persistent storage (SSDs)). Further performance improvements may therefore be possible by optimizing the database.

\noindent {\bf Network and Security Model}. We adopt the now-standard  $\Delta-$synchronous network model for longest chain protocol analysis  \cite{ren2019analysis,dembo2020everything};  here the adversary controls the delivery of messages but the end-to-end network delay between any two nodes is upper bounded by $\Delta$. Also, following standard convention \cite{bitcoin,ren2019analysis,dembo2020everything,gazi2020tight}, we model the block mining process as Poisson with rate $\lambda$ proportional to the hash power of the miner. 
The adversary is assumed to control a fraction $\beta$ of the total hash power.


\noindent {\bf Organization}. 
The rest of the paper is organized as follows. In \S\ref{sec:related} we overview different  approaches to scaling  blockchain performance. In \S\ref{sec:scaling} we discuss the \prism protocol and its limitations.  In \S\ref{sec:new_rule}, we propose a new confirmation rule to \prism along with   formal guarantees on security and low worst-case latency.  \S\ref{sec:design} discusses the practical challenges when turning the algorithm into a working system, as well as  the details of the client implementation with an interface enabling pay-to-public-key transactions.  %\ma{broken reference}. Evaluations are presented in \S\ref{sec:eval} to measure the performance of the system, assess the utilization of network resources (bandwidth, topology, propagation delay) and computation resources (memory, CPU), and impacts of various attacks (balancing attack, censorship attack, spamming). \S\ref{sec:conclusion} concludes the paper.


%%a host of related topics of core interest to the blockchain ecosystem; this includes interfacing Prism to a smart contract programming layer, introduction of light clients (which are simply interested in making and validating specific transactions) and bootstrapping new Prism clients into a running system - each of these is a future direction of research of great interest.


\if 0

% TODO: do we include performance here? Tell the performance first or explain the protocol first?

% TODO: if to compare the performance, what are the baselines? How to compare (cite numbers, run experiments, if so, do we need to optimize their code?) For some of them, modify Prism client into our impelmentation. For algorand, run their code. But what if their implementation is flawed? Explain the results we got (cause of the bottleneck), understand their bottleneck.

% comparisons: Algorand (fame, it could be that their paper is not doing real transactions. use their real code and try to reproduce the number in the paper), Bitcoin (longest chain), OHIE (parallel chain). Remember to point out the security level. This is FINAL.
% mentions: HotStuff
% Point that Conflux is copy cat
% Use Prism 1.0 to help rationale the protocol in Design section.
% Make other system actually do transactions

% Scale of the evaluation
% Hope that the scalability curves are flat, so that reader can assume the scalability (we could provide a breakdown of the CPU/IO resource spent)

% Mention that we have included all possible functions of the client so it is real.

% TODO: make full use of the code. Change parameters to show the idea of other systems.

Text...

Takeaways from experiments. Maybe insert a figure here. % TODO: possibilities: throughput - latency, different protocols take different positions (curve for parameterized ones)

% other potential comparisons: Conflux, Prism 1.0, Bitcoin-NG



Figure 1: comparison of throughput and latency with other blockchain protocols: 

Algorand - best permissionless PoS BFT protocol

longest chain - the original blockchain protocol (frontier as we vary mining rate and block size)

Ohie - parallel chain protocol (give state execution for free)

Prism - our protocol

Network setting (first draft)

100 nodes

artificial delay 300 ms per hop (exponential)

network bandwidth: whatever is sufficient for Prism to achieve 100K Tps. (around 200 to 300Mbps)


\fi


==> Prism Systems Paper (CCS)/intro3.tex <==
\section{Introduction}
In 2008, Satoshi Nakamoto invented \bitcoin and the concept of {\em blockchains}~\cite{bitcoin}. Since then, blockchains have attracted considerable interest for their applications in cross-border payments~\cite{hileman2017global,kazan2015value}, digital contracts~\cite{cong2019blockchain,wust2018you,pilkington201611} and more. At the heart of \bitcoin and many other blockchain projects is the {\em Nakamoto longest chain protocol}. It enables an open (permissionless) network of nodes to reach consensus on an ordered log of transactions. 

A distinguishing feature Nakamoto's protocol is the use of proof-of-work (PoW) consensus. A node gets the right to propose a block of transactions by solving a cryptographic puzzle, a process called ``mining''. Each mined block refers to a previous block, extending a chain, and an honest miner always tries to extend the longest chain. A block is ``confirmed'' when it is embedded $k$-deep in the longest chain, where $k$ is a parameter controlling the probability of reversal, i.e. the probability that another chain could ever overtake the longest chain. 
%The confirmation depth $k$ is the number of blocks mined on top of the confirmed block, and can be interpreted as the number of votes on that block. 
The protocol is secure against Byzantine adversaries controlling no more than 50\% of the network’s compute power. However, achieving this high level of security comes at severe cost to throughput and latency, since it requires the block mining time to be long to reduce forking and the confirmation depth $k$ to be large to make the reversal probability small.  \bitcoin, for example, supports 3--7 transactions per second and can take hours to confirm a transaction with a high level of reliability~\cite{bitcoin}.  

Improving the throughput of PoW consensus has received significant attention in recent years. Proposals range from simply increasing the block size~\cite{bitcoinsize} to restructuring the protocol to scale throughput arbitrarily on top of a slowly growing (and hence secure) longest chain~\cite{bitcoin-ng, ohie, fruitchains}. Improving {\em latency}, however, is much more difficult.  No existing protocol can achieve low latency (e.g., a small multiple of the network delay) while maintaining the security of longest chain protocol. A recent attempt, Prism~\cite{prism-theory}, took an important step: sortition blocks into proposer blocks and voter blocks, and the voter blocks are further sortitioned into multiple parallel ``voter chains’’ to reduce confirmation latency. The idea is to confirm a proposer block using voter blocks from  many chains, each mined independently using the longest chain protocol. With many votes, one can confirm much faster, because although each such vote is not very deep in its respective longest chain (hence not reliable), overall high reliability can still be achieved because there are many independent voting chains.

While the idea of multiple voter chains is elegant, the Prism protocol’s latency is far from ideal. Confirming blocks requires a confirmation rule to compute the reversal probability as a function of the state of the voter chains (analogous to the standard k-deep rule for the longest chain protocol). Prism provides such a rule and proves that it guarantees latency that is a constant multiple of the network delay. But the constant is huge and crucially depends on the time horizon of the blockchain’s operation, making the bound useless in practice. Our analysis shows that Prism's confirmation rule implies a latency bound of several hours depending on the adversarial mining power assumed. To ensure security, there is no choice but to wait until the confirmation rule guarantees the desired level of reliability; we show that in practice this leads to a high latency in \prism. Moreover, the reliability of the confirmation rule depends on using a large number of voter chains (tens of thousands), which is difficult if not impossible to realize in real systems. 

%Therefore, a confirmation rule with large constants is not merely of theoretical concern: it makes the protocol useless in practice.

The second challenge is that parallel voting chain protocols are much more complex to implement than the longest chain protocol. Nodes must process hundreds to thousands of blocks per second in real time, putting significant strain on system. The high block rate and intricate state updates impose a particularly high I/O requirements on databases and persistent storage. Thus it is unclear to what extent the theoretical performance properties can translate to real-world performance. 

In this paper, we present \newprism, the first practical PoW consensus protocol to achieve low latency, high throughput, and Bitcoin-level security. \newprism solves the two challenges above by providing the following contributions:
\begin{itemize}
  \item The first confirmation rule for parallel voting chains that has provably low latency and Bitcoin-level security. This rule is designed to enable explicit identification of the worst-case adversarial attack, which allows us to sharply characterize the confirmation error probability in a general, continuous-time model over an infinite time horizon of operation. Identifying worst-case attacks on consensus protocols is challenging, and our approach of co-designing a confirmation rule along with a worst-case attack is novel, to the best of our knowledge. This methodology also allows us to sharply characterize the worst-case latency of confirmation, which we show to be a small constant of the block interarrival time (e.g., for adversarial hash power $\beta$ of 20\%, the latency bound is roughly a factor of 12 of the block interarrival time). This is elaborated in   \S\ref{sec:new_rule}.

  \item An end-to-end system implementation and evaluation of \newprism, showing that it can achieve both low latency and high throughput (near theoretical predictions) in practice. Our implementation, written in 10,000 lines of Rust, supports pay-to-public-key UTXO transactions (similar to \bitcoin) and includes several crucial performance optimizations, such as asynchronous ledger updates and a scoreboarding technique to enable multi-threaded transaction execution. We evaluate it on a testbed of up to 900 EC2 machines connected via an emulated wide-area network. Fig.~\ref{fig:compare} shows the main results: \newprism achieves 30$\times$ lower latency than the longest chain protocol, and delivers a high throughput of 80,000 tps.
  \end{itemize}

\noindent {\bf Network and  Security Model}. We adopt the now-standard  $\Delta-$ 
synchronous network model for longest chain protocol analysis  \cite{ren2019analysis,dembo2020everything};  here the adversary controls the delivery of messages but the end-to-end network delay between any two nodes is upper bounded by $\Delta$. Also, following standard convention \cite{bitcoin,ren2019analysis,dembo2020everything,gazi2020tight}, we model the block mining process as Poisson with rate $\lambda$ proportional to the hash power of the miner. 
The adversary is assumed to control a fraction $\beta$ of the total hash power.

\smallskip
\noindent {\bf Organization}. 
The rest of the paper is organized as follows. In \S\ref{sec:related} we overview different  approaches to scaling  blockchain performance. In \S\ref{sec:scaling} we provide a short background on the \prism protocol and explain its limitations. In \S\ref{sec:new_rule}, we propose our novel confirmation rule for parallel voting chain, along with formal guarantees on security and low worst-case latency. \S\ref{sec:design} discusses the practical challenges when turning the algorithm into a working system, as well as the details of the client implementation with an interface enabling pay-to-public-key transactions. 

\begin{figure} 
    \centering
    \includegraphics{figures/compare-fig.pdf}
    \caption{\small Throughput and confirmation latency of \newprism, \algorand, \bng, and the longest chain protocol on the same testbed. Note that the axes are on log scales. For \algorand and the longest chain protocol, parameters are tuned to span an optimized tradeoff between throughput and latency at a given security level (details in \S\ref{sec:eval}). 
     For \bng and \newprism, throughput and latency are decoupled so one can simultaneously optimize both at one operating point for a given security level. However, the throughput of Bitcoin-NG drops to that of the longest chain protocol under attack, while that of \newprism remains high. More details in \S\ref{sec:related} and \S\ref{sec:eval-performance}.
    }
    \label{fig:compare}
\end{figure}


==> Prism Systems Paper (CCS)/newprism.tex <==
\section{A New Confirmation Rule for \prism}
\label{sec:new_rule}

In this section, we propose the confirmation rule of \newprism, a simple confirmation rule for Prism-style parallel voting that is secure with high probability and guarantees fast confirmation.

\noindent {\bf Intuition}. The high-level idea of the confirmation rule is that we can confirm a proposer block $B$ at a certain level $\ell$ when no other proposer block at level $\ell$ can ever receive more votes than $B$ in the future. Suppose that an $h$-fraction of voter chains have \textit{stabilized} with high probability, i.e., their votes will not change in the future. Further, suppose that $V$  voter chains vote for some other proposer block instead of $B$ at level $\ell$. 
Then, with high probability, $B$ will eventually receive at least $h m - V$ votes while any other proposer block at level $\ell$ could receive at most $V + m(1-h)$ votes. As a result, we can confirm $B$ if $h m-V>V+m(1-h)$, i.e., $h>\frac{V}{m}+\frac{1}{2}$. Note that $V$ is observable from the blockchain, so the only task now is to estimate $h$.

The key observation is that $h$ is a monotonically increasing function of time. This is because each voter chain follows the longest chain rule, where a prefix of the longest chain will stabilize as the chain grows longer (which happens as time passes). Although time is not observable in a PoW blockchain, it can be estimated from the growth of the voter chains. The large number of voter chains in \prism makes this estimation accurate even for short time periods because of the law of large numbers. 

\noindent {\bf Confirmation rule}.  Let $\tau_\ell$ be the time when a proposer block at level $\ell$ is mined or received by an honest node for the first time. According to the $\Delta$-synchronous model, at $\tau_\ell + \Delta$, all honest nodes will start voting for a proposer block at level $\ell$. 

Let $B_\ell(t)$ be the proposer block at level $\ell$ that receives the most votes at time $\tau_\ell + \Delta + t$, and let $\bar V_\ell(t)$ be the number of votes received by proposer blocks at level $\ell$ other than $B_\ell(t)$.
Let $d_i(t)$ be the depth of the voter block on the $i$-th voter chain which votes for a proposer block of level $\ell$ at time $\tau_\ell +\Delta + t$. If the $i$-th voter chain has not voted for any block on level $\ell$ at time $\tau_\ell +\Delta + t$, then $d_i(t)=0$.

For a single voter chain, let $q_t(\lambda_h,\lambda_a,\Delta,\pi)$ be the success probability of a certain attack $\pi$ to reverse the voter block that votes for a proposer block at level $\ell$ after time $\tau_\ell+\Delta+t$. Here, $\lambda_h = (1-\beta)\lambda$ is the honest mining rate, $\lambda_a = \beta \lambda$ is the adversarial mining rate, and $\Delta$ is the upper bound of the network delay.
Let $\pi^*(\lambda, \Delta)$ be the worst-case attack in terms of maximizing the success probability $q_t$.
Then, we define the {\em effective vote} for a proposer block at level $\ell$ from a voter chain at time $t + \tau_\ell+\Delta$ to be the fraction 
\begin{equation*}
    h^\Delta(t) := 1 - q_t(\lambda_h,\lambda_a,\Delta,\pi^*). 
\end{equation*}
We will derive an expression for $h^\Delta(t)$ later in this section. Now with all these definitions, we can propose the \newprism confirmation rule.

\begin{defn}[\newprism Confirmation Rule]
\label{def:rule}
We confirm $B_\ell(T)$ at time $\tau_\ell + \Delta + T$ if 
$$h^\Delta\left(\frac{1}{(1+\delta)m\lambda}\sum_{i=1}^{m} d_i(T)\right) \geq \frac{1}{m} \bar V_\ell(T) + \frac{1}{2} +\delta$$ 
for some small constant $\delta >0$ which controls the confirmation confidence. Note that $\tau_\ell + \Delta + T$ is an arbitrary time that an honest node chooses to observe the blockchain.
\end{defn}

\subsection{Deriving the New Confirmation Rule}

\noindent {\bf Outline}. Although the confirmation rule described above is simple, its security proof hinges on several building blocks. We start by focusing on the ideal case where the network delay is zero ($\Delta = 0$), all users are online (so that they observe when blocks appear), and only one public proposer block exists on each level. This allows us to focus on the voter chains.

We first revisit the security of the $k$-deep confirmation rule in the longest chain protocol, and introduce an alternative time-based confirmation rule (applicable for online users) on the single voter chain case. This time-based confirmation rule is readily extended to \prism-style parallel voting (with the proof for security similarly extensible) and achieves a much shorter confirmation latency compared to the longest chain protocol for the same reversal probability. Finally, we strengthen the time-based confirmation rule to handle the general setting: (a) offline users (making the confirmation rule only depend on the depth of the voter chains); (b) non-zero network delay $\Delta$; (c) multiple proposer blocks on the same level. This leads to the new \newprism confirmation rule as in Definition \ref{def:rule}.

{\bf \noindent \prism with one voter chain}. Before heading into the full Prism structure, we first take a look at the behavior of \prism with one voter chain ($m=1$), where the stabilized prefix of the single voter chain selects one leader proposer block at each level. The voter chain follows the Nakamoto longest chain protocol, which has a simple $k$-deep confirmation rule: confirm a block when it is buried $k$-blocks deep in the longest chain. This rule is remarkable in that it can be verified by nodes that join the protocol at any time, even much later than when the confirmed blocks first arrived. If we make the assumption that all nodes are {\em online} so that they observe when exactly a block arrives, then we can confirm a voter block (or equivalently the proposer block voted by it) based on time: a proposer block at level $\ell$ is confirmed $t$ seconds after the first block at level $\ell$ is received. Here, $t$ is a parameter to be chosen. We call this time-based confirmation rule the $t$-wait confirmation rule of this single voter chain scheme.

The reversal probability (the probability that a different proposer block at the same level will be selected in the future) of the $t$-wait confirmation rule is also the success probability of the worst-case attack  $q_t(\lambda_h,\lambda_a,0,\pi^*)$ by our definition. For the special case of $\Delta = 0$, a recent work~\cite{dembo2020everything} identified the worst-case attack on the $k$-deep rule: Theorem 5.1 of \cite{dembo2020everything} shows that the \textit{private attack} (with pre-mining proposed in \cite{sompolinsky2016bitcoin}) is the worst-case attack for every sample path. Following a similar logic, we prove that the same private attack is the worst case attack on the $t$-wait rule (see Appendix~\ref{app:proof}). 
To simplify the notation, we let $q_t^0(\lambda_h,\lambda_a) \triangleq q_t(\lambda_h,\lambda_a,0,\pi^*)$.

In the pre-mining phase of the worst-case attack $\pi^*(\lambda, 0)$ (before any proposer block at level $\ell$ is received by all honest nodes, which, say, happens at time $\tau$), the adversary builds up a private chain with the maximum lead over the public voter chain, and the (random) length of such maximum lead at time $\tau$ is stochastically dominated by a Geometric distribution with parameter $p = 1-\frac{\lambda_a}{\lambda_h}$. After a proposer block is received by all honest nodes at time $\tau$, the honest nodes will start mining voter blocks to vote for that block, while the adversary starts a private attack from the maximum lead. The numbers of adversarial blocks and honest blocks mined in the time interval $(\tau, \tau+t)$ follow Poisson distributions with mean $\lambda_a t$ and $\lambda_h t$. If the pre-mined lead plus the newly-mined adversarial blocks is no less than the number of honest blocks at time $\tau+t$, then the attack succeeds; otherwise, from  simple random walk theory, the probability that the adversary will ever catch up from $z$ blocks behind is given by $\left(\frac{\lambda_a}{\lambda_h}\right)^z$ when $\lambda_a < \lambda_h$. 
Therefore, we have a closed-form expression for  $q_t^0(\lambda_h,\lambda_a)$: 
\begin{eqnarray*}
    &&~~~~~q_t^0(\lambda_h,\lambda_a) = 1 - \sum_{l = 0}^{\infty} \left(1 - \frac{\lambda_a}{\lambda_h}\right) \left( \frac{\lambda_a}{\lambda_h} \right)^l \cdot \\
    &&\left( \sum_{k = l}^{\infty} e^{-\lambda_h t} \frac{(\lambda_h t)^k}{k!} \cdot \sum_{n=0}^{k-l} e^{-\lambda_a t} \frac{(\lambda_a t)^n}{n!} \left (1-(\frac{\lambda_a}{\lambda_h})^{k-n-l} \right) \right).
\end{eqnarray*}
As a result, $h^0(t) = 1 - q_t^0((1-\beta)\lambda,\beta \lambda)$ is simply a function of $\lambda$ and $\beta$. 
%\begin{eqnarray*}
%    h^0(t) = \sum_{l = 0}^{\infty} \frac{1-2\beta}{1-\beta} \big( \frac{\beta}{1-\beta} \big)^l \cdot ~~~~~~~~~~~~~~\\
%    \Big( \sum_{k = l}^{\infty} e^{-(1-\beta)\lambda t} \frac{((1-\beta) \lambda t)^k}{k!} \cdot ~~~~~~~~~~~\\
%    \sum_{n=0}^{k-l} e^{-\beta \lambda t} \frac{(\beta \lambda t)^n}{n!} \big (1-(\frac{\beta}{1-\beta})^{k-n-l} \big) \Big).
%\end{eqnarray*}
Fig.~\ref{fig:h0_t} shows $h^0(t)$ for $\beta = 0.3$, where we see the exponential rise to unity. Recall that $h^0(t)$ is the probability that a proposer block is stabilized forever after duration $t$ since the block is mined. Indeed, this scheme achieves the same exponential security level as the longest chain protocol~\cite{ren2019analysis,backbone}, i.e., 
$$h^0(t) \geq 1 - A e^{-a\lambda t}$$
for large $t$, where positive constants $A$ and $a$ only depend on $\beta$. So, in order to achieve a very small error probability $\epsilon$ (we use $\epsilon = 10^{-9}$ in our experiments), the latency of this scheme $\tau_{single}$ should satisfy $h^0(\tau_{single}) \geq 1 - \epsilon$, i.e.,
\begin{equation*}
    \tau_{single} = O\left(\frac{1}{\lambda} \cdot \log{\frac{1}{\epsilon}}\right).
\end{equation*}
For example, we can compute that $\tau_{single} \approx 225/\lambda$ when $\beta = 0.3$ and $\epsilon = 10^{-9}$.

\begin{figure}
    \centering
    \includegraphics[width=0.35\textwidth]{figures/h0_t.png}
    \caption{Fraction of effective votes on the single proposer block (blue) and a potential private block (green).}
    \label{fig:h0_t}
\end{figure}

{\bf \noindent A time-based confirmation rule}. Returning to the Prism structure with many voter chains, we look for a similar time-based confirmation rule. Suppose an online node is aware of the arrival time $\tau_\ell$ of the only \textit{public} proposer block at level $\ell$ (\textit{private} proposer blocks could potentially exist), then when can the node confirm that proposer block? If the node had to wait long enough for every voter block that votes for this proposer block to stabilize, i.e., $h^\Delta \to 1$, then there would be no latency improvement over the longest chain protocol.

In fact, this is not necessary, because we only care about the sum of the votes. 
As long as $h^{\Delta}$, the probability of one voter block staying stable, is greater than 0.5, the adversary cannot reverse more than half of the votes except for probability exponentially small in $m$. This is because of the law of large numbers and the large deviation effect. % In Prism, we can achieve arbitrarily small error probability $\epsilon$ by scaling the number of voter chains $m$. By Law of Large Numbers, the probability that the adversary gets more than half of the votes for its private block is exponentially small in $m$ as long as the probability that a vote that can be displaced from its longest chain is less than $1/2$ in each voter chain. 
So, when there is only one public proposer block at level $\ell$, we can simply confirm it when $h^{\Delta}(\cdot) > 1/2$. %\ly{I think $\delta$ accounts for the finite $m$. Should we give a hint here? Otherwise $\delta$ is discussed only later in the text.} 
Although a vote from a particular voter chain may be reversed in the future with non-negligible probability (around $1/2$), the majority of the votes will stay stable when $m$ is large. The only challenge is that all online nodes may not agree on the proposer block arrival time $\tau_\ell$ due to network delay -- but this is not a problem when $\Delta = 0$. As a result, assuming $\Delta = 0$, we have the following time-based confirmation rule for Prism. 

\begin{defn}[CR1]
Assume nodes are aware of $\tau_\ell$, the arrival time of the only public proposer block at level $\ell$. Then, they confirm the proposer block at time $t_c$ such that $t_c = \tau_\ell + t_\delta^* $, where $h^0(t_\delta^*) = \frac{1}{2} + \delta$ for  some small constant $\delta > 0$ which controls the confirmation error probability.
\end{defn}

{\bf \noindent From time to depth}. Conventionally, we prefer a confirmation rule based on block depth rather than time, following the idea of the $k$-deep rule in the longest chain protocol. We can easily convert CR1 to a depth-based version: confirm the proposer block when more than $m\lambda t_\delta^*$ voter blocks are mined after $\tau_\ell$.
However, an offline node cannot execute this rule, because it does not know $\tau_\ell$. Instead, we can estimate the time by counting the depth of the voter blocks that vote for the public proposer block at level $\ell$, which is observable even for offline users. Therefore, we propose the following depth-based confirmation rule depending entirely on the {\em observable} blockchain.

\begin{defn}[CR2]
At time $\tau_\ell + t$, let $d_i(t)$ be the depth of the voter block on the $i$-th voter chain that votes for a proposer block of level $\ell$, or $d_i(t)=0$ if no such a voter block exists yet. Let $t_\delta^*$ satisfy $h^0(t_\delta^*) = \frac{1}{2} + \delta$ for $0 < \delta < \frac{1}{2}$ as in CR1. Then, at time $\tau_\ell + T$, if there is only one public proposer block on level $\ell$ and $\sum_{i=1}^{m} d_i(T) \geq (1+\delta)m\lambda t^*_\delta$, we can confirm this proposer block. Note that $\tau_\ell + T$ is an arbitrary time chosen by an honest node to observe the blockchain.
\end{defn}

\begin{remark}
Note that the conversion from time to block depth here is conservative as we assume each voter chain grows at the full rate $\lambda$ and the estimated time is an upper bound of the actual time elapsed. However, under the worst-case attack (private attack with pre-mining for $\Delta = 0$), each public voter chain grows at rate $(1-\beta) \lambda$. So a possibly better confirmation rule with lower latency would be to confirm the proposer block when $\sum_{i=1}^{m} d_i(T) \geq (1+\delta)m(1-\beta)\lambda t^*_\delta$. We conjecture this rule is also secure but defer a formal security proof as a future direction. 
\end{remark}

%\begin{remark}
%The confirmation rule in Appendix A assumes that the adversary launches private attack on all the voter chains and the sum of the depths of the votes in the public voter chains is also used to estimate the time that has passed. Then the time is further used to estimate the length of the private chains and the effective vote on each voter chain is calculated individually by applying $k$-deep confirmation rule based on the observed depth of the voter block. Here in CR3 we directly apply the $t$-wait confirmation rule on each voter chain. \ly{does it refer to the old rule?} \xw{can we cite the earlier arxiv version?} \pv{This is a distraction for the reviwer. I propose we get rid of the review. We can bring it back with a detailed discussion in the final publication.}
%\end{remark}

Note that under the normal path (with no adversarial action), each voter chain grows as a Poisson process with rate $\lambda$, so the confirmation latency of CR2 is concentrated around $t^*_\delta$ as $m$ is large. Later, we will show that for a fixed error probability $\epsilon$, we can choose very small slack $\delta$ by increasing $m$. Therefore, the confirmation latency is around $t^*_0$, where $h^0(t^*_0)=1/2$.%\ly{our experiment results differs from this conclusion. should we explain that the real latency is longer because of forking, proposer, etc.?} \pv{not at this stage. any explanation will confuse the reader. Lei: It would be good to discuss the discrepancy between theory and practice in the evaluation section} \xw{I agree. This theoretical value assumes $m = \infty$ and $\Delta = 0$. In the evaluation section, you can say finite $m$ and the network delay make the actual latency to be longer. }
So the latency of \prism $\tau_{Prism}$ under the normal path would be
\begin{equation*}
    \tau_{Prism} = O\left(\frac{1}{\lambda}\right),
\end{equation*}
which is independent of the error probability $\epsilon$ when we choose $m$ to be large enough. For example, $\tau_{Prism} \approx 5/\lambda$ when $\beta = 0.3$. 

{\bf \noindent From $\Delta = 0$ to $\Delta > 0$}.  For a non-zero $\Delta$, characterizing the worst-case attack is challenging, but we are only interested in the regime where the mining rate of each voter chain is low, i.e., $\lambda \Delta \ll 1$. In Appendix \ref{app:proof_sketch}, we show that $q_t(\lambda_h,\lambda_a,\Delta, \pi^*(\lambda, \Delta)) =  q_t(\lambda_h,\lambda_a,\Delta, \pi^*(\lambda, 0)) + O(\lambda^2 \Delta^2)$. In words, for small $\lambda \Delta$, we can use the error probability under the private attack to approximate the error probability under the worst-case attack. 
To further simplify the calculation, we can approximate the honest chain growth using a Poisson process
%$$q_t(\lambda_h,\lambda_a,\Delta, \pi^*(0)) = q_t(\lambda_h',\lambda_a, 0, \pi^*(0)) + O(\bar \Delta^2),$$
with rate $\lambda_h' = \frac{\lambda_h}{1+\lambda_h \Delta}$ when $\lambda \Delta \ll 1$ as justified in Appendix \ref{app:latency}. %\ly{maybe also mention that the appendix provides justification of this approximation}
So we have the approximation 
\begin{align*}
    h^\Delta(t) &= 1 - q_t(\lambda_h,\lambda_a,\Delta,\pi^*(\lambda, \Delta))  \\
    &\approx 1 - q_t^0(\lambda_h',\lambda_a).
\end{align*}

With this approximation, we can have a confirmation rule similar to CR2 for positive $\Delta$ when there is only one public proposer block. 

\begin{defn}[CR3]
At time $\tau_\ell +\Delta + t$, let $d_i(t)$ be the depth of the voter block on the $i$-th voter chain that votes for a proposer block of level $\ell$, or $d_i(t)=0$ if no such a voter block exists yet. Let $t_\delta^*$ satisfy $h^\Delta(t_\delta^*) = \frac{1}{2} + \delta$ for $0 < \delta < \frac{1}{2}$ as in CR1. At time $\tau_\ell + \Delta + T$, if there is only one public proposer block on level $\ell$ and $\sum_{i=1}^{m} d_i(T) \geq (1+\delta)m\lambda t^*_\delta$, then we confirm this proposer block. Note that $\tau_\ell + \Delta + T$ is an arbitrary time chosen by an honest node to observe the blockchain.
\end{defn}

{\bf \noindent Full \newprism confirmation rule}. So far, we have considered the  normal path where there is only one public proposer block when confirmation happens.
In practice, there could be multiple proposer blocks at the same level either due to a natural fork or an adversarial action. In a very extreme case (with low probability), the adversary may balance votes perfectly between two public proposer blocks, in which case there is no chance to confirm a proposer block any faster than the longest chain protocol. However, this is highly unlikely since we can require honest nodes to vote for the proposer block that receives the most votes -- in this case, the votes converge fast and such a balancing attack is unlikely to succeed.

We now complete the confirmation rule for Prism in the most general case where there could be multiple proposer blocks at any level $\ell$.
Let $B_\ell(t)$ be the proposer block at level $\ell$ that receives the most votes at time $\tau_\ell + \Delta + t$, and $\bar V_\ell(t)$ be the number of votes received by proposer blocks at level $\ell$ other than $B_\ell(t)$.
By our definitions, at time $\tau_\ell + \Delta +t$, about $m \cdot h^\Delta(t)$ voter chains are stabilized forever. So at least $m \cdot h^\Delta(t) - \bar V_\ell(t)$ voter chains that vote for $B_\ell(t)$ are stabilized. Since other proposer blocks can receive at most $\bar V_\ell(t) + m \cdot (1-h^\Delta(t))$ votes in the future, we can confirm $B_\ell(t)$ if $m \cdot h^\Delta(t) - \bar V_\ell(t) >\bar V_\ell(t) + m \cdot (1-h^\Delta(t))$, i.e., $h^\Delta(t)>\frac{1}{m} \bar V_\ell(t) + \frac{1}{2}$.

In this confirmation rule, $\bar V_\ell$ can be observed by counting the votes from each voter chain, but the time $t+\Delta$ passed after the appearance time $\tau_\ell$ is not observable for offline users. %as the PoW blockchain may not implement a true timestamp for each block. 
%However,  the time can be accurately estimated here by measuring the chain growth of the voter chains, the accuracy enabled by the  large number of voter chains operating in parallel. 
We estimate  time as in CR2 by counting  the  depth  of  the  voter  blocks  that  vote  for a proposer block at level $\ell$.
This leads us to  the rule for full \newprism confirmation rule, defined  in Definition \ref{def:rule}.


\iffalse
\section{Confirmation rule}

We first define the following notations:
\begin{itemize}
    \item Let $\beta$ be the proportion of the adversary mining power. 
    \item Let $m$ be the number of voter chains and $\lambda$ be the mining rate of each voter chain.
    \item Let $\Delta$ be the upper bound of the network delay between any pair of honest nodes.
\end{itemize}

Let $\tau_\ell$ be the appearance time of the first proposer block at level $\ell$, i.e, a proposer block at level $\ell$ is mined or received by an honest node at $\tau_\ell$ for the first time. Then after $\tau_\ell + \Delta$, all honest nodes will start voting for a proposer block at level $\ell$. 

For a single voter chain, let $q_t(\lambda_h,\lambda_a,\Delta,\pi)$ be the success probability of a certain attack $\pi$ to reverse the voter block that votes for a proposer block at level $\ell$ after time $\tau_\ell+\Delta+t$ assuming that $\lambda_h = (1-\beta)\lambda$ is the honest mining rate, $\lambda_a = \beta \lambda$ is the adversary mining rate, and $\Delta$ is the upper bound of the network delay.
Let $\pi^*(\Delta)$ be the worst case attack in term of maximizing the success probability $q_t$.  Then we say that the effective vote for a proposer block at level $\ell$ from a voter chain at time $\tau_\ell+\Delta+t$ is 

\begin{equation*}
    h^\Delta(t) = 1 - q_t(\lambda_h,\lambda_a,\Delta,\pi^*(\lambda, \Delta)). 
\end{equation*}

Each voter chain follows Nakamoto's longest chain protocol and the worst case attack $\pi^*(0)$ when $\Delta = 0$ has been studied in the literature \cite{sompolinsky2016bitcoin,dembo2020everything}. \cite{dembo2020everything} showed that the private attack with pre-mining proposed in \cite{sompolinsky2016bitcoin} is the sample path based worst case attack in the sense of achieving both persistence and liveness violation.
Hence we have a close formed expression for $q_t^0(\lambda_h,\lambda_a)$:

\begin{eqnarray*}
    q_t^0(\lambda_h,\lambda_a) = 1 - \sum_{l = 0}^{\infty} \frac{\lambda_h - \lambda_a}{\lambda_h} \big( \frac{\lambda_a}{\lambda_h} \big)^l \cdot \\
    \Big( \sum_{k = l}^{\infty} e^{-\lambda_h t} \frac{(\lambda_h t)^k}{k!} \cdot \sum_{n=0}^{k-l} e^{-\lambda_a t} \frac{(\lambda_a t)^n}{n!} \big (1-(\frac{\lambda_a}{\lambda_h})^{k-n-l} \big) \Big).
\end{eqnarray*}

In the pre-mining phase of $\pi^*(0)$ (before time $\tau_\ell$), the adversary builds up a private chain with the maximum lead over the public chain, and the length of the maximum lead at time $\tau_\ell$ is stochastically dominated by a Geometric distribution with parameter $p = 1-\frac{\lambda_a}{\lambda_h}$. After time $\tau_\ell$, the adversary starts a private attack from the maximum lead. The number of adversary blocks and honest blocks mined in the time interval $(\tau_\ell, \tau_\ell+t)$ follow Poisson distributions with mean $\lambda_a t$ and $\lambda_h t$. If the lead plus the number of adversary blocks is no less than the number of honest blocks at time $\tau_\ell+t$, then the attack already succeeds; otherwise, from the simple random walk theory, the probability that the adversary will ever catch up from $z$ blocks behind is given by $(\frac{\lambda_a}{\lambda_h})^z$ when $\lambda_a < \lambda_h$. Therefore, we can write $q_t^0(\lambda_h,\lambda_a)$ as above. 

For positive $\Delta$, characterizing the worst case attack is challenging, but we are only interested in the regime where the block speed of each voter chain is very slow (i.e. $\lambda 
\Delta \ll 1$). We will show that $q_t(\lambda_h,\lambda_a,\Delta, \pi^*(\lambda)) =  q_t(\lambda_h,\lambda_a,\Delta, \pi^*(0)) + O(\lambda^2 \Delta^2)$, i.e., for small $\lambda \Delta$ we can use the error probability under the private attack to approximate the error probability under the worst attack. Further note that for $\lambda \Delta > 0$, the pure honest chain does not grow as a Poisson process. To further simplify the calculation, we show that 
$$q_t(\lambda_h,\lambda_a,\Delta, \pi^*(0)) = q_t(\lambda_h',\lambda_a, 0, \pi^*(0)) + O(\lambda^2 \Delta^2),$$
where $\lambda_h' = \frac{\lambda_h}{1+\lambda_h \Delta}$.
Hence we can approximate $h^{\Delta}(t)$ by

\begin{eqnarray*}
    h^\Delta(t) &=& 1 - q_t(\lambda_h,\lambda_a,\Delta,\pi^*(\Delta))  \\
    &\approx& 1 - q_t(\lambda_h',\lambda_a,0,\pi^*(0)).
\end{eqnarray*}

Let $B_\ell(t)$ be the proposer block at level $\ell$ that receives the most votes at time $\tau_\ell + \Delta + t$, $V_\ell(t)$ be the number of votes received by $B_\ell(t)$ at time $\tau_\ell + \Delta + t$, and $\bar V_\ell(t)$ be the number of votes received by other proposer blocks at level $\ell$ at time $\tau_\ell + \Delta + t$.
Note that at time $\tau_\ell + \Delta +t$, about $m \cdot h^\Delta(t)$ voter chains are stabilized forever. Then at least $m \cdot h^\Delta(t) - \bar V_\ell(t)$ voter chains that vote for $B_\ell(t)$ are stabilized. Since other proposer blocks can receive at most $\bar V_\ell(t) + m \cdot (1-h^\Delta(t))$ votes in the future, we can confirm $B_\ell(t)$ if $m \cdot h^\Delta(t) - \bar V_\ell(t) >\bar V_\ell(t) + m \cdot (1-h^\Delta(t))$, i.e., $h^\Delta(t)>\frac{1}{m} \bar V_\ell(t) + \frac{1}{2}$. Note that when there is only one single block, i.e., we always have $\bar V_\ell(t) = 0$ before confirmation, the confirmation rule simply becomes confirming the single proposer block at time $\tau_\ell + \Delta +t$ such that $h^\Delta(t) > \frac{1}{2}$.

Note that in the above confirmation rule, $\bar V_\ell$ can be observed by counting the votes from each voter chain, but the time $t+\Delta$ passed after the appearance time $\tau_\ell$ is not observable as the proof-of-work block chain may not implement a true timestamp for each block. 
However, the time can be accurately estimated here by measuring the chain growth of the voter chains as we have a large number of voter chains in parallel. Hence, mimicking Nakamoto's so-called ''$k$-deep`` confirmation rule for the longest chain protocol, we also use the depths of voter blocks as observable measurement and formally propose the following implementable confirmation rule for Prism.

\begin{defn}[\newprism Confirmation Rule]
Let $d_i(t)$ be the depth of the voter block which votes for a proposer block of level $\ell$ on the $i$-th voter chain at time $\tau_\ell +\Delta + t$. If the $i$-th voter chain does not vote for any proposer block of level $\ell$ at time $\tau_\ell +\Delta + t$, then $d_i(t) = 0$. We confirm $B_\ell(T)$ at time $\tau_\ell + \Delta + T$ if $h^\Delta(\frac{1}{(1+\delta)m\lambda}\sum_{i=1}^{m} d_i(T)) \geq \frac{1}{m} \bar V_\ell(T) + \frac{1}{2} +\delta$.
\end{defn}


\section{Intuition}


\begin{enumerate}
    \item Point out that we will give an intuition about how the confirmation rule works in the normal path (single proposer block and online user) when $\Delta = 0$.
    \item Take a time-based look at LC. Propose a time-based confirmation rule. Argue security for online users -- this will require you to use the worst-case attack property we proved in the earlier ``everything is a race..." paper. Highlight this result -- most people wouldn't know this before hand. This rule involves $h^0(t)$ and which is directly related to the error probability of the ``t-wait'' confirmation rule for LC. Discuss a bit about the properties of $h^0(t)$. Plot it for sample values of $\beta$. Now point out that  LC requires $h^0(t)$ to be close to 1, hence the latency of LC is $O(\frac{1}{\lambda} \cdot \log{\frac{1}{\epsilon}})$.
    \item Prism has $m$ parallel voter chains. how do we come up with time-based confirmation rule? Propose the main  rule and discuss normal path behavior. Argue why you require ``no adversaries" until confirmation and then assume private attack afterwards -- how this conservative setting helps you prove security. 
    \begin{itemize}
        \item Security: By LLN, the probability that a attacker gets more than half of the votes for its private block is exponentially small in $m$ as long as the probability that a vote that can be displaced from its longer chain is less than 1/2 in each voter chain (i.e., $h^0(t) >1/2$). formally introduce the time-based confirmation rule. at the end of the para, reader should have a belief in the security of this time-based confirmation rule.
        \item Latency: Since we can confirm when $h^0(t) >1/2$, this only requires small $t$ and also $t$ is independent with the error probability $\epsilon$, hence the latency of Prism is $O(\frac{1}{\lambda})$.
    \end{itemize}
    \item discussion on how to convert time-based rule to depth-based rule. Easy for LC but tricky for Prism. Discuss the complications and suggest 3 different ways to convert (these are the old, new, new-new rules). 
    \item Come up with a confirmation rule that is depth-based. Argue that this works but it is conservative. 
    \item Discuss latency in the normal path. empirically plot latency for different values of $\beta$. 
    \item Now bring in $\Delta > 0$. Use worst-case forked tree to convert to $\Delta = 0$ case. Point out that this was successfully done for security analysis of LC in an earlier paper. This para ends with a formal confirmation rule for normal path (i.e., one-proposer block at each depth). 
    \item Now allow more proposer blocks at each depth. This is the full confirmation rule.
\end{enumerate}

In this section, we provide high level idea to explain why the proposed Prism Confirmation Rule works and how it can achieve fast confirmation. For simplicity, we use the case $\Delta = 0$ for illustration. We first rewrite $h^0(t)$ here with parameters $\beta$ and $\lambda$.

\begin{eqnarray*}
    h^0(t) = \sum_{l = 0}^{\infty} \frac{1-2\beta}{1-\beta} \big( \frac{\beta}{1-\beta} \big)^l \cdot ~~~~~~~~~~~~~~\\
    \Big( \sum_{k = l}^{\infty} e^{-(1-\beta)\lambda t} \frac{((1-\beta) \lambda t)^k}{k!} \cdot ~~~~~~~~~~~\\
    \sum_{n=0}^{k-l} e^{-\beta \lambda t} \frac{(\beta \lambda t)^n}{n!} \big (1-(\frac{\beta}{1-\beta})^{k-n-l} \big) \Big).
\end{eqnarray*}

Note that $h^0(t)$ is the probability that a block is stabilized forever in the longest chain after time $t$ since the block is mined. It has been proved that Nakamoto's longest chain protocol achieves exponential security \cite{ren2019analysis,backbone}, i.e., 
$$h^0(t) \geq 1 - A \exp{(-a\lambda t)}$$
for large $t$, where positive constants $A$ and $a$ only depend on $\beta$. Hence in order to achieve very small error probability $\epsilon$ (we use $\epsilon = 10^{-9}$ in our implementation), the latency of the longest chain protocol $\tau_{LC}$ would satisfy $h^0(\tau_{LC}) \geq 1 - \epsilon$, i.e.,

\begin{equation*}
    \tau_{LC} = O(\frac{1}{\lambda} \cdot \log{\frac{1}{\epsilon}}).
\end{equation*}

However, in Prism, we can reduce the error probability $\epsilon$ by scaling $m$. Under the normal path when there is only one proposer block at a certain level $\ell$, we can simply confirm the single proposer block at time $t$ when $h^0(t) > 1/2$. Although each voter chain may be reversed in the future with non-negligible probability (around $1/2$), we can still guarantee that horizontally majority of the votes have been stabilized By Law of Large Numbers when $m$ is very large. Hence the latency of Prism $\tau_{Prism}$ under normal path would be

\begin{equation*}
    \tau_{Prism} = O(\frac{1}{\lambda}),
\end{equation*}
which is independent of the error probability $\epsilon$ when we choose $m$ to be large enough. For example, $\tau_{Prism} \approx 5/\lambda$ when $\beta = 0.3$ as shown in Fig. \ref{fig:h0_t}. Therefore, in Prism by decoupling voting and proposing, we are able to scale voting in a way that allows latency to not depend on the confirmation error probability, but solely on the mining rate.


However, under some abnormal paths, there could be multiple proposer blocks at the same level (this is caused by a natural fork or an adversary action). Note that in some extreme cases, the votes can be perfectly balanced between two public proposer blocks by the adversary, in which case there is no chance to fast confirm one proposer block and hence the latency is back to longest chain latency. However, if one of the proposer block receives much more votes than other proposer blocks, then it can still be fast confirmed by our rule. Further, under our honest voting strategy where honest nodes will vote for the proposer block that receives the most votes if there are more than one proposer block, the votes should converge fast and balancing attack is unlikely to happen.

\fi

\subsection{Main Result}
Here, we state the core security property of this new confirmation rule for \prism blockchain structure. 

\begin{theorem}[Security of \newprism Confirmation Rule]
\label{thm:main}
If $B_\ell(T)$ is confirmed at time $\tau_\ell + \Delta + T$ such that the rule in Definition \ref{def:rule} is satisfied, i.e., $h^\Delta(\frac{1}{(1+\delta)m\lambda}\sum_{i=1}^{m} d_i(T)) \geq \frac{1}{m} \bar V_\ell(T) + \frac{1}{2} +\delta$,
then the number of votes received by $B_\ell(T)$ will be greater than the number of votes received by any other proposer block at any time $t>\tau_\ell + \Delta + T$, except for probability $e^{-\Omega(\delta^2 m)}$. $\tau_\ell + \Delta + T$ is an arbitrary time chosen by an honest node to observe the blockchain.
\end{theorem}

The proofs have been delegated to Appendices \S\ref{sec:delta=0} and \S\ref{app:proof_sketch}  due to space limitations. %, we give a formal proof for Theorem \ref{thm:main} for the special case $\Delta = 0$ and provide a proof sketch on how to extend the result to general case when $\Delta$ is positive.

Our second main contribution is in identifying the worst attack to slow down the confirmation time, denoted as the ``slow-down attack" (defined formally in Appendix \S\ref{app:latency}). Such an identification along with the simplicity of the confirmation rule allow us to bound the worst case latency, as stated below.

\begin{theorem}[Latency of \newprism Confirmation Rule]
\label{thm:latency}
If $B_\ell$ is the only public proposer block at level $\ell$, then it will be confirmed with latency upper bounded by $O(\Delta)$, except for probability $e^{-\Omega(\delta^2 m)}$.
\end{theorem}

The proof is deferred to Appendix \ref{app:latency}. The constants involved in Theorem~\ref{thm:latency} are all small and can be explicitly evaluated. A sample evaluation is illustrated in  Fig.~\ref{fig:latency} which plots the confirmation latency for different $\beta$  under three scenarios: no attack, private mining attack, and the worst case (slow-down) attack; here $\lambda \Delta = 0.1$ and $\delta = 0$. 

\begin{figure}
    \centering
    \includegraphics[width=0.35\textwidth]{figures/latency.png}
    \caption{Latency under three attacks for different $\beta$. The latency is normalized over the upper bound on network latency  $\Delta$.}
    \label{fig:latency}
\end{figure}





==> Prism Systems Paper (CCS)/overview.tex <==
\section{Overview of \prism}
\label{sec:overview}
In this section we  discuss the key ideas behind the design of \prism. We  start with Nakamoto's longest chain protocol, explore the limitations in scaling its throughput and latency, and present \prism as a natural design to remove these limitations. 
%%We will explain the design of \prism incrementally, first addressing throughput and then latency.



\subsection{Longest chain protocol}

The most basic blockchain consensus protocol is Nakamoto's longest chain protocol, used in many blockchain projects including \bitcoin and \ethereum.  The basic object is a {\em block}, consisting of transactions and links to other blocks. Starting with the {\em genesis} block as the root, each new block mined by a miner is added to create an evolving {\em block tree}. In the longest chain protocol, each block is appended to the leaf block of the longest chain in the current block tree, and the transactions in that block are added to the transaction ledger maintained by the blocks in the longest chain. 
 A miner earns the right to append a block after solving a cryptographic puzzle based on the hash of the leaf block \ma{and the contents of the block being mined?}. The cryptographic puzzle is solved by random attempts at finding a solution to a hash inequality. The miner includes the solution in the block as a {\em proof of work}, which other nodes can verify.  The time to solve the puzzle is random and exponentially distributed with a mining rate $f$ that can be tuned by adjusting the difficulty of the puzzle. How fast an individual miner can solve the puzzle and mine the block is proportional to its hashing power, i.e. how fast it can compute hashes. 
 A block is confirmed to be in the ledger when it is $k$-deep in the ledger, i.e. the block is on the longest chain and a chain of $k-1$ blocks have been appended to it. It is proven that as long as the adversary has less than $50\%$ hashing power, the ledger has consistency and liveness properties \cite{backbone}: blocks that are deep enough in the longest chain will not be reverted, and honest miners will be able to enter a non-zero fraction of blocks into the ledger. 

\subsubsection{Latency limitation}

A critical attack on the longest chain protocol is the {\em private  double-spend} attack \cite{bitcoin}, as shown in Figure \ref{fig:double-spend}(a). Here, an adversary is trying to de-confirm a block after it is confirmed, by mining a chain in private and broadcasting it when it is longer than the public chain. If the hashing power of the adversary is greater than that of aggregate of the honest nodes, this attack can be easily executed no matter what $k$ is, since the adversary can mine blocks faster on the average than the honest nodes and will eventually  overtake the public chain. Hence, the system is not secure when the adversary controls more than half of the computing power of the network. On the other hand, when the adversary has less than half the computing power, the probability of success of this attack can be made arbitrarily small by choosing the confirmation depth $k$ to be large \cite{bitcoin}. When $k$ is small, there is still a decent chance that the adversary can mine a longer chain even though it has less power, by getting lucky and solving a few puzzles faster than the average. The probability of this event becomes exponentially smaller as $k$ grows, as the adversary has to get lucky on solving many puzzles. 


The price to pay for choosing $k$ large is increased latency in confirmation. For example, to achieve a probability of deconfirmation of $0.001$, a depth of $24$ blocks is needed if the adversary has fraction $\beta =0.3$ of the total hashing power \cite{bitcoin}. With a block mining rate of $1$ block per $10$ seconds, this translates into a latency of $240$ seconds. To achieve a deconfirmation probability of $10^{-6}$, a depth of $50$ blocks is required, translating into a latency of $500$ seconds. Figure ~\ref{fig:rd} shows Bitcoin's tradeoff between latency and reliability. \ma{I've been assuming this figure also shows the reliability-depth tradeoff for Prism?}

\begin{figure}
\begin{center}
\includegraphics[width=0.4\textwidth]{fast_confirmation_comparision.pdf}
\end{center}
\caption{ Depth of confirmation: longest chain vs \prism. (a) The longest chain protocol requires a block to be many blocks deep for reliable confirmation, so that an adversary mining in private cannot create a longer chain. (b) \prism allows each voter block to be very shallow but relies on many voter chains to increase the reliability. \ma{It's a little odd that the prism figure doesn't show a block tree for the proposer blocks. Can we have a chain, with a level corresponding to each level of the voter trees?}}
\label{fig:double_spend}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=0.4\textwidth]{reliability-depth.jpg}
\end{center}
\caption{\label{fig:rd} Reliability-depth }
\end{figure}


\subsubsection{Throughput limitation}

If $B$ is the block size in number of transactions, then the throughput of \bitcoin \ma{I think we should use `longest chain' protocol instead of `Bitcoin'. In this section, we're talking about the protocol, whereas Bitcoin is a specific system.} is $fB$ transactions per second (tps). 
\red{GF: Should we point out that it's less if there is forking? Or say at most $fB$ tps?} \ma{I like at most $fB$.}
However, the mining rate $f$ and the block size $B$ are constrained by the security requirement. Increasing the mining rate increases the amount of {\em forking} of the blockchain due to multiple blocks being mined on the same leaf block by multiple miners within the network delay $\Delta$. \ma{suggestion: Forking reduces throughput since it reduces the growth rate of the longest chain, and hence, the ledger. More importantly, forking hurts the security of the protocol because the adversary requires less compute power to overtake the longest chain.} This reduces the security of the protocol because the growth rate of the longest chain is reduced by forking while the adversary's compute power can be co-located and hence its attack chain does not experience forking. In fact, the adversarial power that can be tolerated by the longest chain protocol goes from $50\%$ to $0\%$ as the mining rate $f$ increases (Figure \ref{fig:forking}). Increasing the block size $B$ increases the amount of forking as well since the network delay $\Delta$ increases with the block size \cite{decker}.

A back-of-the-envelope calculation of the impact of the forking can be done based on a simple model of the network delay: 
$$ \Delta = \frac{hB}{C},$$
where $h$ is the average number of hops for a block to travel and $C$ transactions per second is the communication bandwidth per link. This model is consistent with the linear relation between the network delay and the block size as measured empirically by \cite{decker}. Hence, the utilization, i.e. the throughput as a fraction of the communication bandwidth, is given by 
$$ \frac{fB}{C} = \frac{f\Delta}{h}.$$
$f\Delta$ is the average number of blocks ``in flight'' per network delay time, and this has to be kept much smaller than $1$ to avoid excessive forking. 
Hence, the security requirement (as well as the number of hops) limits the utilization. \ma{Can we discuss the impact of mining rate on security here instead of the paragraph above? One idea is to state how security depends on $f\Delta$ here, and replace Figure 3 or get rid of the figure. The next sentence gives the specific point $\beta=0.45$ as an example. The nice thing about this is that it highlights that in the longest chain protocol, to meet the security requirement, one cannot have too many blocks in flight at the same time. Prism doesn't have this limitation.} For example, to achieve security against an adversary with $\beta = 0.45$ of the total hashing power, one needs $f\Delta = 0.1$. With $h = 5$, this translates to a utilization of $2\%$.
\red{GF: Maybe explain in words why we can hope to fix this problem? The dependency on  graph diameter is fundamental, since all honest nodes have to come to consensus, but the effect of Bitcoin's security requirement could  be circumvented by designing a system that trades latency for communication in its confirmation rule.}

\begin{figure}
\begin{center}
\includegraphics[width=0.3\textwidth]{forking.png}
\end{center}
\caption{ Increasing mining rate or block size increases forking and reduces security. 
\red{GF: Are we going to add numbers to the x-axis? This looks a bit cartoonish, I think having actual nubmers on the axes would help,  if we want to keep this figure at all (not sure it clarifies too much?).} \ly{Shall I redo the plot to put numbers on x-axis and make it the same style as figure 8 to 12?}
}
\label{fig:forking}
\end{figure}







%%To understand the impact 


%%Problem: For single-longest-chain increase the throughput, we need to increase the mining %%rate or the block size. Theory proves that only so far you can get. 

%%Solution: Have transaction blocks that are not a chain, so we can have high mining rate. %%Proposer chain have low mining rate. Proposer chain has low mining rate and form a chain, %%and refer to those transaction blocks. Latency is still not solved, because we still base confidence on depth.

\subsection{\prism: Factorizing the blockchain}

\ma{I think we need to refer to the Prism theory paper in this section. We are giving the intuition behind the protocol here, but it's important to state that the security properties have been formally proved.}

The selection of a main chain in a blockchain protocol can be viewed as electing a leader block among all the blocks at each level of the block tree. \ma{The level for a block is defined as its distance to the genesis block.} 
In this light, the blocks in the longest chain protocol can be viewed as serving three distinct roles: (1) they stand for election to be leaders;  (2) they add transactions to the main chain; and (3) they vote for ancestor blocks through parent link relationships. Our principal observation is that the latency and throughput limitations of the longest chain protocol are due to the {\em coupling} of the roles carried by the blocks. \prism removes these limitations by factorizing the blocks into three types of blocks: proposer blocks, transaction blocks and voter blocks. (Figure \ref{fig:prism}). Each block mined by a miner is randomly picked (sortitioned) to be of one of the types based on the value of the hash computed for its proof of work, 
% \red{GF: I don't think proof of work was defined earlier--either define it in 2.1, or clarify meaning here} \ma{I added something to Sec. 2 please check}
and if it is a voter block, will be further chosen randomly to be in one of several {\em voter trees} \red{GF: Haven't mentioned or defined voter trees yet...} (More details on this process in Section \ref{sec:key_design}.)
The voter blocks vote for transactions indirectly by voting for proposer blocks, which in turn link to transaction blocks. Proposer blocks are grouped according to their level in the original block tree \ma{not clear what this means. what is the `original block tree'? does a proposer block have a link to a parent proposer block (this is not shown in the figure)}, and each voter tree votes for exactly one proposer block at each level to select a leader block among them. The leader block is the proposer block which has the highest number of votes among all the proposer blocks at the same level (ties broken by hash of the proposer blocks.) The elected leader blocks can then bring in the transactions to form the final ledger. \ma{Can we explain this more precisely, e.g., To obtain the final ledger, one traverses the elected leader blocks level by level, including the transactions that they link to in order.}
The vote from a voter tree is represented by the reference link from a voter block in the longest chains of the voter tree; the longest chains in all the $m$ voter trees maintain the security of the whole system, as explained next.


\begin{figure}
\begin{center}
\includegraphics[width=0.45\textwidth]{Prism_main.pdf}
\end{center}
\caption{\prism: Factorizing the blocks into three types of blocks: proposer blocks, transaction blocks and voter blocks. \ma{can we increase the font size a bit?} }
\label{fig:prism}
\end{figure}

%%Thus, the parent links in the original block tree have two implicit functionalities which are explicitly separated in this representation: 1) they provide a partial ordering of the proposal blocks according to their levels, and 2) they allow blocks to vote for each other. 
% they help the voting blocks to vote for each other.
%%\blue{It's unclear here what is meant by having a block ``support" another block.}

\subsubsection{Security and Latency}

The ledger is maintained by the leader proposal blocks \ma{proposal block, or proposer block. we used proposer block to this point} at all the levels. Each leader proposal block is secured by the votes from the voter trees. Each vote is in turn secured by the longest chain protocol in its voter tree. If the adversary has less than $50\%$ hash power, and the mining rate in each of the voter trees and the proposer tree is kept small to minimize forking, then the consistency and liveness of each of the voter trees guarantee the consistency and liveness of the ledger maintained by the leader proposer blocks. However, this requires long latency to wait for each voter block to get sufficiently deep in its chain. What is interesting is that when there are many voter trees, the same guarantee can be achieved without requiring each and every vote to be secured, thus drastically improving over the latency of the longest chain protocol. 

The private double-spend attack on the longest chain protocol has a natural analog in \prism. Figure \ref{fig:double_spend}(b) shows the scenario. A honest proposer block $H$ at a particular level has collected votes from the voter chains. Over time, each of these votes will become deeper in its voter chain. An attack by the adversary is to mine a private proposal block $A$ at the same level, and on each of the voter trees fork off and mine a private alternate chain and send its vote to block $A$. After leader block $H$ is confirmed, the adversary continues to mine on each of the voter alternate chains to attempt to overtake the public longest chain and shift the vote from $H$ to $A$. If the adversary can thereby get more votes on $A$ than on $H$, then its attack is successful. The question is how deep do we have to wait for each vote to be in its voter chain in order to confirm the proposer block $H$?

Nakamoto's calculations will help us answer this question. As an example, at tolerable adversary power $\beta = 0.3$, the reversal probability \ma{in section 2, we used deconfirmation probability instead of reversal probability. i actually like reversal better, and its probably better to use the same term} in a single chain is $0.45$ when a block is $2$-deep \cite{bitcoin}. With $1000$ voter chains and each vote being $2$-deep, the expected number of chains that can be reversed by the adversary is $450$. The probability that the adversary got lucky and can reverse more than half the votes, i.e. $500$, is about  $0.001$. Hence to achieve $\epsilon = 0.001$, we only need to wait for the votes to be  $2$-deep, as opposed to the $24$ block depth needed in the longest chain protocol.  This reduction in latency is conceptually similar to averaging many unreliable  classifiers to form a strong aggregate classifier:  the more voter chains there are, the less certainty of permanence each individual vote requires, thereby reducing confirmation time.  This gain comes without sacrificing security: each voter chain is operating slowly enough to tolerate $\beta$ adversarial hash power. \ma{I like this section a lot. I think it's at just the right level.} Furthermore, increasing the number of voter chains can further improve the confirmation reliability without sacrificing latency; for example, doubling the number of voter chains from $1000$ to $2000$ can reduce the deconfirmation probability from $0.001$ to $10^{-6}$. Figure \ref{fig:rd} compares the latency-reliability tradeoffs of \prism and the longest chain protocol. 

\subsubsection{Throughput}

To keep \prism secure, the mining rate and the size of the voter blocks have to be chosen such that each voter chain has little forking. The mining rate and the size of the proposer blocks have to be also chosen such that there is very little forking in the proposer tree. Otherwise, the adversary can propose a block at each level, breaking the liveness of the system. Hence, the throughput of \prism would be as low as the longest chain protocol if transactions were carried by the proposer blocks directly. To decouple security from throughput, transactions are instead carried by separate transaction blocks. The transaction blocks enter into a pool after they are mined. Each proposer block when it is mined refers to the transaction blocks in the pool that have not been referred to by previous proposer blocks. When a proposer block is confirmed to be the leader of its level, the transactions in all the transaction blocks it refers to enter into the ledger. The throughput of the system can be increased by increasing the mining rate of the transaction blocks, without affecting the security of the system. This throughput is only limited by the computing or communication bandwidth limit $C$ of each node, thus potentially achieving $100\%$ utilization. In contrast, the throughput of the longest chain protocol is {\em security-limited} and has very low network  utilization. \ma{If we include the figure I mentioned at the end of 2.1, which shows the relationship between $f\Delta$ and security, then we can recall that in the section and explain that transaction blocks overcome this problem}


%%Show that Prism is the optimal (theory). See Fig.~\ref{fig:protocols-comparison}. Optimal in terms of communication limit. But the implementation is limited by state execution. Compare to Hotstuff. 










\begin{figure}
\begin{center}
\includegraphics[width=0.4\textwidth]{chains-table.jpg}
\end{center}
\caption{\label{fig:protocols-comparison} Table: Comparison }
\end{figure}


==> Prism Systems Paper (CCS)/overview2.tex <==

\section{ \prism Overview}
\label{sec:overview}

%\ma{I think we need to refer to the Prism theory paper in this section. We are giving the intuition behind the protocol here, but it's important to state that the security properties have been formally proved.}

The selection of a main chain in a blockchain protocol can be viewed as electing a leader block among all the blocks at each level of the blocktree. In this light, the blocks in the longest chain protocol can be viewed as serving three distinct roles: they stand for election to be leaders;  they add transactions to the main chain; they vote for ancestor blocks through parent link relationships. The latency and throughput limitations of the longest chain protocol are due to the {\em coupling} of the roles carried by the blocks. \prism removes these limitations by factorizing the blocks into three types of blocks: proposer blocks, transaction blocks and voter blocks. (Figure \ref{fig:prism}). Each block mined by a miner is randomly sortitioned into one of the three types of blocks, and if it is a voter block, it will be further  sortitioned into one of the voter trees. (Mining is described in detail in \S\ref{sec:mining}).

The proposer blocktree anchors the \prism blockchain. 
Each proposer block contains a list of reference links to transaction blocks, which contains transactions, as well as a single reference to a parent proposer block.
Honest nodes mine proposer blocks on the longest chain in the proposer tree, but the longest chain does not determine the final confirmed sequence of proposer blocks, known as the  \emph{leader sequence}. 
We define the \emph{level} of a proposer block as its distance from the genesis proposer block, and the \emph{height} of the proposer tree as the maximum level that contains any proposer blocks. 
The leader sequence of proposer blocks contains one block at every level up to the height of the proposer tree, and is  determined by the \emph{voter chains}. 

%\gw{Voter tree (blocktree) or voter chain (blockchain)? Since unlike proposer tree, only voter longest chain will participate in voting.}

There are $m$ voter chains, where $m \gg 1$ is a fixed parameter chosen by the system designer. For example, we choose $m=1000$ in our experiments.  The $i$th voter chain is comprised of voter blocks that are mined on the longest chain of the $i$th voter trees. A voter block votes for a proposer block by containing a reference link to that proposer block, with the requirements that: 1) a vote is valid only if the voter block is in the longest chain of its voter tree; 2) each voter chain votes for one and only one proposer block at each level. The leader block at each level is the one which has the highest number of votes among all the proposer blocks at the same level (tie broken by hash of the proposer blocks.) The elected leader blocks then provide a unique ordering of the transaction blocks to form the final ledger. (Ledger formation is explained in detail in \S\ref{sec:confirmation}.)





%%The security of the system rests on the security of the $m$ voter chains, which is guaranteed by longest chain protocol. However, as we discuss next, by relying on many parallel voter chains, \prism significantly reduces the latency required to achieve a desired reversal probability compared to the vanilla longest chain protocol.


\if 0
The voter blocks vote for transactions indirectly by voting for proposer blocks, which in turn link to transaction blocks. Proposer blocks are grouped according to their level in the original block tree \ma{not clear what this means. what is the `original block tree'? does a proposer block have a link to a parent proposer block (this is not shown in the figure)}, and each voter tree votes for exactly one proposer block at each level to select a leader block among them. The leader block is the proposer block which has the highest number of votes among all the proposer blocks at the same level (ties broken by hash of the proposer blocks.) The elected leader blocks can then bring in the transactions to form the final ledger. \ma{Can we explain this more precisely, e.g., To obtain the final ledger, one traverses the elected leader blocks level by level, including the transactions that they link to in order.} The vote from a voter tree is represented by the reference link from a voter block in the longest chains of the voter tree; the longest chains in all the $m$ voter trees maintain the security of the whole system, as explained next.

\fi

%\begin{figure}
%    \centering
%    \input{figures/prism-chains.tex}
%    \caption{\prism: Factorizing the blocks into three types of blocks: proposer blocks, transaction blocks and voter blocks. \ma{can we increase the font size a bit?} }
%    \label{fig:prism}
%\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=0.45\textwidth]{figures/Prism_main.pdf}
\end{center}
\vspace{-2mm}
\caption{\small \prism: Factorizing the blocks into three types of blocks: proposer blocks, transaction blocks and voter blocks.}
\label{fig:prism}
\vspace{-5mm}
\end{figure}

%%Thus, the parent links in the original block tree have two implicit functionalities which are explicitly separated in this representation: 1) they provide a partial ordering of the proposal blocks according to their levels, and 2) they allow blocks to vote for each other. 
% they help the voting blocks to vote for each other.
%%\blue{It's unclear here what is meant by having a block ``support" another block.}

\if 0

\subsection{Security Model}
\vb{Let $\mathcal{N}$ denote  the nodes in the system and with of loss of generality, we assume each node has equal mining power. Let $\mathcal{H} \subseteq \mathcal{N}$ denote the set of honest nodes and $\mathcal{N} \setminus \mathcal{H}$ is set the adversarial nodes. The fraction of adversarial nodes, $\beta = 1 - \frac{|\mathcal{H}|}{|\mathcal{N}|}$, is assumed to be less then $0.5$. 
%We assume a network model where the delay for a block of size $B$ is equal to $\Delta = \frac{B}{C}+D$, where $B/C$ is the processing delay and $D$ is the propagation delay.
%We model the protocol as running in rounds where each round is of duration equal to the delay ($\Delta$) corresponding to the largest sized block in the \prism protocol. 
The adversarial nodes do not have to follow the \prism protocol - they can mine new blocks with any content and anywhere on the blockchain, and  unlike honest users, they can keep their mined block in private and release it anytime in future. 
%c) their action in a given round is a function of the action of the honest nodes up to and including that round.
However, the adversary cannot perform certain actions such as modifying the block content of blocks mined by honest nodes or withholding blocks mined by an honest node from reaching other honest nodes.
}

\fi

\subsection{Security and Latency}
\label{sec:prism-latency}

%The ledger is maintained by the leader proposer blocks at all the levels. 

The votes from the voter trees secure each leader proposer block, because changing an elected leader requires reversing enough votes to give them to a different proposer block in that level. 
Each vote is in turn secured by the longest chain protocol in its voter tree. If the adversary has less than $50\%$ hash power, and the mining rate in each of the voter trees is kept small to minimize forking,  then the consistency and liveness of each voter tree guarantee the consistency and liveness of the ledger maintained by the leader proposer blocks. 
However, this would appear to require a long latency to wait for each voter block to get sufficiently deep in its chain. What is interesting is that when there are many voter chains, the same guarantee can be achieved without requiring each and every vote to have a very low reversal probability, thus drastically improving over the latency of the longest chain protocol. 


To get some intuition, consider the natural analog of the private double-spend attack on the longest chain protocol in \prism. Figure \ref{fig:double_spend}(b) shows the scenario. An honest proposer block $Ho$ at a particular level has collected votes from the voter chains. Over time, each of these votes will become deeper in its voter chain. An attack by the adversary is to mine a private proposer block $A$ at the same level, and on each of the voter trees, fork off and mine a private alternate chain and send its vote to block $A$. After leader block $Ho$ is confirmed, the adversary continues to mine on each of the alternate voter chains to attempt to overtake the public longest chain and shift the vote from $Ho$ to $A$. If the adversary can thereby get more votes on $A$ than on $Ho$, then its attack is successful. The question is how deep do we have to wait for each vote to be in its voter chain in order to confirm the proposer block $Ho$?

Nakamoto's calculations will help us answer this question. As an example, at tolerable adversary power $\beta = 30\%$, the reversal probability in a single chain is $0.45$ when a block is $2$-deep \cite{bitcoin}. With $m=1000$ voter chains and each vote being $2$-deep, the expected number of chains that can be reversed by the adversary is $450$. The probability that the adversary can get lucky and reverse more than half the votes, i.e. $500$, is about  $0.001$. Hence to achieve a reversal probability, $\epsilon = 0.001$, we only need to wait for the votes to be  $2$-deep, as opposed to the $24$ block depth needed in the longest chain protocol (\S\ref{s:lc-latency}). This reduction in latency comes without sacrificing security: each voter chain can operate at a slow enough mining rate to tolerate $\beta$ adversarial hash power. Furthermore, increasing the number of voter chains can further improve the confirmation reliability without sacrificing latency; for example, doubling the number of voter chains from $1000$ to $2000$ can reduce the reversal probability from $0.001$ to $10^{-6}$.

We have discussed one specific attack, focusing on the case when there is a single public proposer block on a given level. Another possible attack is when there are two or more such proposer blocks and the adversary tries to balance the votes between them to delay confirmation. It turns out that the attack space is quite huge and these are formally analyzed in \cite{prism-theory} to obtain the following guarantee on the confirmation latency, regardless of the attack:

 \begin{theorem}[Latency, Thm. 4.8 \cite{prism-theory}] \label{cor:latency_fast}
For an adversary with $\beta< 50\%$ of hash power, network propagation delay $D$, \prism with $m$ chains confirms  \textit{honest}\footnote{Honest transactions are ones which have no conflicting double-spent transactions broadcast in public.} transactions at reversal probability $\epsilon$ guarantee with latency upper bounded by
\begin{equation}
\label{eq:latency}
 Dc_1(\beta) +  \frac{Dc_2(\beta)}{m} \log \frac{1}{\epsilon}\;\; \text{ seconds},
\end{equation}
where $c_1(\beta)$ and $c_2(\beta) $ are $\beta$ dependent constants.
\end{theorem}

For large number of voter chains $m$, the first term dominates the above equation and therefore Prism achieves near optimal latency, i.e. proportional to the propagation delay $D$ and independent of the reversal probability. Figure \ref{fig:rd} compares the latency-reliability tradeoffs of \prism and the longest chain protocol. Note that (\ref{eq:latency}) is a worst-case latency bound that holds for {\em all} attacks. In Section \ref{sec:balancing}, we will evaluate the latency of our system under the balancing attack. 


\subsection{Throughput}
\label{sec:thruput}

To keep \prism secure, the mining rate and the size of the voter blocks have to be chosen such that each voter chain has little forking. The mining rate and the size of the proposer blocks have to be also chosen such that there is very little forking in the proposer tree. Otherwise, the adversary can propose a block at each level, breaking the liveness of the system. Hence, the throughput of \prism would be as low as the longest chain protocol if transactions were carried by the proposer blocks directly. 


To decouple security from throughput, transactions are instead carried by separate transaction blocks. Each proposer block when it is mined refers to the transaction blocks that have not been referred to by previous proposer blocks. This design allows throughput to be increased by increasing the mining rate of the transaction blocks, without affecting the security of the system. The throughput is only limited by the computing or communication bandwidth limit $C$ of each node, thus potentially achieving $100\%$ utilization. In contrast, as we discussed in \S\ref{s:lc-thput}, the throughput of the longest chain protocol is security-limited, resulting in low network utilization. \cite{prism-theory} formally proves that \prism achieves near optimal throughput:

\begin{theorem}[Throughput, Thm. 4.4\cite{prism-theory} ]
\label{thm:throughput} For an adversary with $\beta < 50\%$ fraction of hash power and network capacity C, Prism can achieve  $(1-\beta)C$ throughput and maintain liveness in the ledger.
\end{theorem}

%Note that the reference links from a proposer block to its transaction blocks are sealed in the proof-of-work of the proposer block. Hence, once a proposer block is mined, there is no way for an attacker to change the reference links to the transaction blocks. In contrast, the transactions that a miner in \bitcoin-NG adds onto the ledger after its block enters the main chain are {\em not} sealed by the proof-of-work. Hence, \bitcoin-NG is susceptible to censorship attacks.

\smallskip
\noindent{\bf Remark on security model:} The Prism theory paper~\cite{prism-theory} analyzed the protocol in a synchronous round-based network model under standard assumptions about the adversary. In particular, the delay for a block of size $B$ was assumed to be equal to $\Delta = \frac{B}{C}+D$, where $B/C$ is the processing delay and $D$ is the propagation delay, and the protocol was assumed to run in rounds where each round is of duration equal to the delay ($\Delta$) corresponding to the largest sized block. The adversarial nodes do not have to follow protocol - they can mine new blocks with any content and anywhere on the blockchain, and  unlike honest users, they can keep their mined blocks in private and release them at anytime in the future. However, the adversary cannot modify the content of blocks mined by honest nodes or withhold blocks mined by an honest node from reaching other honest nodes. Refer to \S2 of~\cite{prism-theory} for the full specification of the model. This model does not capture the impact of artifacts like queuing delay or asynchronous communication on performance. Nevertheless our implementation shows that the overall performance characteristics predicted by the theory hold in a practical setting. 


% To decouple security from throughput, transactions are instead carried by separate transaction blocks. The transaction blocks enter into a pool after they are mined. Each proposer block when it is mined refers to the transaction blocks in the pool that have not been referred to by previous proposer blocks. When a proposer block is confirmed to be the leader of its level, the transactions in all the transaction blocks it refers to enter into the ledger. \ma{The last three sentences could be cut from here and discussed in the design section} The throughput of the system can be increased by increasing the mining rate of the transaction blocks, without affecting the security of the system. This throughput is only limited by the computing or communication bandwidth limit $C$ of each node, thus potentially achieving $100\%$ utilization. In contrast, as we discussed in \S\ref{s:lc-thput}, the throughput of the longest chain protocol is security-limited, resulting in low network utilization. 





%\ma{If we include the figure I mentioned at the end of 2.1, which shows the relationship between $f\Delta$ and security, then we can recall that in the section and explain that transaction blocks overcome this problem}


%%Show that Prism is the optimal (theory). See Fig.~\ref{fig:protocols-comparison}. Optimal in terms of communication limit. But the implementation is limited by state execution. Compare to Hotstuff. 



% \subsection{Formal guarantees}
% The results established about the \prism protocol in a recent theoretical paper~\cite{prism-theory} provide the following throughput and latency guarantees. \ly{update the bib file to reflect that the paper has been published. also consider anonymous issues}




% The above two results show that of Prism achieves near optimal throughput and latency.

% \ma{@Vivek: please summarize the main results from the theory paper here.}
% \vb{done.}



\if 0

\begin{figure}
\begin{center}
\includegraphics[width=0.4\textwidth]{chains-table.jpg}
\end{center}
\caption{\label{fig:protocols-comparison} Table: Comparison }
\end{figure}

\fi


==> Prism Systems Paper (CCS)/proofs.tex <==
\section{Proofs}
\label{app:proof}

\subsection{Proof of Theorem \ref{thm:main} for $\Delta = 0$}
\label{sec:delta=0}
In this section, we prove the security of \newprism Confirmation Rule when $\Delta = 0$.
As a warm-up, we first prove the security of a time-based confirmation for online users in the following lemma.

\begin{lemma}
\label{lem:lem:main_0}
Assume $\Delta = 0$. If an online node is aware of $\tau_\ell$ and confirms $B_\ell(T)$ at time $\tau_\ell + T$ such that $h^0(T) \geq \frac{1}{m} \bar V_\ell(T) + \frac{1}{2} +\delta$, then number of votes received by $B_\ell(T)$ will be greater than number of votes received by any other proposer block at time $t$ for all $t>\tau_\ell + T$, except for probability $e^{-2\delta^2 m}$. Note that $\tau_\ell + T$ is a random time chosen by an honest node to observe the blockchains.
\end{lemma}

\begin{proof}
For $1 \leq i \leq m$, let $H_i(t_1,t_2)$ and $Z_i(t_1,t_2)$ be the number of honest blocks and adversary blocks mined at the $i$-th voter chain in the time interval $(t_1, t_2]$, respectively. Then $H_i(t_1,t_2)$ and $Z_i(t_1,t_2)$ follow Poisson distributions $\texttt{Poi}((1-\beta)\lambda(t_2-t_1))$ and $\texttt{Poi}(\beta\lambda(t_2-t_1))$ respectively.
Let $L_i$ be the maximum lead built by the adversary over the public longest chain on the $i$-th voter chain at time $\tau_\ell$. It have been shown in \cite{sompolinsky2016bitcoin} (Lemma 3) that $L_i$ is first order stochastically dominated by a Geometric random variable $Y \sim \texttt{Geo}(p)$ with $p = \frac{1-2\beta}{1-\beta}$ (i.e., $P(L_i \geq l) \leq P(Y \geq l) = \big( \frac{\beta}{1-\beta} \big)^l$ for $l \in \mathbb{N}$).

Let $U_i(t) = 1$ if the $i$-th voter chain votes for $B_\ell(T)$ at time $\tau_\ell + t$; and 0 otherwise. Then we have $V_\ell(t) = \sum_{i=1}^{m} U_i(t)$.

We prove the theorem by contradiction. Suppose at time $t_1 > \tau_\ell + T$, $V_\ell(t_1)$ is smaller than number of votes received by another proposer block, which implies that $V_\ell(t_1) \leq m/2$.

For $1 \leq i \leq m$, let event $E_i$ be the event that there exists $t_2 \in [\tau_\ell + T, \tau_\ell + t_1]$ such that $L_i + Z_i(\tau_\ell,t_2) \geq H_i(\tau_\ell, t_2)$ on the $i$-th voter chain; let event $F_i$ be the event that there exists $t_2 \in [\tau_\ell + T, +\infty)$ such that $L_i + Z_i(\tau_\ell,t_2) \geq H_i(\tau_\ell, t_2)$ on the $i$-th voter chain. Let event $W_i$ be the event that $i$-th voter chain votes for 
a proposer block at level $\ell$ other than $B_\ell(T)$ at time $T$. Note that $E_i \subset F_i$, and also we have the following important {\bf claim 1}:
\begin{equation*}
   \{U_i(t_1) = 0\} \subseteq E_i \cup W_i, 
\end{equation*}
thus
\begin{equation*}
    U_i(t_1) \geq 1 - \indicator_{E_i\cup W_i} \geq 1 - \indicator_{F_i\cup W_i} \geq 1 - \indicator_{F_i} - \indicator_{W_i}.
\end{equation*}

Sum them up over $1 \leq i \leq m$, we have
\begin{equation*}
    V_\ell(t_1) = \sum_{i=1}^{m} U_i(t) \geq m - \sum_{i=1}^m \indicator_{F_i} - \bar V_\ell(T),
\end{equation*}
then we have
\begin{eqnarray*}
    \sum_{i=1}^m \indicator_{F_i} &\geq& m - \bar V_\ell(T) - V_\ell(t_1) \\
    &\geq& m - \bar V_\ell(T) - m/2 \\
    &=& m/2 - \bar V_\ell(T) \\
    &\geq& m \big (1-h^0(T)\big ) + m\delta.
\end{eqnarray*}

Here we first check the expectation,
\begin{equation*}
    E[\sum_{i=1}^m \indicator_{F_i}] = \sum_{i=1}^m P(F_i) = m P(F_1) = m(1-h^0(T)),
\end{equation*}
by the definition of event $F_i$ and $h^0(t)$. Then we have
\begin{eqnarray}
    \label{eqn:hoeffding_prob}
    &&P(V_\ell(t_1) \leq m/2) \nonumber \\
    &\leq& P(\sum_{i=1}^m \indicator_{F_i} \geq  m(1-h^0(T)) + m\delta)  \nonumber\\
    &=& P(\sum_{i=1}^m \indicator_{F_i} - E[\sum_{i=1}^m \indicator_{F_i}] \geq m\delta)  \nonumber \\
    &\leq& e^{-2\delta^2 m},
\end{eqnarray}
where the last inequality is due to Hoeffding's inequality. (\ref{eqn:hoeffding_prob}) concludes the lemma.

\end{proof}

To complete the proof of Lemma~\ref{lem:lem:main_0}, we now prove {\bf Claim 1}.

\begin{proof}[Proof of Claim 1]
Note that an equivalent expression of event $E_i$ would be the event that there exists time $t_2 \in [\tau_\ell+T,\tau_\ell + t_1]$ such that on the $i$-th voter chain,
\begin{equation*}
    \max_{t_0,t_2:t_0 \leq \tau_\ell, t_2 \in [\tau_\ell+T,\tau_\ell + t_1]}(Z_i(t_0,t_2) - H_i(t_0,t_2)) \geq 0.
\end{equation*}

First, observe that 
\begin{eqnarray*}
&& \{U_i(t_1)=0\} \\
&=&  (\{U_i(t_1)=0\} \cap W_i) \cup (\{U_i(t_1)=0\} \cap W^c_i) \\ 
&\subseteq& W_i \cup (\{U_i(t_1)=0\} \cap W^c_i).
\end{eqnarray*}
Hence, to conclude the proof, it is sufficient to show that
\begin{equation*}
\{U_i(t_1)=0\} \cap W^c_i \subseteq E_i.
\end{equation*}

Second, we make the following observation, hereafter denoted as observation (1):
If the voter chain $i$ does not vote for any proposer block at level $l$ at some time $t>\tau_\ell$, then none of the honest blocks mined over the interval $(\tau_\ell,t]$ (if there are any) are in the voter chain $i$ at time $t$.


Now, define $A_i$ as the event that the voter chain $i$ does not vote for any proposer block at level $l$ at time $T$.
Then, by observation (1), either (i) no honest block was mined over the interval $(\tau_\ell,\tau_\ell+T]$, i.e $H_i(\tau_\ell,\tau_\ell+T)=0$; or (ii) honest blocks were mined over the interval $(\tau_\ell,\tau_\ell+T]$, yet, none of them are in the voter chain $i$ at time $T$.
Since $Z_i(\tau_\ell,\tau_\ell+T)$ is lower bounded by $0$, (i) clearly implies
\begin{equation*}
\max_{t_0,t_2:t_0 \leq \tau_\ell, t_2 \in [\tau_\ell+T,\tau_\ell + t_1]}(Z_i(t_0,t_2) - H_i(t_0,t_2)) \geq 0.
\end{equation*}

\begin{center}
\begin{figure}
     \includegraphics[width=9cm]{Slide1.JPG}
     \caption{Chain $C$ of adversary blocks. Filled blocks are adversary. Honest blocks mined over the interval $(\tau_\ell,\tau_\ell+T]$ are shown on the same chain below the chain $C$. (In general, they do not have to lie on the same chain.)}
     \label{fig:case_1}
\end{figure}
\end{center}

Next, let's assume that case (ii) happens.
Because every honest block is mined at a different level higher than the previous one, all of the honest blocks mined over the interval $(\tau_\ell,\tau_\ell+T]$ are at a unique level.
Moreover, since none of these honest blocks are in the voter chain $i$ at time $\tau_\ell+T$, there exists a chain $C$ at time $\tau_\ell+T$ that has length larger than or equal to the level of all of these honest blocks and does not contain any of them. See Figure~\ref{fig:case_1} for illustration.
The last honest block, $b_{\mathrm{last}}$, on chain $C$ was mined before time $\tau_\ell$, thus, it is at a level that is smaller than the levels of the honest blocks mined over the interval $(\tau_\ell,\tau_\ell+T]$.
Then, the levels of $C$ that are larger than this last honest block are occupied by adversary blocks.
Let $t_{\mathrm{last}} \leq \tau_\ell$ and $d_{\mathrm{last}}$ respectively be the mining time and level of this last honest block on $C$.
Observe that any honest block mined after time $t_{\mathrm{last}}$ is at a unique level larger than $d_{\mathrm{last}}$ that is matched by a unique adversary block on $C$ that was mined after time $t_{\mathrm{last}}$.
Hence, under case (ii),
\begin{equation*}
Z_i(t_{\mathrm{last}},\tau_\ell+T) - H_i(t_{\mathrm{last}},\tau_\ell+T) \geq 0.
\end{equation*}
Since $t_{\mathrm{last}} \leq \tau_\ell$,
\begin{equation*}
\max_{t_0,t_2:t_0 \leq \tau_\ell, t_2 \in [\tau_\ell+T,\tau_\ell + t_1]}(Z_i(t_0,t_2) - H_i(t_0,t_2)) \geq 0.
\end{equation*}

Finally, together with case (i), we can conclude that $A_i$ implies $E_i$:
\begin{equation*}
A_i \subseteq E_i.
\end{equation*}


Next, we express $W^c_i$ as the disjoint union of the events $A_i$ and $A^c_i \cap W^c_i$.
Observe that $A^c_i \cap W^c_i$ is the event that the voter chain $i$ votes for $B_l(T)$ at time $T$:
\begin{equation*}
A^c_i \cap W^c_i = \{U_i(T)=1\}.
\end{equation*}
Then,
\begin{equation*}
\{U_i(t_1)=0\} \cap A^c_i \cap W^c_i = \{U_i(T)=1\} \cap \{U_i(t_1)=0\}.
\end{equation*}

The event $\{U_i(T)=1\}$ implies the existence of a (possibly adversary) block $b^*$ mined at some level $d^*$ before time $\tau_\ell+T$ that votes for $B_l(T)$ and is in the voter chain $i$ at time $\tau_\ell+T$.
Similarly, $\{U_i(T)=1\} \cap \{U_i(t_1)=0\}$ implies the existence of a time $t_2 \in (\tau_\ell+T,\tau_\ell + t_1]$ such that $b^*$ leaves the voter chain $i$ for the first time after $\tau_\ell+T$ at time $t_2$.
Then, at time $t_2$, there exists a chain $C^*$ that contains $b^*$ and has length $D^*$ and a chain $C$ that does not contain $b^*$ and has length $D \geq D^*$. See Figure~\ref{fig:case_2} for illustration.
Notice that no honest block can be at a level larger than $D^*$ at time $t_2$ because $C^*$ \emph{was} the (public) voter chain $i$ just before time $t_2$.

\begin{figure}
     \includegraphics[width=9cm]{Slide2.JPG}
     \caption{Chains $C^*$ and $C$ with heights $D^*$ and $D$. Filled blocks are adversary.}
     \label{fig:case_2}
\end{figure}

Due to observation (1), none of the honest blocks mined before $b^*$ and after time $\tau_\ell$ are in the prefix of $b^*$ in $C^*$, implying that all of the blocks mined after time $\tau_\ell$ in the prefix $b^*$ are adversary blocks. 
Let $b_{\mathrm{com}}$ with mining time $t_{\mathrm{com}}$ and level $d_{\mathrm{com}}$ denote the last honest common block on the chains $C$ and $C^*$.
Note that $b_{\mathrm{com}}$ lies in the prefix of $b^*$ and is an honest block.
Then, as all of the blocks mined after time $\tau_\ell$ in the prefix $b^*$ are adversary blocks, we know that $t_{\mathrm{com}} \leq \tau_\ell.$ Refer to Figure~\ref{fig:case_2}.

Now, at every level in the interval $(d_{\mathrm{com}},D^*]$, either the chains $C$ and $C^*$ have a common adversary block, or the chains have two distinct blocks, one of which has to be an adversary block.
Hence, every level in the interval $(d_{\mathrm{com}},D^*]$ contains an adversary block that is a descendant of $b_{\mathrm{com}}$.
Then, any honest block mined in the interval $(t_{\mathrm{com}},t_2]$ arrives at a unique level $d$, $d_{\mathrm{com}} < d \leq D^*$, that also contains an adversary block descending from $b_{\mathrm{com}}$.
Since these adversary blocks descending from $b_{\mathrm{com}}$ should have been mined after time $t_{\mathrm{com}}$, i.e in the interval $(t_{\mathrm{com}},t_2]$, we conclude that
\begin{equation*}
Z_i(t_{\mathrm{com}},t_2) - H_i(t_{\mathrm{com}},t_2) \geq 0.
\end{equation*}
Since $t_{\mathrm{com}} \leq \tau_\ell$,
\begin{equation*}
\max_{t_0,t_2:t_0 \leq \tau_\ell, t_2 \in [\tau_\ell+T,\tau_\ell + t_1]}(Z_i(t_0,t_2) - H_i(t_0,t_2)) \geq 0.
\end{equation*}


Finally, we observe that
\begin{equation*}
\{U_i(T)=1\} \cap \{U_i(t_1)=0\} \subseteq E_i,
\end{equation*}
which further implies
\begin{eqnarray*}
&&\{U_i(t_1)=0\} \cap W^c_i \\
&=& (\{U_i(t_1)=0\} \cap A^c_i \cap W^c_i) \cup (\{U_i(t_1)=0\} \cap A_i \cap W^c_i) \\
&\subseteq& (\{U_i(T)=1\} \cap \{U_i(t_1)=0\}) \cup A_i \\
&\subseteq& E_i,
\end{eqnarray*}
which concludes the proof.



\end{proof}

Then we can prove the main theorem. We restate it for $\Delta = 0$ in the following theorem.

\begin{theorem}[Restatement of Theorem \ref{thm:main} for $\Delta = 0$]
\label{thm:main_0}
Assume $\Delta = 0$. If $B_\ell(T)$ is confirmed at time $\tau_\ell + T$,i.e., 
$$h^0(\frac{1}{(1+\delta)m\lambda}\sum_{i=1}^{m} d_i(T)) \geq \frac{1}{m} \bar V_\ell(T) + \frac{1}{2} +\delta,$$ 
then number of votes received by $B_\ell(T)$ will be greater than number of votes received by any other proposer block at time $t$ for all $t>\tau_\ell + T$, except for probability $e^{-2\delta^2 m} + 2e^{-\frac{\delta^2 t_\delta^* \lambda m}{3}}$, where $t_\delta^*$ is the time such that $h^0(t_\delta^*) = \frac{1}{2} + \delta$ for $0 < \delta < \frac{1}{2}$. Note that $\tau_\ell + T$ is a random time chosen by an honest node to observe the blockchains.
\end{theorem}

\begin{remark}
When there is only one single proposer block at level $\ell$ (i.e., $\bar V_\ell(T) = 0$), the confirmation rule is simply confirming the single proposer block when $\sum_{i=1}^{m} d_i(T) \geq (1+\delta)m\lambda t^*_\delta$ by the monotonicity of $h^0(t)$.
\end{remark}

\begin{proof}
We define random variables $H_i$, $Z_i$ and $U_i(t)$, events $E_i$ and $F_i$ ($1\leq i \leq m$) the same as in Lemma~\ref{lem:lem:main_0}.
And again we prove the theorem by contradiction. Suppose at time $t_1 > \tau_\ell + T$, $V_\ell(t_1)$ is smaller than number of votes received by another proposer block, which implies that $V_\ell(t_1) \leq m/2$.
Then similar to the arguments in Lemma \ref{lem:lem:main_0}, we have
\begin{eqnarray*}
    \sum_{i=1}^m \indicator_{F_i} &\geq& m - \bar V_\ell(T) - V_\ell(t_1) \\
    &\geq& m - \bar V_\ell(T) - m/2 \\
    &=& m/2 - \bar V_\ell(T) \\
    &\geq& m \big (1-h^0(\frac{1}{(1+\delta)m\lambda}\sum_{i=1}^{m} d_i(T))\big ) + m\delta.
\end{eqnarray*}
Let event $G$ be the event that $\sum_{i=1}^m d_i(T) \geq (1+\delta) m\lambda T$, i.e., the sum of the depths of the voter blocks is atypically large at time $\tau_\ell + T$. Then we have
\begin{eqnarray}
    \label{eqn:total_prob}
    && P(V_\ell(t_1) \leq m/2)  \nonumber\\
    &\leq& P(\sum_{i=1}^m \indicator_{F_i} \geq  m \big (1-h^0(\frac{1}{(1+\delta)m\lambda}\sum_{i=1}^{m} d_i(T))\big ) + m\delta) \nonumber\\
    &=& P(G,\sum_{i=1}^m \indicator_{F_i} \geq  m \big (1-h^0(\frac{1}{(1+\delta)m\lambda}\sum_{i=1}^{m} d_i(T))\big ) + m\delta) \nonumber\\
    &+& P(G^c,\sum_{i=1}^m \indicator_{F_i} \geq  m \big (1-h^0(\frac{1}{(1+\delta)m\lambda}\sum_{i=1}^{m} d_i(T))\big ) + m\delta) \nonumber\\
    &\leq& P(G) + P(\sum_{i=1}^m \indicator_{F_i} \geq  m \big (1-h^0(T))\big ) + m\delta).
\end{eqnarray}

We first bound the probability $P(G)$. Since we have 
$$h^0(\frac{1}{(1+\delta)m\lambda}\sum_{i=1}^{m} d_i(T)) \geq \frac{1}{m} \bar V_\ell(T) + \frac{1}{2} +\delta \geq \frac{1}{2} +\delta,$$
by the definition of $t^*_\delta$ and the monotonicity of $h^0(t)$, we know $\sum_{i=1}^m d_i(T) \geq (1+\delta)m\lambda t^*_\delta$. And since the depth of a voter block is maximized when no fork happens, we know $\sum_{i=1}^{m} (H_i(\tau_\ell,\tau_\ell + T)+Z_i(\tau_\ell,\tau_\ell + T)) \geq \sum_{i=1}^{m} d_i(T) \geq (1+\delta)m\lambda t^*_\delta$. Let event $\hat G$ be the event that $\sum_{i=1}^{m} (H_i(\tau_\ell,\tau_\ell + T)+Z_i(\tau_\ell,\tau_\ell + T)) \geq (1+\delta) m\lambda T$.
Then we have
\begin{eqnarray}
\label{eqn:first_prob}
    && P(G) \nonumber \\
    &\leq& P(\hat G, T> t^*_\delta) + P(\hat G, T \leq t^*_\delta) \nonumber \\
    &\leq& P(\texttt{Poi}(m\lambda T) \geq (1+\delta) m\lambda T, T> t^*_\delta) + P(T \leq t^*_\delta) \nonumber \\
    &\leq& P(\texttt{Poi}(m\lambda T) \geq (1+\delta) m\lambda T, T> t^*_\delta) \nonumber \\
    &+& P(\texttt{Poi}(m\lambda t^*_\delta) \geq (1+\delta) m\lambda t^*_\delta) \nonumber \\
    &\leq& 2e^{-\frac{\delta^2 t_\delta^* \lambda m}{3}},
\end{eqnarray}
where the last inequality is due to Poisson tail bound.

For the second term in (\ref{eqn:total_prob}), by Lemma \ref{lem:lem:main_0} we have
\begin{equation}
    \label{eqn:second_prob}
     P(\sum_{i=1}^m \indicator_{F_i} \geq  m(1-h^0(T)) + m\delta)  \leq e^{-2\delta^2 m}.
\end{equation}
Combine (\ref{eqn:total_prob}), (\ref{eqn:first_prob}) and (\ref{eqn:second_prob}), we have
\begin{equation*}
    P(V_\ell(t_1) \leq m/2) \leq e^{-2\delta^2 m} + 2e^{-\frac{\delta^2 t_\delta^* \lambda m}{3}},
\end{equation*}
which concludes the proof.
\end{proof}


\subsection{Proof  of Theorem \ref{thm:main} for $\Delta > 0$}
\label{app:proof_sketch}
We outline the steps needed to extend the proof technique in Theorem \ref{thm:main_0} to general cases when $\Delta > 0$.

{\bf \noindent Worst case attack}. For positive $\Delta$, characterizing the worst case attack for the longest chain protocol is challenging, but we are only interested in the regime where the block speed of each voter chain is very slow (i.e. $\lambda \Delta \ll 1$). 
Without loss of generality, we renormalize time such that $\lambda = 1$ to simplify notations.
Recall that $q_t(\lambda_h,\lambda_a,\Delta,\pi)$ is the reversal error probability of a block that has been mined for time $t$ under adversary strategy $\pi$, where $\lambda_h = (1-\beta)$ is the honest mining rate and $\lambda_a = \beta$ is the adversary mining rate. We fix $\beta$ and $t$, and write $f(\Delta, \pi) = q_t(\lambda_h,\lambda_a,\Delta,\pi)$. Let
$$g(\Delta) = \max_{\pi} f(\Delta, \pi),$$
$$\pi^*(\Delta) = \arg \max_{\pi} f(\Delta, \pi).$$
And we know $\pi^*(0)$ is the private attack with pre-mining. For $\Delta > 0$, we have
\begin{eqnarray*}
    &&g(\Delta)  \\
    &=& f(\Delta, \pi^*(\Delta)) \\
    &=& f(0, \pi^*(0)) + \frac{\partial f}{\partial \Delta}(0,\pi^*(0))\cdot \Delta \\
    &~~~~+& \frac{\partial f}{\partial \pi^*}(0,\pi^*(0))\cdot \frac{\partial \pi^*(0)}{\partial \Delta} \cdot \Delta + O(\Delta^2) \\
    &=& f(0, \pi^*(0)) + \frac{\partial f}{\partial \Delta}(0,\pi^*(0))\cdot \Delta + O(\Delta^2) \\
    &=& f(\Delta, \pi^*(0)) + O(\Delta^2).
\end{eqnarray*}
Thus  reintroducing $\lambda$ into the result, we have 
$$q_t(\lambda_h,\lambda_a,\Delta,\pi^*(\lambda,\Delta)) = q_t(\lambda_h,\lambda_a,\Delta, \pi^*(\lambda,0)) + O(\lambda^2\Delta^2),$$ 
i.e., for small $\lambda \Delta$ we can use the error probability under the private attack to approximate the error probability under the worst attack. 

{\bf \noindent Poisson approximation}. Further note that for $\lambda \Delta > 0$, the pure honest chain does not grow as a Poisson process because of forking. \cite{dembo2020everything} showed that the worst case forking and hence the worst case chain growth is achieved when every honest block is delivered with maximum delay $\Delta$. In the worst case forking, let $T_d$ be the time it takes for pure honest chain to reach depth $d$ after reaching depth $d - 1$. Then by the memoryless property of the mining process, $T_d$'s are i.i.d. random variables and we can write $T_d$ as $T_d = \Delta + S_d $, where $S_d$'s are i.i.d.\ and exponentially distributed with rate $\lambda_h$. So we have 
\begin{equation*}
    E[T_d] = \Delta + E[S_d] = \Delta + \frac{1}{\lambda_h}.
\end{equation*}

To further simplify the calculation, we approximate the distribution of $Y_d$ with an exponential distribution with rate $\lambda_h'$, where $\lambda_h' = \frac{\lambda_h}{1+\lambda_h \Delta}$, which is equivalent to model the honest chain growth as Poisson process with rate $\lambda_h'$. 

With the two approximations above, we can simply calculate $h^{\Delta}(t)$ by

\begin{eqnarray*}
    h^\Delta(t) &=& 1 - q_t(\lambda_h,\lambda_a,\Delta,\pi^*(\lambda,\Delta))  \\
    &\approx& 1 - q_t^0(\lambda_h',\lambda_a,).
\end{eqnarray*}

{\bf \noindent Correlation across voter chains}. Note that $h^\Delta(t)$ only captures the behavior of one single voter chain. To complete the proof of the main theorem, we still need some independence across all the voter chains. In the proof of Theorem \ref{thm:main_0}, we implicitly assume that the mining processes or arrival of blocks on different voter chains are independent, which is achieved by the Cryptographic sortition mechanism proposed in Prism. The sortition splits the aggregate mining process, which we model it as a Poisson process when the number of miners is very large, into $m$ independent Poisson processes with equal rates.

\iffalse
We model the sortition in Prism as a random oracle $\texttt{PoW}_\texttt{Prism}(X): X \to (S_1,S_2,\cdots,S_m)$, where $X$ is an input binary string with arbitrary length, the output is a random binary vector such that $\sum_{i=1}^m S_i = 1$ with probability $p$ and 0 with probability $1-p$, and each $S_i = 1$ with equal probability. We compare $\texttt{PoW}_\texttt{Prism}(X)$ with an ideal random oracle consist of $m$ independent random oracles: $\texttt{IPoW}(X): X \to (S_1,S_2,\cdots,S_m)$, where $X$ is an input binary string with arbitrary length, and each $S_i$ in the output equals to 1 with probability $p/m$ and all $S_i$'s are independent. 
Indeed, the sortition in Prism is equivalent to the $m$-for-$1$-PoW proposed in \cite{cryptoeprint:2020:675}, and thus  Lemma 7 in \cite{cryptoeprint:2020:675} also applies for $\texttt{PoW}_\texttt{Prism}(X)$. We restate it here.

\begin{lemma}[Lemma 7 in \cite{cryptoeprint:2020:675}]
\label{lem:ind}
For any $x \in {0,1}^*$, we have 
$$\delta(\texttt{PoW}_\texttt{Prism}(x), \texttt{IPoW}(x)) \leq p^2,$$
where $\delta(\cdot,\cdot)$ denotes the total variation distance of two random variables.
\end{lemma}

Lemma \ref{lem:ind} justifies the use of sortition in Prism for achieving independence on the mining processes. To be specific, observe that the use of $\texttt{IPoW}$ would provide full independence across the mining on the $m$ voter chains, and by Lemma \ref{lem:ind} the sortition with $\texttt{PoW}_\texttt{Prism}$ will only differ from $\texttt{IPoW}$ with negligible probability (e.g., $p \approx 10^{-22}$ currently for Bitcoin).
\fi

Further, following the proof of Lemma 16 in \cite{cryptoeprint:2020:675}, not only the events related to block arrivals are independent, the adversary attacks on different voter chains are also negatively correlated.
That is, $P(\cap F_i) \leq \prod P(F_i)$ conditioned on some events occurring with probability at least $1-\varepsilon$, where $F_i$ is the persistence or liveness failure events on the $i$-th voter chain and $\varepsilon$ is negligible in the security parameter. This result directly implies that the correlations across the voter chains are simply negative for the adversary. Armed with this negative correlation property, the proof of Theorem $\ref{thm:main_0}$ can now be extended to the general non-zero delay case. 


\subsection{Proof of Theorem \ref{thm:latency}}
\label{app:latency}

In this section, we discuss the latency of our proposed confirmation rule. We focus on the single proposer block case, i.e., the latency of CR3. Note that although the depth of a voter block is observable for both online and offline nodes, it also greatly depends on the adversary actions. For example, under private attack, each voter chain does not grow with the full rate $\lambda$, hence the confirmation will get delayed compared with the scenario where the adversary follows the protocol. Further, we will see that the adversary can even reduce the depth of the vote by revealing a private chain consist of voter blocks with null votes. Fortunately, we are able to obtain the upper bound of the latency in the single proposer block case by identifying the worst case attack in term of delaying the confirmation.  

{\bf \noindent No attack}. The best case latency of CR3 is achieved when the adversary follows the voting rule and longest chain rule in each voter chain. Under this no attack case, the depth of the vote grows as a Poisson process with rate $\lambda$. Hence the expected latency under no attack is $(1+\delta)m\lambda t^*_\delta/(m\lambda) = (1+\delta) t^*_\delta$.

{\bf \noindent Private attack}. In the private attack, the adversary mines private chains forked from the voter blocks that vote for the single proposer block at level $\ell$, and delays the delivery of every honest voter block with the maximum network delay $\Delta$. We have already seen that the pure honest chain growth under the worst case forking can be approximated with a Poisson process with rate $\lambda_h' = \frac{\lambda_h}{1+\lambda_h \Delta}$. Hence the expected latency under private attack is $(1+\delta)m\lambda t^*_\delta/(m\lambda_h') = (1+\delta) t^*_\delta\lambda/\lambda_h'$.

{\bf \noindent Slow-down attack}.   Next we  show that the worst case latency of CR3 is achieved when the adversary uses the following ``slow down'' attack on all the voter chains.

\begin{defn}[Slow down attack]
\label{def:slow}
On each voter chain, the adversary mines a private chain with null votes forked from the voter block that votes for the single proposer block at level $\ell$. Meanwhile, the adversary delays the delivery of every honest voter block with the maximum network delay $\Delta$. Whenever the length of the private chain is greater than or equal to the public honest chain, the adversary reveals some private blocks to match the length of the public chain and force all honest nodes to mine on the adversary block (we assume tie breaking is in favor of the adversary in the longest chain rule). 
%See Fig. \ref{fig:slow_down} for an example.
\end{defn}

%\begin{figure}
%    \centering
%    \includegraphics[width=0.5\textwidth]{figures/slow_down.png}
%    \caption{Slow down attack}
%    \label{fig:slow_down}
%\end{figure}

\begin{lemma}[Optimality of slow down attack]
\label{lem:slow_down}
The slow down attack is the worst case attack in term of reducing the depth of the vote on a voter chain.
\end{lemma}

\begin{proof}
We show that for each sample path, the slow down attack will lead to the smallest depth of the voter block that votes for the single public proposer block at level $\ell$. Since the slow down attack is independent and identical on all the voter chains, we will only focus on one of the voter chains and WLOG let it be voter chain one.

Given a sample path (a sequence of block arrival times $t_1, t_2, \cdots, t_n$ in the time interval $(\tau_\ell + \Delta, \tau_\ell + \Delta + t)$). Let $B_\ell$ be the single public proposer block at level $\ell$, then all honest nodes will receive $B_\ell$ at time $\tau_\ell + \Delta$. By the honest voting rule, the depth of the vote for $B_\ell$ is the depth of the first honest block mined after $\tau_\ell + \Delta$ in the public longest chain, that is also the difference between the length of the public longest chain and the length of the public adversary chain (here the length of a chain only counts blocks mined in the time interval $(\tau_\ell + \Delta, \tau_\ell + \Delta + t)$).

We recall that the minimal length of the public longest chain can be achieved by keeping every adversary block private and delivering every honest block with maximum delay $\Delta$. Although the slow down attack may reveal some private blocks at some time, it never increase the length of the public chain. Therefore, the slow down attack achieves the minimal length of the public longest chain at time $\tau_\ell + \Delta + t$.

On the other hand, the maximum length of the public adversary chain is obtained at the last time when the adversary mines more blocks than the length of the public chain. i.e., the largest $t' \in [0,t]$ such that the number of adversary blocks is no less than the length of the honest chain under the worst case forking in the time interval $(\tau_\ell+\Delta,\tau_\ell+\Delta+t')$ (if the adversary never catches up the honest chain before $\tau_\ell + \Delta + t$, then $t' =0$). Since in the slow down attack the adversary reveals its private blocks whenever it can match the public chain, it also achieves the maximum length of the public adversary chain. Therefore, the slow down attack achieves the minimal depth of the vote for $B_\ell$.
\end{proof}

Let $d_i^{SD}(t)$ be the depth of the vote on the $i$-th voter chain at time $\tau_\ell + \Delta + t$ under slow down attack for $1 \leq i \leq m$. Then $d_1^{SD}(t)$, $d_2^{SD}(t)$, \dots, $d_m^{SD}(t)$ are i.i.d. random variables. Again for simplicity we will approximate the arrival of honest blocks as a Poisson process with rate $\lambda_h' = \frac{\lambda_h}{1+\lambda_h \Delta}$. Let the effective total mining rate be $\lambda' = \lambda_h'+\lambda_a$ and the effective adversary fraction be $\beta' = \lambda_a/\lambda'$. Then the distribution of $D = d_1^{SD}(t)$ is given by the following equations. 

\begin{eqnarray}
    && P(D=0)  \nonumber\\
    &=& P(H_1(\tau_\ell +\Delta,\tau_\ell +\Delta +t) \leq Z_1(\tau_\ell+\Delta,\tau_\ell+\Delta + t))  \nonumber \\
    &=& \sum_{j=0}^{+\infty} e^{-(1-\beta')\lambda' t} \frac{((1-\beta')\lambda' t)^j}{j!} \Big( \sum_{i=j}^{+\infty} e^{-\beta'\lambda' t} \frac{(\beta'\lambda' t)^i}{i!} \Big) \nonumber \\
    &&\label{eqn:dist1}\\
    && P(D=d) \nonumber \\
    &=& \sum_{n=d}^{+\infty} e^{-\lambda' t} \frac{(\lambda' t)^n}{n!} \cdot \Big(\sum_{c = \lceil \frac{n-2d}{2} \rceil_+}^{\lfloor \frac{n-d}{2} \rfloor} \binom{2c}{c} \binom{n-2c}{d} \cdot\nonumber \\
    &&~~~~~\beta'^{n-c-d} (1-\beta')^{c+d} \frac{2d+2c-n}{n-2c}\Big) \nonumber \\
    &&\label{eqn:dist2}
\end{eqnarray}

For $d \geq 1$ in (\ref{eqn:dist2}), conditioned on that $n$ blocks are mined in the interval $(\tau_\ell+\Delta,\tau_\ell+\Delta + t)$, the depth of the vote is equal to $d$ when (i) for the first $2c$ blocks, the number of adversary blocks is equal to the number of honest blocks; (ii) for the remaining $n-2c$ blocks, there are $d$ honest blocks and $n-2c-d$ adversary blocks, and also the number of honest blocks is strictly greater than the number of adversary blocks in any prefix of the sample path (which is a Ballot problem). (i) happens with probability $\binom{2c}{c} \beta'^c (1-\beta')^c$ and (ii) happens with probability $\binom{n-2c}{d} \beta'^{n-2c-d} (1-\beta')^d \frac{2d+2c-n}{n-2c}$. By choosing the proper range for $c$, we get (\ref{eqn:dist2}).

\begin{lemma}[Latency of CR3]
\label{lem:latency_cr0'}
The expected worst case latency of CR3 is $t^w$, where $t^w$ is the solution of the equation $E[d_1^{SD}(t)] = (1+\delta)t_\delta^*\lambda$.
\end{lemma}

\begin{proof}
By Lemma \ref{lem:slow_down}, we have $E[\sum_{i=1}^m d_i(t^w)] \geq E[\sum_{i=1}^{m} d_i^{SD}(t^w)] = m \cdot E[ d_1^{SD}(t^w)] = (1+\delta)t_\delta^* \lambda m$.
\end{proof}

Lemma \ref{lem:latency_cr0'} directly implies Theorem \ref{thm:latency}.



\iffalse
\subsection{Numerical Evaluations of Latency}
In the experiment, we set adversary fraction $\beta = 0.2$, voter chain mining rate $\lambda_v = 0.2$, proposer chain mining rate $\lambda_p = 0.1$, network delay upper bound $\Delta = 4s$ and the slack in the confirmation rule $\delta = 0.1$. 

Then for each voter chain, the effective honest mining rate would be $\lambda_h' =\frac{(1-\beta)\lambda}{1+(1-\beta)\lambda \Delta} = 0.0976$, the adversary rate $\lambda_a = \beta \lambda = 0.04$, hence the effective adversary fraction $\beta' =\frac{\lambda_a}{\lambda_a+\lambda_h} = 0.29$ and the effective mining rate $\lambda' = \lambda_a + \lambda_h' = 0.1376$.

Let $t_\delta^*$ be the solution of the equation $h^\Delta(t_\delta^*) = \frac{1}{2} + \delta = 0.6$, then we have $t_\delta^* = 44.4s$. We further check that the error probability $\epsilon$ given by Theorem \ref{thm:main_0} is
$$\epsilon = e^{-2\delta^2 m} + 2e^{-\frac{\delta^2 t_\delta^* \lambda m}{3}} = 2 \times 10^{-9}.$$

Then the normal path (no attack and no fork) latency is given by $(1+\delta)t_\delta^* = 48.84s$. However, in the experiment, the voter chains will fork. Suppose the actual network delay is $\Delta_\text{true} = 1.6s$, then the fork rate is $1 - \frac{1}{1+\lambda \Delta_\text{true}} = 24\%$. Therefore, in the experiment, the voter chains would grow slower. Also it takes $1/\lambda_p = 10s$ for a proposer block to be mined. So we should expect the latency measured in the experiment to be $48.84/(1-24\%) + 10 = 74.3s$, which matches with the experiment result.
\fi

==> Prism Systems Paper (CCS)/propagation.tex <==
\section{Block Propagation Delay Distribution}
\label{apx:propagation}

 Here we present the distribution plots of the block propagation delay ($\Delta$) in topologies tested in our scalability experiment (\S\ref{sec:eval-scale}). The data are shown in Figures~\ref{fig:propagation1}, \ref{fig:propagation2}, \ref{fig:propagation3}, \ref{fig:propagation4}, \ref{fig:propagation5}. In each plot, the concrete lines mark the mean of the propagation delay of that type of blocks, and the dashed lines mark the $25\%$ and $75\%$ quantiles. Comparing Figures~\ref{fig:propagation1}, \ref{fig:propagation3}, \ref{fig:propagation5} we observe that as long as the network diameter is kept constant, the block propagation delay is barely affected by the increase of clients.


\begin{figure}[t]
   \centering
   \includegraphics[width=\linewidth]{figures/delay100nodes.pdf}
   \caption{Block propagation delay. Nodes$=100$, Degree$=4$, Diameter$=5$}%\vspace{-6mm}
   \label{fig:propagation1}
 \end{figure}
 
 \begin{figure}[t]
   \centering
   \includegraphics[width=\linewidth]{figures/delay300nodes4.pdf}
   \caption{Block propagation delay. Nodes$=300$, Degree$=4$, Diameter$=7$}%\vspace{-6mm}
   \label{fig:propagation2}
 \end{figure}
 
 \begin{figure}[t]
   \centering
   \includegraphics[width=\linewidth]{figures/delay300nodes6.pdf}
   \caption{Block propagation delay. Nodes$=300$, Degree$=6$, Diameter$=5$}%\vspace{-6mm}
   \label{fig:propagation3}
 \end{figure}
 
 \begin{figure}[t]
   \centering
   \includegraphics[width=\linewidth]{figures/delay1000nodes4.pdf}
   \caption{Block propagation delay. Nodes$=1000$, Degree$=4$, Diameter$=9$}%\vspace{-6mm}
   \label{fig:propagation4}
 \end{figure}
 
 \begin{figure}[t]
   \centering
   \includegraphics[width=\linewidth]{figures/delay1000nodes8.pdf}
   \caption{Block propagation delay. Nodes$=1000$, Degree$=8$, Diameter$=5$}
   \label{fig:propagation5}
 \end{figure}
 



==> Prism Systems Paper (CCS)/pseudocode.tex <==
\section{Pseudocode}
\label{sec:pseudocode}

\begin{algorithm}
{\fontsize{8pt}{8pt}\selectfont \caption{Prism: Mining}\label{alg:prism_minining}
\begin{algorithmic}[1]

\Procedure{Main}{ }
    \State \textsc{Initialize}()
    \While{True}
        \State $header, Ppf, Cpf$ =  \textsc{PowMining}() \label{code:blockBody1}
        \State \maincolorcomment{Block contains header, parent, content and merkle proofs}
        \If{header is a \textit{tx block}}
        \State $block \gets \langle header, txParent, txPool, Ppf, Cpf\rangle$
        \ElsIf{header is a \textit{prop block}}
        \State $block \gets \langle header, prpParent, unRfTxBkPool, Ppf, Cpf\rangle$\label{code:blockBody2}
        \ElsIf{header is a \textit{block in voter} blocktree $i$}
        \State $block \gets \langle header, vtParent[i], votesOnPrpBks[i], Ppf,\label{code:blockBody3} Cpf\rangle$
        % \State \textbf{and} \textsc{ReceiveMessage}($\langle$ header, $TxP$ $\rangle$)
        \EndIf
        \State \textsc{BroadcastMessage}($block$)  \colorcomment{Broadcast to peers}

    \EndWhile
\EndProcedure

\Procedure{Initialize}{ } \colorcomment{ All variables are global}
\vspace{0.5mm} \State \maincolorcomment{Blockchain data structure $C  = (prpTree, vtTree) $}
\State $prpTree \gets genesisP$ \label{code:prpGenesis} \colorcomment{Proposer Blocktree}
\For{$i \gets 1 \; to \; m$}
\State $vtTree[i] \gets genesisM\_i$ \colorcomment{Voter $i$ blocktree} \label{code:voterGenesis}
\EndFor
\State \maincolorcomment{Parent blocks to mine on} \label{code:VarprpParent}
\State $prpParent$ $\gets genesisP $ \colorcomment{ Proposer block to mine on} 
\For{$i \gets 1 \; to \; m$}
\State $vtParent[i]$ $\gets genesisM\_i $ \colorcomment{Voter tree $i$ block to mine on}
\EndFor \label{code:VarvtParent}
\vspace{00.4mm}\State \maincolorcomment{Block content} \label{code:allcontent}
\State  $txPool$ $\gets \phi$ \colorcomment{Tx block content: Txs to add in tx bks} \label{code:txblockcontent}
\State $unRfTxBkPool$ $ \gets \phi$ \colorcomment{Prop bk content1: Unreferred tx bks} \label{code:prblockcontent1}
\State $unRfPrpBkPool$ $ \gets \phi$ \colorcomment{Prop bk content2: Unreferred prp bks} \label{code:prblockcontent2}
\For{$i \gets 1 \; to \; m$}
\State $votesOnPrpBks(i) \gets \phi$ \colorcomment{Voter tree $i$ bkbk content } \label{code:vtblockcontent}
\EndFor

\EndProcedure
\vspace{1mm}
\Procedure{PowMining}{ }
\While{True}
\State  $txParent \gets prpParent$ \label{code:initParent}
\State \maincolorcomment{Assign content for all block types/trees}
\For{$i \gets 1 \;  to \; m$} $vtContent[i] \gets votesOnPrpBks$[i] \label{code:voteIneffcient}
\EndFor
\State $txContent \gets txPool$
\State $prContent \gets (unRfTxBkPool, unRfPrpBkPool)$
\vspace{00.4mm}\State \maincolorcomment{Define parents and content Merkle trees}
\State $parentMT\gets$MerklTree($vtParent,txParent,prpParent$) %\colorcomment{Store all the potential ancestors in a Merkle Tree}
\State $contentMT\gets$MerklTree($vtContent,txContent,prContent$) \label{code:endContent}
\State nonce $ \gets $ RandomString($1^\kappa$)
\State \maincolorcomment{Header is similar to Bitcoin}
\State header $\gets \langle$ $parentMT.$root, $contentMT.$root, nonce $\rangle$
\vspace{00.4mm} \State \maincolorcomment{Sortition into different block types/trees } \label{code:sortitionStart}
\If {Hash(header)  $\leq mf_v$} \colorcomment{Voter block mined}
    \State $i\gets  \lfloor $Hash(header)/$f_v\rfloor$
    \textbf{and} \textit{break} \colorcomment{on tree $i$ }
\ElsIf{ $mf_v < $Hash(header)  $ \leq mf_v+f_t$} 
    \State  $i \gets m+1$ \textbf{ and} \textit{break}\colorcomment{Tx block mined}
\ElsIf{ $mf_v+f_t< $ Hash(header) $\leq mf_v+f_t+f_p$} 
    \State  $i \gets m+2$ \textbf{ and} \textit{break}\colorcomment{Prop block mined}
\EndIf
\EndWhile \label{code:sortitionEnd}
\maincolorcomment{Return header along with Merkle proofs}
\State \Return $\langle header, parentMT.$proof($i$),  $contentMT.$proof($i) \rangle$ \label{code:minedBlocm}
\EndProcedure
\\

\Procedure{ReceiveBlock}{\textsf{B}} \colorcomment{Get block from peers}    
\If {\textsf{B} is a valid \textit{transaction block}} \label{code:txblk_r1}
    \State $txPool$.removeTxFrom(\textsf{B}) \label{code:updateTxContent} %\colorcomment{Remove the txs present in  \textsf{B} } 
    \State $unRfTxBkPool$.append(\textsf{B})\label{code:txblk_r2}

\ElsIf{\textsf{B} is a valid \textit{block on $i^{\text{th}}$ voter tree}} \label{code:vtblk_r1}
%    \State \maincolorcomment{Append \textsf{B} and (if required) all its ancestors}
    \State $vtTree[i]$.append(\textsf{B}) \textbf{and} $vtTree[i]$.append(\textsf{B}.ancestors())    
    \If{\textsf{B}.chainlen $> vtParent[i]$.chainlen} 
    \State $vtParent[i] \gets \textsf{B} $ \textbf{and} $votesOnPrpBks$($i$).update(\textsf{B}) \label{code:updateVoteMine}
    \EndIf\label{code:vtblk_r2}

\ElsIf{\textsf{B} is a valid \textit{prop block}} \label{code:prpblk_r1}
    \If{\textsf{B}.level $==prpParent$.level+$1$}
    \State $prpParent \gets \textsf{B}$ \label{code:updatePropToMine}
    \For{$i \gets 1 \;  to \; m$}  
    \colorcomment{Add vote on level $\ell$ on all $m$ trees}
    \State $votesOnPrpBks($i$)[\textsf{B}.level] \gets \textsf{B}$   \label{code:addVote} 
    \EndFor
    % \State ChangeMainChain() \colorcomment{Similar as  Bitcoin protocol}
    \ElsIf{\textsf{B}.level $ > prpParent$.level+$1$}
        \State \maincolorcomment{Miner doesnt have block at level $prpParent$.level+$1$}
        \State \textsc{RequestNetwork(\textsf{B}.parent)} 
    \EndIf
    \State  $prpTree[\textsf{B} $.level].append(\textsf{B}),\; $unRfPrpBkPool$.append(\textsf{B})
%    \State \maincolorcomment{Remove the tx blocks and prop blocks referred by \textsf{B} }
    \State $unRfTxBkPool$.removeTxBkRefsFrom(\textsf{B}) \label{code:updateTxBkContent}
    \State $unRfPrpBkPool$.removePrpBkRefsFrom(\textsf{B}) \label{code:updatePrpBkContent}`
    % \State $[$\ell$] \gets X.ancestor[-i]$ 
        % \textsc{ReceiveMessage}(\textsf{B} .ancestor$[n-i]$)
    

\EndIf
\vspace{1mm}
\EndProcedure

\Procedure{ReceiveTx}{\textsf{tx}} 
\If {\textsf{tx} has valid signature }   $txPool$.append(\textsf{B})
\EndIf    
\EndProcedure
\end{algorithmic}
}
\end{algorithm}

\begin{algorithm}
{\fontsize{8pt}{8pt}\selectfont \caption{Prism: Tx confirmation}\label{alg:prism_con}
\begin{algorithmic}[1]

\Procedure{IsTxConfirmed}{$tx$}\label{code:fastConf}
    \State $\Pi \gets \phi$         \colorcomment{Array of set of proposer blocks}
    \For{$\ell \gets 1 \;  to \; prpTree.$maxLevel}  
        \State $votesNdepth \gets \phi$ %\colorcomment{Votes from all $m$ voter trees on level $\ell$}
        \For{$i$ in $1\;to\;m$} \label{code:getvotes_start}
        \State  $votesNdepth[i] \gets \textsc{GetVoteNDepth}(i, \ell)$ 
        % \State $vtMCs[i] = vtTree[i].$LongestChain()
        \EndFor
            \If{IsPropSetConfirmed($votesNdepth$)}
        \State $\Pi[\ell] \gets$ {GetProposerSet}$(votesNdepth)$ \label{code:confirmPrpList}
        \Else $\;$ \textbf{break}\label{code:appendPrpList}
        \EndIf
    \EndFor
%    \vspace{3mm}
    \State \maincolorcomment{Ledger list decoding: Check if tx is confirmed in all ledgers}
    \State $prpBksSeqs \gets \Pi[1]\times \Pi[2]\times\cdots\times\Pi[\ell]$  \colorcomment{outer product} \label{code:outerproduct}
\For{$prpBks$ in $prpBksSeqs$} \label{code:ledgers_for_start}
                \State $ledger$ = \textsc{BuildLedger}($prpBks$)
    \If{$tx$ is \textbf{not confirmed} in \av{ledger}} \Return False
    \EndIf
    \EndFor
    \Return True \colorcomment{Return true if tx is confirmed in all ledgers} \label{code:fastConfirmTx}
\EndProcedure
\vspace{1mm}
\State \maincolorcomment{Return the vote of voter blocktree $i$ at level $\ell$ and  depth of the vote}
\Procedure{GetVoteNDepth}{$i, \ell$}
    \State $voterMC \gets vtTree[i].LongestChain()$
    \For{$voterBk$ in $voterMC$} \label{code:voteCountingStart}
%        \State \maincolorcomment{A valid voter block references one proposer block per level.}
        \For{$prpBk$ in $voterBk$.votes}
%            \State \maincolorcomment{Skip the votes on the first $\ell-1$ levels.}
%            \If{$prpBk$.level $ < \ell$} continue 
            \If{$prpBk$.level $ = \ell$} 
                    \State \maincolorcomment{Depth is \#of children bks of voter bk on main chain}
\State  \Return ($prpBk$, $voterBk$.\text{depth}) \label{code:voteCountingEnd}
            \EndIf
        \EndFor
    \EndFor
\EndProcedure
\vspace{1mm}
\Procedure{BuildLedger}{\av{propBlocks}} \colorcomment{Input: list of prop blocks}\label{code:buildLedgerFunc}
\State \av{ledger} $\gets []$ \colorcomment{List of valid transactions}
\For{\av{prpBk} in \av{propBlocks}} 
%    \State \maincolorcomment{\av{prpBk} defines the epoch} 
    \State $refPrpBks \gets prpBk.$getReferredPrpBks() \label{code:epochStarts}
    \State \maincolorcomment{Get all directly and indirectly referred transaction blocks.}
    \State  $txBks \gets\;  ${GetOrderedTxBks}$(prpBk, refPrpBks)$ \label{code:txbksOrdering}
    \For{\av{txBk} in \av{txBks}}
        \State $txs \gets txBk$.getTxs() \colorcomment{Txs are ordered in \av{txBk}}
        \For{$tx$ in $txs$}
        \State \maincolorcomment{Check for double spends and duplicate txs} 
            \If{$tx$ is  \textbf{valid} w.r.t to \av{ledger}} \av{ledger}.append($tx$) \label{code:sanitizeLedger}
            \EndIf
        \EndFor
    \EndFor    
\EndFor
\State \Return \av{ledger}
\EndProcedure
% \\
% \Procedure{GetLeader}{$\ell$} %\colorcomment{proposer block at level $\ell$ with most votes}
% \State $votes \gets \phi$ \colorcomment{Stores votes from all $m$ voter trees at level $\ell$}
% \For{$i$ in $\gets\;1\;to\;m$} 
% \State  $votes[i] \gets \textsc{GetVotes}(i, \ell)$ 
% % \State $vtMCs[i] = vtTree[i].$LongestChain()
% \EndFor
% \Return LeaderConfPolicy($votes$)\colorcomment{Refer \ref{}}
% \EndProcedure
\vspace{1mm}
\State \maincolorcomment{Return ordered list of confirmed transactions}
\Procedure{GetOrderedConfirmedTxs()}{} \label{code:slowConf}
   \State $\texttt{L} \gets \phi$          \colorcomment{Ordered list of leader blocks}
    \For{$\ell \gets 1 \;  to \; prpTree.$maxLevel}  
        \State $votes \gets \phi$ \colorcomment{Stores votes from all $m$ voter trees on level $\ell$}
        \For{$i$ in $\gets\;1\;to\;m$} 
        \State  $votesNDepth[i] \gets \textsc{GetVotes}(i, \ell)$ 
        % \State $vtMCs[i] = vtTree[i].$LongestChain()
        \EndFor
        % \State \textbf{bool} $a \gets $
        \If{IsLeaderConfirmed($votesNDepth$)}
        \State \maincolorcomment{Proposer block with maximum votes on level $\ell$}\label{code:appendLeader}
        \State $\texttt{L}[\ell] \gets$ {GetLeader}$(votesNDepth)$        
        \Else $\;$ \textbf{break}
        \EndIf
    \EndFor
    \Return \textsc{BuildLedger}(\texttt{L}) \label{code:slowBuildLedger}
    \EndProcedure

\end{algorithmic}
}
\end{algorithm}


==> Prism Systems Paper (CCS)/related.tex <==
\section{Related Work }
\label{sec:related}
There are broadly three different approaches to scale the performance of blockchains. First, \textit{on-chain scaling} aims to design consensus protocols with inherently high throughput and low  latency. Protocols such as Bitcoin-NG~\cite{bitcoin-ng}, GHOST~\cite{ghost}, Algorand~\cite{algorand}, OHIE~\cite{ohie} are examples of this approach. 
Second, in \textit{off-chain scaling}, users establish cryptographically-locked agreements called ``payment channels''~\cite{payment-channel} and send most of the transactions off-chain on those channels. 
Lightning~\cite{lightning} and Eltoo~\cite{decker2018eltoo} are examples of this approach. 
Third, \textit{sharding} approaches conceptually maintain multiple ``slow'' blockchains that achieve high performance in aggregate. Omniledger~\cite{kokoris2018omniledger}, Ethereum 2.0~\cite{buterin2016ethereum}, and Monoxide~\cite{monoxide} are examples of this approach. 
These three approaches are orthogonal and can be combined to aggregate their individual performance gains. 
% We also point out that off-chain techniques and sharding are relatively new ideas, and they have not been tested out in the wild like on-chain transactions. 

Since \newprism is an on-chain scaling solution, we compare it with other on-chain solutions. 
We explicitly exclude protocols with different trust and security assumptions, like   Tendermint~\cite{kwon2014tendermint},  HotStuff~\cite{yin2019hotstuff}, HoneyBadgerBFT~\cite{miller2016honey}, SBFT~\cite{gueta1804sbft}, Stellar~\cite{stellarsystem}, and Ripple\cite{cachin2017blockchain}, which require clients to pre-configure a set of validators who are responsible for executing the consensus protocol. 
% \gf{May be worth specifying the sense in  which we mean trusted--these protocols all tolerate byzantine behavior, so validators are not trusted in the usual sense}
These protocols target ``permissioned'' settings, and they generally scale to significantly fewer validator nodes than the above-mentioned permisionless protocols.
%;  hence we don't directly compared them with \prism.

%\ly{Apart from the permissionless blockchain protocols mentioned above, another class of protocols target the ``permissioned'' settings where the set of nodes participating in the consensus is always fixed. Protocols such as Tendermint~\cite{kwon2014tendermint},  HotStuff~\cite{yin2019hotstuff}, HoneyBadgerBFT~\cite{miller2016honey}, SBFT~\cite{gueta1804sbft} etc fall into this category. We point out that those protocols target different applications and they scale to significantly to a fewer number of nodes than the above mentioned permisionless protocols,  hence we don't directly compared them with \prism.}
%Stellar~\cite{stellarsystem} and Ripple\cite{cachin2017blockchain}, which require clients to pre-configure a set of trusted nodes..


% Those protocols target goals different from a public blockchain like \prism.}
Among protocols with similar security assumptions to ours,  Bitcoin-NG~\cite{bitcoin-ng}  mines blocks  at a low rate similar to the longest chain protocol. In addition, each block's miner continuously adds transactions to the ledger until the next block is mined. This utilizes the capacity of the network between the infrequent mining events, thereby improving throughput, but latency remains the same as that of the longest-chain protocol. Furthermore,  an adversary that adaptively corrupts miners can reduce its throughput to that of the longest chain protocol by censoring the addition of transactions~\cite{parallel}. \newprism adopts the idea of decoupling the addition of transactions from the election into the main chain but avoids this adaptive attack. We compare to \bng in \S\ref{sec:eval-performance}.
%We were not able to find an implementation of Bitcoin-NG for use in our experiments.
%\ma{isn't it actually implemented in some projects? be careful about this one; there are 3 cornel profs on pc, and they will know about bitcoin-ng and could talk to Gun Sirer too}
%\ly{bitcoin-ng is implemented (see https://blog.aeternity.com/introduction-to-æternitys-bitcoin-ng-implementation-331d0a1393b4).}

DAG-based solutions like GHOST~\cite{ghost}, Inclusive~\cite{inclusive}, and Conflux~\cite{conflux} were designed to operate at high mining rates, and their blocks form a directed acyclic graph (DAG). 
However, these protocols were later shown to be insecure because they don't guarantee liveness, i.e. the ledger stops growing under certain balancing attacks \cite{ghost_attack}. Spectre\cite{spectre} and Phantom \cite{phantom} protocols were built along the ideas in GHOST and Inclusive to defend against the balancing attack, however, they don't provide any formal guarantees. Also, Spectre doesn't give a total ordering and
Phantom has a liveness attack \cite{conflux}.
To the best of our knowledge, the GHOST, Inclusive, Spectre and Phantom protocols have no publicly available implementation, and hence we were not able to compare these protocols with \newprism in our performance evaluation. 

\newprism maintains the same blockchain structure as \prism: a DAG with many parallel chains, and a clear separation of blocks into different types with different functionalities (Figure \ref{fig:prism}). 
OHIE~\cite{ohie} and Parallel Chains~\cite{parallel} build on these lessons by running many slow, secure longest chains in parallel, which gives high aggregate throughput at the same latency as the longest-chain protocol. To our knowledge, Parallel Chains has not been implemented. 
% In OHIE's latest implementation~\cite{ohiecode}, clients do not maintain the unspent transaction output (UTXO) state of the blockchain and  transactions are signed messages without any context, so it is hard to compare with OHIE in our experiments, where all nodes maintain the full UTXO state.
% \gf{This seems a little too implicit. How about something like this? ``
In OHIE's latest implementation~\cite{ohiecode}, transactions are placeholder signed messages that do not depend on prior transactions; because of this, clients do not need to maintain the unspent transaction output (UTXO) state of the blockchain. 
This makes comparison with \cite{ohiecode} difficult because in practice, we observed that transaction processing (including UTXO state management) is a major computational bottleneck for high-throughput systems (see \S\ref{sec:eval}).

Algorand~\cite{algorand} takes a different approach by adopting a proof of stake consensus protocol and tuning various parameters to maximize the performance. We compare to Algorand in Figure~\ref{fig:compare} and in \S\ref{sec:eval-performance}. Importantly, none of the above protocols simultaneously achieve both high throughput and low latency. 
Their reported throughputs are all lower than \newprism's, and their latencies are all higher than \newprism's, except for Algorand which has a lower latency.



%%\ma{Should we mention Avalanche?}
%%\vb{Yes. They also claim high throughput and low latency. Currently their protocol is not fully specified in the paper and no implementation available} \ly{one available with only the consensus layer}

%%\ly{TODO: talk about stellar, read algorand's description}

%\ma{One general comment is give credit (generously) if there's an idea in related work that inspired something in prism.}
%\vb{We are inspired by all the DAG approaches. We took the idea of a) changing the main chain rule from GHOST, b) `referencing` blocks from Inclusive, and c) ledger sanitization  from Conflux.}

==> Prism Systems Paper (CCS)/reviews.tex <==
\clearpage

\section{Prior Reviews and Revisions}

\begin{table}[htbp]
	\centering
	\caption{Scores}
	\begin{tabular}{ r | c | c } 
	 \hline
	 Reviewer & Merit & Expertise \\ [0.5ex] 
	 \hline\hline
	 Reviewer A & 3 (weak accept) & 2 \\
	 Reviewer B & 3 (weak accept)  & 2 \\
	 Reviewer C & 1 (reject) & 2 \\
	 Reviewer D & 3 (weak accept) & 3 \\
	 Reviewer E & 2 (weak reject) & 2 \\
	 \hline
	\end{tabular}
	\label{table:scores}
\end{table}

The paper was submitted to NSDI 20 Fall deadline. The scores are in Table~\ref{table:scores}. The major revisions to address the comments are:

\begin{itemize}
    \item Implemented \bng using our \prism codebase, measured its performance and added to the evaluation section (Fig~\ref{fig:compare} and \S\ref{sec:eval-performance}).
    \item Added a discussion of the spamming problem and proposed a solution. Added an experiment to demonstrate the effectiveness of the solution (\S\ref{sec:spamming-eval})
    \item Added a discussion about Spectre and Phantom, two protocols that focus on improving blockchain throughput (\S\ref{sec:related}).
    \item Added a discussion about BFT-based protocol like HotStuff and HoneyBadgerBFT (\S\ref{sec:related}).
    \item Clarified that Prism has high CPU efficiency, and does not inherently require powerful machines (\S\ref{sec:eval-resource}).
\end{itemize}

\subsection{Review A}

Merit: 3 (weak accept), Expertise: 2.

\noindent{\bf Paper Summary:}
The authors propose to evaluate in practice a recently proposed
theoretical blockchain protocol (Prism) that would allow the scaling
of Bitcoin's performance while maintaining security guarantees. The
protocol relies on the use of three types of blocks to decouple
throughput from voting for a leader. The authors evaluate their
implementation of the protocol in Rust in a distributed setting. They
demonstrate that a network of 100 instances running on Amazon EC2
large machines can achieve 75,000 tps regardless of the chosen
adversarial ratio, and the latency is below 1 minute in most of the
cases. The authors also demonstrate via experiments that the system is
robust to a variety of known attacks, and that it's comparable or
better than Algorand, another well-studied consensus protocol for
blockchains.

\noindent{\bf Comments for Author:}\\
Pros:\\
- simple yet novel and impressive design\\
- great framework to evaluate PoW-based protocols

\noindent Cons:\\
- questionable practical use of PoW-based protocol with high resource requirements for users

\rp{We point out that \prism does not inherently require powerful machines.  Our implementation attains a throughput of over 70,000 tps on a machine with 8 cores, 16 GB RAM, and 400 GB of SSD, specs that are common today even on laptops for \$2-3K. Of course, our system can be configured for lower throughput to further reduce resource requirements. As Figures~\ref{fig:bw} and~\ref{fig:cpu} show, Prism's CPU and bandwidth requirements scale linearly with throughput.  The main point, as discussed in \S\ref{sec:eval-resource}, is that our \prism implementation does not waste resources: it has very high CPU efficiency, and reasonable bandwidth efficiency ($\sim$50\%), which we believe can be further improved with straightforward optimizations. We added more explanation on this in \S\ref{sec:eval-resource}.}

- protocol is intuitive to comprehend, but it is not intuitive to understand all of its security implications

\rp{The protocol's security was formally analyzed in the Prism theory paper~\cite{prism-theory}. We have added a short remark on the security model and referenced the theory paper in \S\ref{sec:overview}. We also added a discussion of spamming attacks that were not analyzed in the theory paper and demonstrated the effectiveness of a simple solution.}


My suggestions:

- explain if there is a practical need for something in-between the permissionless cheap-to-join PoW-based consensus like Bitcoin and expensive-to-join BFT-based consensus like Libra

\rp{We explain in \S\ref{sec:related} that BFT-based consensus protocols target very different applications and have their own limitations, such as being unable to scale to many nodes. Also, as explained in \S\ref{sec:eval-resource}, \prism is not inherently expensive to join. It has high CPU efficiency and its parameters can be tuned to operate at a lower throughput (at reduced cost) if the application requires. 
%Also, the throughput of \prism is required for applications like large scale payments.
}

- discuss wide threat model more thoroughly and provide intuition for why the protocol is robust to those attacks which were not included in experiments. For example, variations of the GoldFinger attacks.

\rp{We would like to point out that \prism shares many security properties with the longest chain protocol, and would like to refer the reviewer to~\cite{prism-theory} and the literature on the security of Bitcoin~\cite{securityofpow}. The simplest version of the GoldFinger attack is when the adversary controls $>51\%$, and in this case both \prism and the longest chain (Bitcoin) protocol are not secure.}

I liked that the authors of the paper create a security/throughput evaluation framework and apply it to both their protocol and Bitcoin. This alone is a valuable contribution to the research area, and also makes comparing Prism to Bitcoin much easier.

The design of the overall system is very comprehensible based on the paper, despite the introduction of several new sub-blocks primitives. However, after reading the paper I didn't have confidence that it's as robust as Bitcoin, due to the increased complexity.

I also like that the authors  propose non-trivial performance optimizations (asynchronous updates, parallel transactions, block pruning, etc) to make the system more practical.

It is not clear to me what is the rationale behind building the system on top of this protocol (although the theoretical results are very interesting!). It seems to me that to realize the full performance of the system it should be run on expensive hardware and with an extremely fast and reliable internet connection.  In this case, is PoW necessary? 
I wish the authors explained in the discussion why in this setting PoW is better than HotStuff (BFT protocol based on leadership used in Libra). It is clear why this is the case in Bitcoin, where both performing validation and mining blocks is permissionless (Bitcoin's original whitepaper even mentions 1 CPU = 1 vote rationale, although we know that mining works differently today), but not in your context.
I guess there is a niche for high-performance PoW-based system, but this is not obvious. 

\rp{It is true that the benefits of \prism compared to other protocols are most apparent on high-end hardware with reliable network connections. 
However, (a) \prism has good performance even on lower-end hardware, and (b) PoW can be useful even if we assume miners have high-end hardware. 
On  lower-end hardware, Figure~\ref{fig:cpu} illustrates that even if clients have only two cores at their disposal (which  is a very modest requirement), they can still get about $30,000$ tps, which is still an order of magnitude more throughput than Algorand, several orders of magnitude more than Bitcoin, and comparable to \bng.
Therefore the requirements to observe good performance with  \prism are  well within reach for most modern computers. 
Even if we assume that miners should have high-end hardware, the most performant BFT-based protocols have been shown to scale to up to tens or hundreds of nodes \cite{yin2019hotstuff,ibm}, and  they typically require knowledge of participants (i.e.,  are designed for permissioned settings). 
PoW protocols in contrast are most useful in settings where participants are not known \emph{a priori} and/or if the goal is to scale to thousands or more  validators.  
}
% More generally, \prism exhibits benefits even on lower-end hardware; the point is that \prism is designed to maximally utilize whatever hardware and network it is running on. However, when run on low-end hardware, the bottleneck ends up being the hardware.}

3. The Longest Chain Protocol (Section 3)

It would be more accurate to call that ``heaviest chain'': the chain which has the biggest amount of ``work''. It is possible that longer chain has less work because of the difficulty adjustments in Bitcoin's PoW. I guess you may choose to still use ``the longest chain'', but please clarify that you mean the biggest amount of work.

\rp{Correct. We use the term longest chain for simplicity and since it is common in the literature, but we added a footnote on this point in \S\ref{sec:background}}.

\subsection{Review B}

Merit: 3 (weak accept), Expertise: 2.

\noindent{\bf Paper Summary:}
The paper presents Prism, a blockchain implementation that achieves a high throughput of over 70,000 transactions per second and confirmation latency of tens of seconds on networks. Prism was evaluated on a network of 1000 EC2 Virtual Machines.

\noindent{\bf Comments for Author:}
The paper was interesting.  It demonstrates good tput and latency under attack. However there were several issues that need to be addressed in both the writing, design, and evaluation.

First, an issue was that there was not conclusion which is often a red flag.  For instance, the paper was rushed last minute and conclusion removed or it was a resubmit from a separate conference with different formatting requirements.  Neither one is a deal breaker, but a red flag about proofreading at the very least.

\rp{The paper was not rushed. In the previous submisssion we decided  to  use the space for a longer discussion on ideas for extensions (e.g., light clients, bootstrapping, etc.). In this version, we have added a conclusion section and summarized the discussion on future work  in this section.}

Second, spamming where miners do not validate transactions seems dangerous and raises practical concerns as described in the paper.  The paper described an interesting approach to reduce the window of vulnerability to this attack. However, spamming was not evaluated.

\rp{We have added a discussion of spamming and how to mitigate it in  \S\ref{sec:spamming-design}, and we evaluate it experimentally in \S\ref{sec:spamming-eval}. Our results show that it reduces spamming by more than 80\% while only adding less than 5 seconds to the confirmation latency.}

Third, the evaluation did not actual mine.  This is cited as practice in other papers, but it seems to throw off the evaluation without any actual proof of work.

\rp{As mentioned in the text, the model of proof-of-work mining as a Poisson process is precise. So we are able to simulate the mining process with great accuracy using exponential-distributed random delays. This is a standard practice in evaluations of PoW-based blockchain protocols (see \cite{conflux,ohie}).}

Finally, this is becoming more of a crowded space where many papers are attempting to increase the tput rate and commit latency.  As a result, it is difficult to have significant and unique contribution.  This paper is interesting with good contribution. However, some of the issues discussed need to be addressed to improve the paper more.

\rp{We have given a comprehensive comparison with other related works in \S\ref{sec:related}. We have also demonstrated that \prism has the highest throughput among all the protocols out there and is a close second in terms of latency.}

\subsection{Review C}

Merit: 1 (reject), Expertise: 2.

\noindent{\bf Paper Summary:}
The paper describes Prism, which is a high throughput blockchain protocol that is documents in an upcoming CCS paper, and provides performance evaluation on Prism.

\noindent{\bf Comments for Author:}
This paper reads not like a detailed systems paper, but a detailed white paper advocating for the use of a particular technology, in this case, Prism.  There are questions of fit and scope for NSDI, as well as issues of anonymity.

\rp{We respectfully disagree with characterizing our paper as a ``white paper''. We set out to implement and evaluate Prism precisely because we felt that despite promising theoretical results, it is difficult to assess the real-world performance of such a complex protocol based only on theory. Our paper provides a  systematic evaluation the protocol in a practical setting, compares it to state-of-the-art baselines, and addresses practical concerns such as spamming.}

First, I find this paper difficult to parse as a systems paper. Much of the detailed operations of the protocol is not in this paper, since the protocol itself is described in detail in the CCS 2019 paper (by presumably the same authors as this paper). The high level design of the protocol is described as is, with little justification or explanation of why particular choices were made. The only nugget I could tease out is that Prism is fast because it decouples multiple properties that used to be accomplished using the same blocks on the traditional blockchain architectures.  The fact that many details are in a separate paper makes this a frustrating paper to read.

\rp{We have attempted to provide an overview of the main ideas behind the Prism protocol by contrasting it with the longest chain protocol in Sections \ref{sec:background} and \ref{sec:overview}. In particular, Section \ref{sec:prism-latency} explains how Prism overcomes the latency limitation of the longest chain protocol using voter chains, and Section~\ref{sec:thruput} discusses how it decouples throughput from security using transaction blocks. Also, at the risk of some overlap with the theory paper, we included a detailed design in \S\ref{sec:design} to make this paper self-contained to the extent possible. The main aspect that is in a separate paper is the security analysis of the protocol.} 


Much of what makes a systems paper useful is missing here. Outside of the high level idea of separation of concerns, there's little explanation of why the system is designed this way, and what direct implications there are on performance. Instead, there are LOTS of protocol details describing both normal and corner cases of operation.  Some of the performance optimizations are discussed, but not justified beyond differentiation over BTC, and details of implementations vs design are not clearly identified.  One gets the impression that there could be a much more systemsy version of this paper if 6.2 was greatly expanded to much more fine grain discussion and comparison of alternatives.

\rp{As mentioned above, we discuss design details for completeness, but provide intuition for the main protocol design decisions in Sections~\ref{sec:background} and~\ref{sec:overview}. Regarding our performance optimizations, it is not difficult to see that they are essential for high performance. For example, without the scorboarding technique, we cannot process transactions in parallel and our throughput would be limited to the single-core performance in Figure \ref{fig:cpu}.}

There is plenty of evaluation, but again from a microcosm of prism microbenchmarks. Given the number of alternative faster txn blockchain designs in the last few years, why are there no performance comparisons against them, e.g. bitcoin-ng?

\rp{We implemented \bng by modifying our \prism codebase and measured its performance. Results are in Fig~\ref{fig:compare}. Also, we would like to point out that most of these designs do not have a publicly available implementation.}

I think there are potentially interesting lessons to be learned from this protocol and its implementation, but they are not available in a paper written in the current style.

\subsection{Review D}

Merit: 3 (weak accept), Expertise: 3.

\noindent{\bf Paper Summary:}
The paper presents the implementation and evaluation of Prism, an on-chain scaling solution for Bitcoin that enables scaling the number of transactions on Bitcoin by 10000x while keeping transaction confirmation latency within 13-120s. The basic Prism protocol and its security properties has already been published. This paper is more a validation of the Prism protocol through careful implementation and experimentation at scale (up to 1000 VMs on AWS).

\noindent{\bf Comments for Author:}
The paper is quite dense even though the authors spend the first several pages describing the Prism protocol. I basically had to read the original Prism paper to get a full understanding of the protocol and it is pretty neat: instead of using the longest chain, Prism uses a DAG and by separating the blocks into transaction blocks, proposer blocks and voter blocks, they decouple security from throughput/latency. Specifically, by having a large number of voter blocks (m > 1000), they can confirm transactions at low latency after depth 2 with extremely low probability of reversal unlike Bitcoin that needs a depth of 24 or more (10x latency reduction though each voter chain can operate at slow/similar speed as Bitcoin). Second, by allowing fast mining of transaction blocks, they can arbitrarily increase the throughput of the system, again without impacting security. 

One issue with the protocol compared to Bitcoin is that nodes cannot choose transactions (transactions have to be selected randomly for achieving the security properties of the protocol.) In current Bitcoin, there is the notion of transaction fees and miners typically prioritise transactions with higher fees, which in turn provides these transactions with lower latency. This feature/incentive is missing in Prism but perhaps given the overall low latency, lack of this incentive is perhaps not a major issue.

\rp{We would like to point out that in \bitcoin, transaction fees only provide limited benefits for improving the latency for a specific transaction. Even if a transaction is immediately mined into the next block, the confirmation latency is still significantly higher than \prism for the same security property. Also, \prism provides much higher throughput than \bitcoin, therefore we believe it's unlikely to have a backlog of unmined transactions.}

However, the protocol itself has already been published, so the contribution of this paper is only on the design and implementation of the protocol.   Here, the authors claim that they solve many challenging aspects to optimising the implementation but  this is not really convincing. Many of the optimisations are standard techniques and/or possible as a the direct result of the protocol design (e.g., asynchronous ledger updates is possible in Prism but hard to do/not necessary for Bitcoin; transactions need not be broadcast when received etc.).  To enable parallel transaction execution, the authors borrow the scoreboarding technique (basically ensure no conflict in transactions during execution) and a functional design such that state is passed around. Still, I can see value to validating a complex protocol such as Prism through implementation and evaluation, hence my overall rating.

\rp{As we have clarified in the introduction section, we believe that the system implementation and its evaluation represent significant contributions. (a) It validates Prism's theoretical analysis in a practical setting. Due to the complexity of the Prism protocol, it was not clear that such protocol can be implemented as a real system and scale both throughput and latency without affecting security. (b) We discovered that through careful optimizations, CPU is not a performance bottleneck. Instead, I/O and database is the main bottleneck. We hope this motivates future research in blockchain-specific database design. (c) We evaluate Prism under active attacks in a real implementation. Such evaluation can not be performed in a realistic way without the system implementation due to the complex nature of a networked system. Our evaluations shows that Prism is robust to those attacks. Additionally, in this submission, we discuss a spamming attack and provide a simple solution that mitigates it, reducing spam traffic by 80\% with little impact on performance.}

Also, the authors claim that the latency of their system is similar to Algorand but this seems like a stretch to me. Algorand provides latency as low as 2s while the lowest latency of Prism is 13s (at beta=20\%). If one is using these systems for transactions, one can live with 2s latency while 13s seems prohibitive, so I would not claim that the latencies are similar!

\rp{We have revised the wording to avoid saying our latency is similar to Algorand. For a $\beta=20$\% adversary, Algorand's latency is 2.35s, and Prism's latency is 12.5s.}
%However, please note that Algorand can only operate at $\beta<33\%$, and Prism's latency would be lower than for higher $\beta$,  } 



Other comments:

What is the value of m parameter for Prism used in your experiments?

\rp{$m=1000$ is used across the paper. We added a note in \S\ref{sec:eval-performance}. Also, we report all parameters in Appendix B.}

What are the number of duplicate transactions and how does it vary in your experiments? What happens to this and other overhead when users (attackers) submit multiple small/valid transactions by connecting to hundreds of nodes?  Note that this is different from spamming as users may be incentivized to submit to multiple nodes to reduce transaction latency/improve reliability, so I can see a user who connects to hundred or more nodes to submit their transaction and if multiple users do the same, this can result in lots of wasted work/duplicate transaction? Sure, the system will still not double-spend/be secure but what happens to throughput/latency of the system.

\rp{Duplicate transactions submitted to multiple miners have the same impact on performance as conflicting transactions in spamming attacks. We discuss these attacks and propose a simple mitigation in \S\ref{sec:spamming-design} and evaluate it in \S\ref{sec:spamming-eval}.}

Typos in discussion point 4: trasnaction, s->As

missing related work such as spectre and phantom that target the same problem.

\rp{Fixed both.}

\subsection{Review E}

Merit: 2 (weak reject), Expertise: 2.

\noindent{\bf Paper Summary:}
The proposed PRISM scheme is a scaling blockchains with an on-scaling solution, by decoupling the addition of transactions from election into the main chain. It delivers low latency and high throughput, compared to Bitcoin's and other PoW/PoS consensus protocols.

\noindent{\bf Comments for Author:}
Prims splits blocks into three types: proposer blocks, transaction blocks, and voter blocks; The goal is to decouple the roles of the blocks in the chain (usually there is only one block type which carries all those functionalities - e.g. Bitcoin)

Proposer block: each proposer block contains a list of references to transaction blocks and a single reference to a parent proposer block. Miners mine (longest) chain of proposer blocks.

Voter block: each voter blocks casts a vote for a proposer block. A voter block can only reference one proposer block; a voter block is valid if it is part of the longest chain. The longest chain protocol secures the voter blockchain security (as well as the overall system). The adversary needs more than 50\% hashing power to gain advantage and cast voting blocks at will.

Since there are many voter chains, each vote does not need to get sufficiently deep in the chain for confirmation (and thus increase latency). This improves the latency of the system considerably when compared with, e.g., Bitcoins (2-deep instead of 24-deep for same reversal probability).

Increasing the number of voter chains improves security (and decreases the size of k-deep for the same degree of security)

Leader block: is the one with the highest number of votes (at a certain level). All the leader blocks provide a unique ordering of the transaction blocks. 

Latency improved because Prism decouples the blocks into voter and transaction + proposed blocks. The voter blocks are mined in n chains and define the consensus of the protocol. The proposed blocks (referencing transaction blocks) with more votes cast are the consensual blocks that are part of the blockchain. Latency improved because the consensus of the voter chains do not require leader blocks to be deep in the tree to be secure against reversal attacks (since there are many parallel chains).

Throughout improved, again, due to separation of concerns in the different block types. Since the mining of transaction blocks is not part of the security assumptions of the system (as in Bitcoin), the transactions can be processed at node utilization (i.e. limited by miner's CPU and bandwidth). This achieves near-optimal throughput.

Questions/comments

5.5 (page 5) Cryptographic sortition needs more background. It is mentioned throughout the paper but without going deeper in the details (does it use VRFs? zksnars?, etc). In addition, it is important to discuss what are the security assumptions of this and how does it affect the overall system assumptions and security? etc..)

\rp{Sortition does not use VRFs or SNARKs. Please see the detailed explanation in \S\ref{sec:mining}.}

5.5 (page 5) Miners simultaneous mine one voter block for each of the m voter chains. For security, the system requires many voter chains. How does a large m affect latency?

\rp{The confirmation latency actually decreases as $m$ increase, as discussed in \S\ref{sec:prism-latency}. Please note that the voter blocks actually contribute a small fraction of the bandwidth usage compared to the transactions. For example, as shown in Table~\ref{table:bw-profiling}, in our implementation with $m=1000$, the voter blocks represent only 0.21\% of the bandwidth (compared to over 50\% for transactions).}

Each client must keep the state of the blockchain. Splitting the transaction blocks and into different types and keeping m (relatively large) number of voter blockchains in memory might become expensive for clients. It would be good if the authors would present how maintaining all that state locally would affect miner's performance and resources spent. [this is actually addressed in 7.3. Resource Utilization section]

\rp{We keep all the state in RocksDB on SSD instead of the memory, so that the client is crash-tolerant. As pointed out by the reviewer, \S\ref{sec:eval-resource} provides a detailed breakdown of resource consumption.}

Miners do not validate transactions before including them to proposed blocks. This opens up (I believe) a lot of surface for denial of service attacks and targeted attacks to miners. What would be the cost of adding transaction validation to the mining pipeline?

\rp{We would like to point out that miners do perform basic validation like signature checks and proof-of-work validation. Such checks would prevent the most naive ways of DDoS. However, as explained in \S\ref{sec:spamming-eval}, not checking transactions for double spends during mining could indeed introduce the possibility of spamming. Our mitigation strategies described in \S\ref{sec:spamming-design} protect against such spamming attacks and are effective as shown in \S\ref{sec:spamming-eval}.}

6. (Implementation) ``We have implemented a Prism client in about 10,000 lines of Rust code'' where is it? it'd be great to take a look at the code.

\rp{The code is available at \cite{prismcode}.}


==> Prism Systems Paper (CCS)/reviews2.tex <==
\clearpage

\section{Prior Reviews and Revisions}

\begin{table}[htbp]
	\centering
	\caption{Scores}
	\begin{tabular}{ r | c | c } 
	 \hline
	 Reviewer & Merit & Expertise \\ [0.5ex] 
	 \hline\hline
	 Reviewer A & 2 (weak reject) & 3 \\
	 Reviewer B & 2 (weak reject) & 4 \\
	 Reviewer C & 2 (weak reject) & 3 \\
	 \hline
	\end{tabular}
	\label{table:scores}
\end{table}

An earlier version of the paper was submitted to CCS 2020 Winter deadline. The present version is a substantially revised paper with significant new content. Specifically, in this major revision, we:

\begin{itemize}
    \item Propose a new confirmation rule for Prism and prove its security. This new rule is much more practical than the one in \cite{prism-theory} and yields better confirmation latency (details in \S1 and \S\ref{sec:scaling}). Meanwhile, just as the one in \cite{prism-theory}, this new rule is provably secure. %The new rule replaces the heuristic-based rule in the previous version of the paper. 
    We believe this addition significantly boosts the technical contribution: a new confirmation rule that makes \prism practical and a new blockchain security proof methodology (co-design of the confirmation rule of the protocol jointly with an explicit identification of the worst-case attack). (The previous submitted version used a heuristic confirmation rule in our implementation which did not have a formal security guarantee.)
    \item For this revision, we have redone almost all the experiments to evaluate the \prism protocol our new confirmation.  The performance  (throughput/latency) is improved by a factor of 10,000 compared to Bitcoin and the only limiting factor is physical limits (disk I/O and network limits). 
  
    \item We have cut back didactic material   about the longest chain protocol and the Prism protocol to provide enough space to formally introduce the new confirmation rule, the system design, and the experimental results.
\end{itemize}

We believe that this paper is justified as a new submission, with over 40\% of the content being new. However, in the interest of transparency, we include the previous review (scores are in Table~\ref{table:scores}) and our response.

\subsection{Review A}

\noindent{\bf Paper Summary:}
This paper describes an implementation of a Bitcoin-like system on top of the Prism blockchain protocol, which is reported to have excellent performance. The paper evaluates the performance of the implementation, including how performance is affected by various attacks that can be mounted against the system.

\noindent{\bf Strengths:}
The performance of the implemented system is impressive, and implementers of blockchain systems may find the details of the implementation interesting.

The paper is well written and pleasant to read.

\noindent{\bf Weaknesses:}
Much of the text of the paper is not novel, but is rather a recap of the previously published work on Prism. New content only starts around page 6, though the background up to that point is certainly useful to a reader who hasn't seen the previous publication.

\rp{The paper has been heavily revised. We try to provide a succinct background of the longest chain protocol and the Prism protocol in this new paper in page 1 -- 3. Page 4 -- 7 present our new practical confirmation rule that is provably fast and secure. Page 8 -- 10 provides the detailed design decisions which is useful as a reference by practitioners who design real-world cryptocurrency systems. Page 11 -- 13 is our extensive evaluation of Prism, which validates the theoretical results.}

This doesn't seem like a standalone paper to me; it strengthens the evidence that Prism is a good protocol, but the level of technical innovation is low. There are many implementation details in the paper, but we don't know which implementation choices have novelty or are even critical to the system's performance. Hence, the implementation design is not evaluated scientifically. The spamming defense seems like the most novel aspect of the system, but it's rather simple.

\rp{As mentioned earlier, this paper is now heavily revised. The new confirmation rule, the system implementation, and the large-scale evaluation are all new and innovative. Only page 1 -- 3 describes existing work which serves as a background for the paper. Also, we believe that all design techniques are innovative especially in the context of blockchain. No existing blockchain client can  support such a high throughput. Our implementation detail shows one way of designing a high-throughput system and its performance is extensively validated by our evaluation. As mentioned before, many unknowns exist around the Prism protocol if one only looks at \cite{prism-theory}, e.g. is it possible to turn the seemingly-complex protocol into a real-world system? Our paper answers these questions for the first time. In this sense, we believe the implementation and the evaluation are important contributions in themselves.}

\noindent{\bf Comments for author:}
I think the authors should take the content in this paper and use it to extend the previous Prism paper into a journal paper.

\rp{As mentioned before, this paper is now heavily revised with half of the content being new. We believe that with innovations in the theory (the new confirmation rule and its strong, provable security guarantees) and in the system (the first end-to-end system that achieves 80,000 tps and less than 1 minute of latency), this paper is fully justified as a standalone paper. }

\subsection{Review B}

\noindent{\bf Paper Summary:}
The paper presents an implementation and extensive experimental evaluation of Prism, a proof-of-work based blockchain that improves both the latency and the throughput of PoW cryptocurrencies. The original system design was described and analyzed at CCS 2019, and is in my opinion a very interesting and important contribution introducing and combining a number of nice ideas.

The main scope of the current paper is reporting on implementation challenges, evaluating the implementation, and comparing it with alternative approaches from the blockchain literature. Asides from the software engineering challenge of implementing the system, there are two main challenges that the implementation addresses: the bottleneck introduced by the traditional synchronous ledger update, and (2) the bottleneck introduced by the need to process too many transactions and compare them to the ledger. The paper also evaluates the effect of some additional attacks that intuitively slow-down Prism’s performance such as spamming (for which an idea is proposed to reduce it) and censorship.

\noindent{\bf Strengths:}
I am quite excited about the original ideas in Prism and I appreciate the effort invested in implementing, emulating, evaluating, and comparing the implementation with existing systems that claim state-of-the-art throughput and latency. I think the paper does a good job in documenting the challenges and discussing how they are tackled.

\noindent{\bf Weaknesses:}
I am worried that having a system implementing a design proposed last year in CSS is counterproductive and sets the wrong precedent for the conference. As expected and discussed above, there is a number of challenges that one needs to tackle when implementing the system, and the paper properly documents and resolves them (with the asterisk of asynchrony deviating from the analysis of \cite{prism-theory} as discussed above). Yet, I don’t see considerably novel ideas, so given \cite{prism-theory} the scientific advancement in terms of systems security research is in my opinion marginal for CCS.

\rp{We believe that the system implementation and evaluation is crucial in showing that Prism is practical, and in guiding practitioners to incorporate the algorithm in real-world systems. Also, in this major revision, we propose a new, more practical confirmation rule that is provably secure. We believe that this combination of algorithm innovation and system evaluation possesses significant value for a security conference.}

\noindent{\bf Comments for author:}
Regarding synchrony/asynchrony: The paper observes that the Prism protocol does not need to update the ledger in a synchronous manner. I am a bit skeptical about this statement. The original analysis of Prism assumes a synchronous model and so does the proof of security, as the authors discuss in the introduction. But running a system designed and analyzed over a synchronous environment in an asynchronous manny might be insecure. I did not see any argument that the system preserves its security in the asynchronous model. Does the analysis from \cite{prism-theory} extend directly to the asynchronous setting? Is there no issue with variable difficulty? How is it guaranteed that that miners executing Bitcoin-style readjustment in an asynchronous manner will not end up with different puzzle targets?

\rp{We would like to point out that ledger update does not affect the execution of the consensus protocol itself. That is, the thread updating the ledger monitors the \textit{output} of the consensus protocol (i.e. the blockchain state), but does not provide \textit{input} into the consensus. The reviewer is absolutely correct that Prism is designed for and analyzed under the synchronous setting. Indeed, our testbed runs on a synchronous network and everything related to updating the blockchain state (i.e. running the consensus protocol itself) is done synchronously. Although we don't dive into dynamically adjusting the mining difficulty in this paper, as long as the adjustment only depends on the blockchain state (as in the case of Bitcoin), it will work in Prism because nodes update the blockchain state synchronously.}

Regarding the parallel processing of transactions, I agree that using ideas from concurrency in hardware is indeed the way to go. I liked the parallel drawn between race conditions on a processor and race conditions when validating transactions.

The paper also proposes and evaluates experimentally approaches for countering spamming attacks that are introduced by the high degree of parallelization of the Prism design. The idea is relatively straight-forward, add a small time-jitter when processing transactions. This is validated and the reported experiments demonstrate a considerable reduction in the effect of spamming. A question that was unclear to me is whether or not this jitter needs to be readjusted depending on the actual latency of the network. Such a latency will not appear in the simulations, but when executed on a global scale, e.g., nodes over the Internet, it could be considerable and even variable.

\rp{The reviewer is totally correct that the jitter needs to be adjusted based on the real network latency. However, the reviewer may have missed the fact we indeed simulated the real Internet latency in our testbed. Actually, we added a 120ms one-way propagation delay between \textit{every} pair of nodes. This corresponds to the one-way latency from Tokyo to Paris. So we believe that our eval results of the spam mitigation already represents its real-world effectiveness.}

\noindent{\bf Required improvements:}
It would be useful to address the above comments.

\subsection{Review C}

\noindent{\bf Paper Summary:} This paper extends \cite{prism-theory} with mainly with measurement analysis. In general it's impolite to inflate academic papers (I was once reprimanded by a highly accomplished professor regarding this practice), instead it'd have been nicer to supplement the public archive version of \cite{prism-theory} with this discussion.

\rp{We would like to respectfully point out that even in its previous version, this paper was in no way intended as an inflation of an existing paper. The implementation, the evaluation, and the design details are all new. Although we used some pages to provide a gradual introduction into the longest chain protocol and Prism, we felt that such background was useful in making the paper more self-contained. That said, in this extensive revision, we have condensed the background section significantly assuming the audience to have sufficient background on blockchains.}

\noindent{\bf Strengths:}
The strengths of this paper are the implementation demo (Section 6) and measurements (section 7).

\noindent{\bf Weaknesses:}
Prism itself is bad, basically it has all the complexities of DAG (it's similar to \cite{ohie} but with even more indirect complexities), without several of the advantages (such as incentive compatibility in the sense that honest block are never orphaned, see for example eprint.iacr.org/2017/300 and eprint.iacr.org/2016/916). \rp{We would like to point out that although Prism is indeed more complex than the longest chain protocol, the design is based on the first principles. We believe that complexity itself is not a sin, only \textit{unjustified} complexity is. To that end, Prism is a very natural scaling of the longest chain protocol, achieved by first analyzing the roles of the blocks in the longest chain protocol and then scaling each one of them. Also, the extra complexity in the protocol does not impose significant overhead in terms of computational and network resource consumption. Our evaluation has proven this point.  In fact, understanding any practical bottlenecks and hurdles for achieving Prism's theoretical performance was precisely our motivation for building the system. Regarding incentive-compatibility: unlike what the reviewer implied, in Prism, honest transaction and proposer blocks are always included. } The introduction makes silly remarks about being "the first such protocol", and false claims about other works such as \cite{phantom} (just because one paper pointed out a particular issue (that was later improved doesn't mean that you may brag that it lacks proof of security). \rp{We believe our claims are factually correct. Still, we have eliminated all editorializing in this version.}

\noindent{\bf Comments for author:}
Suppose that you are required to design a reward scheme for Prism where the money is derived only from transaction fees (and not newly minted money), can you do it in a convincing way?

\rp{Incentives for consensus algorithms are a complicated topic. Indeed, four decades of BFT consensus algorithms have resulted in hundreds of publications but hardly any with incentive analysis. We respectfully submit that proposing incentive mechanisms is an altogether different research topic and outside the scope of this paper.} %   \ly{This response does not feel strong enough. What to do?}

You should add a brief note in the paper that because the protocols requires the unpredictable stochastic process for security (no a priori knowledge of block role) it requires PoW and doesn't work with PoStake or other kinds of resources, whereas there are other DAG protocols then work well with a resource other than PoW.

\rp{We politely point out that this is not true and refer the reviewer to a recent arxiv preprint (https://arxiv.org/abs/1910.02218v2) that could serve as the building block of \prism with PoS (proof of stake).} %\ly{could we cite some paper?}

Section 5.4 and 7.4: what about an analysis of liveness, i.e., under what conditions an honest transaction be included in the ledger, given the spam protection? \rp{Honest, non-conflicting transactions are always included. Spam protection only provides extra time for miners to see if other miners have already mined the same transaction.} More importantly, can you measure the complexity of maintaining the local ledger in Prism (for spam protection) versus the complexity in Bitcoin (if it's say 10000 times more complex that you should make clear that the range of the added complexity is in that ball park). \rp{Unlike what is implied by the reviewer,   the cost of maintaining the ledger in \prism is not inherently higher than in Bitcoin. Actually, we addressed this point in our evaluation when we discuss the CPU consumption of the system. In our real-world experience, 10,000 tps per CPU core (with all cryptographic checks enabled) is a very reasonable computation cost.}



==> Prism Systems Paper (CCS)/scaling.tex <==
\section{Background}
\label{sec:scaling}

\iffalse
Outline:
1. Why is it hard to scale the latency? Use the content of the current section 3. Use just the results from section 3. (“Mining rate controls everything”. Throughput is easier to scale. Latency is harder and that’s the challenge.)
2. Prism solved it, and how. (The first three paragraphs of current section 4.)
3. Limitation of Prism (NEW).
- Security proof has round-by-round model
- Finite horizon.
- The constants are very bad. (Demonstrate by some examples. Pick different Rmax and plot the latency.)
- Also, point out that the state of art back then was not the same as today so that we don’t beat up Prism too much. Things has improved much on the Bitcoin side.
\fi



Several recent blockchain proposals have succeeded in scaling the throughput of the longest chain, such as Bitcoin-NG \cite{bitcoin-ng}, GHOST \cite{ghost}, and Fruitchains \cite{fruitchains}. However, how to scale the latency has been a major challenge in blockchain research for years. \newprism borrows an idea from \prism~\cite{prism-theory}, a recent attempt to scale PoW consensus, by systematically decoupling the functions of the blocks in the longest chain protocol. Specifically, \newprism retains the mining and blockchain structure of \prism. In this section, we provide an overview of this idea, and explain why \prism does not deliver low latency in practice. 


\iffalse

\subsection{Limitation of Longest Chain Protocol}
\label{sec:limitation_LC}

The most basic blockchain consensus protocol is Nakamoto's longest chain protocol, used in many systems including \bitcoin and \ethereum. 
The longest chain protocol is simple: at any time, a node adopts the longest chain to its knowledge and attempts to mine a new block that extends this longest chain via solving a cryptographic puzzle; a block is confirmed when buried $k$-deep in the longest chain, i.e. the block is on the longest chain and a chain of $k-1$ blocks have been appended to it.
It is proven that as long as the adversary has less than $50\%$ hashing power, the longest chain has consistency and liveness properties~\cite{backbone,ren2019analysis,dembo2020everything}: blocks that are deep enough in the longest chain will remain in the longest chain with high probability, and honest miners will be able to enter a non-zero fraction of blocks into the longest chain.

However, the longest chain protocol has poor performance in both latency and throughput. For example, \bitcoin supports 3--7 transactions per second and can take hours to confirm a transaction with a high level of reliability~\cite{bitcoin}. A natural question is: {\em Can we improve the latency or throughput significantly by tuning parameters in the longest chain protocol?}

The longest chain protocol has two key parameters: the mining rate $\lambda$ (blocks per second), which can be tuned by adjusting the difficulty of the puzzle, and the block size $B$ (in number of transactions). Roughly speaking, the longest chain protocol with $k$-deep confirmation will have latency $k/\lambda$ seconds and throughput $\lambda B$ transactions per
second~(tps). Hence increasing $\lambda$ and $B$ can potentially reduce latency and increase throughput. However, these parameters are restricted by the security requirement. 

Let $\Delta$ be the network delay, i.e. the time it takes to broadcast a block to other nodes in the network. Empirical results show that increasing the block size would also increase the network delay $\Delta$ \cite{decker}. The relationship between $\Delta$ and $B$ can be captured by a simple model of the network delay: 
$$ \Delta = \frac{hB}{C} + D,$$
where $h$ is the average number of hops for a block to travel, $C$ is the communication bandwidth per link in transactions per second, and $D$ is the end-to-end propagation delay.   
Hence, the {\em utilization}, i.e. the throughput as a fraction of the communication bandwidth, is upper bounded by
$$ \frac{\lambda B}{C} < \frac{\lambda\Delta}{h}.$$
In the longest chain protocol, to be secure against an adversary with $\beta < 50\%$ of hash power, $\lambda\Delta$ should satisfy \cite{dembo2020everything}
$$\lambda\Delta<\frac{1-2\beta}{\beta(1-\beta)}.$$
%For example, to achieve security against an adversary with $\beta = 45\%$ of the total hashing power, one needs $f\Delta \approx 0.2$. With $h = 5$, this translates to a utilization of at most $4\%$. The above bound holds regardless of block size; the utilization of the longest chain protocol cannot exceed 4\% for $\beta = 45\%$ and $h=5$.
To not compromise on security, $\lambda\Delta$ must generally be kept much smaller than $1$. 
Hence, the security requirement of the longest chain protocol limits the throughput. Moreover, the latency normalized by the network delay $\Delta$ is given by $k/\lambda \Delta$, and therefore the security requirement also limits latency. 
\fi



\subsection{Prism and Decoupling the Longest Chain}
\label{sec:prism}

The selection of a main chain in a blockchain protocol can be viewed as electing a leader block among all the blocks at each level of the blocktree. In this light, the blocks in the longest chain protocol can be viewed as serving three distinct roles: they stand for election to be leaders;  they add transactions to the main chain; they vote for ancestor blocks through parent link relationships. The latency and throughput limitations of the longest chain protocol are due to the {\em coupling} of the roles carried by the blocks. \prism~\cite{prism-theory} proposes to remove these limitations by factorizing the blocks into {\em three types} of blocks: {\em proposer blocks}, {\em transaction blocks}, and {\em voter blocks} (Figure \ref{fig:prism}). Each block mined by a miner is randomly sortitioned into one of the three types of blocks, and if it is a voter block, it will be further  sortitioned into one of several voter chains. (Mining is described in more detail below.)

\begin{figure}
\begin{center}
\includegraphics[width=0.45\textwidth]{figures/Prism_main.pdf}
\end{center}
\caption{\small Factorizing the blocks into three types of blocks: proposer blocks, transaction blocks and voter blocks.}
\label{fig:prism}
\end{figure}

The \textit{proposer} blocktree anchors the blockchain. 
Each proposer block contains a list of reference links to \textit{transaction} blocks which contain transactions, as well as a single reference to a parent proposer block.
Honest nodes mine proposer blocks on the longest chain in the proposer tree, but the chain structure does \textit{not} determine the final confirmed sequence of proposer blocks.
We define the \emph{level} of a proposer block as its distance from the genesis proposer block, and the \emph{height} of the proposer tree as the maximum level that contains any proposer blocks.
To determine the ordering of proposer blocks (and thus transaction blocks and transactions), we elect one \textit{leader} proposer block from each level. The sequence of leader blocks up to the height of the proposer tree is called the  \textit{leader sequence}, and is determined by the \emph{voter} chains. 

%\gw{Voter tree (blocktree) or voter chain (blockchain)? Since unlike proposer tree, only voter longest chain will participate in voting.}

There are $m$ voter chains, where $m \gg 1$ is a fixed parameter chosen by the system designer. For example, we choose $m=1000$ in our experiments. New blocks are mined on each voter chain according to the longest chain rule. A voter block votes for a proposer block by including its hash, and the votes are cast such that each voter chain votes for one and only one proposer block at each level of the proposer tree. We consider a vote \textit{valid} if it is cast by a voter block on a longest voter chain. For each level in the proposer tree, we define the proposer block that receives the most valid votes as the \textit{leader block} (ties are broken by the hash of the proposer blocks). The sequence of the leader blocks decides a unique ordering of the transaction blocks, which forms the final ledger (ledger formation is explained in more detail below).

\smallskip \noindent
\textbf{Mining}.\label{sec:mining} In Prism, miners should not be able to choose \emph{a priori} which type of block they are mining; this is essential for the security of the scheme, since otherwise the adversary could concentrate its mining power on a subset of block trees and overpower the honest nodes.
\emph{Cryptographic sortition} is used to ensure that miners cannot choose which type of block they mine.
Nodes combine the contents of the transaction block, the proposer block, and the $m$ voter blocks (one for each voter chain) they are mining into a \emph{superblock} and perform proof-of-work mining on it.
We divide the range of a valid proof of work into $m+2$ sections, each corresponding to one type of block.
The concrete type \textbf{T} of a superblock is then decided by looking at which section its proof-of-work falls into.
Here, the proof-of-work value essentially serves as a random oracle
 that dictates the type of a mined block.
However, there is still one problem: once we know the concrete type \textbf{T} of a superblock, we want it to contain only the content of type \textbf{T} but not other types, otherwise we will waste bandwidth. As a solution, miners summarize the contents of the $m+2$ candidate blocks using a Merkle tree, and perform mining on the Merkle root instead of the plain hash of the combined content. When the concrete type \textbf{T} of the superblock is decided, the miner keeps only the content of type \textbf{T} and inserts a Merkle proof to show that it had committed to this particular content when the block was mined.

\smallskip \noindent
\textbf{Ledger Formation}.\label{sec:confirmation} In Prism, transaction blocks are mined at a high rate.
A key consequence is that transaction blocks mined concurrently may contain redundant or conflicting transactions.
If Prism were to discard blocks that contain inconsistent transactions, it would waste bandwidth because transactions that \emph{are} consistent are also discarded.
To prevent this, Prism separates the process of confirming blocks and forming a ledger.
The key observation is that given a confirmed leader sequence of proposer blocks, the ordering of transaction blocks is uniquely determined. This gives us a total ordering of transactions since the inception of the protocol, and enables us to determine the validity of each individual transaction by executing them following this ordering. For example, among transactions that try to spend the same coin, only the first is considered valid.

\smallskip \noindent
\textbf{Summary}. At a high level, Prism achieves high throughput by decoupling it from security: transactions are carried by separate transaction blocks and hence throughput can be increased by simply increasing the mining rate of transaction blocks, while the security stays the same because the mining rate of proposer blocks remains low. The throughput is only limited by the computing or communication bandwidth $C$ of each node, thus enabling a $100\%$ utilization.
For latency, the key idea is that even though it takes a long time to achieve low reversal probability of \textit{individual} votes (same as in \bitcoin), the collective opinion on leader blocks can converge much faster because there are many parallel voter chains. Next, we will discuss some nuances of this idea, and explain why Prism does not deliver low latency in practice.


\subsection{Limitations of Prism}
\label{sec:limitation_Prism}

%\ma{This section needs to be much more specific and clear about what is the problem with Prism's confirmation rule. We need to briefly explain what is a confirmation rule, what is Prism's rule (before this paper), and what is the problem with it. I would also discuss the confirmation rule before any limitations of the analysis. It seems these are different things -- we're improving some aspect of the protocol, and we're also providing a better analysis (relying on fewer assumptions).}

\noindent {\bf \prism's confirmation rule~\cite{prism-theory}}. The confirmation rule in a blockchain defines when nodes can consider a block to be part of the immutable ledger. For example, the longest chain protocol famously uses the $k$-deep confirmation rule. In \prism, the ledger is determined by the proposer leader blocks, so the confirmation rule needs to decide when the leader block of a proposer level is immutable.

The immutability of a leader block depends on the immutability of the votes, which in turn depends on how deep they appear in the respective voter chains, or, their \textit{depths}. The key challenge is to consider the depths of all $m$ votes for a proposer level, such that we can confirm a leader block quickly, and the leader block will not change once confirmed (except for negligible probability). 

 For each proposer block at a level, \prism calculates a {\em confidence interval} for the total number of votes it will \textit{eventually} receive. When the confidence interval of any single proposer block is above that of all other blocks on the same level, it confirms the block. Bagaria et al.~\cite{prism-theory} prove a security theorem for this rule in a round-by-round synchronous model. We now explain the limitations of this confirmation rule regarding security and confirmation latency. 

\noindent {\bf Limitations of security guarantee}. In \cite{prism-theory}, the confidence interval of the number of votes a proposer block receives depends on a finite bound on the lifespan of the blockchain in rounds ($r_{\rm max}$). As $r_{max}$ increases, the probability of a successful attack increases in this analysis (via a union bound). Specifically, the exact expression of error probability is $r_{\rm max}^2 e^{-\frac{(1-2\beta)m}{16 \log{m}}}$. To compensate for the effect of $r_{\rm max}$, \cite{prism-theory} increases the number of voter chains ($m$) to keep the confirmation error probability low.
%The confirmation error probability in \cite{prism-theory} is kept low by choosing $m$ large enough (so that latency can be essentially decoupled and kept low as well);
Table \ref{table:num_voter} shows the number of voter chains $m$ needed for a low error probability ($\epsilon = 10^{-9}$), which is impractically large and grows with the expected life span of the blockchain. 
%which is impractical.


\begin{table}
	\centering
	\caption{Relationship between the number of voter chains $m$ and the life span of the blockchain according to the security theorem in \cite{prism-theory}. We target a confirmation error probability of $\epsilon = 10^{-9}$. \cite{prism-theory} adopts a round-by-round model and we set the round duration to 1 second.}
	\begin{tabular}{ c || c | c | c | c | c | c } 
	 \hline
	  & \multicolumn{3}{c|}{$\beta = 0.2$} & \multicolumn{3}{c}{$\beta = 0.33$} \\
	 \hline
	 $r_{\rm max}$ (year)  & 1  &10  &100  & 1  &10  &100  \\ 
	 \hline
	 $m$ & 14075 & 15388  & 16716 &  26479 & 28939 & 31474 \\
	 \hline
	\end{tabular}
	\label{table:num_voter}
\end{table}


\noindent {\bf Limitation of the latency guarantee}. Although the confirmation rule in \cite{prism-theory} guarantees to confirm transactions within a constant factor of the network latency, the constant introduced in the analysis is large and leads to poor latency in practice.
To be specific, Theorem 4.8 in \cite{prism-theory} shows that the confirmation latency of an honest transaction (a transaction without public double spending) is upper bounded by $c_1(\beta) = \frac{5400(1-\beta)}{(1-2\beta)^3 \log{\frac{1-\beta}{\beta}}} \log{\frac{50}{1-2\beta}}$ rounds when $m$ is very large. Table \ref{table:old_latency} lists this bound for several different $\beta$, which is too large to provide any practical guarantee.

\begin{table}
	\centering
	\caption{Upper bound on the confirmation latency guaranteed by \cite{prism-theory}. \cite{prism-theory} adopts a round-by-round model and we set the round duration to be 1 second. The poor latency bounds are due to the large constants introduced in the analysis.}
	\begin{tabular}{ c || c | c | c } 
	 \hline
     $\beta$ &0.1  & 0.2 & 0.33 \\
	 \hline
	 Latency upper bound & 4.96h & 17.72h & 180h \\ 
	 \hline
	\end{tabular}
	\label{table:old_latency}
\end{table}

\medskip
\noindent {\bf \newprism's approach}. At the time of the analysis in \cite{prism-theory}, the state-of-the-art proof technique for longest chain  protocols were still rudimentary  \cite{backbone,pss16}, relying on finite execution time horizons. The proof techniques for the longest chain protocol, and corresponding security models and guarantees, have significantly advanced. Latest techniques can model continuous-time block arrivals with infinite time horizon  \cite{ren2019analysis,li2020continuous}, and provide sharp characterizations of the relation between network delay $\Delta$ and adversary fraction $\beta$ for secure blockchain operation \cite{dembo2020everything,gazi2020tight}. 
However, it is still unclear how to bring these techniques (or the ones in \cite{cryptoeprint:2020:675} on parallel ledger combining) to bear on the idea of \prism and its security analysis, given the multiple parallel voting chains coupled via a single block sortition procedure. We take a different approach in this paper: identifying the worst case attack and directly calculating the associated confirmation probability, {\em without resorting to a union bound}. We elaborate on our approach in the next section.

==> Prism Systems Paper (CCS)/spam-exp-dis-jitter.tex <==
\section{Spamming Attacks}
\subsection{Exponential-distributed random jitter\label{app-spam}}
\gw{Added the whole section.}
Here we present an analysis of adding exponential-distributed random jitter to mitigate spam attacks. Suppose that one arbitrary spam transaction is received by $N$ nodes at the same time. For node $j\in[N]$, the time to mine the transaction into a block is the sum of random jitter $X_j$ and mining time $M_j$. We assume $\{X_j\}_{j\in[N]}$ are i.i.d. exponential random variables with parameter $\lambda$. Also we assume mining time $M_j$ is significantly smaller than jitter $X_j$, such that we can approximate $X_j+M_j\approx X_j$.

Without loss of generality, let node $s=\arg\min_{j\in[N]} X_j$ be the first to mine the transaction, and define random variable $Z_j\in\{0,1\}$ such that
\[Z_j=1\text{ if the spam transaction gets mined by node $j$.}\]

We know that $Z_s=1$ and for $j\neq s$, $E[Z_j]\le P(X_j<X_s+\Delta)$ where $\Delta$ is the maximal network delay of a transaction block. The reason is that if the  transaction gets mined by node $j$, the time gap between two jitters $X_j$ and $X_s$ must be less than the network delay, otherwise node $j$ would remove the spam transaction from the memory pool.

By our assumption, $\{X_j\}_{j\in[N]}$ are i.i.d. exponential random variables with parameter $\lambda$, and we know $X_j\ge X_s$. By the memoryless property of exponential distribution, we have
\[P(X_j<X_s+\Delta|X_j\ge X_s)=P(X_j<\Delta)=1-e^{-\lambda \Delta}.\]

Then consider without the random jitter, the transaction would be mined by all the $N$ miners since the mining time is very small for a transaction block. So to normalize the number of spam, we normalize with $N$.

The expected normalized spam should be
\begin{align*}
    E[\sum_j Z_j]/N&= \frac{E[Z_s+\sum_{j\neq s} Z_j]}{N}\\
    &= \frac{1+\sum_{j\neq s}E[Z_j]}{N}\\
    &\le \frac{1+\sum_{j\neq s}(1-e^{-\lambda \Delta})}{N}\\
    &=1-\frac{N-1}{N}\cdot e^{-\lambda \Delta}\\
    &\approx 1-e^{-\lambda \Delta}.
\end{align*}

Fig.~\ref{fig:attack-spamming-exp} shows the case under $\Delta=2$s. With a mean of 10s, we can reduce spam to 20\%.
\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/exp-jitter.pdf}
    \caption{Effectiveness of random jitter in defending against spam attack. The maximal network delay is $\Delta=2$s. Jitters follow exponential distributions and we report the mean ($1/\lambda$).}
    \label{fig:attack-spamming-exp}
    %\vspace{-4mm}
\end{figure}


==> background.tex <==
\section{The Longest Chain Protocol}
\label{sec:background}
% In this section, we review Nakamoto's longest chain protocol~\cite{bitcoin} and discuss the fundamental limitations in scaling its latency and throughput. These limitations motivate \prism's design, as we discuss in the next section. 

% %as a natural design to remove these limitations. 
% %%We will explain the design of \prism incrementally, first addressing throughput and then latency.



% \subsection{The longest chain protocol}

The most basic blockchain consensus protocol is Nakamoto's longest chain protocol, used in many systems including \bitcoin and \ethereum.  The basic object is a {\em block}, consisting of {\em transactions} and a reference link to another block. 
%A transaction is a payment signed by a sender's public key, and addressed to a recipient's public key. 
As transactions arrive into the system, a set of nodes, called {\em miners}, construct blocks and broadcast them to other nodes. The goal of the protocol is for all nodes to reach consensus on an ordered log of blocks (and the transactions therein), referred to as the {\em ledger}.

Starting with the {\em genesis} block as the root, each new block mined by a miner is added to create an evolving {\em blocktree}. In the longest chain protocol, honest miners append each block to the leaf block of the longest chain\footnote{In case of variable proof of work, honest miners mine on the "heaviest chain".} in the current blocktree, and the transactions in that block are added to the transaction ledger maintained by the blocks in the longest chain. 
A miner earns the right to append a block after solving a cryptographic puzzle, which requires finding a solution to a hash inequality.
 %the leaf block \ma{and the contents of the block being mined?}.  
 The miner includes the solution in the block as a {\em proof of work} (PoW), which other nodes can verify.  The time to solve the puzzle is random and exponentially distributed, with a mining rate $f$ that can be tuned by adjusting the difficulty of the puzzle. How fast an individual miner can solve the puzzle and mine the block is proportional to its hashing power, i.e. how fast it can compute hashes. 
 
 A block is confirmed to be in the ledger when it is $k$-deep in the ledger, i.e. the block is on the longest chain and a chain of $k-1$ blocks have been appended to it. It is proven that as long as the adversary has less than $50\%$ hashing power, the ledger has consistency and liveness properties~\cite{backbone}: blocks that are deep enough in the longest chain will remain in the longest chain with high probability, and honest miners will be able to enter a non-zero fraction of blocks into the ledger. 

\begin{figure}
\begin{center}
\includegraphics[width=0.4\textwidth]{fast_confirmation_comparision_2.pdf}
\end{center}
\caption{\small Depth of confirmation: longest chain vs. \prism. (a) The longest chain protocol requires a block $Ho$ to be many blocks deep for reliable confirmation, so that an adversary mining in private cannot create a longer chain to reverse block $Ho$. (b) \prism allows each voter block to be very shallow but relies on many voter chains to increase the reliability.}
\label{fig:double_spend}
\end{figure}

\subsection{Latency Limitation}
\label{s:lc-latency}
A critical attack on the longest chain protocol is the {\em private  double-spend} attack \cite{bitcoin}, as shown in Figure \ref{fig:double_spend}(a). Here, an adversary is trying to revert a block after it is confirmed, by mining a chain in private and broadcasting it when it is longer than the public chain. If the hashing power of the adversary is greater than that of aggregate of the honest nodes, this attack can be easily executed no matter what $k$ is, since the adversary can mine blocks faster on the average than the honest nodes and will eventually  overtake the public chain. On the other hand, when the adversary has less than half the power, the probability of success of this attack can be made exponentially small by choosing the confirmation depth $k$ to be large \cite{bitcoin}. The price to pay for choosing $k$ large is increased latency in confirmation. For example, to achieve a reversal probability of  $0.001$, a depth of $24$ blocks is needed if the adversary has $\beta = 30\%$ of the total hashing power~\cite{bitcoin}.  Figure ~\ref{fig:rd} shows the tradeoff between confirmation depth (and therefore latency) and reliability.


%%With Bitcoin's block mining rate of 1 block every 10 minutes, this translates into a latency of 4 hours! Increasing the block mining rate to, say, 1 block per 10 seconds, improves latency to 240 seconds, but the latency to achieve a high level of reliability is still very high. To achieve a reversal probability of $10^{-6}$, a depth of $50$ blocks is required, translating into a latency of $500$ seconds. Figure ~\ref{fig:rd} shows the tradeoff between confirmation depth (and therefore latency) and reliability. \pv{This is a pretty long section and if we are in a space crunch, then its fine to cut a bit.} 

%In Bitcoin, the mining rate is set much more conservatively, a block roughly every 10 minutes, leading to very long confirmation latency. 

%\ma{I've been assuming this figure also shows the reliability-depth tradeoff for Prism?}
% \begin{figure}
%     \centering
%     \begin{subfigure}[b]{\textwidth}
%         \centering
%         \includegraphics[width=0.35\linewidth]{fast_confirmation_comparision_a.pdf}%
%         \hfill
%         \includegraphics[width=0.35\linewidth]{fast_confirmation_comparision_b.pdf}
%     \end{subfigure}
%     \tion{\small Depth of confirmation: longest chain vs. \prism. (a) The longest chain protocol requires a block to be many blocks deep for reliable confirmation, so that an adversary mining in private cannot create a longer chain. (b) \prism allows each voter block to be very shallow but relies on many voter chains to increase the reliability. \ma{please increase the font size of the subfigure labels, or better, separate this into two figures and use latex's subfig environment}} 
% \end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=0.32\textwidth]{figures/reliability-depth.pdf}
\end{center}
\caption{\label{fig:rd} \small Reliability as a function of confirmation depth. The reversal probability of \prism has a factor $m$ improvement over the longest chain protocol in the exponential rate of decrease, where $m$ is the number of voter chains (introduced in \S\ref{sec:overview}).}
\end{figure}
\subsection{Throughput Limitation}
\label{s:lc-thput}

If $B$ is the block size in number of transactions, then the throughput of the longest chain protocol is at most $fB$ transactions per second (tps). 
However, the mining rate $f$ and the block size $B$ are constrained by the security requirement. Increasing the mining rate increases the amount of {\em forking} of the blockchain due to multiple blocks being mined on the same leaf block by multiple miners within the network delay~$\Delta$. Forking reduces throughput since it reduces the growth rate of the longest chain; recall that only blocks on the longest chain contribute to the ledger. More importantly, forking hurts the security of the protocol because the adversary requires less compute power to overtake the longest chain. In fact, the adversarial power that can be tolerated by the longest chain protocol goes from $50\%$ to $0\%$ as the mining rate $f$ increases \cite{backbone}. 
%(Figure \ref{fig:forking}). 
Similarly, increasing the block size $B$ also increases the amount of forking since the network delay $\Delta$ increases with the block size \cite{decker}.

A back-of-the-envelope calculation of the impact of the forking can be done based on a simple model of the network delay: 
$$ \Delta = \frac{hB}{C} + D,$$
where $h$ is the average number of hops for a block to travel, $C$ is the communication bandwidth per link in transactions per second, and $D$ is the end-to-end propagation delay.  This model is consistent with the linear relation between the network delay and the block size as measured empirically by \cite{decker}. 
%\ma{do we have to mention the possibility of cut-through routing? i think we can skip it and maybe mention it in the discussion section towards the end.}
%\vb{Thats a good idea. There are works (like bloxroute) out there which propose cut-through routing to improve the latency.}
Hence, the utilization, i.e. the throughput as a fraction of the communication bandwidth, is upper bounded by
$$ \frac{fB}{C} < \frac{f\Delta}{h},$$
where $f\Delta$ is the average number of blocks ``in flight'' at any given time, and reflects the amount of forking in the block tree.  %%which is nothing but the \textit{forking rate} on the longest chain. \ma{how is forking rate defined?}
In the longest chain protocol, to be secure against an adversary with $\beta < 50\%$ of hash power, this parameter should satisfy \cite{backbone}
$$f\Delta<\frac{1-2\beta}{\beta}.$$
For example, to achieve security against an adversary with $\beta = 45\%$ of the total hashing power, one needs $f\Delta \approx 0.2$. With $h = 5$, this translates to a utilization of at most $4\%$. The above bound holds regardless of block size; the utilization of the longest chain protocol cannot exceed 4\% for $\beta = 45\%$ and $h=5$.
In summary, to not compromise on security, $f\Delta$ must be kept much smaller than $1$. 
Hence, the security requirement (as well as the number of hops) limits the bandwidth utilization.  

%%$$ \ma{I still don't understand why this is different from the analysis in Appendix %%D.2 of the Prism paper.}
%%\vb{The analysis in D.2 is a conservative necessary condition. Whereas the above %%formula is only a necessary condition. It comes from the simple fact that the %%honest nodes grow at rate $\frac{(1-\beta)}{1+f\Delta}$ and adversary grows at rate %%$f\beta$.}
%%\gf{The phrasing above the equation makes it sound like a necessary condition.} %%\vb{Typo. It is indeed a necessary condition

% \ma{Can we state how security depends on $f\Delta$ here precisely, and replace Figure 3 with one that shows maximum possible $f\Delta$ vs. $\beta$. The next sentence gives the specific point $\beta=0.45$ as an example. The nice thing about this is that it highlights that in the longest chain protocol, to meet the security requirement, one cannot have too many blocks in flight at the same time. Prism doesn't have this limitation. However, if my understanding is correct, it will show that $f\Delta$ can be 1 for $\beta < 0.33$, and drops sharply only for higher security levels. This would mean that the possible utilization for Bitcoin in practice is really $1/h$. Is this correct? Prism can only improve throughput from $1/h$ to $1$, unless we're concerned with very high security?} 
% \vb{The effective throughput due to forking is $fB\big(\frac{1}{1+f\Delta}\big)$} \ly{$f\Delta = \frac{1-2\beta}{\beta}$ See Figure~\ref{fig:forking-new}} \ma{Is this consistent with the Prism theory paper, Appendix D.2? I'm still not happy with our explanation here. My hope is that we can remove Fig. 3, and use the fact that f$\Delta$ must be small for security, and the equation above to show that the utilization of the longest chain protocol is limited. @Vivek: please see if this makes sense and update this section.}


%%In summary, in the longest chain protocol, security of the system is fundamentally at odds with low latency and high throughput. To achieve a low reversal probability, blocks must be deep in the longest chain, increasing confirmation latency. At the same time, increasing the mining rate or block size would compromise security because of forking. As we discuss next, \prism removes these limitations to achieve high throughput, low latency, and security simultaneously. 

%\red{GF: Maybe explain in words why we can hope to fix this problem? The dependency on  graph diameter is fundamental, since all honest nodes have to come to consensus, but the effect of Bitcoin's security requirement could  be circumvented by designing a system that trades latency for communication in its confirmation rule.}

\if 0
\begin{figure}
\begin{center}
\includegraphics[width=0.4\textwidth]{figures/forking_security.pdf}
\end{center}
\caption{ Increasing mining rate or block size increases forking and reduces security. 
\red{GF: Are we going to add numbers to the x-axis? This looks a bit cartoonish, I think having actual nubmers on the axes would help,  if we want to keep this figure at all (not sure it clarifies too much?).} \ly{Shall I redo the plot to put numbers on x-axis and make it the same style as figure 8 to 12?}
\vb{I have added numbers to x-axis for now.}
\gw{Caption says "or block size", but it's not in the figure.}}
\label{fig:forking}
\end{figure}

\fi

% \begin{figure}
% \centering
% \input{figures/fdelta-fig.tex}
% \caption{ Increasing mining rate or block size increases forking and reduces security. \gw{Is this the correct caption for the figure?}} \ma{No. This figure might actually work better with $f\Delta$ on the x-axis. The focus should probably be the region where $f\Delta$ is small, say less than 2 or 3. I'm not sure the figure is correct. @Vivek: please double check} \vb{This figure look correct}
% \label{fig:forking-new}
% \end{figure}






==> commands.tex <==

\usepackage[utf8]{inputenc}
\usepackage[english]{babel}

\setcounter{secnumdepth}{3} % numbering section depth
\setcounter{tocdepth}{4}
\newtheorem{thm}{Theorem}[section]
\newtheorem{defn}[thm]{Definition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{prop}{Proposition}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{constr}[thm]{Construction}


\newcommand{\bpf}{\begin{proof}}
\newcommand{\epf}{\end{proof}}
\newcommand{\bprf}{{\em Proof: }}
\newcommand{\bproof}{{\em Proof of }}
\newcommand{\eproof}{\hfill $\Box$}
\newcommand{\argmin}{\operatornamewithlimits{arg \ min}}
\newcommand{\argmax}{\operatornamewithlimits{arg \ max}}
\newcommand{\indep}{\mathrel{\text{\scalebox{1.07}{$\perp\mkern-10mu\perp$}}}}


\newcommand{\red}[1]{\textcolor{red}{#1}}

\newcommand{\beqa}{\begin{eqnarray}}

\newcommand{\eeqa}{\end{eqnarray}}

\newcommand{\beqan}{\begin{eqnarray*}}

\newcommand{\eeqan}{\end{eqnarray*}}

\newcommand{\beq}{\begin{equation}}

\newcommand{\eeq}{\end{equation}}

\newcommand{\prf}{\noindent {\bf Proof}\ \ \ }

\newcommand{\lra}{\Longleftrightarrow}

\newcommand{\lbr}{\left \{ }

\newcommand{\rbr}{\right \} }

\newcommand{\Lbr}{\left [}

\newcommand{\Rbr}{\right ]}

\newcommand{\lp}{\left (}

\newcommand{\rp}{\right )}

\renewcommand{\r}{\right}

\renewcommand{\l}{\left}

\newcommand{\df}{\stackrel{{\rm def}}{=}}

\newcommand{\real}{{\Bbb {R}}}

\newcommand{\complex}{{\Bbb {C}}}

\newcommand{\prob}{{\Bbb {P}}}

\newcommand{\expect}{{E}}

% \newcommand{\eqref}[1]{(\ref{#1})}




\renewcommand{\C}{{\cal C}}
\newcommand{\X}{{\mathcal X}}

\renewcommand{\S}{{\cal S}}

\newcommand{\bmk}{\beta_m^{(K)}}



\newcommand{\vu}{{\bf u}}

\newcommand{\vd}{{\bf d}}

\newcommand{\Ummse}{U_{{\rm mmse}}}

\newcommand{\vp}{{\bf p}}

\newcommand{\vq}{{\bf q}}

\newcommand{\vone}{{\bf 1}}

\newcommand{\vh}{{\bf h}}
\newcommand{\hh}{\hat h}
\newcommand{\vw}{{\bf w}}

\newcommand{\SNR}{\sf SNR}
\newcommand{\SINR}{\sf SINR}
\newcommand{\rot}{\sf RoT}
\newcommand{\penal}{\sf penalty}
\newcommand{\PR}{\sf PR}

\newcommand{\eapprox} {\stackrel {.}{=}}
\newcommand{\al}{\stackrel{.}{<}}
\newcommand{\ag}{\stackrel{.}{>}}

\newcommand{\SINRt}{{\sf SINR^{(t)}}}
\newcommand{\lambdat}{\lambda^{(t)}}
\newcommand{\It}{I^{(t)}}
\newcommand{\vwt}{{\bf w}^{(t)}}
\newcommand{\vwn}{{\bf w}^{(t+1)}}
\newcommand{\vv}{{\bf v}}
\newcommand{\uu}{{\bf u}}
\newcommand{\ww}{{\bf w}}
\newcommand{\eps}{\varepsilon}
\newcommand{\vz}{{\bf z}}
\newcommand{\bvh}{\bar{\vh}}



\newcommand{\singlespacing}{\let\CS=\@currsize\renewcommand{\baselinestretch}{0.95}\tiny\CS}



\newcommand{\oneandahalfspacing}{\let\CS=\@currsize\renewcommand{\baselinestretch}{1.25}\tiny\CS}



\newcommand{\doublespacing}{\let\CS=\@currsize\renewcommand{\baselinestretch}{1.39}\tiny\CS}



% Start with double spacing:

%%\singlespacing

%\oneandahalfspacing

%\doublespacing

\newcommand{\be}{\begin{equation}}

\newcommand{\ee}{\end{equation}}

\newcommand{\tr}{{\rm trace}}

\newcommand{\rref}[1]{(\ref{#1})}

\newcommand{\CN}{{\cal CN}}





\newcommand{\bc}{\begin{center}}

\newcommand{\ec}{\end{center}}

\newcommand{\bfl}{\begin{flushleft}}

\newcommand{\efl}{\end{flushleft}}

\newcommand{\blob}{\hfill \rule{.1in}{0.1in}}

\newcommand{\scheme}{{\sf Prism} }
\newcommand{\schemenosp}{{\sf Prism}\ignorespaces}
\newcommand{\schemelite}{{\sf Prism 1.0 } }
\newcommand{\schemelitenosp}{{\sf Prism 1.0}\ignorespaces}
\newcommand{\schemebackbone}{{\sf Prism Backbone} }
\newcommand{\schemebackbonenosp}{{\sf Prism Backbone}\ignorespaces}
\newcommand{\fruitchains}{{\sf Fruitchains } }
\newcommand{\fruitchainsnosp}{{\sf Fruitchains}\ignorespaces}
\newcommand{\bitcoinNG}{{\sf BitcoinNG } }
\newcommand{\bitcoinNGnosp}{{\sf BitcoinNG}\ignorespaces}
\newcommand{\disccoin}{{\sf DiscCoin } }
\newcommand{\disccoinnosp}{{\sf DiscCoin}\ignorespaces}
\newcommand{\byzcoin}{{\sf ByzCoin } }
\newcommand{\byzcoinnosp}{{\sf ByzCoin}\ignorespaces}
\newcommand{\hybrid}{{\sf Hybrid } }
\newcommand{\thunderella}{{\sf Thunderella }}
\newcommand{\inclusive}{{\sf Inclusive }}
\newcommand{\spectre}{{\sf Spectre }}
\renewcommand{\phantom}{{\sf Phantom }}
\newcommand{\conflux}{{\sf Conflux }}
\newcommand{\avalanche}{{\sf Avalanche }}

\newcommand{\bitcoin}{{\sf Bitcoin} }
\newcommand{\bitcoinnosp}{{\sf Bitcoin}\ignorespaces}

\newcommand{\ghost}{{\sf GHOST} }
\newcommand{\ghostnosp}{{\sf GHOST}\ignorespaces}

\newcommand{\prism}{{\sf Prism} }

\newcommand{\pois}{{\sf Poiss}}
\newcommand{\geom}{{\sf Geometric}}
\newcommand{\bin}{{\sf Bin}}

\makeatletter
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                       {-18\p@ \@plus -4\p@ \@minus -4\p@}%
                       {4\p@ \@plus 2\p@ \@minus 2\p@}%
                       {\normalfont\normalsize\bfseries\boldmath
                        \rightskip=\z@ \@plus 8em\pretolerance=10000 }}

\newcommand{\ext}{{\sf ext} }

\newcommand{\N}{{\mathcal{N}}}
\newcommand{\Z}{{\mathcal{Z}}}
\newcommand{\fv}{\bar{f}_v}
\newcommand{\fp}{\bar{f}_p}
\newcommand{\Rl}{R_{\ell}}



\newcommand{\Vo}{{\sf{V}}}
\renewcommand{\H}{{\mathcal{H}}}
\renewcommand{\C}{{\mathcal{C}}}
\newcommand{\A}{{\mathcal{A}}}
\newcommand{\T}{{\mathcal{T}}}
\newcommand{\R}{{\mathcal{R}}}
\newcommand{\rmax}{r_{\rm max}}
\newcommand{\rmin}{r_{\rm min}}
\newcommand{\bmin}{b_{\rm min}}
\newcommand{\kmin}{k_{\rm min}}
\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\E}{\mathbb{E}}
\renewcommand{\P}{{\mathcal P}}
\newcommand{\Dr}{{\Delta_r}}
\newcommand{\Dmax}{{\Delta_{\text{max}}}}
\newcommand{\cone}{\frac{1-2\beta}{16}}


\makeatother
\newcommand{\blue}{\color{blue}}

\newcommand{\tE}{\texttt{E}}
\newcommand{\tT}{\texttt{T}}
\newcommand{\tF}{\texttt{F}}
\newcommand{\Rc}{R^{\text{stop}}}
\newcommand{\Rconf}{R^{\text{conf}}}
\newcommand{\Dll}{D_{\ell', \ell}}
\newcommand{\Dllf}{\big\{D_{\ell', \ell}\big\}_{\ell'\leq \ell}}
\newcommand{\Rfirst}{R_0}
\newcommand{\Rlast}{R_{\text{last}}}
\newcommand{\LS}{\texttt{LedSeq}}
\renewcommand{\epsilon}{\varepsilon}

\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{xcolor}
\definecolor{azure}{rgb}{0.54, 0.17, 0.89}
\newcommand{\colorcomment}[1]{\Comment{ {\color{azure} #1}} }
\newcommand{\av}[1]{$#1$}
\newcommand{\maincolorcomment}[1]{{\color{azure}// #1 } }
\def\NoNumberLine#1{{\def\alglinenumber##1{}\State #1}\addtocounter{ALG@line}{-1}}
\usepackage{enumitem,kantlipsum}

\renewcommand{\bmin}{B_{\rm min}}

==> confirmation-rule.tex <==
\section{Confirmation Rule}
\label{apx:confirmation}

In this section we give the detailed calculation of the confidence intervals of the votes a proposer block receives. It is used when confirming a leader proposer block, as mentioned in Section~\ref{sec:confirmation}.

Consider the scenario where there are $n$ proposer blocks at level $l$, and let $\mathcal P =\{B^P_1, B^P_2, \ldots, B^P_n\}$ denote the set of proposer blocks at level $l$. Now we want to count the number of votes each block will get with confidence $1-\epsilon$.

Suppose $B^P_i$ gets $v_i$ votes. Here a vote stands for a voter block which is on the longest chain of its voter tree and votes for $B^P_i$. 
Let $\mathcal V_i =\{B^V_{i_1}, B^V_{i_2}, \ldots, B^V_{i_{v_i}}\}$ denote the set of votes that $B^P_i$ has. For every vote $B^V_{i_j}$, let $d_{i_j}$ denote its depth, which is the number of blocks appended to voter block $B^V_{i_j}$ in the longest chain, plus one.

Now, for each vote $B^V_{i_j}$ with depth $d_{i_j}$, we want to calculate the probability $P_{i_j}$ of it being permanent. 
% \textit{not} being overtaken by a hypothetical, unreleased adversarial chain any time in the future. 
To do so, we consider a potential private double-spend attack, assuming an adversarial party is trying to overturn the voting results to elect a different proposer block $B^P_A$ as the leader block of level $l$. 
Note that $B^P_A$ could either be a block in $\mathcal P$, i.e. publicly known, or a block the adversary has privately mined but not released. 
To elect $B^P_A$ as the leader block of level $l$, the adversarial party would need to mine its own voter chains to overturn some existing votes to vote for $B^P_A$. 

We want to compute the probability of this happening.
% we need to reason about the blocks the adversary has already mined as well as those it will mine in the future. 
However, we do not know when the adversary started mining voter blocks for $B^P_A$.
% , which means we do not know how long the adversary could have been mining its private blocks. 
% However, from the visible state of the blockchain, we can estimate when $B^P_i$ was mined; assuming $B^P_A$ was mined at least as late as $B^P_i$, this gives us a bound. 
Notice that the adversary has no incentive to mine voter blocks for $B^P_A$ until $B^P_i$ has been mined and released. 
%Since the honest nodes are always releasing blocks, we can use the average depth of the votes for $B^P_i$ in the public voter trees to estimate the time passed since $B^P_i$ was released, hence  bounding the expected number of votes the adversary could have accumulated on their private fork in the same amount of time. 
Since the honest nodes are always releasing blocks, we can use the average depth of the votes in the public voter trees to estimate the time passed since level $l$ was released, hence  bounding the expected number of votes the adversary could have accumulated on their private fork in the same amount of time. 
That is, since block inter-arrivals are exponentially distributed, the number of blocks mined since blocks in $\mathcal P$ was proposed is a Poisson random variable, with rate equal to its mean. 
This quantity can be related to the time elapsed since blocks in $\mathcal P$ was released via the block mining rate.
%That is, since block inter-arrivals are exponentially distributed, the number of blocks mined since block $B^P_i$ was proposed is a Poisson random variable, with rate equal to its mean. 
%This quantity can be related to the time elapsed since $B^P_i$ was released via the block mining rate.
% To do this, we estimating how deep those private voter chains are on average. 

More precisely, as an honest node, we assume the fraction of adversarial hashing power is $\beta$, and we can empirically estimate the average depth of existing public votes as $\bar{d}=\sum_{ij}{d_{i_j}}/\sum_{i}{v_i}$ and the forking rate $\alpha$~\footnote{The fraction of blocks not on the longest chain out of all blocks.} of public voter chains. 
Since there are many voter chains, these estimates converge quickly to their true means. 
Then, we calculate the estimated average depth of a \emph{private} voter chain, denoted as $\bar{d_A}$, to be
% \gf{Yes, the sentences starting with "we observe that" to the end of this para  (through the following equations) need a good bit more explanation. Minor nits: In the defn of $\bar{d}$, $v_i$ was earlier defined as the total number of votes, not the honest number  of votes,
% but $\bar{d}$ is defined as the average depth of honest votes. How are you defining an "honest vote" here? 
% Also, the sentence starting with "We observe" doesn't parse.}
% \ly{``honest'' is better defined as ``public'' here, and I have changed the definitions correspondingly. Also, I added the sentence below the next equation. Does this sound like enough explanantion?}
$$\bar{d_A} = \frac{\beta \bar{d}}{(1-\alpha)(1-\beta)}.$$
Here the $1/(1-\alpha)$ term accounts for forking in public voter chains and assumes that the malicious private voter chains do not fork. The $\beta / (1-\beta)$ term accounts for the ratio of hashing power between the honest users ($1-\beta$) and the malicious users ($\beta$).
This expected depth $\bar{d_A}$ can be used as an estimate of the rate of the Poisson random variable of the number of blocks in the adversary's  private chain. 


Since each voter chain follows the longest-chain rule, the calculation for $P_{i_j}$ is the same as in \bitcoin
$$P_{i_j} = F_{\text{Pois}}(d_{i_j};\bar{d_A}) - \sum_{k=0}^{d_{i_j}}f_{\text{Pois}}(k;\bar{d_A})\frac{\beta}{1-\beta}^{d_{i_j} + 1 - k}.$$
Here $F_{\text{Pois}}(x;\lambda)$ is the cumulative distribution function and $f_{\text{Pois}}(x;\lambda)$ is the probability mass function of Poisson distribution with rate parameter $\lambda$.
In this expression, the first term is the probability that the adversary has mined fewer than $d_{i_j}+1$ blocks, in which case it cannot currently overtake the main chain. 
The second term computes, for each possible length of the adversary's chain, the probability that the adversary overtakes the public voter chain in the future by mining faster. 

Given $P_{i_j}$, we can now calculate the confidence interval of votes on each proposer block. For proposer block $B_i^P$ and each of its votes $B^V_{i_j}$, let $\tilde V_{i_j}$ be the random variable where
$$\tilde V_{i_j} = \begin{cases}
    1, & \text{if vote } B^V_{i_j} \text{ is secure forever (permanent)} \\
    0, & \text{if vote } B^V_{i_j} \text{ will be overturned}
  \end{cases}.$$
With some abuse of notation, let $v_i$ be the random variable equal to the number of secure votes of $B^P_i$. We have
$$v_i = \sum_{j}B^V_{i_j}.$$
Note that $\tilde V_{i_j}\sim \text{Bernoulli}(P_{i_j})$. Then the lower confidence bound of votes on $B_i^P$ (denoted as $\left \lfloor v_{i} \right \rfloor$) can be obtained by calculating in $\epsilon$-quantile of random variable $v_i$.

In real-world implementations, given the complexity of such computation, its closed-form approximation may be used. We can approximate $v_i$ using a Gaussian distribution $\mathcal N(\mu_i, \sigma_i^2)$ where
$$\mu_i=\sum_j P_{i_j}.$$
$$\sigma_i^2 = \sum_j P_{i_j}(1-P_{i_j}).$$
Using the closed-form approximation of the quantile function of normal distribution, we have
$$\left \lfloor v_{i} \right \rfloor \approx \mu_i - \sigma_i \sqrt{\ln{
\frac{1}{\epsilon^2}} - \ln{\ln{\frac{1}{\epsilon^2}}} - \ln{(2\pi)}}.$$

Now, we consider the upper confidence bound of votes on $B_i^P$ (denoted as $\left \lceil v_{i} \right \rceil$). Here, we want to defend against the worst case where for each $B_i^P$, only $\left \lfloor v_{i} \right \rfloor$ votes are retained, and the adversarial party controls the remaining votes (we let $\left \lceil v_A \right \rceil$ denote the number of such votes). Recall that each voter chain can only vote for each proposer level once. For a system with $m$ voter chains, we have
$$\left \lceil v_A \right \rceil = m - \sum_{i}\left \lfloor v_{i} \right \rfloor.$$
The adversarial party will use those votes to vote for $B^P_A$. Since $B^P_A$ could be any block in $\mathcal P$, we have
$$\left \lceil v_i \right \rceil = \left \lfloor v_{i} \right \rfloor + \left \lceil v_A \right \rceil.$$
$B^P_A$ could also be a block which the adversarial party mines but has not released. In such case, the upper bound of votes on $B^P_A$ is just $\left \lceil v_A \right \rceil$. Finally, to select the leader of level $l$, we search for the block $B^P_L \in \mathcal P$ satisfying $\left \lfloor v_{L} \right \rfloor > \left \lceil v_i \right \rceil$ for every $i \neq L$ and $\left \lfloor v_{L} \right \rfloor > \left \lceil v_A \right \rceil$. In words, we select the block whose lower bound of votes is higher than the upper bound of any other known or unknown proposer block in the same level.

==> datapoints.tex <==
\section{Parameters Used in Evaluations}
\label{apx:datapoints}

Here we present the parameters used in the experiment in \S\ref{sec:eval-performance} for \prism (Table~\ref{table:prism-params}, Table~\ref{table:prism-beta}), \algorand (Table~\ref{table:algorand-params}), \bng (Table~\ref{table:bng-params}), and the longest chain protocol (Table~\ref{table:lc-params}).

\begin{table}[t]
	\centering
	\caption{Parameters of \prism.}
	%\resizebox{\columnwidth}{!}{
	\begin{tabular}{ r | c } 
	 \hline
	 Parameter & Value \\ [0.5ex] 
	 \hline\hline
	 Transaction Block Size & 228 transactions \\
	 Voter Block Size & 1000 votes \\
	 Proposer Block Size & 7000 references \\
	 Voter Chains ($m$) & 1000 \\
	 Transaction Mining Rate & 350 Blocks/s \\
	 Voter Mining Rate & Table~\ref{table:prism-beta}\\
	 Proposer Mining Rate & Table~\ref{table:prism-beta}\\
	 \hline
	\end{tabular}
	%}
\label{table:prism-params}
\end{table}

\begin{table}[t]
	\centering
	\caption{Mining rate $f$ of proposer and voter blocks for different $\beta$ in \prism. The unit is Blocks/s.}
	%\resizebox{\columnwidth}{!}{
	\begin{tabular}{ r | c } 
	 \hline
	 $\beta$ & Mining Rate ($f$) \\ [0.5ex] 
	 \hline\hline
	 0.20 & 0.535 \\
	 0.33 & 0.185 \\
	 0.40 & 0.097 \\
	 0.42 & 0.081 \\
	 0.43 & 0.069 \\
	 0.44 & 0.054 \\
	 \hline
	\end{tabular}
	%}
\label{table:prism-beta}
\end{table}


\begin{table}[t]
	\centering
	\caption{Parameters of \algorand. Block Size: number of transactions in a block. Assembly Time: maximum time spent on assembling a block (this limit was never hit in the experiment). $\lambda$: expected time to reach consensus on block hash. $\Lambda$: expected time to reach consensus on the actual block. Detailed definition in~\cite{algorand}.}
	%\resizebox{\columnwidth}{!}{
	\begin{tabular}{ r | c | c | c } 
	 \hline
	 Block Size & Assembly Time (s) & $\lambda$ (s) & $\Lambda$ (s) \\ [0.5ex] 
	 \hline\hline
	 1287 & 0.5 & 0.6 & 1.6 \\
	 4366 & 0.8 & 1.2 & 3.0 \\
	 8733 & 1.6 & 1.9 & 6.5 \\
	 13100 & 1.6 & 1.9 & 10.0 \\
	 17294 & 1.6 & 2.0 & 13.0 \\
	 21504 & 1.9 & 2.3 & 16.0 \\
	 42334 & 3.5 & 3.9 & 38.0 \\
	 64614 & 5.0 & 5.4 & 56.0 \\
	 85513 & 7.0 & 7.4 & 73.0 \\
	 85836 & 7.0 & 7.4 & 68.0 \\
	 103004 & 8.4 & 8.8 & 84.0 \\
	 116580 & 9.5 & 9.9 & 99.0 \\
	 133766 & 11.0 & 11.4 & 110.0 \\
	 \hline
	\end{tabular}
	%}
\label{table:algorand-params}
\end{table}

\begin{table}[t]
	\centering
	\caption{Parameters of \bng.}
	\begin{tabular}{ r | c } 
	 \hline
	 Parameter & Value \\ [0.5ex] 
	 \hline\hline
	 Key Block Mining Rate & 0.10 Block/s \\
	 Micro Block Interval & 15000 $\mu\text{s}$ \\
	 Block Size & 500 transactions \\
	 \hline
	\end{tabular}
\label{table:bng-params}
\end{table}

\begin{table}[t]
	\centering
	\caption{Mining rate $f$ for different $\beta$ and block sizes in the longest chain protocol. Here block sizes are in terms of transactions.}
	%\resizebox{\columnwidth}{!}{
	\begin{tabular}{ r | r | c } 
	 \hline
	 $\beta$ & Block Size & Mining Rate ($f$) \\ [0.5ex] 
	 \hline\hline
	 \multirow{8}{*}{0.20} & 10 & 0.404 \\
	                       & 260 & 0.262 \\
	                       & 1000 & 0.221 \\
	                       & 4000 & 0.144 \\
	                       & 10000 & 0.110 \\
	                       & 20000 & 0.079 \\
	                       & 60000 & 0.064 \\
	                       & 200000 & 0.027 \\
	 \hline
	 \multirow{4}{*}{0.33} & 10 & 0.168 \\
	                       & 260 & 0.117 \\
	                       & 1000 & 0.119 \\
	                       & 4000 & 0.065 \\
	 \hline
	\end{tabular}
	%}
\label{table:lc-params}
\end{table}






==> design2.tex <==
\section{Design}
\label{sec:design}

% \vb{ A possible notation is to use capital letters for tuples and small letters otherwise. Header $H$, Content $C$, Block $B=(H,C)$.
% $H=(P,n,D)$, $P$ is the content, $n$ is nonce and $D$ is $\texttt{digest}(C)$.
% Tx block $B^T$, Tx header $H^T$, Tx parent $P^T$, Tx digest $D^T$ and Tx content $C^T$ (similar for prop. and voter block). $B \in \{B^T, B^P, B^V\}$ and so on..}

\subsection{Notation}
\label{sec:blocktypes}
Each block $B=(H,C)$ is a tuple containting a header $H$ and content $C$.
As discussed in  \S\ref{sec:overview}, there are three types of blocks: transaction blocks, proposer blocks,  and voter blocks.
In all three types, the header $H=(P, n, D)$ is a tuple containing: (1) the hash $P$ of the parent block,
%(\vb{conceptually parent blocks also differ}) \ma{seems ok to me} 
(2)  a valid PoW nonce $n$, and (3) a content digest $D=\texttt{Digest}(C)$. % proving that the block was mined in the correct category (transaction, proposer, or voter). 
We add a superscript to the above notations to denote the type of block being referred. 
For example, we refer  to proposer blocks by $B^P$, transaction blocks by $B^T$, and voter blocks by $B^V$.
% Along the same lines, a proposer block's header, content, and parent are denoted by $H^P$, $C^P$, and $P^P$, respectively, and its content digest by $D^P$.

% The nonce $n$ and content digest $D$ are explained further in the mining procedure (\S\ref{sec:mining}).

%\todo{I intentionally did not  describe what is actually done in the code w.r.t. parent blocks because I think it may confuse people more. Let me know what you think.}
% \ma{I think this is at the right level}

%\paragraph{Transaction blocks.}
% \smallskip
% \noindent{\bf Transaction blocks.}
% Transaction blocks do not need a parent block,  so  $P^T=\emptyset$.
% The content of a transaction block is an ordered list of transactions: $C^T := [t_1, \ldots, t_m]$.
% drawn from the miner's local a memory pool \texttt{mempool} of transactions that have not yet been  incorporated into a transaction block.
% Note that a transaction $t$ is a payment from a sender's public key to a recipient's public key, signed by the sender. 
% \gw{Do we want to mention about multiple senders and recipients?}


% They contain a list of transactions, and a pointer to a parent proposer block. \ma{why do transaction blocks need a pointer to a proposer block? this is also not shown in in Fig. 4} \ma{It might be useful to define a transaction, e.g., it is a payment from a sender public key to a recipient public key, signed by the sender}

% \vb{Below we have described both the content and the mining procedure of the proposer and voter blocks. We can explicitly state that perhaps} \ma{I think this is ok} 

% \smallskip
% \noindent{\bf Proposer blocks.}
% Since the proposer tree is built in a longest-chain fashion, proposer blocks choose as their parent $P^P$  the tip of the longest chain in the proposer tree. 
% Each proposer block's content, $C^P$, is an ordered list of references to other proposer and/or transaction blocks.  
% We compute $B$'s set of \emph{ancestors} by following the chain of parent links in the proposer tree.
% For proposer block $B$, let $C^P_1 =[B^P_{i_1}, B^P_{i_2}, \ldots]$ denote an ordered list of proposer blocks that are neither indirectly referenced or among content of $B$'s ancestors.
% Let $C^P_2 = [B^T_{j_1}, B^T_{j_2},\ldots]$ denote an ordered list of transaction blocks that are not referenced (directly or indirectly) by any of $B$'s ancestors or by any of the proposer blocks in $C^P_1$.
% The content of the proposer block is the concatenation of these two ordered lists: $C^P  :=(C^P_1, C^P_2)$.
% Note that $C^P$ actually stores references to the listed blocks, but we describe them as blocks here to reduce notation.
% Honest nodes mine proposer blocks on the longest chain in the proposer blocktree, but the longest chain does not determine the final confirmed sequence of proposer blocks, known as the  \emph{leader sequence}. 
% We define the \emph{level} of a proposer block as its distance from the genesis block (Figure \ref{}), and the \emph{height} of the proposer tree as the maximum level that contains any proposer blocks. 
% The confirmed leader sequence of proposer blocks contains one block at every level up to the height of the proposer blocktree, and is  determined by the \emph{voter trees}. 
% \smallskip
% \noindent{\bf Voter blocks.}
% There are $m$ voter trees, where $m \gg 1$ is a fixed parameter chosen by the system designers. 
% The $i^{th}$ voter tree is comprised of voter blocks that are mined on the longest chain of the voter tree. 
% Voter trees are also  built in a longest-chain fashion,  so for a voter block  $B^{V_i}$ in the $i^{th}$ voter tree,  its parent $P^{V_i}$ is the tip of the longest chain in the $i^{th}$ voter tree.
% The block's contents $C^{V_i}$ are a list of references to proposer blocks, or \emph{votes}.
% Recall that the \emph{level} of a proposer block denotes its distance from the genesis block, and the \emph{height} $h$ of the proposer tree is the maximum level that contains any proposer blocks.
% Let $L=\{1,\ldots, h\}$ denote the set of all levels in the proposer blocktree.
% Voter trees are built in a longest-chain fashion; each voter tree's longest chain is allowed to vote at most once on any level in  $L$.
% For a voter block $B^V$, let $\ell'_{B}$ be the latest level of proposer block voter by $B^V$'s ancestors and thus $B^V$ has to vote on levels $\{\ell'_{B}+1,\cdots,h\}$.
% % let $L'_{B}$ denote the set of levels that have already been voted on by $B$'s ancestors. (\vb{$L'_{B}$ is a continuous set. To simplify the notation we can say that `for voter block $B$, let $\ell'_{B}$ be the latest level of proposer block voter by $B$'s ancestors and thus $B$ has to vote on levels $\{\ell'_{B}+1,\cdots,h\}$})
% % Let $L_{B} = L \cap L'_{B}$ be the set of remaining levels, and let $\mathcal P_i$ denote the set of proposer blocks at level  $i$. \gw{You mean $L - L'_B$?}
% The content of the voter block, $C^V := [B^P_{\ell'_{B}+1},\ldots,B^P_{h}]$ is a list of proposer blocks where with some abuse of notation, $B^P_{\ell}$ denotes a vote for  (pointer to) a proposer block at level $\ell$. 
% In words,  the voter block contains a list of one vote per unvoted level in the block's ancestor list. 
% \ma{It seems we can simplify this description per Vivek's suggestion} \vb{done}
% this list includes at most one pointer to a proposer block at every level of the proposer blocktree that has not yet been voted on by any of $B$'s ancestors in the $i$th voter tree. 
% We call such a pointer a \emph{vote}, since it is effectively endorsing a given proposer block. 
% In other words, each voter tree is allowed  at most one vote for each level of the proposer tree, where only the votes contained in the longest chain of each voter tree are counted. 
% We explain how these votes are used to confirm transactions in Section \ref{sec:confirmation}


% \todo{Mention database, mempool, etc. data structures as well. These will be discussed in more detail in the Implementation subsection, but we just explain what they are here so that the pseudocode makes sense. }

% \subsection{Protocol}
% The protocol has two primary components: mining and ledger formation. 

% \ma{One thing that would be good to mention is that the lists in the different blocks have bounded length. Perhaps discuss how a block picks among its options when the list doesn't fit everything.}
% \vb{The list of different blocks will vary in length but for simplicity we can leave it unbounded. In expectation, the size of the list is $1$.}

\subsection{Mining}
\label{sec:mining}
Miners should not be able to choose \emph{a priori} which type of block they are mining; this is essential for the security of the scheme, since otherwise the adversary could concentrate all  of its power on a subset of block trees and overpower them. 
\emph{Cryptographic sortition} is used to ensure that miners cannot choose which type of block they mine.
Nodes simultaneously mine one transaction block, one proposer block, and $m$ voter blocks (one for each tree). 
Only after a valid proof of work is found does the miner learn if the mined block is a transaction, proposer, or voter block. 
The mining process has three steps (four including validation): 

\noindent \textbf{(1) Superblock generation.} 
When a miner starts mining, it creates a \emph{superblock} that simultaneously contains the parents and contents for all $m+2$ possible sub-blocks (1 transaction sub-block, 1 proposer, and $m$ voter sub-blocks). The parents and contents differ for each type of block.
This superblock is updated whenever the miner receives a new network message that changes either the header or the content of any of the sub-blocks. 

\emph{Transaction sub-block $B^T$:} 
%The miner chooses a parent $R_{B^T}$ as described in Section  \ref{sec:blocktypes}. 
Transaction blocks do not need a parent block,  so  $P^T=\emptyset$.
The content of a transaction block, $C^T$, is an ordered list of transactions,  drawn from a data structure similar to the Bitcoin \texttt{mempool}, except in Bitcoin, \texttt{mempool} stores all transactions that have not yet been included in the main chain; in Prism, once a transaction is included in a valid transaction block, it is permanently removed from the \texttt{mempool}.
This is because the transaction block (hence its contained transactions), is guaranteed to eventually be included in the ledger (\S\ref{sec:confirmation}).
Upon receiving a new transaction block over the network, the miner should remove the transactions in the new block from its own mempool and transaction block content. 

\emph{Proposer sub-block $B^P$:} 
Proposer tree is built in a longest-chain fashion; proposer blocks choose as their parent $P^P$  the tip of the longest chain in the proposer tree. 
Each proposer block's content, $C^P  :=(C^P_1, C^P_2)$, is an ordered list of references to other proposer and transaction blocks, where
$C^P_1$ is an ordered list of proposer blocks that are neither referenced nor among content of $B^P$'s ancestor block\footnote{ Ancestor blocks are computed by following the chain of links from $B^P$ in the prop. tree.}, and
 $C^P_2$ is an ordered list of transaction blocks that are not referenced (directly or indirectly) by any of $B^P$'s ancestors or by any of the proposer blocks in $C^P_1$.
% Note that $C^P$ actually stores references to the listed blocks.
A miner updates content $C^P$ upon receiving a new transaction block or a new proposer block. 
% The miner chooses a parent $P^P$ and block contents $C^P$ as described in  \S\ref{sec:blocktypes}. 
% That  is, miners store a list of references to proposer and transaction blocks that have not been referenced by any other proposer blocks in $B^P$'s ancestry. 
% In the former case, it can choose to add a reference to the new transaction block to the miner's proposer block content.
% In the latter case, if the newly-received proposer block is at the same level as the miner's in-progress block, the miner should update the in-progress proposer block's parent so as to extend the longest chain and also update the content $C^P$.
%(\vb{and the content?)} \ma{yep, i think it should be `parent and content'}. 

\emph{Voter sub-block $B^{V_i}$ in the $i^{th}$ voter tree:} 
Voter trees are also  built in a longest-chain fashion; the  parent of voter block  $B^{V_i}$, $P^{V_i}$, is the tip of the longest chain in the $i^{th}$ voter tree.
The content, $C^{V_i}$, is a list of references to proposer blocks, or \emph{votes}.
% , and the \emph{height} $h$ of the proposer tree is the maximum level that contains any proposer blocks.
Each voter tree's longest chain is allowed to vote at most one proposer block on any level\footnote{
Level of a proposer block is its distance from the genesis block.} of the proposer tree.
Let $h$ denote the last level in the proposer blocktree and $\ell_B$ denote the last level voted by $B_{V_i}$'s ancestors.
% For a voter block $B^{V_i}$, let $\ell'_{B}$ be the latest level of proposer block voter by $B^{V_i}$'s ancestors and thus $B^{V_i}$ has to vote on levels $\{\ell'_{B}+1,\cdots,h\}$.
% let $L'_{B}$ denote the set of levels that have already been voted on by $B$'s ancestors. (\vb{$L'_{B}$ is a continuous set. To simplify the notation we can say that `for voter block $B$, let $\ell'_{B}$ be the latest level of proposer block voter by $B$'s ancestors and thus $B$ has to vote on levels $\{\ell'_{B}+1,\cdots,h\}$})
% Let $L_{B} = L \cap L'_{B}$ be the set of remaining levels, and let $\mathcal P_i$ denote the set of proposer blocks at level  $i$. \gw{You mean $L - L'_B$?}
Then the content of the voter block $B^{V_i}$ is $C^V := [B^P_{\ell'_{B}+1},\ldots,B^P_{h}]$, list of proposer blocks where with some abuse of notation, $B^P_{\ell}$ denotes a vote for  (pointer to) a proposer block at level $\ell$. 
In words,  the voter block contains a list of one vote per unvoted level in the block's ancestors. 

% The miner chooses a parent $P^{V_i}$ as described in   \S\ref{sec:blocktypes}. 
% Its content $C^{V_i}$  is references to one proposer block on each level that have not yet been voted on by any of its ancestors. 
% \ma{Feels a bit repetitive with 4.1, but i think it's OK}
By default, nodes will vote for the first proposer block they see at a given level.
Notice that the content $C^{V_i}$ is updated if the miner receives either a new proposer block at a previously-unseen level or a new voter block for the $i^{th}$ tree that changes the longest chain of that voter tree. 
In  the former case, the miner adds a vote for that level. 
In the latter case, the miner updates its parent block $P^{V_i}$ so as to extend the longest chain and also updates the content $C^{V_i}$.
All the contents and parent links are concatenated into a superblock $B=(H,C)$ with header 
$H=(P:=[P^T,  P^P, P^{V_1}, \ldots, P^{V_m}], n, D)$ 
% \ma{nit. do we need the $\emptyset$?} \vb{nope..}
and content 
$ C := [ C^T, C^P, C^{V_1}, \ldots, C^{V_m}]$.
The content digest $D$ is explained next.


\noindent \textbf{(2) PoW and sortition.}
Once the superblock is formed, the miner mines by searching for a nonce $n$ such that $Hash( H)\leq q$, where $Hash(\cdot)$ denotes a hash function, and $q$ denotes a difficulty threshold. 
For a one-way hash function, the miner can do no better than brute-force search, so it cycles through difference values of nonces $n$ until  finding one such that $Hash(H) \leq q$. Upon finding a valid nonce,  sortition  occurs. 
We divide the numbers from $0$ to $q$ into regions corresponding to different block types. 
For example, $[0,q_T]$ denotes a transaction block, $[q_T+1,q_P]$ denotes a  proposer block, and $[q_P+1,q]$ denotes voter blocks,  split evenly into  $m$ regions, one per voter tree.
The output region of $Hash(H)$ determines the block type.


\noindent \textbf{(3) Block pruning.}
Passing around a large superblock after mining would waste unnecessary bandwidth. 
Hence, to improve space efficiency, instead of using the full concatenated parent block and content lists, only the relevant content is retained after mining and the type of the block is known.
For example, a mined proposer block would contain only the proposer parent reference , $P^P$, and proposer content, $ C^P$; it would \emph{not} store transactions or votes.
However,  if we do this naively, block validators would not be able to tell if the cryptographic sortition was correctly executed.
To address this, we alter our header to contain the following:
$H=\left(\textsf{MerkleRoot}(P), n, D := \textsf{MerkleRoot}(C)\right)$, 
 where $\textsf{MerkleRoot}(\cdot)$ denotes the Merkle root of a Merkle tree \cite{merkle} 
%  \ma{cite something for Merkle tree} 
generated from the contained array.
%To avoid the overhead of including all $m+2$ parents and content hashes in every block, Prism block headers contain: a) the Merkle root of a tree with $m+2$ parent blocks, b) the Merkle root of a tree with $m+2$ contents, and c) a nonce. \gw{"a)" is different from our implementation. In implementation, every block has a proposer parent. And every voter block has a voter parent which is stored inside content.}
%Upon finding a valid nonce, the hash of the block deterministically determines if the block is a proposer block, a transaction block, or a voter block on one  of the $m$ voter trees.  
%The mined, sortitioned block includes a header, the appropriate parent and content for the soritioned block type, and the respective Merkle proofs.
In addition to the pruned content and header, we include \textit{sortition proofs}, Merkle proofs attesting to the fact that the block  was mined correctly.
In our proposer block example, the Merkle proof would include the sibling node for every  node in the path from the proposer content $C^P$ to the root $\textsf{MerkleRoot}(C)$ in the Merkle tree. 
Hence $\textsf{MerkleProof}( C)$ (resp. $\textsf{MerkleProof}(P)$) is an array of  size $\log_2 (m)$ -- a primary source of storage overhead in Prism blocks. 


\noindent \textbf{(4) Block validation.}
Upon  receiving a mined Prism block $B=(H,C)$, a validator checks two things. 
First, it  checks that $Hash( H) \leq q$ and that the cryptographic sortition is correct  (i.e., that the hash  maps to the correct region for the block type).
Next, it checks the sortition proof.  
To do this, it takes content $C$ (resp. parent) in  the block, and ensures that the Merkle proof validation gives the content (resp. parent) digest in the header \cite{merkle}. 
% \ma{This is perfect}


\begin{figure}
   \centering
   \includegraphics[width=\linewidth]{figures/ledger_generation.png}
   \vspace{-5mm}
    \caption{\small Ledger formation has three parts:  
   (1)  confirming a leader  sequence of proposer blocks;
   (2)  creating a list  of transactions;
   and (3) sanitizing the transaction list for conflicts. 
   In this figure, each transaction  block has only one transaction; suppose transactions  (c) and (d) are inconsistent (e.g., a double spend).
   A proposer block's black reference link denotes a parent link. 
    Blue links denote reference links; a proposer block can include reference links to transaction blocks as well as proposer blocks.}
   %   \gw{A typo: unrefererred $\to$ unreferred? Do we need to use the word unrefererred? Referred blocks are okay in links.}
%   Each shade of grey corresponds to an epoch. In Step 1 (line:\ref{code:txbksOrdering}), all the transaction blocks are incorporated, and in Step 2 (line:\ref{code:sanitizeLedger}), they are combined to build the ledger.
   \label{fig:leader_ledger}
    \vspace{-5mm}

 \end{figure}


\subsection{Ledger Formation}
\label{sec:confirmation}
% Unlike many blockchain designs, Prism allows transactions to be confirmed before they are ordered. 
% This is possible because confirmation is often an easier task than ordering. 
% For example, consider the following two transactions: a) Alice pays Bob 10\$, and b) Carol pays Drake 10\$. Both these transactions can be individually confirmed without deciding which transaction occurred first.
% The decision to separate transaction confirmation from ordering helps Prism achieve low latency. 
% However, as a result, conflicting or duplicate transactions can become part of the blockchain; these conflicts must be eliminated during transaction ordering (i.e., during ledger formation). 
% % It handles such conflicts by separating the process of confirming blocks and that of generating a ledger from the set of confirmed blocks. 
% % Without it, blockchains must maintain a single, self-consistent sequence of blocks; this causes simultaneously-mined blocks to be wasted, while slowing down the generation of the ledger. 
% % We separately discuss the two procedures of block confirmation and ledger formation. 

% \paragraph{Transaction confirmation}
Prism achieves high throughput in part by mining multiple transaction blocks simultaneously and allowing all of them to contribute to the final ledger. 
A key consequence is that blocks mined concurrently may contain redundant or conflicting transactions.
If Prism were to discard blocks that contain inconsistent transactions, it would needlessly reduce throughput by not confirming the transactions that \emph{are} consistent.
% This would also slow down transaction confirmation, because it means 
To prevent this, Prism separates the process of confirming blocks and forming a ledger. 
This is a key difference between Prism and many other blockchain protocols.
% Since the same transaction can appear in multiple Prism transaction blocks \ma{we need to give more context about why this is a problem. it's all about having a large number of transaction blocks in flight at the same time, so it's fundamentally impossible for a miner to know that a transaction it is mining has not already been included in some other transaction block by another miner}, transaction confirmation is not necessarily the same thing as transaction block confirmation. 
The formation of a ledger in Prism  occurs in three steps, as shown in Figure \ref{fig:leader_ledger}. 

\noindent{\bf (1) Proposer block confirmation.}
First, we must confirm a contiguous sequence of leader proposer blocks at each level.  
    Recall that the proposer block with the most votes on level $\ell$ is defined as the \textit{leader block} at level $\ell$, and the sequence of leader blocks for each level of the proposer tree is defined as the {\em leader sequence}. 
Once we can guarantee that this leader sequence is permanent for all levels up to some level $\ell$ with probability at least $1-\epsilon$, where $\epsilon$ is the target reversal probability, we can confirm a leader block sequence. This process is described in more detail below.

\noindent{\textbf{(2) Transaction  ordering.}}
    Given a proposer block leader sequence, we iterate over the sequence and list the referred transaction blocks in the  order they are referred. 
    We use $L_i$ to denote the leader at level $i$. 
    In Figure \ref{fig:leader_ledger}, we  start  with the leader at level 1 $L_1$, the left proposer block.
    $L_1$ refers to only one transaction  block containing transaction $a$, so our ledger starts with $a$.
    Next, we consider $L_2$. It starts by referring to its parent, the right proposer block at level 1.
    Since that proposer block has not yet been included in the ledger, we include its referred transactions---namely, $a$ and $b$. 
    $L_2$ then adds $L_1$, followed by transaction blocks containing $d$ and $c$, in that order.
    Since $L_1$ was already added to our ledger, we ignore it, but add $d$ and $c$.
    This process continues until we reach the end of our leader sequence.

\noindent{\textbf{(3) Ledger sanitization.}} In the previous step, we may have added redundant or conflicting transactions. 
    Hence, we now execute the transaction list in the previously-specified order. Any duplicate or invalid transactions are discarded. 
    In Figure~\ref{fig:leader_ledger}, we discard the second instance of $a$ (since it's a duplicate), and we discard $c$ (since it conflicts with $d$).

\if 0
\begin{enumerate}
    \item  \textbf{Proposer block confirmation.} First, we must confirm a contiguous sequence of leader proposer blocks at each level.  
    Specifically, the proposer block with the most votes on level $\ell$ is defined as the \textit{leader block} at level $\ell$. 
% This phenomenon is at the core of \schemenosp's security.
The sequence of leader blocks for each level of the proposer blocktree is defined as the {\em leader sequence}. 
Once we can guarantee that this leader sequence is permanent for all levels up to some level $\ell$ with probability at least $1-\epsilon$, we can confirm a leader block sequence. This process is described in more detail below.
    \item \textbf{Transaction  ordering.} 
    Given a proposer block leader sequence, we iterate over the sequence and list the referred transaction blocks in the  order they are referred. 
    We use $L_i$ to denote the leader at level $i$. 
    In Figure \ref{fig:leader_ledger}, we  start  with the leader at level 1 $L_1$, the left proposer block.
    $L_1$ refers to only one transaction  block containing transaction $a$, so our ledger starts with $a$.
    Next, we consider $L_2$. It starts by referring to its parent, the right proposer block at level 1.
    Since that proposer block has not yet been included in the ledger, we include its referred transactions---namely, $a$ and $b$. 
    $L_2$ then adds $L_1$, followed by transaction blocks containing $d$ and $c$, in that order.
    Since $L_1$ was already added to our ledger, we ignore it, but add $d$ and $c$.
    This process continues until we reach the end of our leader sequence.
    \item \textbf{Ledger sanitization.} In the previous step, we may have added redundant or conflicting transactions. 
    Hence, we now execute the transaction list in the previously-specified order. Any duplicate or invalid transactions are discarded. 
    In Figure \ref{fig:leader_ledger}, we discard the second instance of $a$ (since it's a duplicate), and we discard $c$ (since it conflicts with $d$).
\end{enumerate}

\fi
   
%   (3) Iterate over the transactions ledger and \emph{sanitize} it by  removing all  transactions  that conflict with a prior transaction.

% Ultimately, transaction confirmation hinges on confirmation of the proposer blocks that refer to transaction block(s) containing the transaction.
% A transaction block is confirmed once a proposer block pointing to the transaction block is confirmed.
% We thus start by explaining the confirmation of proposer blocks, then explain how this leads to transaction confirmation.


% Specifically, the proposer block with the most votes on level $\ell$ is defined as the \textit{leader block} at level $\ell$. 
% % This phenomenon is at the core of \schemenosp's security.
% The sequence of leader blocks for each level of the proposer blocktree is defined as the {\em leader sequence}. 
% Once we can confirm a contiguous leader sequence, e.g. at levels $1,\ldots, \ell$ with our desired reliability $1-\epsilon$, we can confirm an ordered ledger of transactions. 
% This ledger is formed by iterating over the sequence, and for each leader block, looping over all the transaction blocks referenced within. 
% The list of transactions from each transaction block is added sequentially to the ledger; each transaction's validity is checked for validity (e.g., double spends) and duplicate entries (since the same transaction can be added to multiple transaction blocks). 
% This process is illustrated in Figure \ref{fig:leader_ledger}. \ma{I don't really like Fig. 6. It would be better to create an example which actually shows duplicate transactions and double spends after the ordering step, and than shows the sanitized ledger. BTW, the step of going from ordered transaction blocks to order transactions doesn't seem that important (it's pretty obvious). But the most important point is that you have to do sanitization, and this has to be done after transactions are ordered. }


%\paragraph{Proposer block confirmation.} 
\smallskip
The key to the above confirmation process is leader proposer block confirmation (step 1).
The leader block at a given level $\ell$ can initially fluctuate when the voter trees start voting on level $\ell$. 
However, as the voter trees grow, votes on level $\ell$ are embedded deeper into their respective voter trees, which (probabilistically) prevents the votes from being reverted.
% A leader proposer block at a given level $\ell$ is confirmed based on the votes of the voter trees. 
Hence, we can confirm the leader block when: (1) a plurality of voter trees have voted for it, and (2) that plurality is guaranteed not to change with probability at least $1-\epsilon$, where $\epsilon$ is a user-selected target reversal probability.

%Because there are many voter trees, each individual voter tree needs  only a weak confirmation guarantee to still give a strong confirmation guarantee to the aggregate majority vote. 
% \gw{Do we need to define what is weakly confirm?}

Our confirmation procedure calculates this probability by computing a $(1-\epsilon)$-confidence interval over the number of votes on each leader block, as well as a hypothetical ``private'' block that has not yet been released by a hypothetical adversary that controls a fraction $\beta$ of the hash power. 
Once the leader block's confidence interval is strictly larger than any of the other candidates' confidence intervals, we can be sure (with probability at least $1-\epsilon$) that the current leader will remain the leader for all time, so we confirm that proposer block. 
The details of this confidence interval calculation are included in Appendix~\ref{apx:confirmation}.

\subsection{Spam Mitigation}
\label{sec:spamming-design}

In Prism, miners do not validate transactions before including them in blocks.
This introduces the possibility of spamming, where an adversary could generate a large number of conflicting transactions and send them to different nodes across the network.  
The nodes would then mine all of these transactions into blocks, causing miners and validators to waste storage  and computational  resources.\footnote{While a discussion of incentives is beyond the scope of this paper, it is important to note that fees alone cannot prevent such spamming. Assuming nodes only pay for transactions that make it to into the ledger, the adversary would not be charged for conflicting transactions that get removed during sanitization.}
%spam/duplicate transactions
% There are a few practical mechanisms for circumventing this. 
Notice that protocols like the longest chain are not susceptible to this attack because transactions are validated prior to block creation. 
We propose a simple mechanism to mitigate spamming. Miners validate transactions with respect to their latest ledger state and other unconfirmed transactions, giving the adversary only a small window of network delay to spam the system. 
This then allows miners to mitigate spamming attacks by adding a random timing jitter prior to mining transactions, thus increasing the chance that a miner can detect that a conflicting transaction is already present in a transaction block, in  which case it will choose to not include that transaction.
We evaluate the effectiveness of this method in \S\ref{sec:spamming-eval}.

% \smallskip


%We believe such practical countermeasures will be important in  practical settings.
%mitigations:  jitter,  mempool optimization, sortition? 

%\ma{more generally, i think we need to expand this section to explain the important parts of the design in more detail. I don't think the long pseudocode blocks are that helpful. no one will read them, and they don't distinguish the important stuff from the mundane. let's remove the pseudocode to make room to expand on things like: (1) more formal description of block contents (a diagram might help); (2) what exactly is the proof of work puzzle in prism; (3) how does sortition work; (4) how do you get the final block that is sent over the network; (5) how do we get a ledger from all these blocks; (6) how does transaction confirmation work; how and why is it different from bitcoin. there might be other stuff worth mentioning, but we should ideally describe at least each of these points at a decent level of detail} 




% Consider a proposer block sequence from levels $1$ to $\ell$, $\{p_1,\cdots,p_{\ell}\}$, represented by blue blocks in Fig. \ref{fig:leader_ledger}(a).
% Let $L_{p_i}$, represented by green blocks in the grey shaded area in Fig. \ref{fig:leader_ledger}(a), be an ordered list of all the transaction blocks directly or indirectly referred by block $p_i$. 
% Let $\{L_{p_1}, \cdots, L_{p_{\ell}}\}$ be the \textit{transaction block list} of sequence $\{p_1,\cdots,p_{\ell}\}$ as shown in Fig. \ref{fig:leader_ledger}(b). 
% We consider this transaction block list confirmed once each proposer block in the underlying sequence is confirmed. 
% Our proposer block confirmation policy is a simplified version of the policy from \cite{prism}. 
% To confirm a proposer block as leader with reliability parameter $\epsilon$, we consider the votes from all $m$ voter trees. 
% Each voter tree has some maximum probability of ending up with a vote against the block at level $1\leq i \leq \ell$.
% Once we


% While confirming a leader block can take time, 
% we quickly narrow down a set of proposer blocks, defined as the \textit{proposer set}, which is guaranteed probabilistically to contain the eventual leader block for that level. 
% The proposer set is defined as in \todo{XXX--HOW MUCH DETAIL DO WE WANT TO GO INTO? }
% % This procedure first gets all the votes from the voter trees and then gets the proposer set for each 
% % level from the genesis to the last level for which the proposer set can be realized (lines:\ref{code:getvotes_start}-\ref{code:appendPrpList}). 
% Upon  defining a proposer set for each realizable level, Prism takes an outer product of all the proposer sets to  enumerate the set of all possible proposer block leader sequences (line:\ref{code:outerproduct}). 
% Note that by design, one of these sequence will eventually be the leader block sequence.
% It then builds a ledger for each of these proposer block sequences and confirms the given transaction if it is present in \textit{all} of these ledgers (lines:\ref{code:ledgers_for_start}-\ref{code:fastConfirmTx}). 



% \textit{Confirmation and Ordering:} A set of transactions can often be individually confirmed before being ordered among themselves. 
% For this reason, confirming transactions is easier than ordering the transactions.
% For example, consider the following two transactions a) Alice pays Bob 10\$, and b) Carol pays Drake 10\$. Both these transactions can be individually confirmed without deciding which transaction occurred first.
% In Bitcoin, transactions are simultaneously confirmed and ordered; 
% however, in Prism, transactions can be confirmed before being ordered.
% The procedure \textsc{IsTxConfirmed()} in Algorithm \ref{alg:prism_con} defines the transaction confirmation rule $g$ and the procedure \textsc{GetOrderedConfirmedTxs()} defines the rule for ordering the confirmed transactions. Both these procedures use \textsc{BuildLedger()} which is described next.



% \paragraph{Transaction Ordering}
% Once a sequence of leader blocks is confirmed, the ledger is formed by iterating over the sequence, and for each leader block, looping over all the transaction blocks referenced within. 
% The list of transactions from each transaction block is added sequentially to the ledger; each transaction's validity is checked for validity (e.g., double spends) and duplicate entries (since the same transaction can be added to multiple transaction blocks). 
% This process is illustrated in Figure \ref{fig:leader_ledger}(c). 




%\ma{let's move discussion of spamming to the discussion section}


==> discussion.tex <==

\section{Discussion}
\label{sec:discussion}

% \ly{
% \begin{enumerate}
%     \item throttling
%     \item Compare with existing blockchain protocols and discuss their practicability (performance on a store-and-forward network)
% \end{enumerate}
% }

We discuss some potential extensions to \prism.


% \smallskip

 
% \smallskip
\noindent \textbf{Light clients.} 
 SPV (Simple payment verification) are short proofs~\cite{spv} to verify the validity of a given transaction (payment) for a \textit{light user} who only downloads the blocks headers in a blockchain.
In the longest chain protocol, every transaction in the block is valid so a Merkle proof of a transaction with respect to its block header proves payment validity.
However, this is not enough in \prism, where transaction blocks can potentially contain invalid transactions. We can facilitate SPV proofs in \prism by this simple modification: We store all the unspent coins in the ledger formed by leader blocks until level $\ell$ in a Merkle-Patricia tree and add the root of this tree to the proposer block(s) at level $\ell+e$ (for a large value of $e$, say $20$). Since this tree contains only unspent coins generated by valid transactions, the merkle proof of the output coins of a payment with respect to to this commit proves the validity of the payment.

% \smallskip
\noindent \textbf{Bootstrapping a new user.} 
Longest chain blockchains like Bitcoin use a small fraction of network bandwidth, so new users can simply download and process all the blocks to join the system. 
Since Prism runs near network capacity,  expecting a new user to download and process all the old blocks is not practical. 
The modification suggested in the previous paragraph can be also used to bootstrap as follows: a new user downloads all proposer and voter tree blocks (which consume less than $0.1\%$ of the capacity). Say the new user's proposer tree has confirmed leader block at level $\ell$. 
We know that this leader block stores the commit of all the unspent coins up to level $\ell-e$. 
Now the new user asks an existing user for the UTXO set for the ledger up to level $\ell-e$. The user can verify the correctness of this set by comparing it with the UTXO set commitment stored in the leader block at level $\ell$.
% \gw{"the commit of stored the leader block" contains a typo?}
This UTXO set contains all the information required from transaction blocks
% \gw{can we abbr transaction to tx?}
referred by proposer blocks until level $\ell-e$ and thus the new user can join the system by downloading full blocks starting from level $\ell-e$.



\noindent \textbf{Smart contracts.} 
 Our current implementation achieves high throughput and low latency on an UTXO based scripting layer. 
 A natural question is whether we can achieve similar performance on a smart contract layer. 
 \prism's latency depends only on the block structure at the consensus layer and is independent of the scripting layer. Thus a smart contract version of Prism will also achieve low confirmation latency. As described in \S\ref{sec:scoreboarding}, parallelizing transaction execution (via \textit{scoreboarding}) was vital in achieving high throughput. The ability to parallelize transaction execution of smart contracts will also be the key to exploit the high throughput provided by \prism consensus. 
 
 
 %%As described in section  \ref{sec:scoreboarding}, parallelizing transaction execution via \textit{scoreboarding}~\cite{scoreboarding} was vital in achieving high throughput. This technique can be extended to parallelize execution of a more generic scripting layer such as smart contracts and this is left for future work.


==> figures/prism-chains.tex <==
\tikzstyle{proposer} = [draw, fill=blue!20, rectangle, rounded corners, minimum height=1em, minimum width=1.6em, text centered]
\tikzstyle{voter} = [draw, fill=green!20, rectangle, rounded corners, minimum height=1em, minimum width=1.6em]
\tikzstyle{transaction} = [draw, circle, fill=yellow!20]

% The block diagram code is probably more verbose than necessary
\begin{tikzpicture}[auto, node distance=0.8cm,>=latex']
\node [proposer] (p0l) {\tiny L};
\node [proposer, below of=p0l] (p1l) {\tiny L};
\node [proposer, left=0.1cm of p1l] (p1s) {};
\node [proposer, below of=p1l] (p2l) {\tiny L};
\node [proposer, right=0.1cm of p2l] (p2s) {};
\node [proposer, below of=p2l] (p3l) {\tiny L};

\node[transaction, above left = 0.01cm and 0.45cm of p0l] (t00){};
\node[transaction, below right = 0.06cm and 0.02cm of t00] (t01){};
\node[transaction, left = 0.25cm of p1s] (t10){};
\node[transaction, above right = 0.07cm and 0.02cm of t10] (t11){};
\node[transaction, below right = 0.10cm and 0.07cm of t10] (t12){};
\node[transaction, below left = 0.05cm and 0.25cm of p2l] (t20){};
\node[transaction, above left = 0.07cm and 0.13cm of t20] (t21){};
\node[transaction, left = 0.35cm of p3l] (t30){};
\node[transaction, above left = 0.05cm and 0.11cm of t30] (t31){};
\node[transaction, left = 0.25cm of t30] (t32){};
\draw[densely dashed, <-] (t00)  to [looseness=0.4] (p0l);
\draw[densely dashed, <-] (t01)  to [looseness=0.4] (p0l);
\draw[densely dashed, <-] (t10)  to [looseness=0.4] (p1l);
\draw[densely dashed, <-] (t11)  to [looseness=0.4] (p1l);
\draw[densely dashed, <-] (t12)  to [looseness=0.4] (p1l);
\draw[densely dashed, <-] (t20)  to [looseness=0.4] (p2l);
\draw[densely dashed, <-] (t21)  to [looseness=0.4] (p2l);
\draw[densely dashed, <-] (t30)  to [looseness=0.4] (p3l);
\draw[densely dashed, <-] (t31)  to [looseness=0.4] (p3l);
\draw[densely dashed, <-] (t32)  to [looseness=0.4] (p3l);


\node [voter, right=1cm of p0l] (v00) {};
\node [voter, below of=v00] (v01) {};
\node [voter, below of=v01] (v02) {};
\node [voter, below of=v02] (v03) {};
\draw[<-] (v00) to (v01);
\draw[<-] (v01) to (v02);
\draw[<-] (v02) to (v03);

\node [voter, right=0.3cm of v00] (v10) {};
\node [voter, below of=v10] (v11) {};
\node [voter, below of=v11] (v12) {};
\node [voter, below of=v12] (v13) {};
\draw[<-] (v10) to (v11);
\draw[<-] (v11) to (v12);
\draw[<-] (v12) to (v13);

\node [right=0.3cm of v10] (space0) {$\cdots$};
\node [below of=space0] (space1) {$\cdots$};
\node [below of=space1] (space2) {$\cdots$};
\node [below of=space2] (space3) {$\cdots$};

\node [voter, right=0.3cm of space0] (v20) {};
\node [voter, below of=v20] (v21) {};
\node [voter, below of=v21] (v22) {};
\node [voter, below of=v22] (v23) {};
\draw[<-] (v20) to (v21);
\draw[<-] (v21) to (v22);
\draw[<-] (v22) to (v23);

\draw[densely dashed, <-] (p0l)  to [looseness=0.3] (v00);
\draw[densely dashed, <-] (p1l)  to [looseness=0.3] (v01);
\draw[densely dashed, <-] (p2l)  to [looseness=0.3] (v02);
\draw[densely dashed, <-] (p3l)  to [looseness=0.3] (v03);

\draw[densely dashed, <-] (p0l)  to [looseness=0.3] (v10);
\draw[densely dashed, <-] (p1l)  to [looseness=0.3] (v11);
\draw[densely dashed, <-] (p2l)  to [looseness=0.3] (v12);
\draw[densely dashed, <-] (p3l)  to [looseness=0.3] (v13);

\draw[densely dashed, <-] (p0l)  to [looseness=0.3] (v20);
\draw[densely dashed, <-] (p1l)  to [looseness=0.3] (v21);
\draw[densely dashed, <-] (p2l)  to [looseness=0.3] (v22);
\draw[densely dashed, <-] (p3l)  to [looseness=0.3] (v23);

\end{tikzpicture}

==> implementation.tex <==
\section{Implementation}
\label{sec:implementation}

We have implemented a basic Prism client and wallet in about 10,000 lines of Rust code. We describe the architecture of our implementation and several design decisions that are key to its high performance.




\begin{figure}[t]
\begin{center}
\includegraphics[width=3.2in]{prism.png}
\end{center}
\caption{\label{fig:prism-system} Prism system diagram. \todo{Add persistent storage for raw blocks?}}
\end{figure}

\subsection{Architecture}

Our implementation features a simplified version of Bitcoin's scripting language, processing only pay-to-public-key (P2PK) transactions, similar to that implemented in Algorand~\cite{algorand, algorandcode}. \ma{talk about UTXO here}


Although Prism is compatible with more complex scripting languages (e.g., smart contracts), we made this choice to enable a fair comparison with other baselines \cite{algorand,ohie},
% \ly{is "alogrand1" the theory paper?} 
which make a similar choice in their  implementations \cite{ohiecode,algorandcode}. \ma{I'm not sure we should claim too strongly that Prism, as is, is compatible with smart contracts. For instance, I'm not entirely sure how miners should execute a smart contract without knowing the state of the ledger (e.g., VM state) on top of which they are mining.}
% Hence, the following design decisions will be based on the assumption that the system is processing only P2PK transactions. 


Our system architecture is illustrated in Figure \ref{fig:prism-system}. \ma{this is a useless figure!}
At a high level, it is divided into various handlers running on separate threads:
\begin{enumerate}
    \item {\em Peer handler},  which parses messages passed over the network; these messages can encapsulate protocol-relevant information such as relayed blocks.
    \item {\em Transaction/block handlers}, which process new transactions or blocks as they arrive. % For parallelism, these handlers are deployed in a worker pool with 16 threads.
    \item {\em Miner}, which updates the miner's context, i.e., its current estimate of what votes to cast and how to structure each of its block types. \gw{There are two "miner"s in this sentence and it may cause confusion.}
    \item {\em Ledger generator}, which periodically updates the confirmed order of transaction blocks. \ma{The ledger generator also updates the pending list of transactions as it confirms transaction blocks. (Is this correct? Which component is responsible for removing transactions that are already in some transaction block from the pending transaction list? I assume that can happen without  confirmation.}
    \item {\em Sanitizer}, which applies the confirmed sequence of transaction blocks to the UTXO set. \ma{Explain when this is run. It's everytime following ledger generation?}
\end{enumerate}

\ma{talk about which components have multiple threads to enable parallelism (transaction/block handlers, ledger generater/sanitizer?) and which run as a single thread}  

First, we have a network server, or \emph{peer handler}, that parses messages passed over the network; 
these messages can encapsulate protocol-relevant information such as relayed blocks.
Next, we have a worker pool of 16 threads that are opportunistically deployed as \emph{transaction or block handlers}, depending on what the system needs at a given point in time. 
These handlers deal with new transactions or blocks; because blocks are produced at such a high rate in Prism, parallelism is needed to prevent this processing from becoming a system bottleneck. 
Third, we have a \emph{miner thread}, which updates the miner's context, i.e., its current estimate of what votes to cast and how to structure each of its block types.
The \emph{ledger generation} thread periodically updates the confirmed order of transaction blocks. \gw{\emph{ledger generation} thread or ledger generator?}
Finally, the \emph{sanitization} thread applies the confirmed sequence of transaction blocks to the unspent transaction output (UTXO) set. \gw{Sanitization actually has multiple threads?}
Because ledger generation and sanitization are operating at a high rate on closely-related data, we use the scoreboarding technique from computer architecture to ensure that these processes are self-consistent.
This will be discussed further in Section \ref{sec:key_design}. \ma{I think i covered all of this.}

\smallskip
\noindent{\bf Persistent storage.} Discuss all the databases. Block database. Block DAG database (this only maintains graph structure, i.e. there aren't two copies of actual blocks). UTXO database. Wallet database (is this one important to explain. it seems this could have been a separate piece of software anyway). 

\smallskip
\noindent{\bf In-memory state.} Unresolved blocks. Mempool. Highly accessed DBs are cached in memory -- explain.


We have six types of storage. 
The first is the \emph{block database}, which stores raw blocks.
Related to the block database, the \emph{blockchain database} stores the DAG-structured relation between blocks.
Both are stored in persistent storage backed by RocksBD \cite{}.
The \emph{UTXO database} stores the set of unspent coins, and the \emph{wallet database} stores a user's own unspent coins. 
Both the UTXO and wallet databases are also kept in persistent storage (RocksDB) to enable our implementation to run for long periods of time without running out of memory. 
The \emph{unresolved blocks} database stores blocks that contain pointers to blocks that have not yet been received; 
whenever a new block is received over the network,  this database is accessed to attempt to resolve already-received blocks. 
The unresolved blocks database is stored in memory, as it does not grow with time. \ma{It doesn't grow with time only if the system is behaving correctly, right? If under attack, one could easily get a huge number of unresolved blocks. We'll have to revisit this decision.} 
Similarly, the memory pool (mempool) stores received transactions that have not yet been mined into a transaction block. 
The mempool is also stored in memory.






\subsubsection{Implementation Design Decisions}
\label{sec:key_design}
Here we outline a number of implementation design decisions that affect our performance metrics. 
Many of these issues arise implicitly in related literature \cite{ohie,algorand,conflux}; we highlight them explicitly to facilitate a fair comparison.


\paragraph{Asynchronous confirmation} 
% More tolerant on delays and frequent shift of longest chains.
In classical blockchains like Bitcoin, every block generally confirms a new set of transactions in the ledger. 
This is not the case in Prism, where confirmation occurs based on the aggregate behavior of many blockchains: each new block is individually unlikely to confirm a new transaction. 
For this reason, we have decoupled the processing of blocks from transaction confirmation by using a separate thread to periodically check the confirmation status of transactions. \gw{This thread is ledger generator?}
This wastes less processing power than checking each transaction's confirmation status every time a new block is received, and alleviated a system bottleneck for us.


\paragraph{Parallel transaction execution} 
The \emph{state} of a P2PK blockchain is the set of unspent transaction outputs, also known as the UTXO set. 
Processing transactions requires both evaluating their validity and executing them, i.e., updating the state. 
Both of these processes require accessing the UTXO database, often in quick succession. 
However, because we operate at high throughput levels (tens of thousands of transactions per second), these database accesses quickly become a bottleneck if processed sequentially. 
Hence,  we have a worker pool of eight threads accessing the UTXO database for simultaneous transaction processing. \ma{These threads are distinct from the event handler threads described in 4.1?} 
To avoid race conditions, we implement scoreboarding. \ma{We definitely need to explain this in more detail}
\todo{Lei, add more details here?}
We expect that this implementation choice would have even greater repercussions for more complex scripting languages, since the cost of processing each transaction increases. 
% (benchmark and show the advantage of parallel execution, note that the advantage on more complex transactions could be higher.)

\paragraph{State updates} 
Each node maintains a local copy of the state; different nodes' views of the state may differ due to network delays. 
In a real blockchain \ma{what do you mean `real blockchain'? traditional blockchains?}, nodes update their local state each time a new transaction is processed; this update involves checking the validity of each transaction by ensuring that the transaction draws only upon valid UTXOs, and updating the corresponding UTXO database. 
Several academic blockchain implementation papers have chosen not to implement state updates \cite{algorand,ohie}, instead generating random transactions that are not necessarily valid with respect to the current state. 
Nodes in turn do not check the validity of these transactions. 
This design choice reduces the computational load of transaction validation, which can be a substantial bottleneck in high-performance blockchains. 
Indeed, we find that state updates (e.g., transaction validation and processing updates to the UTXO database) are a bottleneck in our current implementation. 
Notice that this will also be the bottleneck in efficient centralized implementations. \ma{This discussion of previous implementations should go in the related work section. The purpose of this section is to discuss our implementation, and what we had to do to achieve good performance. So the more relevant question here is, what enables our implementation to achieve fast state updates}

% For example, Figure \ref{} illustrates the difference in throughput achievable in our implementation when we disable state updates. 
% We observe up to a \red{XXX}\% difference. 

% Talk about how many academic implementations choose to not include state updates for efficiency, which ends up being a bottleneck in practice. Show plots comparing with and without state updates. 

\paragraph{Transaction broadcasting}
Most blockchains broadcast transactions prior to incorporating them into blocks. 
This is done because it is unknown ahead of time which node will mine the next block, so transactions are widely disseminated to ensure that they are included in a block as quickly as possible. 
In contrast, our implementation does not broadcast transactions.
Prism generates blocks at much higher rate than other blockchain protocols. 
This elevated block rate means that any individual miner is likely to mine a transaction block in time comparable to the delay associated with broadcasting a block to the rest of the network (i.e., seconds).
Hence, unlike other blockchain protocols, there is little incentive for a Prism miner to broadcast its transactions.
In practice, non-mining nodes can transmit their transactions to one or more miners; however, those miners need not relay the transaction for the same reason as before.
 % Indeed, even miners may choose to broadcast transactions to ensure that their own transactions are confirmed as quickly as possible. 
% This broadcasting process may consume additional computational and network resources that are not modeled in our implementation. 
% However, such overhead can easily be limited by throttling the amount of computation and/or bandwidth used for transaction relaying. 
% In a high-performance Prism implementation, the bulk of the computation and bandwidth should be spent on processing and relaying blocks.
We want to emphasize that this decision to not broadcast transactions is \emph{not} the same thing as sharding the blockchain; all transactions end up on the same main chain and therefore have the same security guarantees. \ma{we should explain that there's nothing preventing miners from broadcasting transactions, and the impact on performance won't be significant. this is an optimization to reduce network bandwidth consumption} 
% Talk about fact that we do not broadcast transactions, why this is ok, and mention that other implementations do the same. 

\paragraph{Mining simulation} Like other academic implementations of PoW systems \cite{ohie,conflux}, we do not implement the actual proof-of-work loop used to generate blocks.
Instead, we simulate the time to mine a block by drawing an exponentially-distributed random delay for each block. 
This is done for two reasons:
first, simulating PoW wastes energy for no reason, since we have good analytical models of the (random) mining time. 
Second, in practice, PoW will happen primarily on dedicated hardware (e.g., ASICS), so the cost of mining will not contribute to the computational bottlenecks of the consensus protocol. 
Therefore, this simplification does not introduce unrealistic artifacts. 



==> intro.tex <==

\section{Introduction}

In 2008, Satoshi Nakamoto invented \bitcoin and the concept of {\em blockchains}~\cite{bitcoin}. Since then, blockchains have attracted considerable interest for their applications in cross-border payments~\cite{hileman2017global,kazan2015value}, digital contracts~\cite{cong2019blockchain,wust2018you,pilkington201611} and more. At the heart of \bitcoin and many other blockchain projects is the {\em Nakamoto longest chain protocol}. It enables an open (permissionless) network of nodes to reach consensus on an ordered log of transactions and is tolerant to Byzantine adversarial attacks with no more than 50\% of the compute power in the network. To achieve this high level of security, however, the longest chain protocol severely limits transaction throughput and latency  (\S\ref{sec:background}). \bitcoin, for example, supports 3--7 transactions per second and can take hours to confirm a transaction with a high level of reliability~\cite{bitcoin}.  

%Today's cryptocurrencies have poor transaction throughput and slow confirmation times. Bitcoin supports 3--7 transactions per second and can take hours to confirm a transaction with a high level of reliability~\cite{bitcoin}.  The root cause for this poor performance is the {\em Nakamoto longest chain protocol} (\S\ref{sec:background}), a Byzantine fault-tolerant consensus protocol that lies at the heart of Bitcoin and many other cryptocurrencies~\cite{buterin2016ethereum, citeothers}. Roughly speaking, the longest chain protocol enables an open (permissionless) network of nodes to reach consensus on an ordered log of transactions, provided that at least 50\% of the compute power in the network belongs to honest nodes that follow protocol. 

The limitations of the longest chain protocol have led to a flurry of work in recent years on more scalable blockchain consensus protocols (\S\ref{sec:related} discusses related work). However, until recently, no protocol has been shown to guarantee Bitcoin-level security (up to 50\% adversarial power) as well as high throughput and low latency. Prism~\cite{prism-theory} is the first such protocol. Prism is a Proof-of-Work (PoW) blockchain consensus protocol that is  (1) secure against 50\% adversarial compute power, (2) can achieve optimal throughput (up to the network communication bandwidth), and (3) can achieve near-optimal confirmation latency (on the order of the network's propagation delay). Prism removes the throughput and latency limitations of the longest chain protocol by systematically decoupling security and throughput in the blockchain  (\S\ref{sec:overview}).  
%transaction proposal, validation, and confirmation in the blockchain (\S\ref{sec:overview}). 
A recent theoretical paper described the core protocol and analyzed its security properties~\cite{prism-theory}.

While these theoretical results are promising, there are three main limitations. (1) First, the security analysis of \prism in \cite{prism-theory} is in a limited setting (round-by-round synchronous model with a finite time horizon of blockchain operation). Further, the theoretical latency guarantees for \prism \cite{prism-theory} involve large constants (that get larger with increasing time horizon of blockchain operation) -- this  results in  large values of latency in practice.  (2) Second,  the \prism consensus protocol is much more complex than the longest chain protocol: clients must maintain over 1000 distinct blockchains, which refer to each other to create an intricate directed acyclic graph (DAG) structure, and they must process blocks at very high rates (e.g., 100-1000s of blocks per second at 100s of Mbps) to update these blockchains and confirm transactions. %Second, Prism's theoretical analysis relies on several simplifying assumptions (e.g., round-based synchronous communication and a simple network model that ignores queuing delay), and to make the analysis tractable, the performance bounds are specified up to large constants that may not be indicative of real-world performance.  
(3) Third, Prism's theory focuses on the network as the primary performance bottleneck, but a real high-throughput blockchain system must overcome other potential performance bottlenecks. For example, in addition to achieving consensus on a transaction order, clients must also {\em execute} transactions and maintain the {\em state} of the ledger to confirm transaction. Though some academic prototypes ignore transaction execution (e.g., \cite{ohiecode, conflux}),
%\cite{cite-codebases-better-than-papers},
in practice, it often turns out to be the bottleneck due to its high I/O overhead, c.f.,~\cite{raju2018mlsm},  \S\ref{sec:eval-resource}.
Finally, Prism could be vulnerable to spamming, a practical security concern that has not been fully analyzed. 


% the performance of a blockchain system depends on more than the consensus protocol. The consensus protocol orders transactions, but to confirm them, the client must {\em execute} the transactions in order and keep track of the {\em state} of the ledger. 

\begin{figure} 
    \centering
    \includegraphics{figures/compare-fig.pdf}
    \caption{\small Throughput and confirmation latency of \prism, \algorand, \bng, and the longest chain protocol on the same testbed. Note that the axes are on log scales. For \algorand and the longest chain protocol, parameters are tuned to span an optimized tradeoff between throughput and latency at a given security level. For \bng and \prism, throughput and latency are decoupled so one can simultaneously optimize both at one operating point for a given security level. However, the throughput of Bitcoin-NG drops to that of the longest chain protocol under attack, while that of \prism remains high. More details in \S\ref{sec:related} and \S\ref{sec:eval-performance}. }
    \label{fig:compare}
    \vspace{-5mm}
\end{figure}

\noindent {\bf Main Contributions}. 
In this paper, we present the design (\S\ref{sec:design}) and  implementation (\S\ref{sec:implementation}) of a Bitcoin-like system based on the \prism consensus protocol. Our implementation features payments as multi-input-multi-output transactions (payments) similar to pay-to-public-key (P2PK) in Bitcoin and Algorand~\cite{algorand, algorandcode}. We evaluate our system on a testbed of up to 1000 EC2 Virtual Machines connected via an emulated wide area network. Figure \ref{fig:compare} summarizes the results. \prism consistently achieves a throughput of over 70,000 tps for a range of security levels $\beta$ denoting the fraction of adversarial compute power.  To guarantee a reversal probability of less than $10^{-9}$, \prism's latency ranges from 13 seconds against an adversary of power $\beta = 20\%$, to $296$ seconds for $\beta = 44\%$. To our knowledge, this makes our system by far the fastest  implementation of a blockchain system with Bitcoin-level security guarantees. Compared to the longest chain protocol, \prism provides about 10,000$\times$ higher throughput and 1,000$\times$ lower latency. Compared to Algorand~\cite{algorand}, the state-of-the-art proof-of-stake system, \prism achieves 70$\times$ the throughput with about 10 seconds higher latency, and can provide a higher level of security  (up to $\beta = 50\%$ vs. $\beta=33\%$ for Algorand).

We make the following contributions:
\begin{CompactItemize}
    \item We implement a Prism client in roughly 10,000 lines of {\tt Rust} code, and quantify its performance in extensive experiments on EC2. Our result validate Prism's core modeling decisions and theory by showing that it can scale both throughput and latency of the longest chain protocol (without compromising security) in a practical setting. Our code is available here~\cite{prismcode}.
    
    \item Our implementation highlights several performance optimizations, e.g., asynchronous ledger updates, and a scoreboarding technique that enables parallel transaction execution without race conditions (see ~\S\ref{sec:implementation-highlights}). We show that with these careful optimizations, it is possible to alleviate CPU performance bottlenecks and provide linear CPU scaling up to at least 8 cores. At this point, the primary bottleneck for our implementation is the underlying database (RocksDB~\cite{rocksdb} and I/O to the SSD persistent storage). This suggests that future research on databases optimized for blockchain-specific access patterns could further improve performance. 
    
    \item We evaluate practical security concerns like censorship attack, balancing attack, and spamming (see ~\S\ref{sec:eval-attack}). Additionally, we propose a simple solution to the spamming problem that reduces spam traffic by 80\% while only adding 5 seconds to the confirmation delay. Our implementation illustrates that \prism performs well even under these attacks, and makes a stronger case for the practical viability of the system.
    
\end{CompactItemize}

%Our implementation and evaluation provide several key takeaways. First, our results validate Prism's core modeling and design decisions in a practical setting by demonstrating that it can scale both throughput and latency of the longest chain protocol independently of one another without compromising the security guarantee. Second, our implementation shows that with careful performance optimization (see ~\S\ref{sec:implementation-highlights}), it is possible to alleviate CPU performance bottlenecks and provide linear CPU scaling up to \ma{XXX cores}. At this point, the primary bottleneck for our implementation is the underlying database (RocksDB~\cite{rocksdb} and I/O to persistent storage (SSDs)). Therefore future research on databases optimized for blockchain-specific access patterns could provide further performance improvements. 


% e.g., asychoronous ledger updates, and a scoreboarding technique that enables parallel transaction execution without race conditions. We show that these optimizations alleviate CPU performance bottlenecks and provide linear CPU scaling, such that the primary bottleneck is the underlying database (RocksDB~\cite{rocksdb} and I/O to persistent storage (SSDs)). Further performance improvements may therefore be possible by optimizing the database.

The rest of the paper is organized as follows. In \S\ref{sec:related} we discuss different scaling approaches taken in blockchains. In \S\ref{sec:background} we discuss the longest chain protocol and its limitations to motivate the design of the \prism protocol in \S\ref{sec:overview} and \S\ref{sec:design}. We discuss the details of the client implementation with an interface enabling pay-to-public-key transactions in \S\ref{sec:implementation}. Evaluations are presented in \S\ref{sec:eval} to assess the impact of network resources (bandwidth, topology, propagation delay) and computation resources (memory, CPU) on the overall performance. \S\ref{sec:conclusion} concludes the paper.


%%a host of related topics of core interest to the blockchain ecosystem; this includes interfacing Prism to a smart contract programming layer, introduction of light clients (which are simply interested in making and validating specific transactions) and bootstrapping new Prism clients into a running system - each of these is a future direction of research of great interest.


\if 0

% TODO: do we include performance here? Tell the performance first or explain the protocol first?

% TODO: if to compare the performance, what are the baselines? How to compare (cite numbers, run experiments, if so, do we need to optimize their code?) For some of them, modify Prism client into our impelmentation. For algorand, run their code. But what if their implementation is flawed? Explain the results we got (cause of the bottleneck), understand their bottleneck.

% comparisons: Algorand (fame, it could be that their paper is not doing real transactions. use their real code and try to reproduce the number in the paper), Bitcoin (longest chain), OHIE (parallel chain). Remember to point out the security level. This is FINAL.
% mentions: HotStuff
% Point that Conflux is copy cat
% Use Prism 1.0 to help rationale the protocol in Design section.
% Make other system actually do transactions

% Scale of the evaluation
% Hope that the scalability curves are flat, so that reader can assume the scalability (we could provide a breakdown of the CPU/IO resource spent)

% Mention that we have included all possible functions of the client so it is real.

% TODO: make full use of the code. Change parameters to show the idea of other systems.

Text...

Takeaways from experiments. Maybe insert a figure here. % TODO: possibilities: throughput - latency, different protocols take different positions (curve for parameterized ones)

% other potential comparisons: Conflux, Prism 1.0, Bitcoin-NG



Figure 1: comparison of throughput and latency with other blockchain protocols: 

Algorand - best permissionless PoS BFT protocol

longest chain - the original blockchain protocol (frontier as we vary mining rate and block size)

Ohie - parallel chain protocol (give state execution for free)

Prism - our protocol

Network setting (first draft)

100 nodes

artificial delay 300 ms per hop (exponential)

network bandwidth: whatever is sufficient for Prism to achieve 100K Tps. (around 200 to 300Mbps)


\fi


==> intro2.tex <==

\section{Introduction}

In 2008, Satoshi Nakamoto invented \bitcoin and the concept of {\em blockchains}~\cite{bitcoin}. Since then, blockchains have attracted considerable interest for their applications in cross-border payments~\cite{hileman2017global,kazan2015value}, digital contracts~\cite{cong2019blockchain,wust2018you,pilkington201611} and more. At the heart of \bitcoin and many other blockchain projects is the {\em Nakamoto longest chain protocol}. It enables an open (permissionless) network of nodes to reach consensus on an ordered log of transactions and is tolerant to Byzantine adversarial attacks with no more than 50\% of the compute power in the network. To achieve this high level of security, however, the longest chain protocol severely limits transaction throughput and latency. \bitcoin, for example, supports 3--7 transactions per second and can take hours to confirm a transaction with a high level of reliability~\cite{bitcoin}.  

%Today's cryptocurrencies have poor transaction throughput and slow confirmation times. Bitcoin supports 3--7 transactions per second and can take hours to confirm a transaction with a high level of reliability~\cite{bitcoin}.  The root cause for this poor performance is the {\em Nakamoto longest chain protocol} (\S\ref{sec:background}), a Byzantine fault-tolerant consensus protocol that lies at the heart of Bitcoin and many other cryptocurrencies~\cite{buterin2016ethereum, citeothers}. Roughly speaking, the longest chain protocol enables an open (permissionless) network of nodes to reach consensus on an ordered log of transactions, provided that at least 50\% of the compute power in the network belongs to honest nodes that follow protocol. 

\noindent {\bf Prism}. The limitations of the longest chain protocol have led to a flurry of work in recent years on more scalable blockchain consensus protocols (\S\ref{sec:related} discusses related work). 
However, a central challenge in the space has been to guarantee Bitcoin-level security (up to 50\% adversarial power) while also guaranteeing high throughput \emph{and} low latency. 
% \gf{Can we be more specific what we mean by ``high" throughput and ``low" latency? Otherwise reviewers may argue with this assertion}
Prism~\cite{prism-theory} was recently proposed as a solution to this problem.
Prism is a Proof-of-Work (PoW) blockchain consensus protocol that is theoretically shown to achieve (1) security against 50\% adversarial compute power, (2) optimal throughput (up to the network communication bandwidth), and (3) near-optimal confirmation latency. %\ma{This statement might seem in conflict with the claim in the next paragraph about Prism's current latency guarantees. Is there a better way to put this?}
% Prism removes the throughput and latency limitations of the longest chain protocol by systematically decoupling security and throughput in the blockchain.   
% %transaction proposal, validation, and confirmation in the blockchain (\S\ref{sec:overview}). 
% A recent theoretical paper described the core protocol and analyzed its security properties~\cite{prism-theory}.

\noindent {\bf Limitations of Prism}. 
While these theoretical results are promising, there are three main limitations. 
(1) First, the security analysis of \prism in \cite{prism-theory} is in a limited setting (round-by-round synchronous model with a finite time horizon of blockchain operation). The finite time horizon strictly limits the usability of the security in practice: the resulting confirmation error probability (i.e. the probability of a double-spend) depends on the duration of time horizon, getting worse as the time horizon increases.  
This shortcoming in turn forces the confirmation rule in \cite{prism-theory} to also depend on the finite time horizon, rendering the guarantees practically useless.
% and its theoretical latency bounds involving large 
% Further, the theoretical latency guarantees for \prism \cite{prism-theory} involve large constants that get larger with increasing time horizon of blockchain operation -- this  results in  high latency values in practice.  
(2) Second,  the \prism consensus protocol is more complex than the longest chain protocol: clients must maintain over 1000 distinct blockchains, which refer to each other to create an intricate directed acyclic graph (DAG) structure, and they must process blocks at very high rates (e.g., 100-1000s of blocks per second at 100s of Mbps) to update these blockchains and confirm transactions. 
A naive system design can easily introduce performance bottlenecks that would prevent Prism from achieving the theoretically-promised scaling properties.
For example, in addition to achieving consensus on a transaction order, clients must also {\em execute} transactions and maintain the {\em state} of the ledger to confirm transaction. Though some academic prototypes ignore transaction execution (e.g., \cite{ohiecode, conflux}),
%\cite{cite-codebases-better-than-papers},
in practice, it often turns out to be the bottleneck due to its high I/O overhead, c.f.,~\cite{raju2018mlsm},  \S\ref{sec:eval-resource}.
Unfortunately, \cite{prism-theory} does not explain how to design the Prism client architecture to avoid such bottlenecks. 
% It is unclear if a successful transition from algorithm to an efficient system design can be enabled.  %Second, Prism's theoretical analysis relies on several simplifying assumptions (e.g., round-based synchronous communication and a simple network model that ignores queuing delay), and to make the analysis tractable, the performance bounds are specified up to large constants that may not be indicative of real-world performance.  
(3) Third, to date there is no practical evaluation  of Prism's performance. \cite{prism-theory} provides simulations, but because of limitation (1), these simulations may not be indicative of real-world performance. 

%Finally, Prism could be vulnerable to spamming, a practical security concern that has not been fully analyzed. 

 

\begin{figure} 
    \centering
    \includegraphics{figures/compare-fig.pdf}
    \caption{\small Throughput and confirmation latency of \prism, \algorand, \bng, and the longest chain protocol on the same testbed. Note that the axes are on log scales. For \algorand and the longest chain protocol, parameters are tuned to span an optimized tradeoff between throughput and latency at a given security level (details in \S\ref{sec:eval}). 
    %\gf{This is confusing--it's not clear what parameter(s) are being varied in the Algorand and longest-chain curves. Should we add more detail?} \ly{details of tuning are provided in seciton 7.} 
    %\ly{The circle indicates the performance under the default parameters chosen by the original Algorand implementation.} 
     For \bng and \prism, throughput and latency are decoupled so one can simultaneously optimize both at one operating point for a given security level. However, the throughput of Bitcoin-NG drops to that of the longest chain protocol under attack, while that of \prism remains high. More details in \S\ref{sec:related} and \S\ref{sec:eval-performance}. 
    }
    \label{fig:compare}
    \vspace{-5mm}
\end{figure}

\noindent {\bf Main Contributions}. 
In this paper, we resolve each of these three  limitations of \prism.  Specifically: 
\begin{CompactItemize}
\item 
  {\bf Theory and Algorithms}. We  design a new, simple confirmation rule for \prism that does not depend on a finite time horizon for its security. 
  This new rule is designed to enable explicit identification of the worst-case adversarial attack, 
  which allows us to sharply characterize the confirmation error probability in    a  general, continuous-time  %cryptographic \ly{not sure if cryptographic is precise} 
  model over an infinite time  horizon of blockchain operation.  
  In general, identifying worst-case attacks on consensus protocols is considered challenging; our approach of co-designing a confirmation rule along with a worst-case attack is novel, to the best of our knowledge.
  This methodology also allows us  to sharply characterize the worst-case latency of confirmation, which we show to be a  small constant of the block interarrival time (e.g., for adversarial hash power $\beta$ of 20\%, the latency is roughly a factor of 12 of the block interarrival time). 
%   ; \prism decouples security of confirmation from latency). 
  This is elaborated in   \S\ref{sec:new_rule}.
  
  \item {\bf  Algorithms to System Design and Implementation}. We provide a system design of a Prism client that can be used to evaluate the theoretical performance scaling claims. The design includes several crucial performance optimizations, such as asynchronous ledger updates and a scoreboarding technique that enables parallel transaction execution without race conditions. We subsequently discuss the details of our implementation of a Prism client in roughly 10,000 lines of {\tt Rust} code.
  Our implementation features payments as multi-input-multi-output transactions similar to pay-to-public-key (P2PK) in Bitcoin and Algorand~\cite{algorand, algorandcode}, and includes several Prism-specific optimizations to enhance performance. 
%   Our implementation includes several optimizations
%   It also includes a simple, lightweight solution to out-of-model spamming attacks. 
  This system design is the focus of \S\ref{sec:design}.
  
  \item {\bf  Implementation and Evaluation}. 
  We evaluate our system on a testbed of up to 900 EC2 Virtual Machines connected via an emulated wide area network.   Our result (summarized in Figure~\ref{fig:compare}) validates Prism's core modeling decisions and the new confirmation rule by showing that it can scale both throughput and latency in a practical setting. 
  \prism achieves a consistent throughput of over 80,000 tps for different security levels $\beta$, denoting the fraction of adversarial compute power.  To guarantee a reversal probability of less than $10^{-9}$, \prism incurs a latency of 42 seconds against an adversary of power $\beta = 20\%$, or 182 seconds for $\beta = 33\%$. 
  %To our knowledge, this makes our system the highest-throughput blockchain implementation with Bitcoin-level security guarantees. 
  Compared to Bitcoin, \prism provides about 10,000$\times$ higher throughput and 1,000$\times$ lower latency. Compared to Algorand~\cite{algorand}, the state-of-the-art proof-of-stake system, \prism achieves 70$\times$ the throughput with about 20 seconds higher latency, and can provide a higher level of security  (up to a $\beta = 50\%$ fully-adaptive adversary vs. $\beta=33\%$ for Algorand). This is the focus of  \S\ref{sec:eval}.
  
  
 %\item We show that with these careful optimizations, it is possible to alleviate CPU performance bottlenecks and provide linear CPU scaling up to at least 8 cores. At this point, the primary bottleneck for our implementation is the underlying database (RocksDB~\cite{rocksdb} and I/O to the SSD). This suggests that future research on databases optimized for blockchain-specific access patterns could further improve performance. 

% \item
% We evaluate several practical attacks like censorship attack, balancing attack, and spamming (see ~\S\ref{sec:eval-attack}). Additionally, we propose a simple solution to the spamming problem that reduces spam traffic by 80\% while only adding 5 seconds to the confirmation delay. Our implementation illustrates that \prism performs well even under these attacks, and makes a stronger case for the practical viability of the system.
% \gf{let's remove this bullet? seems second order and raises questions about fig. 1--i.e. wasn't fig. 1 evaluated under attack?}

\end{CompactItemize}

%Our implementation and evaluation provide several key takeaways. First, our results validate Prism's core modeling and design decisions in a practical setting by demonstrating that it can scale both throughput and latency of the longest chain protocol independently of one another without compromising the security guarantee. Second, our implementation shows that with careful performance optimization (see ~\S\ref{sec:implementation-highlights}), it is possible to alleviate CPU performance bottlenecks and provide linear CPU scaling up to \ma{XXX cores}. At this point, the primary bottleneck for our implementation is the underlying database (RocksDB~\cite{rocksdb} and I/O to persistent storage (SSDs)). Therefore future research on databases optimized for blockchain-specific access patterns could provide further performance improvements. 


% e.g., asychoronous ledger updates, and a scoreboarding technique that enables parallel transaction execution without race conditions. We show that these optimizations alleviate CPU performance bottlenecks and provide linear CPU scaling, such that the primary bottleneck is the underlying database (RocksDB~\cite{rocksdb} and I/O to persistent storage (SSDs)). Further performance improvements may therefore be possible by optimizing the database.

\noindent {\bf Network and Security Model}. We adopt the now-standard  $\Delta-$synchronous network model for longest chain protocol analysis  \cite{ren2019analysis,dembo2020everything};  here the adversary controls the delivery of messages but the end-to-end network delay between any two nodes is upper bounded by $\Delta$. Also, following standard convention \cite{bitcoin,ren2019analysis,dembo2020everything,gazi2020tight}, we model the block mining process as Poisson with rate $\lambda$ proportional to the hash power of the miner. 
The adversary is assumed to control a fraction $\beta$ of the total hash power.


\noindent {\bf Organization}. 
The rest of the paper is organized as follows. In \S\ref{sec:related} we overview different  approaches to scaling  blockchain performance. In \S\ref{sec:scaling} we discuss the \prism protocol and its limitations.  In \S\ref{sec:new_rule}, we propose a new confirmation rule to \prism along with   formal guarantees on security and low worst-case latency.  \S\ref{sec:design} discusses the practical challenges when turning the algorithm into a working system, as well as  the details of the client implementation with an interface enabling pay-to-public-key transactions.  %\ma{broken reference}. Evaluations are presented in \S\ref{sec:eval} to measure the performance of the system, assess the utilization of network resources (bandwidth, topology, propagation delay) and computation resources (memory, CPU), and impacts of various attacks (balancing attack, censorship attack, spamming). \S\ref{sec:conclusion} concludes the paper.


%%a host of related topics of core interest to the blockchain ecosystem; this includes interfacing Prism to a smart contract programming layer, introduction of light clients (which are simply interested in making and validating specific transactions) and bootstrapping new Prism clients into a running system - each of these is a future direction of research of great interest.


\if 0

% TODO: do we include performance here? Tell the performance first or explain the protocol first?

% TODO: if to compare the performance, what are the baselines? How to compare (cite numbers, run experiments, if so, do we need to optimize their code?) For some of them, modify Prism client into our impelmentation. For algorand, run their code. But what if their implementation is flawed? Explain the results we got (cause of the bottleneck), understand their bottleneck.

% comparisons: Algorand (fame, it could be that their paper is not doing real transactions. use their real code and try to reproduce the number in the paper), Bitcoin (longest chain), OHIE (parallel chain). Remember to point out the security level. This is FINAL.
% mentions: HotStuff
% Point that Conflux is copy cat
% Use Prism 1.0 to help rationale the protocol in Design section.
% Make other system actually do transactions

% Scale of the evaluation
% Hope that the scalability curves are flat, so that reader can assume the scalability (we could provide a breakdown of the CPU/IO resource spent)

% Mention that we have included all possible functions of the client so it is real.

% TODO: make full use of the code. Change parameters to show the idea of other systems.

Text...

Takeaways from experiments. Maybe insert a figure here. % TODO: possibilities: throughput - latency, different protocols take different positions (curve for parameterized ones)

% other potential comparisons: Conflux, Prism 1.0, Bitcoin-NG



Figure 1: comparison of throughput and latency with other blockchain protocols: 

Algorand - best permissionless PoS BFT protocol

longest chain - the original blockchain protocol (frontier as we vary mining rate and block size)

Ohie - parallel chain protocol (give state execution for free)

Prism - our protocol

Network setting (first draft)

100 nodes

artificial delay 300 ms per hop (exponential)

network bandwidth: whatever is sufficient for Prism to achieve 100K Tps. (around 200 to 300Mbps)


\fi


==> overview.tex <==
\section{Overview of \prism}
\label{sec:overview}
In this section we  discuss the key ideas behind the design of \prism. We  start with Nakamoto's longest chain protocol, explore the limitations in scaling its throughput and latency, and present \prism as a natural design to remove these limitations. 
%%We will explain the design of \prism incrementally, first addressing throughput and then latency.



\subsection{Longest chain protocol}

The most basic blockchain consensus protocol is Nakamoto's longest chain protocol, used in many blockchain projects including \bitcoin and \ethereum.  The basic object is a {\em block}, consisting of transactions and links to other blocks. Starting with the {\em genesis} block as the root, each new block mined by a miner is added to create an evolving {\em block tree}. In the longest chain protocol, each block is appended to the leaf block of the longest chain in the current block tree, and the transactions in that block are added to the transaction ledger maintained by the blocks in the longest chain. 
 A miner earns the right to append a block after solving a cryptographic puzzle based on the hash of the leaf block \ma{and the contents of the block being mined?}. The cryptographic puzzle is solved by random attempts at finding a solution to a hash inequality. The miner includes the solution in the block as a {\em proof of work}, which other nodes can verify.  The time to solve the puzzle is random and exponentially distributed with a mining rate $f$ that can be tuned by adjusting the difficulty of the puzzle. How fast an individual miner can solve the puzzle and mine the block is proportional to its hashing power, i.e. how fast it can compute hashes. 
 A block is confirmed to be in the ledger when it is $k$-deep in the ledger, i.e. the block is on the longest chain and a chain of $k-1$ blocks have been appended to it. It is proven that as long as the adversary has less than $50\%$ hashing power, the ledger has consistency and liveness properties \cite{backbone}: blocks that are deep enough in the longest chain will not be reverted, and honest miners will be able to enter a non-zero fraction of blocks into the ledger. 

\subsubsection{Latency limitation}

A critical attack on the longest chain protocol is the {\em private  double-spend} attack \cite{bitcoin}, as shown in Figure \ref{fig:double-spend}(a). Here, an adversary is trying to de-confirm a block after it is confirmed, by mining a chain in private and broadcasting it when it is longer than the public chain. If the hashing power of the adversary is greater than that of aggregate of the honest nodes, this attack can be easily executed no matter what $k$ is, since the adversary can mine blocks faster on the average than the honest nodes and will eventually  overtake the public chain. Hence, the system is not secure when the adversary controls more than half of the computing power of the network. On the other hand, when the adversary has less than half the computing power, the probability of success of this attack can be made arbitrarily small by choosing the confirmation depth $k$ to be large \cite{bitcoin}. When $k$ is small, there is still a decent chance that the adversary can mine a longer chain even though it has less power, by getting lucky and solving a few puzzles faster than the average. The probability of this event becomes exponentially smaller as $k$ grows, as the adversary has to get lucky on solving many puzzles. 


The price to pay for choosing $k$ large is increased latency in confirmation. For example, to achieve a probability of deconfirmation of $0.001$, a depth of $24$ blocks is needed if the adversary has fraction $\beta =0.3$ of the total hashing power \cite{bitcoin}. With a block mining rate of $1$ block per $10$ seconds, this translates into a latency of $240$ seconds. To achieve a deconfirmation probability of $10^{-6}$, a depth of $50$ blocks is required, translating into a latency of $500$ seconds. Figure ~\ref{fig:rd} shows Bitcoin's tradeoff between latency and reliability. \ma{I've been assuming this figure also shows the reliability-depth tradeoff for Prism?}

\begin{figure}
\begin{center}
\includegraphics[width=0.4\textwidth]{fast_confirmation_comparision.pdf}
\end{center}
\caption{ Depth of confirmation: longest chain vs \prism. (a) The longest chain protocol requires a block to be many blocks deep for reliable confirmation, so that an adversary mining in private cannot create a longer chain. (b) \prism allows each voter block to be very shallow but relies on many voter chains to increase the reliability. \ma{It's a little odd that the prism figure doesn't show a block tree for the proposer blocks. Can we have a chain, with a level corresponding to each level of the voter trees?}}
\label{fig:double_spend}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=0.4\textwidth]{reliability-depth.jpg}
\end{center}
\caption{\label{fig:rd} Reliability-depth }
\end{figure}


\subsubsection{Throughput limitation}

If $B$ is the block size in number of transactions, then the throughput of \bitcoin \ma{I think we should use `longest chain' protocol instead of `Bitcoin'. In this section, we're talking about the protocol, whereas Bitcoin is a specific system.} is $fB$ transactions per second (tps). 
\red{GF: Should we point out that it's less if there is forking? Or say at most $fB$ tps?} \ma{I like at most $fB$.}
However, the mining rate $f$ and the block size $B$ are constrained by the security requirement. Increasing the mining rate increases the amount of {\em forking} of the blockchain due to multiple blocks being mined on the same leaf block by multiple miners within the network delay $\Delta$. \ma{suggestion: Forking reduces throughput since it reduces the growth rate of the longest chain, and hence, the ledger. More importantly, forking hurts the security of the protocol because the adversary requires less compute power to overtake the longest chain.} This reduces the security of the protocol because the growth rate of the longest chain is reduced by forking while the adversary's compute power can be co-located and hence its attack chain does not experience forking. In fact, the adversarial power that can be tolerated by the longest chain protocol goes from $50\%$ to $0\%$ as the mining rate $f$ increases (Figure \ref{fig:forking}). Increasing the block size $B$ increases the amount of forking as well since the network delay $\Delta$ increases with the block size \cite{decker}.

A back-of-the-envelope calculation of the impact of the forking can be done based on a simple model of the network delay: 
$$ \Delta = \frac{hB}{C},$$
where $h$ is the average number of hops for a block to travel and $C$ transactions per second is the communication bandwidth per link. This model is consistent with the linear relation between the network delay and the block size as measured empirically by \cite{decker}. Hence, the utilization, i.e. the throughput as a fraction of the communication bandwidth, is given by 
$$ \frac{fB}{C} = \frac{f\Delta}{h}.$$
$f\Delta$ is the average number of blocks ``in flight'' per network delay time, and this has to be kept much smaller than $1$ to avoid excessive forking. 
Hence, the security requirement (as well as the number of hops) limits the utilization. \ma{Can we discuss the impact of mining rate on security here instead of the paragraph above? One idea is to state how security depends on $f\Delta$ here, and replace Figure 3 or get rid of the figure. The next sentence gives the specific point $\beta=0.45$ as an example. The nice thing about this is that it highlights that in the longest chain protocol, to meet the security requirement, one cannot have too many blocks in flight at the same time. Prism doesn't have this limitation.} For example, to achieve security against an adversary with $\beta = 0.45$ of the total hashing power, one needs $f\Delta = 0.1$. With $h = 5$, this translates to a utilization of $2\%$.
\red{GF: Maybe explain in words why we can hope to fix this problem? The dependency on  graph diameter is fundamental, since all honest nodes have to come to consensus, but the effect of Bitcoin's security requirement could  be circumvented by designing a system that trades latency for communication in its confirmation rule.}

\begin{figure}
\begin{center}
\includegraphics[width=0.3\textwidth]{forking.png}
\end{center}
\caption{ Increasing mining rate or block size increases forking and reduces security. 
\red{GF: Are we going to add numbers to the x-axis? This looks a bit cartoonish, I think having actual nubmers on the axes would help,  if we want to keep this figure at all (not sure it clarifies too much?).} \ly{Shall I redo the plot to put numbers on x-axis and make it the same style as figure 8 to 12?}
}
\label{fig:forking}
\end{figure}







%%To understand the impact 


%%Problem: For single-longest-chain increase the throughput, we need to increase the mining %%rate or the block size. Theory proves that only so far you can get. 

%%Solution: Have transaction blocks that are not a chain, so we can have high mining rate. %%Proposer chain have low mining rate. Proposer chain has low mining rate and form a chain, %%and refer to those transaction blocks. Latency is still not solved, because we still base confidence on depth.

\subsection{\prism: Factorizing the blockchain}

\ma{I think we need to refer to the Prism theory paper in this section. We are giving the intuition behind the protocol here, but it's important to state that the security properties have been formally proved.}

The selection of a main chain in a blockchain protocol can be viewed as electing a leader block among all the blocks at each level of the block tree. \ma{The level for a block is defined as its distance to the genesis block.} 
In this light, the blocks in the longest chain protocol can be viewed as serving three distinct roles: (1) they stand for election to be leaders;  (2) they add transactions to the main chain; and (3) they vote for ancestor blocks through parent link relationships. Our principal observation is that the latency and throughput limitations of the longest chain protocol are due to the {\em coupling} of the roles carried by the blocks. \prism removes these limitations by factorizing the blocks into three types of blocks: proposer blocks, transaction blocks and voter blocks. (Figure \ref{fig:prism}). Each block mined by a miner is randomly picked (sortitioned) to be of one of the types based on the value of the hash computed for its proof of work, 
% \red{GF: I don't think proof of work was defined earlier--either define it in 2.1, or clarify meaning here} \ma{I added something to Sec. 2 please check}
and if it is a voter block, will be further chosen randomly to be in one of several {\em voter trees} \red{GF: Haven't mentioned or defined voter trees yet...} (More details on this process in Section \ref{sec:key_design}.)
The voter blocks vote for transactions indirectly by voting for proposer blocks, which in turn link to transaction blocks. Proposer blocks are grouped according to their level in the original block tree \ma{not clear what this means. what is the `original block tree'? does a proposer block have a link to a parent proposer block (this is not shown in the figure)}, and each voter tree votes for exactly one proposer block at each level to select a leader block among them. The leader block is the proposer block which has the highest number of votes among all the proposer blocks at the same level (ties broken by hash of the proposer blocks.) The elected leader blocks can then bring in the transactions to form the final ledger. \ma{Can we explain this more precisely, e.g., To obtain the final ledger, one traverses the elected leader blocks level by level, including the transactions that they link to in order.}
The vote from a voter tree is represented by the reference link from a voter block in the longest chains of the voter tree; the longest chains in all the $m$ voter trees maintain the security of the whole system, as explained next.


\begin{figure}
\begin{center}
\includegraphics[width=0.45\textwidth]{Prism_main.pdf}
\end{center}
\caption{\prism: Factorizing the blocks into three types of blocks: proposer blocks, transaction blocks and voter blocks. \ma{can we increase the font size a bit?} }
\label{fig:prism}
\end{figure}

%%Thus, the parent links in the original block tree have two implicit functionalities which are explicitly separated in this representation: 1) they provide a partial ordering of the proposal blocks according to their levels, and 2) they allow blocks to vote for each other. 
% they help the voting blocks to vote for each other.
%%\blue{It's unclear here what is meant by having a block ``support" another block.}

\subsubsection{Security and Latency}

The ledger is maintained by the leader proposal blocks \ma{proposal block, or proposer block. we used proposer block to this point} at all the levels. Each leader proposal block is secured by the votes from the voter trees. Each vote is in turn secured by the longest chain protocol in its voter tree. If the adversary has less than $50\%$ hash power, and the mining rate in each of the voter trees and the proposer tree is kept small to minimize forking, then the consistency and liveness of each of the voter trees guarantee the consistency and liveness of the ledger maintained by the leader proposer blocks. However, this requires long latency to wait for each voter block to get sufficiently deep in its chain. What is interesting is that when there are many voter trees, the same guarantee can be achieved without requiring each and every vote to be secured, thus drastically improving over the latency of the longest chain protocol. 

The private double-spend attack on the longest chain protocol has a natural analog in \prism. Figure \ref{fig:double_spend}(b) shows the scenario. A honest proposer block $H$ at a particular level has collected votes from the voter chains. Over time, each of these votes will become deeper in its voter chain. An attack by the adversary is to mine a private proposal block $A$ at the same level, and on each of the voter trees fork off and mine a private alternate chain and send its vote to block $A$. After leader block $H$ is confirmed, the adversary continues to mine on each of the voter alternate chains to attempt to overtake the public longest chain and shift the vote from $H$ to $A$. If the adversary can thereby get more votes on $A$ than on $H$, then its attack is successful. The question is how deep do we have to wait for each vote to be in its voter chain in order to confirm the proposer block $H$?

Nakamoto's calculations will help us answer this question. As an example, at tolerable adversary power $\beta = 0.3$, the reversal probability \ma{in section 2, we used deconfirmation probability instead of reversal probability. i actually like reversal better, and its probably better to use the same term} in a single chain is $0.45$ when a block is $2$-deep \cite{bitcoin}. With $1000$ voter chains and each vote being $2$-deep, the expected number of chains that can be reversed by the adversary is $450$. The probability that the adversary got lucky and can reverse more than half the votes, i.e. $500$, is about  $0.001$. Hence to achieve $\epsilon = 0.001$, we only need to wait for the votes to be  $2$-deep, as opposed to the $24$ block depth needed in the longest chain protocol.  This reduction in latency is conceptually similar to averaging many unreliable  classifiers to form a strong aggregate classifier:  the more voter chains there are, the less certainty of permanence each individual vote requires, thereby reducing confirmation time.  This gain comes without sacrificing security: each voter chain is operating slowly enough to tolerate $\beta$ adversarial hash power. \ma{I like this section a lot. I think it's at just the right level.} Furthermore, increasing the number of voter chains can further improve the confirmation reliability without sacrificing latency; for example, doubling the number of voter chains from $1000$ to $2000$ can reduce the deconfirmation probability from $0.001$ to $10^{-6}$. Figure \ref{fig:rd} compares the latency-reliability tradeoffs of \prism and the longest chain protocol. 

\subsubsection{Throughput}

To keep \prism secure, the mining rate and the size of the voter blocks have to be chosen such that each voter chain has little forking. The mining rate and the size of the proposer blocks have to be also chosen such that there is very little forking in the proposer tree. Otherwise, the adversary can propose a block at each level, breaking the liveness of the system. Hence, the throughput of \prism would be as low as the longest chain protocol if transactions were carried by the proposer blocks directly. To decouple security from throughput, transactions are instead carried by separate transaction blocks. The transaction blocks enter into a pool after they are mined. Each proposer block when it is mined refers to the transaction blocks in the pool that have not been referred to by previous proposer blocks. When a proposer block is confirmed to be the leader of its level, the transactions in all the transaction blocks it refers to enter into the ledger. The throughput of the system can be increased by increasing the mining rate of the transaction blocks, without affecting the security of the system. This throughput is only limited by the computing or communication bandwidth limit $C$ of each node, thus potentially achieving $100\%$ utilization. In contrast, the throughput of the longest chain protocol is {\em security-limited} and has very low network  utilization. \ma{If we include the figure I mentioned at the end of 2.1, which shows the relationship between $f\Delta$ and security, then we can recall that in the section and explain that transaction blocks overcome this problem}


%%Show that Prism is the optimal (theory). See Fig.~\ref{fig:protocols-comparison}. Optimal in terms of communication limit. But the implementation is limited by state execution. Compare to Hotstuff. 










\begin{figure}
\begin{center}
\includegraphics[width=0.4\textwidth]{chains-table.jpg}
\end{center}
\caption{\label{fig:protocols-comparison} Table: Comparison }
\end{figure}


==> overview2.tex <==

\section{ \prism Overview}
\label{sec:overview}

%\ma{I think we need to refer to the Prism theory paper in this section. We are giving the intuition behind the protocol here, but it's important to state that the security properties have been formally proved.}

The selection of a main chain in a blockchain protocol can be viewed as electing a leader block among all the blocks at each level of the blocktree. In this light, the blocks in the longest chain protocol can be viewed as serving three distinct roles: they stand for election to be leaders;  they add transactions to the main chain; they vote for ancestor blocks through parent link relationships. The latency and throughput limitations of the longest chain protocol are due to the {\em coupling} of the roles carried by the blocks. \prism removes these limitations by factorizing the blocks into three types of blocks: proposer blocks, transaction blocks and voter blocks. (Figure \ref{fig:prism}). Each block mined by a miner is randomly sortitioned into one of the three types of blocks, and if it is a voter block, it will be further  sortitioned into one of the voter trees. (Mining is described in detail in \S\ref{sec:mining}).

The proposer blocktree anchors the \prism blockchain. 
Each proposer block contains a list of reference links to transaction blocks, which contains transactions, as well as a single reference to a parent proposer block.
Honest nodes mine proposer blocks on the longest chain in the proposer tree, but the longest chain does not determine the final confirmed sequence of proposer blocks, known as the  \emph{leader sequence}. 
We define the \emph{level} of a proposer block as its distance from the genesis proposer block, and the \emph{height} of the proposer tree as the maximum level that contains any proposer blocks. 
The leader sequence of proposer blocks contains one block at every level up to the height of the proposer tree, and is  determined by the \emph{voter chains}. 

%\gw{Voter tree (blocktree) or voter chain (blockchain)? Since unlike proposer tree, only voter longest chain will participate in voting.}

There are $m$ voter chains, where $m \gg 1$ is a fixed parameter chosen by the system designer. For example, we choose $m=1000$ in our experiments.  The $i$th voter chain is comprised of voter blocks that are mined on the longest chain of the $i$th voter trees. A voter block votes for a proposer block by containing a reference link to that proposer block, with the requirements that: 1) a vote is valid only if the voter block is in the longest chain of its voter tree; 2) each voter chain votes for one and only one proposer block at each level. The leader block at each level is the one which has the highest number of votes among all the proposer blocks at the same level (tie broken by hash of the proposer blocks.) The elected leader blocks then provide a unique ordering of the transaction blocks to form the final ledger. (Ledger formation is explained in detail in \S\ref{sec:confirmation}.)





%%The security of the system rests on the security of the $m$ voter chains, which is guaranteed by longest chain protocol. However, as we discuss next, by relying on many parallel voter chains, \prism significantly reduces the latency required to achieve a desired reversal probability compared to the vanilla longest chain protocol.


\if 0
The voter blocks vote for transactions indirectly by voting for proposer blocks, which in turn link to transaction blocks. Proposer blocks are grouped according to their level in the original block tree \ma{not clear what this means. what is the `original block tree'? does a proposer block have a link to a parent proposer block (this is not shown in the figure)}, and each voter tree votes for exactly one proposer block at each level to select a leader block among them. The leader block is the proposer block which has the highest number of votes among all the proposer blocks at the same level (ties broken by hash of the proposer blocks.) The elected leader blocks can then bring in the transactions to form the final ledger. \ma{Can we explain this more precisely, e.g., To obtain the final ledger, one traverses the elected leader blocks level by level, including the transactions that they link to in order.} The vote from a voter tree is represented by the reference link from a voter block in the longest chains of the voter tree; the longest chains in all the $m$ voter trees maintain the security of the whole system, as explained next.

\fi

%\begin{figure}
%    \centering
%    \input{figures/prism-chains.tex}
%    \caption{\prism: Factorizing the blocks into three types of blocks: proposer blocks, transaction blocks and voter blocks. \ma{can we increase the font size a bit?} }
%    \label{fig:prism}
%\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=0.45\textwidth]{figures/Prism_main.pdf}
\end{center}
\vspace{-2mm}
\caption{\small \prism: Factorizing the blocks into three types of blocks: proposer blocks, transaction blocks and voter blocks.}
\label{fig:prism}
\vspace{-5mm}
\end{figure}

%%Thus, the parent links in the original block tree have two implicit functionalities which are explicitly separated in this representation: 1) they provide a partial ordering of the proposal blocks according to their levels, and 2) they allow blocks to vote for each other. 
% they help the voting blocks to vote for each other.
%%\blue{It's unclear here what is meant by having a block ``support" another block.}

\if 0

\subsection{Security Model}
\vb{Let $\mathcal{N}$ denote  the nodes in the system and with of loss of generality, we assume each node has equal mining power. Let $\mathcal{H} \subseteq \mathcal{N}$ denote the set of honest nodes and $\mathcal{N} \setminus \mathcal{H}$ is set the adversarial nodes. The fraction of adversarial nodes, $\beta = 1 - \frac{|\mathcal{H}|}{|\mathcal{N}|}$, is assumed to be less then $0.5$. 
%We assume a network model where the delay for a block of size $B$ is equal to $\Delta = \frac{B}{C}+D$, where $B/C$ is the processing delay and $D$ is the propagation delay.
%We model the protocol as running in rounds where each round is of duration equal to the delay ($\Delta$) corresponding to the largest sized block in the \prism protocol. 
The adversarial nodes do not have to follow the \prism protocol - they can mine new blocks with any content and anywhere on the blockchain, and  unlike honest users, they can keep their mined block in private and release it anytime in future. 
%c) their action in a given round is a function of the action of the honest nodes up to and including that round.
However, the adversary cannot perform certain actions such as modifying the block content of blocks mined by honest nodes or withholding blocks mined by an honest node from reaching other honest nodes.
}

\fi

\subsection{Security and Latency}
\label{sec:prism-latency}

%The ledger is maintained by the leader proposer blocks at all the levels. 

The votes from the voter trees secure each leader proposer block, because changing an elected leader requires reversing enough votes to give them to a different proposer block in that level. 
Each vote is in turn secured by the longest chain protocol in its voter tree. If the adversary has less than $50\%$ hash power, and the mining rate in each of the voter trees is kept small to minimize forking,  then the consistency and liveness of each voter tree guarantee the consistency and liveness of the ledger maintained by the leader proposer blocks. 
However, this would appear to require a long latency to wait for each voter block to get sufficiently deep in its chain. What is interesting is that when there are many voter chains, the same guarantee can be achieved without requiring each and every vote to have a very low reversal probability, thus drastically improving over the latency of the longest chain protocol. 


To get some intuition, consider the natural analog of the private double-spend attack on the longest chain protocol in \prism. Figure \ref{fig:double_spend}(b) shows the scenario. An honest proposer block $Ho$ at a particular level has collected votes from the voter chains. Over time, each of these votes will become deeper in its voter chain. An attack by the adversary is to mine a private proposer block $A$ at the same level, and on each of the voter trees, fork off and mine a private alternate chain and send its vote to block $A$. After leader block $Ho$ is confirmed, the adversary continues to mine on each of the alternate voter chains to attempt to overtake the public longest chain and shift the vote from $Ho$ to $A$. If the adversary can thereby get more votes on $A$ than on $Ho$, then its attack is successful. The question is how deep do we have to wait for each vote to be in its voter chain in order to confirm the proposer block $Ho$?

Nakamoto's calculations will help us answer this question. As an example, at tolerable adversary power $\beta = 30\%$, the reversal probability in a single chain is $0.45$ when a block is $2$-deep \cite{bitcoin}. With $m=1000$ voter chains and each vote being $2$-deep, the expected number of chains that can be reversed by the adversary is $450$. The probability that the adversary can get lucky and reverse more than half the votes, i.e. $500$, is about  $0.001$. Hence to achieve a reversal probability, $\epsilon = 0.001$, we only need to wait for the votes to be  $2$-deep, as opposed to the $24$ block depth needed in the longest chain protocol (\S\ref{s:lc-latency}). This reduction in latency comes without sacrificing security: each voter chain can operate at a slow enough mining rate to tolerate $\beta$ adversarial hash power. Furthermore, increasing the number of voter chains can further improve the confirmation reliability without sacrificing latency; for example, doubling the number of voter chains from $1000$ to $2000$ can reduce the reversal probability from $0.001$ to $10^{-6}$.

We have discussed one specific attack, focusing on the case when there is a single public proposer block on a given level. Another possible attack is when there are two or more such proposer blocks and the adversary tries to balance the votes between them to delay confirmation. It turns out that the attack space is quite huge and these are formally analyzed in \cite{prism-theory} to obtain the following guarantee on the confirmation latency, regardless of the attack:

 \begin{theorem}[Latency, Thm. 4.8 \cite{prism-theory}] \label{cor:latency_fast}
For an adversary with $\beta< 50\%$ of hash power, network propagation delay $D$, \prism with $m$ chains confirms  \textit{honest}\footnote{Honest transactions are ones which have no conflicting double-spent transactions broadcast in public.} transactions at reversal probability $\epsilon$ guarantee with latency upper bounded by
\begin{equation}
\label{eq:latency}
 Dc_1(\beta) +  \frac{Dc_2(\beta)}{m} \log \frac{1}{\epsilon}\;\; \text{ seconds},
\end{equation}
where $c_1(\beta)$ and $c_2(\beta) $ are $\beta$ dependent constants.
\end{theorem}

For large number of voter chains $m$, the first term dominates the above equation and therefore Prism achieves near optimal latency, i.e. proportional to the propagation delay $D$ and independent of the reversal probability. Figure \ref{fig:rd} compares the latency-reliability tradeoffs of \prism and the longest chain protocol. Note that (\ref{eq:latency}) is a worst-case latency bound that holds for {\em all} attacks. In Section \ref{sec:balancing}, we will evaluate the latency of our system under the balancing attack. 


\subsection{Throughput}
\label{sec:thruput}

To keep \prism secure, the mining rate and the size of the voter blocks have to be chosen such that each voter chain has little forking. The mining rate and the size of the proposer blocks have to be also chosen such that there is very little forking in the proposer tree. Otherwise, the adversary can propose a block at each level, breaking the liveness of the system. Hence, the throughput of \prism would be as low as the longest chain protocol if transactions were carried by the proposer blocks directly. 


To decouple security from throughput, transactions are instead carried by separate transaction blocks. Each proposer block when it is mined refers to the transaction blocks that have not been referred to by previous proposer blocks. This design allows throughput to be increased by increasing the mining rate of the transaction blocks, without affecting the security of the system. The throughput is only limited by the computing or communication bandwidth limit $C$ of each node, thus potentially achieving $100\%$ utilization. In contrast, as we discussed in \S\ref{s:lc-thput}, the throughput of the longest chain protocol is security-limited, resulting in low network utilization. \cite{prism-theory} formally proves that \prism achieves near optimal throughput:

\begin{theorem}[Throughput, Thm. 4.4\cite{prism-theory} ]
\label{thm:throughput} For an adversary with $\beta < 50\%$ fraction of hash power and network capacity C, Prism can achieve  $(1-\beta)C$ throughput and maintain liveness in the ledger.
\end{theorem}

%Note that the reference links from a proposer block to its transaction blocks are sealed in the proof-of-work of the proposer block. Hence, once a proposer block is mined, there is no way for an attacker to change the reference links to the transaction blocks. In contrast, the transactions that a miner in \bitcoin-NG adds onto the ledger after its block enters the main chain are {\em not} sealed by the proof-of-work. Hence, \bitcoin-NG is susceptible to censorship attacks.

\smallskip
\noindent{\bf Remark on security model:} The Prism theory paper~\cite{prism-theory} analyzed the protocol in a synchronous round-based network model under standard assumptions about the adversary. In particular, the delay for a block of size $B$ was assumed to be equal to $\Delta = \frac{B}{C}+D$, where $B/C$ is the processing delay and $D$ is the propagation delay, and the protocol was assumed to run in rounds where each round is of duration equal to the delay ($\Delta$) corresponding to the largest sized block. The adversarial nodes do not have to follow protocol - they can mine new blocks with any content and anywhere on the blockchain, and  unlike honest users, they can keep their mined blocks in private and release them at anytime in the future. However, the adversary cannot modify the content of blocks mined by honest nodes or withhold blocks mined by an honest node from reaching other honest nodes. Refer to \S2 of~\cite{prism-theory} for the full specification of the model. This model does not capture the impact of artifacts like queuing delay or asynchronous communication on performance. Nevertheless our implementation shows that the overall performance characteristics predicted by the theory hold in a practical setting. 


% To decouple security from throughput, transactions are instead carried by separate transaction blocks. The transaction blocks enter into a pool after they are mined. Each proposer block when it is mined refers to the transaction blocks in the pool that have not been referred to by previous proposer blocks. When a proposer block is confirmed to be the leader of its level, the transactions in all the transaction blocks it refers to enter into the ledger. \ma{The last three sentences could be cut from here and discussed in the design section} The throughput of the system can be increased by increasing the mining rate of the transaction blocks, without affecting the security of the system. This throughput is only limited by the computing or communication bandwidth limit $C$ of each node, thus potentially achieving $100\%$ utilization. In contrast, as we discussed in \S\ref{s:lc-thput}, the throughput of the longest chain protocol is security-limited, resulting in low network utilization. 





%\ma{If we include the figure I mentioned at the end of 2.1, which shows the relationship between $f\Delta$ and security, then we can recall that in the section and explain that transaction blocks overcome this problem}


%%Show that Prism is the optimal (theory). See Fig.~\ref{fig:protocols-comparison}. Optimal in terms of communication limit. But the implementation is limited by state execution. Compare to Hotstuff. 



% \subsection{Formal guarantees}
% The results established about the \prism protocol in a recent theoretical paper~\cite{prism-theory} provide the following throughput and latency guarantees. \ly{update the bib file to reflect that the paper has been published. also consider anonymous issues}




% The above two results show that of Prism achieves near optimal throughput and latency.

% \ma{@Vivek: please summarize the main results from the theory paper here.}
% \vb{done.}



\if 0

\begin{figure}
\begin{center}
\includegraphics[width=0.4\textwidth]{chains-table.jpg}
\end{center}
\caption{\label{fig:protocols-comparison} Table: Comparison }
\end{figure}

\fi


==> propagation.tex <==
\section{Block Propagation Delay Distribution}
\label{apx:propagation}

 Here we present the distribution plots of the block propagation delay ($\Delta$) in topologies tested in our scalability experiment (\S\ref{sec:eval-scale}). The data are shown in Figures~\ref{fig:propagation1}, \ref{fig:propagation2}, \ref{fig:propagation3}, \ref{fig:propagation4}, \ref{fig:propagation5}. In each plot, the concrete lines mark the mean of the propagation delay of that type of blocks, and the dashed lines mark the $25\%$ and $75\%$ quantiles. Comparing Figures~\ref{fig:propagation1}, \ref{fig:propagation3}, \ref{fig:propagation5} we observe that as long as the network diameter is kept constant, the block propagation delay is barely affected by the increase of clients.


\begin{figure}[t]
   \centering
   \includegraphics[width=\linewidth]{figures/delay100nodes.pdf}
   \caption{Block propagation delay. Nodes$=100$, Degree$=4$, Diameter$=5$}%\vspace{-6mm}
   \label{fig:propagation1}
 \end{figure}
 
 \begin{figure}[t]
   \centering
   \includegraphics[width=\linewidth]{figures/delay300nodes4.pdf}
   \caption{Block propagation delay. Nodes$=300$, Degree$=4$, Diameter$=7$}%\vspace{-6mm}
   \label{fig:propagation2}
 \end{figure}
 
 \begin{figure}[t]
   \centering
   \includegraphics[width=\linewidth]{figures/delay300nodes6.pdf}
   \caption{Block propagation delay. Nodes$=300$, Degree$=6$, Diameter$=5$}%\vspace{-6mm}
   \label{fig:propagation3}
 \end{figure}
 
 \begin{figure}[t]
   \centering
   \includegraphics[width=\linewidth]{figures/delay1000nodes4.pdf}
   \caption{Block propagation delay. Nodes$=1000$, Degree$=4$, Diameter$=9$}%\vspace{-6mm}
   \label{fig:propagation4}
 \end{figure}
 
 \begin{figure}[t]
   \centering
   \includegraphics[width=\linewidth]{figures/delay1000nodes8.pdf}
   \caption{Block propagation delay. Nodes$=1000$, Degree$=8$, Diameter$=5$}
   \label{fig:propagation5}
 \end{figure}
 



==> pseudocode.tex <==
\section{Pseudocode}
\label{sec:pseudocode}

\begin{algorithm}
{\fontsize{8pt}{8pt}\selectfont \caption{Prism: Mining}\label{alg:prism_minining}
\begin{algorithmic}[1]

\Procedure{Main}{ }
    \State \textsc{Initialize}()
    \While{True}
        \State $header, Ppf, Cpf$ =  \textsc{PowMining}() \label{code:blockBody1}
        \State \maincolorcomment{Block contains header, parent, content and merkle proofs}
        \If{header is a \textit{tx block}}
        \State $block \gets \langle header, txParent, txPool, Ppf, Cpf\rangle$
        \ElsIf{header is a \textit{prop block}}
        \State $block \gets \langle header, prpParent, unRfTxBkPool, Ppf, Cpf\rangle$\label{code:blockBody2}
        \ElsIf{header is a \textit{block in voter} blocktree $i$}
        \State $block \gets \langle header, vtParent[i], votesOnPrpBks[i], Ppf,\label{code:blockBody3} Cpf\rangle$
        % \State \textbf{and} \textsc{ReceiveMessage}($\langle$ header, $TxP$ $\rangle$)
        \EndIf
        \State \textsc{BroadcastMessage}($block$)  \colorcomment{Broadcast to peers}

    \EndWhile
\EndProcedure

\Procedure{Initialize}{ } \colorcomment{ All variables are global}
\vspace{0.5mm} \State \maincolorcomment{Blockchain data structure $C  = (prpTree, vtTree) $}
\State $prpTree \gets genesisP$ \label{code:prpGenesis} \colorcomment{Proposer Blocktree}
\For{$i \gets 1 \; to \; m$}
\State $vtTree[i] \gets genesisM\_i$ \colorcomment{Voter $i$ blocktree} \label{code:voterGenesis}
\EndFor
\State \maincolorcomment{Parent blocks to mine on} \label{code:VarprpParent}
\State $prpParent$ $\gets genesisP $ \colorcomment{ Proposer block to mine on} 
\For{$i \gets 1 \; to \; m$}
\State $vtParent[i]$ $\gets genesisM\_i $ \colorcomment{Voter tree $i$ block to mine on}
\EndFor \label{code:VarvtParent}
\vspace{00.4mm}\State \maincolorcomment{Block content} \label{code:allcontent}
\State  $txPool$ $\gets \phi$ \colorcomment{Tx block content: Txs to add in tx bks} \label{code:txblockcontent}
\State $unRfTxBkPool$ $ \gets \phi$ \colorcomment{Prop bk content1: Unreferred tx bks} \label{code:prblockcontent1}
\State $unRfPrpBkPool$ $ \gets \phi$ \colorcomment{Prop bk content2: Unreferred prp bks} \label{code:prblockcontent2}
\For{$i \gets 1 \; to \; m$}
\State $votesOnPrpBks(i) \gets \phi$ \colorcomment{Voter tree $i$ bkbk content } \label{code:vtblockcontent}
\EndFor

\EndProcedure
\vspace{1mm}
\Procedure{PowMining}{ }
\While{True}
\State  $txParent \gets prpParent$ \label{code:initParent}
\State \maincolorcomment{Assign content for all block types/trees}
\For{$i \gets 1 \;  to \; m$} $vtContent[i] \gets votesOnPrpBks$[i] \label{code:voteIneffcient}
\EndFor
\State $txContent \gets txPool$
\State $prContent \gets (unRfTxBkPool, unRfPrpBkPool)$
\vspace{00.4mm}\State \maincolorcomment{Define parents and content Merkle trees}
\State $parentMT\gets$MerklTree($vtParent,txParent,prpParent$) %\colorcomment{Store all the potential ancestors in a Merkle Tree}
\State $contentMT\gets$MerklTree($vtContent,txContent,prContent$) \label{code:endContent}
\State nonce $ \gets $ RandomString($1^\kappa$)
\State \maincolorcomment{Header is similar to Bitcoin}
\State header $\gets \langle$ $parentMT.$root, $contentMT.$root, nonce $\rangle$
\vspace{00.4mm} \State \maincolorcomment{Sortition into different block types/trees } \label{code:sortitionStart}
\If {Hash(header)  $\leq mf_v$} \colorcomment{Voter block mined}
    \State $i\gets  \lfloor $Hash(header)/$f_v\rfloor$
    \textbf{and} \textit{break} \colorcomment{on tree $i$ }
\ElsIf{ $mf_v < $Hash(header)  $ \leq mf_v+f_t$} 
    \State  $i \gets m+1$ \textbf{ and} \textit{break}\colorcomment{Tx block mined}
\ElsIf{ $mf_v+f_t< $ Hash(header) $\leq mf_v+f_t+f_p$} 
    \State  $i \gets m+2$ \textbf{ and} \textit{break}\colorcomment{Prop block mined}
\EndIf
\EndWhile \label{code:sortitionEnd}
\maincolorcomment{Return header along with Merkle proofs}
\State \Return $\langle header, parentMT.$proof($i$),  $contentMT.$proof($i) \rangle$ \label{code:minedBlocm}
\EndProcedure
\\

\Procedure{ReceiveBlock}{\textsf{B}} \colorcomment{Get block from peers}    
\If {\textsf{B} is a valid \textit{transaction block}} \label{code:txblk_r1}
    \State $txPool$.removeTxFrom(\textsf{B}) \label{code:updateTxContent} %\colorcomment{Remove the txs present in  \textsf{B} } 
    \State $unRfTxBkPool$.append(\textsf{B})\label{code:txblk_r2}

\ElsIf{\textsf{B} is a valid \textit{block on $i^{\text{th}}$ voter tree}} \label{code:vtblk_r1}
%    \State \maincolorcomment{Append \textsf{B} and (if required) all its ancestors}
    \State $vtTree[i]$.append(\textsf{B}) \textbf{and} $vtTree[i]$.append(\textsf{B}.ancestors())    
    \If{\textsf{B}.chainlen $> vtParent[i]$.chainlen} 
    \State $vtParent[i] \gets \textsf{B} $ \textbf{and} $votesOnPrpBks$($i$).update(\textsf{B}) \label{code:updateVoteMine}
    \EndIf\label{code:vtblk_r2}

\ElsIf{\textsf{B} is a valid \textit{prop block}} \label{code:prpblk_r1}
    \If{\textsf{B}.level $==prpParent$.level+$1$}
    \State $prpParent \gets \textsf{B}$ \label{code:updatePropToMine}
    \For{$i \gets 1 \;  to \; m$}  
    \colorcomment{Add vote on level $\ell$ on all $m$ trees}
    \State $votesOnPrpBks($i$)[\textsf{B}.level] \gets \textsf{B}$   \label{code:addVote} 
    \EndFor
    % \State ChangeMainChain() \colorcomment{Similar as  Bitcoin protocol}
    \ElsIf{\textsf{B}.level $ > prpParent$.level+$1$}
        \State \maincolorcomment{Miner doesnt have block at level $prpParent$.level+$1$}
        \State \textsc{RequestNetwork(\textsf{B}.parent)} 
    \EndIf
    \State  $prpTree[\textsf{B} $.level].append(\textsf{B}),\; $unRfPrpBkPool$.append(\textsf{B})
%    \State \maincolorcomment{Remove the tx blocks and prop blocks referred by \textsf{B} }
    \State $unRfTxBkPool$.removeTxBkRefsFrom(\textsf{B}) \label{code:updateTxBkContent}
    \State $unRfPrpBkPool$.removePrpBkRefsFrom(\textsf{B}) \label{code:updatePrpBkContent}`
    % \State $[$\ell$] \gets X.ancestor[-i]$ 
        % \textsc{ReceiveMessage}(\textsf{B} .ancestor$[n-i]$)
    

\EndIf
\vspace{1mm}
\EndProcedure

\Procedure{ReceiveTx}{\textsf{tx}} 
\If {\textsf{tx} has valid signature }   $txPool$.append(\textsf{B})
\EndIf    
\EndProcedure
\end{algorithmic}
}
\end{algorithm}

\begin{algorithm}
{\fontsize{8pt}{8pt}\selectfont \caption{Prism: Tx confirmation}\label{alg:prism_con}
\begin{algorithmic}[1]

\Procedure{IsTxConfirmed}{$tx$}\label{code:fastConf}
    \State $\Pi \gets \phi$         \colorcomment{Array of set of proposer blocks}
    \For{$\ell \gets 1 \;  to \; prpTree.$maxLevel}  
        \State $votesNdepth \gets \phi$ %\colorcomment{Votes from all $m$ voter trees on level $\ell$}
        \For{$i$ in $1\;to\;m$} \label{code:getvotes_start}
        \State  $votesNdepth[i] \gets \textsc{GetVoteNDepth}(i, \ell)$ 
        % \State $vtMCs[i] = vtTree[i].$LongestChain()
        \EndFor
            \If{IsPropSetConfirmed($votesNdepth$)}
        \State $\Pi[\ell] \gets$ {GetProposerSet}$(votesNdepth)$ \label{code:confirmPrpList}
        \Else $\;$ \textbf{break}\label{code:appendPrpList}
        \EndIf
    \EndFor
%    \vspace{3mm}
    \State \maincolorcomment{Ledger list decoding: Check if tx is confirmed in all ledgers}
    \State $prpBksSeqs \gets \Pi[1]\times \Pi[2]\times\cdots\times\Pi[\ell]$  \colorcomment{outer product} \label{code:outerproduct}
\For{$prpBks$ in $prpBksSeqs$} \label{code:ledgers_for_start}
                \State $ledger$ = \textsc{BuildLedger}($prpBks$)
    \If{$tx$ is \textbf{not confirmed} in \av{ledger}} \Return False
    \EndIf
    \EndFor
    \Return True \colorcomment{Return true if tx is confirmed in all ledgers} \label{code:fastConfirmTx}
\EndProcedure
\vspace{1mm}
\State \maincolorcomment{Return the vote of voter blocktree $i$ at level $\ell$ and  depth of the vote}
\Procedure{GetVoteNDepth}{$i, \ell$}
    \State $voterMC \gets vtTree[i].LongestChain()$
    \For{$voterBk$ in $voterMC$} \label{code:voteCountingStart}
%        \State \maincolorcomment{A valid voter block references one proposer block per level.}
        \For{$prpBk$ in $voterBk$.votes}
%            \State \maincolorcomment{Skip the votes on the first $\ell-1$ levels.}
%            \If{$prpBk$.level $ < \ell$} continue 
            \If{$prpBk$.level $ = \ell$} 
                    \State \maincolorcomment{Depth is \#of children bks of voter bk on main chain}
\State  \Return ($prpBk$, $voterBk$.\text{depth}) \label{code:voteCountingEnd}
            \EndIf
        \EndFor
    \EndFor
\EndProcedure
\vspace{1mm}
\Procedure{BuildLedger}{\av{propBlocks}} \colorcomment{Input: list of prop blocks}\label{code:buildLedgerFunc}
\State \av{ledger} $\gets []$ \colorcomment{List of valid transactions}
\For{\av{prpBk} in \av{propBlocks}} 
%    \State \maincolorcomment{\av{prpBk} defines the epoch} 
    \State $refPrpBks \gets prpBk.$getReferredPrpBks() \label{code:epochStarts}
    \State \maincolorcomment{Get all directly and indirectly referred transaction blocks.}
    \State  $txBks \gets\;  ${GetOrderedTxBks}$(prpBk, refPrpBks)$ \label{code:txbksOrdering}
    \For{\av{txBk} in \av{txBks}}
        \State $txs \gets txBk$.getTxs() \colorcomment{Txs are ordered in \av{txBk}}
        \For{$tx$ in $txs$}
        \State \maincolorcomment{Check for double spends and duplicate txs} 
            \If{$tx$ is  \textbf{valid} w.r.t to \av{ledger}} \av{ledger}.append($tx$) \label{code:sanitizeLedger}
            \EndIf
        \EndFor
    \EndFor    
\EndFor
\State \Return \av{ledger}
\EndProcedure
% \\
% \Procedure{GetLeader}{$\ell$} %\colorcomment{proposer block at level $\ell$ with most votes}
% \State $votes \gets \phi$ \colorcomment{Stores votes from all $m$ voter trees at level $\ell$}
% \For{$i$ in $\gets\;1\;to\;m$} 
% \State  $votes[i] \gets \textsc{GetVotes}(i, \ell)$ 
% % \State $vtMCs[i] = vtTree[i].$LongestChain()
% \EndFor
% \Return LeaderConfPolicy($votes$)\colorcomment{Refer \ref{}}
% \EndProcedure
\vspace{1mm}
\State \maincolorcomment{Return ordered list of confirmed transactions}
\Procedure{GetOrderedConfirmedTxs()}{} \label{code:slowConf}
   \State $\texttt{L} \gets \phi$          \colorcomment{Ordered list of leader blocks}
    \For{$\ell \gets 1 \;  to \; prpTree.$maxLevel}  
        \State $votes \gets \phi$ \colorcomment{Stores votes from all $m$ voter trees on level $\ell$}
        \For{$i$ in $\gets\;1\;to\;m$} 
        \State  $votesNDepth[i] \gets \textsc{GetVotes}(i, \ell)$ 
        % \State $vtMCs[i] = vtTree[i].$LongestChain()
        \EndFor
        % \State \textbf{bool} $a \gets $
        \If{IsLeaderConfirmed($votesNDepth$)}
        \State \maincolorcomment{Proposer block with maximum votes on level $\ell$}\label{code:appendLeader}
        \State $\texttt{L}[\ell] \gets$ {GetLeader}$(votesNDepth)$        
        \Else $\;$ \textbf{break}
        \EndIf
    \EndFor
    \Return \textsc{BuildLedger}(\texttt{L}) \label{code:slowBuildLedger}
    \EndProcedure

\end{algorithmic}
}
\end{algorithm}


==> reviews.tex <==
\clearpage

\section{Prior Reviews and Revisions}

\begin{table}[htbp]
	\centering
	\caption{Scores}
	\begin{tabular}{ r | c | c } 
	 \hline
	 Reviewer & Merit & Expertise \\ [0.5ex] 
	 \hline\hline
	 Reviewer A & 3 (weak accept) & 2 \\
	 Reviewer B & 3 (weak accept)  & 2 \\
	 Reviewer C & 1 (reject) & 2 \\
	 Reviewer D & 3 (weak accept) & 3 \\
	 Reviewer E & 2 (weak reject) & 2 \\
	 \hline
	\end{tabular}
	\label{table:scores}
\end{table}

The paper was submitted to NSDI 20 Fall deadline. The scores are in Table~\ref{table:scores}. The major revisions to address the comments are:

\begin{itemize}
    \item Implemented \bng using our \prism codebase, measured its performance and added to the evaluation section (Fig~\ref{fig:compare} and \S\ref{sec:eval-performance}).
    \item Added a discussion of the spamming problem and proposed a solution. Added an experiment to demonstrate the effectiveness of the solution (\S\ref{sec:spamming-eval})
    \item Added a discussion about Spectre and Phantom, two protocols that focus on improving blockchain throughput (\S\ref{sec:related}).
    \item Added a discussion about BFT-based protocol like HotStuff and HoneyBadgerBFT (\S\ref{sec:related}).
    \item Clarified that Prism has high CPU efficiency, and does not inherently require powerful machines (\S\ref{sec:eval-resource}).
\end{itemize}

\subsection{Review A}

Merit: 3 (weak accept), Expertise: 2.

\noindent{\bf Paper Summary:}
The authors propose to evaluate in practice a recently proposed
theoretical blockchain protocol (Prism) that would allow the scaling
of Bitcoin's performance while maintaining security guarantees. The
protocol relies on the use of three types of blocks to decouple
throughput from voting for a leader. The authors evaluate their
implementation of the protocol in Rust in a distributed setting. They
demonstrate that a network of 100 instances running on Amazon EC2
large machines can achieve 75,000 tps regardless of the chosen
adversarial ratio, and the latency is below 1 minute in most of the
cases. The authors also demonstrate via experiments that the system is
robust to a variety of known attacks, and that it's comparable or
better than Algorand, another well-studied consensus protocol for
blockchains.

\noindent{\bf Comments for Author:}\\
Pros:\\
- simple yet novel and impressive design\\
- great framework to evaluate PoW-based protocols

\noindent Cons:\\
- questionable practical use of PoW-based protocol with high resource requirements for users

\rp{We point out that \prism does not inherently require powerful machines.  Our implementation attains a throughput of over 70,000 tps on a machine with 8 cores, 16 GB RAM, and 400 GB of SSD, specs that are common today even on laptops for \$2-3K. Of course, our system can be configured for lower throughput to further reduce resource requirements. As Figures~\ref{fig:bw} and~\ref{fig:cpu} show, Prism's CPU and bandwidth requirements scale linearly with throughput.  The main point, as discussed in \S\ref{sec:eval-resource}, is that our \prism implementation does not waste resources: it has very high CPU efficiency, and reasonable bandwidth efficiency ($\sim$50\%), which we believe can be further improved with straightforward optimizations. We added more explanation on this in \S\ref{sec:eval-resource}.}

- protocol is intuitive to comprehend, but it is not intuitive to understand all of its security implications

\rp{The protocol's security was formally analyzed in the Prism theory paper~\cite{prism-theory}. We have added a short remark on the security model and referenced the theory paper in \S\ref{sec:overview}. We also added a discussion of spamming attacks that were not analyzed in the theory paper and demonstrated the effectiveness of a simple solution.}


My suggestions:

- explain if there is a practical need for something in-between the permissionless cheap-to-join PoW-based consensus like Bitcoin and expensive-to-join BFT-based consensus like Libra

\rp{We explain in \S\ref{sec:related} that BFT-based consensus protocols target very different applications and have their own limitations, such as being unable to scale to many nodes. Also, as explained in \S\ref{sec:eval-resource}, \prism is not inherently expensive to join. It has high CPU efficiency and its parameters can be tuned to operate at a lower throughput (at reduced cost) if the application requires. 
%Also, the throughput of \prism is required for applications like large scale payments.
}

- discuss wide threat model more thoroughly and provide intuition for why the protocol is robust to those attacks which were not included in experiments. For example, variations of the GoldFinger attacks.

\rp{We would like to point out that \prism shares many security properties with the longest chain protocol, and would like to refer the reviewer to~\cite{prism-theory} and the literature on the security of Bitcoin~\cite{securityofpow}. The simplest version of the GoldFinger attack is when the adversary controls $>51\%$, and in this case both \prism and the longest chain (Bitcoin) protocol are not secure.}

I liked that the authors of the paper create a security/throughput evaluation framework and apply it to both their protocol and Bitcoin. This alone is a valuable contribution to the research area, and also makes comparing Prism to Bitcoin much easier.

The design of the overall system is very comprehensible based on the paper, despite the introduction of several new sub-blocks primitives. However, after reading the paper I didn't have confidence that it's as robust as Bitcoin, due to the increased complexity.

I also like that the authors  propose non-trivial performance optimizations (asynchronous updates, parallel transactions, block pruning, etc) to make the system more practical.

It is not clear to me what is the rationale behind building the system on top of this protocol (although the theoretical results are very interesting!). It seems to me that to realize the full performance of the system it should be run on expensive hardware and with an extremely fast and reliable internet connection.  In this case, is PoW necessary? 
I wish the authors explained in the discussion why in this setting PoW is better than HotStuff (BFT protocol based on leadership used in Libra). It is clear why this is the case in Bitcoin, where both performing validation and mining blocks is permissionless (Bitcoin's original whitepaper even mentions 1 CPU = 1 vote rationale, although we know that mining works differently today), but not in your context.
I guess there is a niche for high-performance PoW-based system, but this is not obvious. 

\rp{It is true that the benefits of \prism compared to other protocols are most apparent on high-end hardware with reliable network connections. 
However, (a) \prism has good performance even on lower-end hardware, and (b) PoW can be useful even if we assume miners have high-end hardware. 
On  lower-end hardware, Figure~\ref{fig:cpu} illustrates that even if clients have only two cores at their disposal (which  is a very modest requirement), they can still get about $30,000$ tps, which is still an order of magnitude more throughput than Algorand, several orders of magnitude more than Bitcoin, and comparable to \bng.
Therefore the requirements to observe good performance with  \prism are  well within reach for most modern computers. 
Even if we assume that miners should have high-end hardware, the most performant BFT-based protocols have been shown to scale to up to tens or hundreds of nodes \cite{yin2019hotstuff,ibm}, and  they typically require knowledge of participants (i.e.,  are designed for permissioned settings). 
PoW protocols in contrast are most useful in settings where participants are not known \emph{a priori} and/or if the goal is to scale to thousands or more  validators.  
}
% More generally, \prism exhibits benefits even on lower-end hardware; the point is that \prism is designed to maximally utilize whatever hardware and network it is running on. However, when run on low-end hardware, the bottleneck ends up being the hardware.}

3. The Longest Chain Protocol (Section 3)

It would be more accurate to call that ``heaviest chain'': the chain which has the biggest amount of ``work''. It is possible that longer chain has less work because of the difficulty adjustments in Bitcoin's PoW. I guess you may choose to still use ``the longest chain'', but please clarify that you mean the biggest amount of work.

\rp{Correct. We use the term longest chain for simplicity and since it is common in the literature, but we added a footnote on this point in \S\ref{sec:background}}.

\subsection{Review B}

Merit: 3 (weak accept), Expertise: 2.

\noindent{\bf Paper Summary:}
The paper presents Prism, a blockchain implementation that achieves a high throughput of over 70,000 transactions per second and confirmation latency of tens of seconds on networks. Prism was evaluated on a network of 1000 EC2 Virtual Machines.

\noindent{\bf Comments for Author:}
The paper was interesting.  It demonstrates good tput and latency under attack. However there were several issues that need to be addressed in both the writing, design, and evaluation.

First, an issue was that there was not conclusion which is often a red flag.  For instance, the paper was rushed last minute and conclusion removed or it was a resubmit from a separate conference with different formatting requirements.  Neither one is a deal breaker, but a red flag about proofreading at the very least.

\rp{The paper was not rushed. In the previous submisssion we decided  to  use the space for a longer discussion on ideas for extensions (e.g., light clients, bootstrapping, etc.). In this version, we have added a conclusion section and summarized the discussion on future work  in this section.}

Second, spamming where miners do not validate transactions seems dangerous and raises practical concerns as described in the paper.  The paper described an interesting approach to reduce the window of vulnerability to this attack. However, spamming was not evaluated.

\rp{We have added a discussion of spamming and how to mitigate it in  \S\ref{sec:spamming-design}, and we evaluate it experimentally in \S\ref{sec:spamming-eval}. Our results show that it reduces spamming by more than 80\% while only adding less than 5 seconds to the confirmation latency.}

Third, the evaluation did not actual mine.  This is cited as practice in other papers, but it seems to throw off the evaluation without any actual proof of work.

\rp{As mentioned in the text, the model of proof-of-work mining as a Poisson process is precise. So we are able to simulate the mining process with great accuracy using exponential-distributed random delays. This is a standard practice in evaluations of PoW-based blockchain protocols (see \cite{conflux,ohie}).}

Finally, this is becoming more of a crowded space where many papers are attempting to increase the tput rate and commit latency.  As a result, it is difficult to have significant and unique contribution.  This paper is interesting with good contribution. However, some of the issues discussed need to be addressed to improve the paper more.

\rp{We have given a comprehensive comparison with other related works in \S\ref{sec:related}. We have also demonstrated that \prism has the highest throughput among all the protocols out there and is a close second in terms of latency.}

\subsection{Review C}

Merit: 1 (reject), Expertise: 2.

\noindent{\bf Paper Summary:}
The paper describes Prism, which is a high throughput blockchain protocol that is documents in an upcoming CCS paper, and provides performance evaluation on Prism.

\noindent{\bf Comments for Author:}
This paper reads not like a detailed systems paper, but a detailed white paper advocating for the use of a particular technology, in this case, Prism.  There are questions of fit and scope for NSDI, as well as issues of anonymity.

\rp{We respectfully disagree with characterizing our paper as a ``white paper''. We set out to implement and evaluate Prism precisely because we felt that despite promising theoretical results, it is difficult to assess the real-world performance of such a complex protocol based only on theory. Our paper provides a  systematic evaluation the protocol in a practical setting, compares it to state-of-the-art baselines, and addresses practical concerns such as spamming.}

First, I find this paper difficult to parse as a systems paper. Much of the detailed operations of the protocol is not in this paper, since the protocol itself is described in detail in the CCS 2019 paper (by presumably the same authors as this paper). The high level design of the protocol is described as is, with little justification or explanation of why particular choices were made. The only nugget I could tease out is that Prism is fast because it decouples multiple properties that used to be accomplished using the same blocks on the traditional blockchain architectures.  The fact that many details are in a separate paper makes this a frustrating paper to read.

\rp{We have attempted to provide an overview of the main ideas behind the Prism protocol by contrasting it with the longest chain protocol in Sections \ref{sec:background} and \ref{sec:overview}. In particular, Section \ref{sec:prism-latency} explains how Prism overcomes the latency limitation of the longest chain protocol using voter chains, and Section~\ref{sec:thruput} discusses how it decouples throughput from security using transaction blocks. Also, at the risk of some overlap with the theory paper, we included a detailed design in \S\ref{sec:design} to make this paper self-contained to the extent possible. The main aspect that is in a separate paper is the security analysis of the protocol.} 


Much of what makes a systems paper useful is missing here. Outside of the high level idea of separation of concerns, there's little explanation of why the system is designed this way, and what direct implications there are on performance. Instead, there are LOTS of protocol details describing both normal and corner cases of operation.  Some of the performance optimizations are discussed, but not justified beyond differentiation over BTC, and details of implementations vs design are not clearly identified.  One gets the impression that there could be a much more systemsy version of this paper if 6.2 was greatly expanded to much more fine grain discussion and comparison of alternatives.

\rp{As mentioned above, we discuss design details for completeness, but provide intuition for the main protocol design decisions in Sections~\ref{sec:background} and~\ref{sec:overview}. Regarding our performance optimizations, it is not difficult to see that they are essential for high performance. For example, without the scorboarding technique, we cannot process transactions in parallel and our throughput would be limited to the single-core performance in Figure \ref{fig:cpu}.}

There is plenty of evaluation, but again from a microcosm of prism microbenchmarks. Given the number of alternative faster txn blockchain designs in the last few years, why are there no performance comparisons against them, e.g. bitcoin-ng?

\rp{We implemented \bng by modifying our \prism codebase and measured its performance. Results are in Fig~\ref{fig:compare}. Also, we would like to point out that most of these designs do not have a publicly available implementation.}

I think there are potentially interesting lessons to be learned from this protocol and its implementation, but they are not available in a paper written in the current style.

\subsection{Review D}

Merit: 3 (weak accept), Expertise: 3.

\noindent{\bf Paper Summary:}
The paper presents the implementation and evaluation of Prism, an on-chain scaling solution for Bitcoin that enables scaling the number of transactions on Bitcoin by 10000x while keeping transaction confirmation latency within 13-120s. The basic Prism protocol and its security properties has already been published. This paper is more a validation of the Prism protocol through careful implementation and experimentation at scale (up to 1000 VMs on AWS).

\noindent{\bf Comments for Author:}
The paper is quite dense even though the authors spend the first several pages describing the Prism protocol. I basically had to read the original Prism paper to get a full understanding of the protocol and it is pretty neat: instead of using the longest chain, Prism uses a DAG and by separating the blocks into transaction blocks, proposer blocks and voter blocks, they decouple security from throughput/latency. Specifically, by having a large number of voter blocks (m > 1000), they can confirm transactions at low latency after depth 2 with extremely low probability of reversal unlike Bitcoin that needs a depth of 24 or more (10x latency reduction though each voter chain can operate at slow/similar speed as Bitcoin). Second, by allowing fast mining of transaction blocks, they can arbitrarily increase the throughput of the system, again without impacting security. 

One issue with the protocol compared to Bitcoin is that nodes cannot choose transactions (transactions have to be selected randomly for achieving the security properties of the protocol.) In current Bitcoin, there is the notion of transaction fees and miners typically prioritise transactions with higher fees, which in turn provides these transactions with lower latency. This feature/incentive is missing in Prism but perhaps given the overall low latency, lack of this incentive is perhaps not a major issue.

\rp{We would like to point out that in \bitcoin, transaction fees only provide limited benefits for improving the latency for a specific transaction. Even if a transaction is immediately mined into the next block, the confirmation latency is still significantly higher than \prism for the same security property. Also, \prism provides much higher throughput than \bitcoin, therefore we believe it's unlikely to have a backlog of unmined transactions.}

However, the protocol itself has already been published, so the contribution of this paper is only on the design and implementation of the protocol.   Here, the authors claim that they solve many challenging aspects to optimising the implementation but  this is not really convincing. Many of the optimisations are standard techniques and/or possible as a the direct result of the protocol design (e.g., asynchronous ledger updates is possible in Prism but hard to do/not necessary for Bitcoin; transactions need not be broadcast when received etc.).  To enable parallel transaction execution, the authors borrow the scoreboarding technique (basically ensure no conflict in transactions during execution) and a functional design such that state is passed around. Still, I can see value to validating a complex protocol such as Prism through implementation and evaluation, hence my overall rating.

\rp{As we have clarified in the introduction section, we believe that the system implementation and its evaluation represent significant contributions. (a) It validates Prism's theoretical analysis in a practical setting. Due to the complexity of the Prism protocol, it was not clear that such protocol can be implemented as a real system and scale both throughput and latency without affecting security. (b) We discovered that through careful optimizations, CPU is not a performance bottleneck. Instead, I/O and database is the main bottleneck. We hope this motivates future research in blockchain-specific database design. (c) We evaluate Prism under active attacks in a real implementation. Such evaluation can not be performed in a realistic way without the system implementation due to the complex nature of a networked system. Our evaluations shows that Prism is robust to those attacks. Additionally, in this submission, we discuss a spamming attack and provide a simple solution that mitigates it, reducing spam traffic by 80\% with little impact on performance.}

Also, the authors claim that the latency of their system is similar to Algorand but this seems like a stretch to me. Algorand provides latency as low as 2s while the lowest latency of Prism is 13s (at beta=20\%). If one is using these systems for transactions, one can live with 2s latency while 13s seems prohibitive, so I would not claim that the latencies are similar!

\rp{We have revised the wording to avoid saying our latency is similar to Algorand. For a $\beta=20$\% adversary, Algorand's latency is 2.35s, and Prism's latency is 12.5s.}
%However, please note that Algorand can only operate at $\beta<33\%$, and Prism's latency would be lower than for higher $\beta$,  } 



Other comments:

What is the value of m parameter for Prism used in your experiments?

\rp{$m=1000$ is used across the paper. We added a note in \S\ref{sec:eval-performance}. Also, we report all parameters in Appendix B.}

What are the number of duplicate transactions and how does it vary in your experiments? What happens to this and other overhead when users (attackers) submit multiple small/valid transactions by connecting to hundreds of nodes?  Note that this is different from spamming as users may be incentivized to submit to multiple nodes to reduce transaction latency/improve reliability, so I can see a user who connects to hundred or more nodes to submit their transaction and if multiple users do the same, this can result in lots of wasted work/duplicate transaction? Sure, the system will still not double-spend/be secure but what happens to throughput/latency of the system.

\rp{Duplicate transactions submitted to multiple miners have the same impact on performance as conflicting transactions in spamming attacks. We discuss these attacks and propose a simple mitigation in \S\ref{sec:spamming-design} and evaluate it in \S\ref{sec:spamming-eval}.}

Typos in discussion point 4: trasnaction, s->As

missing related work such as spectre and phantom that target the same problem.

\rp{Fixed both.}

\subsection{Review E}

Merit: 2 (weak reject), Expertise: 2.

\noindent{\bf Paper Summary:}
The proposed PRISM scheme is a scaling blockchains with an on-scaling solution, by decoupling the addition of transactions from election into the main chain. It delivers low latency and high throughput, compared to Bitcoin's and other PoW/PoS consensus protocols.

\noindent{\bf Comments for Author:}
Prims splits blocks into three types: proposer blocks, transaction blocks, and voter blocks; The goal is to decouple the roles of the blocks in the chain (usually there is only one block type which carries all those functionalities - e.g. Bitcoin)

Proposer block: each proposer block contains a list of references to transaction blocks and a single reference to a parent proposer block. Miners mine (longest) chain of proposer blocks.

Voter block: each voter blocks casts a vote for a proposer block. A voter block can only reference one proposer block; a voter block is valid if it is part of the longest chain. The longest chain protocol secures the voter blockchain security (as well as the overall system). The adversary needs more than 50\% hashing power to gain advantage and cast voting blocks at will.

Since there are many voter chains, each vote does not need to get sufficiently deep in the chain for confirmation (and thus increase latency). This improves the latency of the system considerably when compared with, e.g., Bitcoins (2-deep instead of 24-deep for same reversal probability).

Increasing the number of voter chains improves security (and decreases the size of k-deep for the same degree of security)

Leader block: is the one with the highest number of votes (at a certain level). All the leader blocks provide a unique ordering of the transaction blocks. 

Latency improved because Prism decouples the blocks into voter and transaction + proposed blocks. The voter blocks are mined in n chains and define the consensus of the protocol. The proposed blocks (referencing transaction blocks) with more votes cast are the consensual blocks that are part of the blockchain. Latency improved because the consensus of the voter chains do not require leader blocks to be deep in the tree to be secure against reversal attacks (since there are many parallel chains).

Throughout improved, again, due to separation of concerns in the different block types. Since the mining of transaction blocks is not part of the security assumptions of the system (as in Bitcoin), the transactions can be processed at node utilization (i.e. limited by miner's CPU and bandwidth). This achieves near-optimal throughput.

Questions/comments

5.5 (page 5) Cryptographic sortition needs more background. It is mentioned throughout the paper but without going deeper in the details (does it use VRFs? zksnars?, etc). In addition, it is important to discuss what are the security assumptions of this and how does it affect the overall system assumptions and security? etc..)

\rp{Sortition does not use VRFs or SNARKs. Please see the detailed explanation in \S\ref{sec:mining}.}

5.5 (page 5) Miners simultaneous mine one voter block for each of the m voter chains. For security, the system requires many voter chains. How does a large m affect latency?

\rp{The confirmation latency actually decreases as $m$ increase, as discussed in \S\ref{sec:prism-latency}. Please note that the voter blocks actually contribute a small fraction of the bandwidth usage compared to the transactions. For example, as shown in Table~\ref{table:bw-profiling}, in our implementation with $m=1000$, the voter blocks represent only 0.21\% of the bandwidth (compared to over 50\% for transactions).}

Each client must keep the state of the blockchain. Splitting the transaction blocks and into different types and keeping m (relatively large) number of voter blockchains in memory might become expensive for clients. It would be good if the authors would present how maintaining all that state locally would affect miner's performance and resources spent. [this is actually addressed in 7.3. Resource Utilization section]

\rp{We keep all the state in RocksDB on SSD instead of the memory, so that the client is crash-tolerant. As pointed out by the reviewer, \S\ref{sec:eval-resource} provides a detailed breakdown of resource consumption.}

Miners do not validate transactions before including them to proposed blocks. This opens up (I believe) a lot of surface for denial of service attacks and targeted attacks to miners. What would be the cost of adding transaction validation to the mining pipeline?

\rp{We would like to point out that miners do perform basic validation like signature checks and proof-of-work validation. Such checks would prevent the most naive ways of DDoS. However, as explained in \S\ref{sec:spamming-eval}, not checking transactions for double spends during mining could indeed introduce the possibility of spamming. Our mitigation strategies described in \S\ref{sec:spamming-design} protect against such spamming attacks and are effective as shown in \S\ref{sec:spamming-eval}.}

6. (Implementation) ``We have implemented a Prism client in about 10,000 lines of Rust code'' where is it? it'd be great to take a look at the code.

\rp{The code is available at \cite{prismcode}.}


==> reviews2.tex <==
\clearpage

\section{Prior Reviews and Revisions}

\begin{table}[htbp]
	\centering
	\caption{Scores}
	\begin{tabular}{ r | c | c } 
	 \hline
	 Reviewer & Merit & Expertise \\ [0.5ex] 
	 \hline\hline
	 Reviewer A & 2 (weak reject) & 3 \\
	 Reviewer B & 2 (weak reject) & 4 \\
	 Reviewer C & 2 (weak reject) & 3 \\
	 \hline
	\end{tabular}
	\label{table:scores}
\end{table}

An earlier version of the paper was submitted to CCS 2020 Winter deadline. The present version is a substantially revised paper with significant new content. Specifically, in this major revision, we:

\begin{itemize}
    \item Propose a new confirmation rule for Prism and prove its security. This new rule is much more practical than the one in \cite{prism-theory} and yields better confirmation latency (details in \S1 and \S\ref{sec:scaling}). Meanwhile, just as the one in \cite{prism-theory}, this new rule is provably secure. %The new rule replaces the heuristic-based rule in the previous version of the paper. 
    We believe this addition significantly boosts the technical contribution: a new confirmation rule that makes \prism practical and a new blockchain security proof methodology (co-design of the confirmation rule of the protocol jointly with an explicit identification of the worst-case attack). (The previous submitted version used a heuristic confirmation rule in our implementation which did not have a formal security guarantee.)
    \item For this revision, we have redone almost all the experiments to evaluate the \prism protocol our new confirmation.  The performance  (throughput/latency) is improved by a factor of 10,000 compared to Bitcoin and the only limiting factor is physical limits (disk I/O and network limits). 
  
    \item We have cut back didactic material   about the longest chain protocol and the Prism protocol to provide enough space to formally introduce the new confirmation rule, the system design, and the experimental results.
\end{itemize}

We believe that this paper is justified as a new submission, with over 40\% of the content being new. However, in the interest of transparency, we include the previous review (scores are in Table~\ref{table:scores}) and our response.

\subsection{Review A}

\noindent{\bf Paper Summary:}
This paper describes an implementation of a Bitcoin-like system on top of the Prism blockchain protocol, which is reported to have excellent performance. The paper evaluates the performance of the implementation, including how performance is affected by various attacks that can be mounted against the system.

\noindent{\bf Strengths:}
The performance of the implemented system is impressive, and implementers of blockchain systems may find the details of the implementation interesting.

The paper is well written and pleasant to read.

\noindent{\bf Weaknesses:}
Much of the text of the paper is not novel, but is rather a recap of the previously published work on Prism. New content only starts around page 6, though the background up to that point is certainly useful to a reader who hasn't seen the previous publication.

\rp{The paper has been heavily revised. We try to provide a succinct background of the longest chain protocol and the Prism protocol in this new paper in page 1 -- 3. Page 4 -- 7 present our new practical confirmation rule that is provably fast and secure. Page 8 -- 10 provides the detailed design decisions which is useful as a reference by practitioners who design real-world cryptocurrency systems. Page 11 -- 13 is our extensive evaluation of Prism, which validates the theoretical results.}

This doesn't seem like a standalone paper to me; it strengthens the evidence that Prism is a good protocol, but the level of technical innovation is low. There are many implementation details in the paper, but we don't know which implementation choices have novelty or are even critical to the system's performance. Hence, the implementation design is not evaluated scientifically. The spamming defense seems like the most novel aspect of the system, but it's rather simple.

\rp{As mentioned earlier, this paper is now heavily revised. The new confirmation rule, the system implementation, and the large-scale evaluation are all new and innovative. Only page 1 -- 3 describes existing work which serves as a background for the paper. Also, we believe that all design techniques are innovative especially in the context of blockchain. No existing blockchain client can  support such a high throughput. Our implementation detail shows one way of designing a high-throughput system and its performance is extensively validated by our evaluation. As mentioned before, many unknowns exist around the Prism protocol if one only looks at \cite{prism-theory}, e.g. is it possible to turn the seemingly-complex protocol into a real-world system? Our paper answers these questions for the first time. In this sense, we believe the implementation and the evaluation are important contributions in themselves.}

\noindent{\bf Comments for author:}
I think the authors should take the content in this paper and use it to extend the previous Prism paper into a journal paper.

\rp{As mentioned before, this paper is now heavily revised with half of the content being new. We believe that with innovations in the theory (the new confirmation rule and its strong, provable security guarantees) and in the system (the first end-to-end system that achieves 80,000 tps and less than 1 minute of latency), this paper is fully justified as a standalone paper. }

\subsection{Review B}

\noindent{\bf Paper Summary:}
The paper presents an implementation and extensive experimental evaluation of Prism, a proof-of-work based blockchain that improves both the latency and the throughput of PoW cryptocurrencies. The original system design was described and analyzed at CCS 2019, and is in my opinion a very interesting and important contribution introducing and combining a number of nice ideas.

The main scope of the current paper is reporting on implementation challenges, evaluating the implementation, and comparing it with alternative approaches from the blockchain literature. Asides from the software engineering challenge of implementing the system, there are two main challenges that the implementation addresses: the bottleneck introduced by the traditional synchronous ledger update, and (2) the bottleneck introduced by the need to process too many transactions and compare them to the ledger. The paper also evaluates the effect of some additional attacks that intuitively slow-down Prism’s performance such as spamming (for which an idea is proposed to reduce it) and censorship.

\noindent{\bf Strengths:}
I am quite excited about the original ideas in Prism and I appreciate the effort invested in implementing, emulating, evaluating, and comparing the implementation with existing systems that claim state-of-the-art throughput and latency. I think the paper does a good job in documenting the challenges and discussing how they are tackled.

\noindent{\bf Weaknesses:}
I am worried that having a system implementing a design proposed last year in CSS is counterproductive and sets the wrong precedent for the conference. As expected and discussed above, there is a number of challenges that one needs to tackle when implementing the system, and the paper properly documents and resolves them (with the asterisk of asynchrony deviating from the analysis of \cite{prism-theory} as discussed above). Yet, I don’t see considerably novel ideas, so given \cite{prism-theory} the scientific advancement in terms of systems security research is in my opinion marginal for CCS.

\rp{We believe that the system implementation and evaluation is crucial in showing that Prism is practical, and in guiding practitioners to incorporate the algorithm in real-world systems. Also, in this major revision, we propose a new, more practical confirmation rule that is provably secure. We believe that this combination of algorithm innovation and system evaluation possesses significant value for a security conference.}

\noindent{\bf Comments for author:}
Regarding synchrony/asynchrony: The paper observes that the Prism protocol does not need to update the ledger in a synchronous manner. I am a bit skeptical about this statement. The original analysis of Prism assumes a synchronous model and so does the proof of security, as the authors discuss in the introduction. But running a system designed and analyzed over a synchronous environment in an asynchronous manny might be insecure. I did not see any argument that the system preserves its security in the asynchronous model. Does the analysis from \cite{prism-theory} extend directly to the asynchronous setting? Is there no issue with variable difficulty? How is it guaranteed that that miners executing Bitcoin-style readjustment in an asynchronous manner will not end up with different puzzle targets?

\rp{We would like to point out that ledger update does not affect the execution of the consensus protocol itself. That is, the thread updating the ledger monitors the \textit{output} of the consensus protocol (i.e. the blockchain state), but does not provide \textit{input} into the consensus. The reviewer is absolutely correct that Prism is designed for and analyzed under the synchronous setting. Indeed, our testbed runs on a synchronous network and everything related to updating the blockchain state (i.e. running the consensus protocol itself) is done synchronously. Although we don't dive into dynamically adjusting the mining difficulty in this paper, as long as the adjustment only depends on the blockchain state (as in the case of Bitcoin), it will work in Prism because nodes update the blockchain state synchronously.}

Regarding the parallel processing of transactions, I agree that using ideas from concurrency in hardware is indeed the way to go. I liked the parallel drawn between race conditions on a processor and race conditions when validating transactions.

The paper also proposes and evaluates experimentally approaches for countering spamming attacks that are introduced by the high degree of parallelization of the Prism design. The idea is relatively straight-forward, add a small time-jitter when processing transactions. This is validated and the reported experiments demonstrate a considerable reduction in the effect of spamming. A question that was unclear to me is whether or not this jitter needs to be readjusted depending on the actual latency of the network. Such a latency will not appear in the simulations, but when executed on a global scale, e.g., nodes over the Internet, it could be considerable and even variable.

\rp{The reviewer is totally correct that the jitter needs to be adjusted based on the real network latency. However, the reviewer may have missed the fact we indeed simulated the real Internet latency in our testbed. Actually, we added a 120ms one-way propagation delay between \textit{every} pair of nodes. This corresponds to the one-way latency from Tokyo to Paris. So we believe that our eval results of the spam mitigation already represents its real-world effectiveness.}

\noindent{\bf Required improvements:}
It would be useful to address the above comments.

\subsection{Review C}

\noindent{\bf Paper Summary:} This paper extends \cite{prism-theory} with mainly with measurement analysis. In general it's impolite to inflate academic papers (I was once reprimanded by a highly accomplished professor regarding this practice), instead it'd have been nicer to supplement the public archive version of \cite{prism-theory} with this discussion.

\rp{We would like to respectfully point out that even in its previous version, this paper was in no way intended as an inflation of an existing paper. The implementation, the evaluation, and the design details are all new. Although we used some pages to provide a gradual introduction into the longest chain protocol and Prism, we felt that such background was useful in making the paper more self-contained. That said, in this extensive revision, we have condensed the background section significantly assuming the audience to have sufficient background on blockchains.}

\noindent{\bf Strengths:}
The strengths of this paper are the implementation demo (Section 6) and measurements (section 7).

\noindent{\bf Weaknesses:}
Prism itself is bad, basically it has all the complexities of DAG (it's similar to \cite{ohie} but with even more indirect complexities), without several of the advantages (such as incentive compatibility in the sense that honest block are never orphaned, see for example eprint.iacr.org/2017/300 and eprint.iacr.org/2016/916). \rp{We would like to point out that although Prism is indeed more complex than the longest chain protocol, the design is based on the first principles. We believe that complexity itself is not a sin, only \textit{unjustified} complexity is. To that end, Prism is a very natural scaling of the longest chain protocol, achieved by first analyzing the roles of the blocks in the longest chain protocol and then scaling each one of them. Also, the extra complexity in the protocol does not impose significant overhead in terms of computational and network resource consumption. Our evaluation has proven this point.  In fact, understanding any practical bottlenecks and hurdles for achieving Prism's theoretical performance was precisely our motivation for building the system. Regarding incentive-compatibility: unlike what the reviewer implied, in Prism, honest transaction and proposer blocks are always included. } The introduction makes silly remarks about being "the first such protocol", and false claims about other works such as \cite{phantom} (just because one paper pointed out a particular issue (that was later improved doesn't mean that you may brag that it lacks proof of security). \rp{We believe our claims are factually correct. Still, we have eliminated all editorializing in this version.}

\noindent{\bf Comments for author:}
Suppose that you are required to design a reward scheme for Prism where the money is derived only from transaction fees (and not newly minted money), can you do it in a convincing way?

\rp{Incentives for consensus algorithms are a complicated topic. Indeed, four decades of BFT consensus algorithms have resulted in hundreds of publications but hardly any with incentive analysis. We respectfully submit that proposing incentive mechanisms is an altogether different research topic and outside the scope of this paper.} %   \ly{This response does not feel strong enough. What to do?}

You should add a brief note in the paper that because the protocols requires the unpredictable stochastic process for security (no a priori knowledge of block role) it requires PoW and doesn't work with PoStake or other kinds of resources, whereas there are other DAG protocols then work well with a resource other than PoW.

\rp{We politely point out that this is not true and refer the reviewer to a recent arxiv preprint (https://arxiv.org/abs/1910.02218v2) that could serve as the building block of \prism with PoS (proof of stake).} %\ly{could we cite some paper?}

Section 5.4 and 7.4: what about an analysis of liveness, i.e., under what conditions an honest transaction be included in the ledger, given the spam protection? \rp{Honest, non-conflicting transactions are always included. Spam protection only provides extra time for miners to see if other miners have already mined the same transaction.} More importantly, can you measure the complexity of maintaining the local ledger in Prism (for spam protection) versus the complexity in Bitcoin (if it's say 10000 times more complex that you should make clear that the range of the added complexity is in that ball park). \rp{Unlike what is implied by the reviewer,   the cost of maintaining the ledger in \prism is not inherently higher than in Bitcoin. Actually, we addressed this point in our evaluation when we discuss the CPU consumption of the system. In our real-world experience, 10,000 tps per CPU core (with all cryptographic checks enabled) is a very reasonable computation cost.}



==> spam-exp-dis-jitter.tex <==
\section{Spamming Attacks}
\subsection{Exponential-distributed random jitter\label{app-spam}}
\gw{Added the whole section.}
Here we present an analysis of adding exponential-distributed random jitter to mitigate spam attacks. Suppose that one arbitrary spam transaction is received by $N$ nodes at the same time. For node $j\in[N]$, the time to mine the transaction into a block is the sum of random jitter $X_j$ and mining time $M_j$. We assume $\{X_j\}_{j\in[N]}$ are i.i.d. exponential random variables with parameter $\lambda$. Also we assume mining time $M_j$ is significantly smaller than jitter $X_j$, such that we can approximate $X_j+M_j\approx X_j$.

Without loss of generality, let node $s=\arg\min_{j\in[N]} X_j$ be the first to mine the transaction, and define random variable $Z_j\in\{0,1\}$ such that
\[Z_j=1\text{ if the spam transaction gets mined by node $j$.}\]

We know that $Z_s=1$ and for $j\neq s$, $E[Z_j]\le P(X_j<X_s+\Delta)$ where $\Delta$ is the maximal network delay of a transaction block. The reason is that if the  transaction gets mined by node $j$, the time gap between two jitters $X_j$ and $X_s$ must be less than the network delay, otherwise node $j$ would remove the spam transaction from the memory pool.

By our assumption, $\{X_j\}_{j\in[N]}$ are i.i.d. exponential random variables with parameter $\lambda$, and we know $X_j\ge X_s$. By the memoryless property of exponential distribution, we have
\[P(X_j<X_s+\Delta|X_j\ge X_s)=P(X_j<\Delta)=1-e^{-\lambda \Delta}.\]

Then consider without the random jitter, the transaction would be mined by all the $N$ miners since the mining time is very small for a transaction block. So to normalize the number of spam, we normalize with $N$.

The expected normalized spam should be
\begin{align*}
    E[\sum_j Z_j]/N&= \frac{E[Z_s+\sum_{j\neq s} Z_j]}{N}\\
    &= \frac{1+\sum_{j\neq s}E[Z_j]}{N}\\
    &\le \frac{1+\sum_{j\neq s}(1-e^{-\lambda \Delta})}{N}\\
    &=1-\frac{N-1}{N}\cdot e^{-\lambda \Delta}\\
    &\approx 1-e^{-\lambda \Delta}.
\end{align*}

Fig.~\ref{fig:attack-spamming-exp} shows the case under $\Delta=2$s. With a mean of 10s, we can reduce spam to 20\%.
\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/exp-jitter.pdf}
    \caption{Effectiveness of random jitter in defending against spam attack. The maximal network delay is $\Delta=2$s. Jitters follow exponential distributions and we report the mean ($1/\lambda$).}
    \label{fig:attack-spamming-exp}
    %\vspace{-4mm}
\end{figure}

